SoK: Where's the "up"?! A Comprehensive (bottom-up) Study on the Security of Arm Cortex-M Systems

Arm Cortex-M processors are the most widely used 32-bit microcontrollers among embedded and Internet-of-Things devices. Despite the widespread usage, there has been little effort in summarizing their hardware security features, characterizing the limitations and vulnerabilities of their hardware and software stack, and systematizing the research on securing these systems. The goals and contributions of this paper are multi-fold. First, we analyze the hardware security limitations and issues of Cortex-M systems. Second, we conducted a deep study of the software stack designed for Cortex-M and revealed its limitations, which is accompanied by an empirical analysis of 1,797 real-world firmware. Third, we categorize the reported bugs in Cortex-M software systems. Finally, we systematize the efforts that aim at securing Cortex-M systems and evaluate them in terms of the protections they offer, runtime performance, required hardware features, etc. Based on the insights, we develop a set of recommendations for the research community and MCU software developers.

==> Makefile <==
DOC ?= main.tex
DIFF ?= 925952 # The NDSS submission
PDFLATEX = pdflatex 
BIBTEX = bibtex
RERUN = "(There were undefined (references|citations)|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
TARDIR = $(DOC:.tex=-src)
IMG_SRCS = $(wildcard figures/*-source.pdf)
IMG_OBJS = $(patsubst %-source.pdf,%.eps,$(IMG_SRCS))

ALL_TEX_FILES = $(shell find . -type f -name '*.tex')
BIB_FILES = $(wildcard *.bib)

.PHONY: pdf clean

pdf: images $(DOC:.tex=.pdf)

all: pdf

%.pdf: %.tex *.tex $(BIB_FILES) $(IMG_OBJS) $(ALL_TEX_FILES)
	$(eval DOC_BASE := $(GENS)$(shell basename $@ .pdf))
	rm -f $(DOC_BASE).bbl
	${PDFLATEX} $<
	egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(PDFLATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(PDFLATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(PDFLATEX) $<) ; true
	egrep -i "(Reference|Citation).*undefined" $*.log ; true
#	dvips -o $(DOC_BASE).ps -t letter $(DOC_BASE).dvi
#	ps2pdf14 -dPDFSETTINGS=/prepress -dEmbedAllFonts=true $(DOC_BASE).ps

watch:
	make; fswatch -0 `find . -name "*.tex" -o -name "*.bib"` | xargs -0 -n1 make all

diff:
	@bin/diff.sh $(DIFF)

clean:
	find . -name "*.aux" | xargs rm -f
	find . -name "*.log" | xargs rm -f
	find . -name "*.out" | xargs rm -f
	find . -name "*.cut" | xargs rm -f
	find . -name "*.gz"  | xargs rm -f
	find . -name "*.upa" | xargs rm -f
	find . -name "*.upb" | xargs rm -f
	@\rm -f \
        $(DOC:.tex=.dvi) \
        $(DOC:.tex=.pdf) \
        $(DOC:.tex=.ps)  \
        $(DOC:.tex=.bbl) \
        $(DOC:.tex=.blg) \
        $(DOC:.tex=.lof) \
        $(DOC:.tex=.lot) \
        $(DOC:.tex=.loc) \
        $(DOC:.tex=.lol) \
	$(DOC:.tex=-src.tar.gz)

images: $(IMG_OBJS)

%.eps: %-source.pdf
	pdftops -eps $< $(<:-source.pdf=.eps)

veryclean: clean
	@\rm -f *~ *.log
	@\rm -f figures/*.eps

tar: pdf
	@test -d $(TARDIR) || mkdir $(TARDIR)
	@cp Makefile *.{tex,bib,bst,cls} $(TARDIR)
	@tar cz $(TARDIR) > $(TARDIR).tar.gz
	@rm -rf $(TARDIR)



==> arch.tex <==
\section*{Cortex-M Hardware and Architecture}
\label{sec:cortexmapp}

\begin{comment}
\begin{table*}[!tpb]
\center
\scriptsize
\caption{Arm Cortex-M Processors and Their Security-related Features}
\vspace{-0.3cm}
\label{tab:cortexmfamily}
\begin{threeparttable}
\begin{tabular}{llcccccccccccccccccc}
\hline
CPU & ISA & \rotatebox{90}{\# MPU Regions} & \rotatebox{90}{TrustZone}   & \rotatebox{90}{Privileged
eXecute Never (PXN)} & \rotatebox{90}{eXecution Only Memory (XOM)} & \rotatebox{90}{Stack Limit Registers} & \rotatebox{90}{Unprivileged store/load ins.} & \rotatebox{90}{Target Test (TT) ins.} & \rotatebox{90}{Instruction Cache (KB)} & \rotatebox{90}{Data Cache (KB)} & \rotatebox{90}{Instruction Prefetching} & \rotatebox{90}{Branch Prediction} & \rotatebox{90}{Embedded Trace Macrocell (ETM)} & \rotatebox{90}{Micro Trace Buffer (MTB)} & \rotatebox{90}{Data Watchpoint and Trace Unit (DWT)} & \rotatebox{90}{Flash Patch and Breakpoint Unit (FPB)} & \rotatebox{90}{Single Instruction Multiple Data (SIMD)} & \rotatebox{90}{Float Point Unit (FPU)} & Year\\ \hline \hline
 M0 & v6-M 				&00	&00&00&00&00	&00&00&00		&00		&00&00&00	&00&11&55&00&00&2009\\ 
 M0+ & v6-M 			&8	&00&00&00&00	&00&00&00		&00		&00&00&00	&11&11&55&00&00&2012 \\ 
 M1&v6-M 				&00	&00&00&00&00	&00&00&00		&00		&00&00&00	&00&55&55&00&00&2007 \\ 
 M3&v7-M 				&8	&00&00&00&00	&11&00&00		&00		&11&11&I	&00&11&11&00&00&2004 \\ 
 M4&v7-M 				&8	&00&00&00&00	&11&00&00		&00		&11&00&I	&00&11&11&11&11&2010 \\ 
 M7&v7-M 				&16	&00&00&00&00	&11&00&0-64	&0-64	&11&11&11	&00&11&11&11&11&2014 \\ 
 M23&v8-M Baseline		&16	&11&00&00&11	&11&11&00		&00		&00&00&I	&11&11&11&00&00&2016 \\ 
 M33&v8-M Mainline		&16	&11&00&00&11	&11&11&00		&00		&00&00&I	&11&11&55&11&11&2016 \\ 
 M35P&v8-M Mainline		&16	&11&00&00&11	&11&11&2-16	&00		&00&00&I	&11&11&11&11&11&2018 \\ 
 M55&v8.1-M Mainline	&16	&11&11&11&11	&11&11&0-64	&0-64	&11&11&I	&11&11&55&11&11&2020 \\ \hline                     
\end{tabular}
\begin{tablenotes}
%    \item[1] Measured in percentages.
%    \item[2] Measured in kilobytes (KB).
	\item[] \supportlevel{0}: Not support, \supportlevel{10}: Support, \supportlevel{5}: Partially Support, I: Instruction trace only. On M23, ETM and the MTB are exclusive to each other.
 \end{tablenotes}
\end{threeparttable}
\end{table*}
% https://en.wikipedia.org/wiki/Arm_Cortex-M
\end{comment}

%\ziming{We need to make it clear what contributions are in Sec II and III. When I read the current version, as a reader I can learn something but doesn't mean it make contributions. Maybe summarize some technical highlights? maybe there is a way to formalize thing? Summarize some technical findings?}

Table~\ref{tab:cortexmfamily} presents the Cortex-M processors, their instruction set architectures, and the security features they support.
% delete SIMD, TT, Instruction Prefetching, FPU, merge PAC/BTI

In this section, we discuss the Cortex-M architecture, including its registers, execution modes, privilege levels, physical memory map, and exception handling mechanisms. 
We explain the memory protection and debug units, both of which are security related. 
%Interested readers can also refer to the white paper on Cortex-M~\cite{WhitepaperCortexM} for more information.
Table~\ref{tab:cortexmfamily} presents the Cortex-M processors, their instruction set architectures, and the security features they support.
Figure~\ref{fig:func-blocks} shows the hardware functional blocks of Cortex-M System-on-Chip (SoC).
%\subsection{Architecture and Instruction Set}
%Cortex-M processors support both 16-bit and 32-bit Thumb and Thumb-2 instructions.
%Cortex-M0/M0+/M1 are based on the Armv6-M architecture, which only has a small instruction set of 56 instructions.
%Cortex-M3/M4/M7 are based on the Armv7-M architecture.
%Cortex-M23, which supports TrustZone, is based on the Armv8-M Baseline sub-profile extended from Armv6-M.
%Cortex-M33 with TrustZone is based on Armv8-M Mainline sub-profile.
%Cortex-M35P introduces physical security.
%Cortex-M55 is based on Armv8.1-M Mainline.
%The instruction set architecture in the Cortex-M processors is the upward compatibility. 
%For example, the instruction set of Armv7-M is a superset of Armv6-M.
%As a result, a binary image compiled for Cortex-M0 can run directly on other processors.


% \begin{table*}[!htbp]
% 	\centering
% 	% \setlength{\abovecaptionskip}{5pt} 
% 	% \setlength{\belowcaptionskip}{-13pt}
% 	\caption{Banked Registers between Security State}
% 	\label{tab:banked-reg}
%   \begin{tabular}{llll} \hline
%     Register Type               & secure Register   & non-secure Register & P\_O?   \\ \hline\hline
%     General-purpose register    & MSP\_S, PSP\_S    & MSP\_NS, PSP\_NS    & N       \\
%     Special-purpose registers   & PRIMASK\_S        & PRIMASK\_NS         & Y       \\
%                                 & BASEPRI\_S        & BASEPRI\_NS         & Y       \\
%                                 & FAULTMASK\_S      & FAULTMASK\_NS       & Y       \\
%                                 & CONTROL\_S        & CONTROL\_NS         & Y       \\
%     System Control Space (SCS)  & secure SCS including SCB\_S   & non-secure SCS including SCB\_NS  & Y   \\\hline

% 	\end{tabular}
% 	%\vspace{5pt}
% \end{table*}

\subsection{General Registers}
\label{sec:subsec:GeneralReg}

\begin{figure}[!t]
	\begin{centering}
	\includegraphics[width = .48\textwidth]{pics/Function-components.pdf}
	\vspace{-0.4cm}
	\caption{Hardware functional blocks of Cortex-M SoC, including all the units discussed in \S\ref{sec:cortexm} and \S\ref{sec:trustzone}. The green boxes represent units that are allocated to the secure state. The blue boxes represent configurable components. Dotted boxes represent optional units.} %Some processors do not support flash patching, so the star means a partially implemented FPB.}
	\label{fig:func-blocks}
	\end{centering}
	\vspace{-0.5cm}
\end{figure}

Table~\ref{tab:registers} presents all the general and special registers on Cortex-M processors.
A Cortex-M processor has 16 general-purpose registers, namely \verb|R0| to \verb|R15|,
in which \verb|R0| to \verb|R12| are used for general data operations.
The stack pointer (\verb|SP| aka \verb|R13|) is a shadow register that holds the memory address of the top of the stack.
Depending on the processor's \emph{mode} and \verb|CONTROL[1]|, \verb|SP| shadows either the main stack pointer (\verb|MSP|) or the process stack pointer (\verb|PSP|).
\verb|MSPLIM| and \verb|PSPLIM| hold the lower limit of the corresponding stack pointer.
If the stack pointer would be updated to a value lower than the limit, a \verb|UsageFault| or \verb|HardFault|~\cite{ArmFaultHandling} will be generated.
The link register (\verb|LR| aka \verb|R14|) holds the return address for a subroutine, which exits by executing \verb|BX LR|.
%If a subroutine calls another subroutine, the value of \verb|LR| will be preserved onto the stack. 
When an interrupt occurs, \verb|LR| holds a special type of value \verb|EXC_RETURN|, which will be discussed in Section~\ref{sec:ExceptionStacking}.
%The program counter (\verb|PC| aka \verb|R15|) has the address of the next instruction to fetch.

% System control space is a region reserved for system control and configuration registers.

% \begin{table*}[!htpb]
%   \center
%   \scriptsize
%   \caption{Cortex-M Processor Debug Resources}
%   \label{tab:debug}
%   \begin{tabular}{llll}
%   \hline
%   Debug & Description & Banked in &  Privilege\\ 
%   Resources &  & TrustZone? &  Access only?\\ \hline \hline  
%   \verb|Trace|  & & & \\ 
%   $\hookrightarrow$ \verb|ETM|  & Embedded tracec macrocell  & No  & - \\
%   $\hookrightarrow$ \verb|ITM|  & A memory-mapped register interface to generate instrumentation packets & No  & No \\
%   $\hookrightarrow$ \verb|DWT|  & & No  & - \\
%   $\hookrightarrow$ \verb|TPIU| & & No  & - \\
%   \verb|FPB|  & & No  & - \\
%   \verb|SCS|  & Memory region for system control and configuration & Yes & Yes\\
%   $\hookrightarrow$ \verb|SCB|    & Control and configure key features for exception model &  Yes& Yes \\
%   $\hookrightarrow$ \verb|DCB|    & For debug features  & Yes & Yes \\  
  % \hline                                                                
  % \end{tabular}
  % \end{table*}

\subsection{Execution Mode, Privilege Level and Special Registers}
\label{sec:mode}

All Cortex-M processors have two execution modes, namely thread (\verb|T|) and handler (\verb|H|).
All, but the Armv6-M processors, also have two privilege levels, namely privileged (\verb|P|) and unprivileged (\verb|U|). 
Execution in the thread mode can be either privileged or unprivileged and either \verb|PSP| or \verb|MSP| can be used, whereas execution in the handler mode is always privileged and \verb|MSP| is always used.  
Software at the unprivileged level cannot execute privileged instructions and modify some memory regions, such as the Private Peripheral Bus (PPB).

The current mode and privilege level are determined by the combination of the interrupt program status register (\verb|IPSR|) and the \verb|CONTROL| register.
\verb|IPSR| is part of the program status register (\verb|xPSR|).
\verb|IPSR|'s nine least significant bits (\verb|IPSR[8:0]|) indicate the exception number if not 0. 
If \verb|IPSR[8:0]| is 0, the processor is in the thread mode. %, which we will discuss in Section~\ref{sec:mode}.
In the thread mode \verb|CONTROL[0]| determines whether the state is unprivileged or not,
whereas \verb|CONTROL[1]| determines whether \verb|SP| shadows \verb|PSP| or \verb|MSP|.
%Besides \verb|IPSR|, the 32-bit \verb|xPSR| consists of another two non-overlapping special registers: the application program status register (\verb|APSR|) and the execution program status register (\verb|EPSR|).
%\verb|APSR| has the program status flags, such as overflow, negative, carry, etc.
The priority mask register (\verb|PRIMASK|), the base priority mask register (\verb|BASEPRI|), and the fault mask register (\verb|FAULTMASK|) are used to disable and prioritize interrupts.
%\verb|BASEPRI| and \verb|FAULTMASK| are not available for Armv6-M or Armv8-M Baseline processors. 
Special registers can only be read or written using three special privileged instructions, namely \verb|MRS| (move from a special register to a general one), \verb|MSR| (move from a general-purpose register to a special one) and \verb|CPS| (enable or disable interrupts) as shown in Table~\ref{tab:SecInstruction}.
% Another privileged access only instruction CPS is used to change processor state.

On reset, the processor is at the privileged level (\verb|CONTROL[0]| = 0) and the thread mode (\verb|IPSR[8:0]| = 0). %even though it executes the reset handler.
To switch the processor's from privileged to unprivileged, one can simply change \verb|CONTROL[0]| to 1 using the \verb|MSR| instruction.
To switch from unprivileged to privileged, software should use the instruction \verb|SVC| to execute the \verb|SVC| handler. %in the handler mode.
%Then, the SVC handler can use \verb|MSR| to change \verb|CONTROL[0]| from 1 to 0 and returns.
Figure~\ref{fig:ModePLSecure} presents a complete execution mode, privilege level and security state transition diagram. %, which we will explain in detail in \S\ref{sec:subsec:stateswithing}.

\subsection{Physical Memory Map}
\label{sec:physicalmemory}

\begin{table}[!tpb]
\center
\scriptsize
\caption{Cortex-M Processor General and Special Registers}
\vspace{-0.3cm}
\label{tab:registers}
\begin{tabular}{lp{5cm}l}
\hline
Register & Description & Banked in \\ 
 &  & TrustZone? \\ \hline \hline                                                                                                                                                                                                       
\verb|R0|-\verb|R12| & General-purpose registers for data operations & No \\
\verb|R13|/\verb|SP| & Shadowed stack pointer & - \\
$\hookrightarrow$ \verb|MSP| & Main stack pointer & Yes \\
$\hookrightarrow$ \verb|PSP| & Process stack pointer & Yes \\
\verb|R14|/\verb|LR| & Link register & No   \\
\verb|R15|/\verb|PC| & Program counter & No  \\ 
\verb|MSPLIM| & Main stack pointer limit (v8-M and after) & Yes  \\
\verb|PSPLIM| & Process stack pointer limit (v8-M and after) & Yes \\
\verb|xPSR| & Program status register. Combination of \verb|APSR|, \verb|IPSR|, and \verb|EPSR| & Yes \\                                                                 
\verb|CONTROL| & Determining the privilege level and stack register in thread mode & \verb|bit[1,0]| \\ 
\verb|PRIMASK| & Used for interrupt disabling & Yes \\
\verb|BASEPRI| & Priority threshold for interrupt disabling & Yes \\
\verb|FAULTMASK| & Used for interrupt disabling & Yes \\
\hline                                                                
\end{tabular}
\vspace{-0.5cm} 
\end{table}

\begin{table*}[t]
	\centering
	\scriptsize
	% \setlength{\abovecaptionskip}{5pt} 
	% \setlength{\belowcaptionskip}{-13pt}
	\caption{32-bit Physical Memory Map}
	\vspace{-0.3cm}	
	\label{tab:Armv8-system-map}
	\begin{threeparttable}
	\begin{tabular}{l l c p{8cm}} \hline
		Physical Address Range & Region & XN? & Remarks	\\ \hline\hline 
		0x00000000 - 0x1FFFFFFF & Code & No & ROM or flash memory; very bottom is actually aliased memory not code 	\\   
		0x20000000 - 0x3FFFFFFF & SRAM	& No & On-chip RAM	\\    
		0x40000000 - 0x5FFFFFFF & Peripheral & Yes & Address space for on-chip peripherals, such as MPC\\     
		0x60000000 - 0x7FFFFFFF & RAM & No & Memory with write back, write allocate cache attribute	\\    
		0x80000000 - 0x9FFFFFFF & RAM & No & Memory with write through cache attribute	\\      
		0xA0000000 - 0xBFFFFFFF & Device & Yes & Peripherals accessible to all masters \\    
		0xC0000000 - 0xDFFFFFFF & Device & Yes & Peripherals accessible only to this PE	\\      
		0xE0000000 - 0xFFFFFFFF & System & Yes & This region can only be accessed at the privileged level.	\\  		
		$\hookrightarrow$ 0xE0000000 - 0xE00FFFFF & System Private Peripheral Bus (PPB) & Yes & Key resources, including the System Control Space and debug features. \\ 	
		\hspace{.3cm} $\hookrightarrow$ 0xE000E000 - 0xE000EFFF & Secure System Control Space (SCS) & Yes & Registers for control, configuration, and status reporting. Some registers are banked when TrustZone is implemented. \\ 		
		\hspace{.3cm} \hspace{.3cm} $\hookrightarrow$ 0xE000EC00 - 0xE000ED8F & Secure  System Control Block (SCB) &  & 	\\ 	
		\hspace{.3cm} $\hookrightarrow$ 0xE002E000 - 0xE002EFFF & Non-secure System Control Space & Yes & 	\\ 		
		\hspace{.3cm} \hspace{.3cm} $\hookrightarrow$ 0xE002ED00 - 0xE002ED8F & Non-secure System Control Block & Yes & 	\\ 				
		$\hookrightarrow$ 0xE0100000 - 0xFFFFFFFF & Vendor\_SYS & Yes & Implementation defined vendor system region \\ \hline
	\end{tabular}
	\begin{tablenotes}
		\item[] XN: eXecution Never
	 \end{tablenotes}  
	 \end{threeparttable}
	 \vspace{-0.5cm} 
\end{table*}

\begin{table}[!tpb]
\center
\scriptsize
\caption{Instructions That Have Security Implications}
\vspace{-0.3cm}
\label{tab:SecInstruction}
\begin{tabular}{p{11ex}p{6.5cm}}
	\hline
	Instruction & Description                                                                                                                                                                                                              \\ \hline \hline
	\verb|CPS| & Change processor state. Privileged access only. See~\S\ref{sec:mode}.\\
	\verb|MRS|/\verb|MSR| & Data transfer between \verb|xPSR| and general-purpose registers or immediate value. Privileged access only. See~\S\ref{sec:mode}.\\ \hdashline
	\multicolumn{2}{c}{Introduced in TrustZone} \\ \hdashline
	\verb|SG| & Secure entry point to switch from non-secure to the secure state. \verb|SG|s resides in NSC. See~\S\ref{sec:subsec:stateswithing}.\\
	\verb|BXNS| & Branch or return to the non-secure state from the secure state. See~\S\ref{sec:subsec:stateswithing}.\\
	\verb|BLXNS| & Call non-secure functions in the secure state. See~\S\ref{sec:subsec:stateswithing}.\\
	\verb|STR*T|/\verb|LDR*T| & Used at the privileged level to emulate unprivileged store/load operations. Data widths of word, halfword (H), signed halfword (SH) and byte (B) are available. See \S\ref{sec:subsec:STRT}. \\
	\verb|TTA?T?| & The 4 TT instruction variants, i.e., TT, TTT, TTA, TTAT, which query the security state and access permissions of a memory location. See \S\ref{sec:subsec:TT}. \\
	\verb|VLLDM|/\verb|VLSTM| & Save and restore floating-point context if the non-secure function being called and also utilize FPU or Helium feature. \\
	%The insertion of VLSTM and VLLDM is normally handled by C/C++ compilers. 
	\hdashline
	\multicolumn{2}{c}{Introduced in PACBTI. See~\S\ref{sec:subsec:PACBTI}.} \\ \hdashline
	% \verb|STRT|/\verb|LDRT| & Store/Load Register with Translation, Used at the privileged modes to emulate user mode instructions\\
	% If the instruction is executed when the processor is in a privileged mode, the memory system is signaled to treat the access as if the processor was in User mode. \ziming{Is there more instructions like this?} \\
	\verb|PAC| & Sign \verb|LR| using \verb|SP| and a key, store the result in \verb|R12|. \\
	\verb|PACBTI| & Sign \verb|LR| using \verb|SP| and a key, store the result in \verb|R12|. When BTI is enabled, it is a valid target instruction. \\
	\verb|PACG| & Sign \verb|Rn| using \verb|Rm| and a key, store the result in \verb|Rd|. \\
	\verb|AUT| & Authenticate \verb|LR| with \verb|SP| and PAC in \verb|R12|. Generate a \verb|UsageFault| exception on errors. \\
	\verb|BXAUT| & Indirect branch with pointer authentication. Branch to \verb|Rn| if PAC matches. Generate a \verb|UsageFault| exception on errors. \\
	\verb|AUTG| & Authenticate \verb|Rn| with \verb|Rm| and the PAC is in \verb|Rd|. Generate a \verb|UsageFault| exception on errors. \\
	\verb|BTI| & A valid target instruction. \\
	\hline                                                                
	\end{tabular}
	\vspace{-0.5cm} 
\end{table}

The physical memory space of a Cortex-M system is 32 bit, which is equally divided into eight regions 
%to map different types of memories, devices and system peripherals 
as shown in Table~\ref{tab:Armv8-system-map}.
%The 4GB address space is sparsely populated due to the limited sizes of the physical devices.
The first 512MB region is reserved for \emph{code}, and it is mapped to on-chip ROMs or Flash memories. 
%The size of ROMs and Flash range from several KBs to several MBs.
The second 512MB region is mapped to on-chip \emph{SRAM},
which together with two \emph{RAM} regions hold mutable run-time data, e.g., stack, heap, and global data.
%The size of SRAM and RAMs also range from several KBs to several MBs.
The \emph{peripheral} and two \emph{device} regions map I/O device registers.
%which include General Purpose Input and Output (GPIO), Direct memory access (DMA) controller, etc.
The \emph{system} region maps system control registers, 
which include a 1MB system \emph{private peripheral bus} (PPB) for Memory Protection Unit (MPU), Security Attribution Unit (SAU), SysTick timer, etc.
PPB is further divided into configurations for the secure and the non-secure state if TrustZone is implemented.
A fixed eXecution Never (XN) attribute is associated with each region in that only \emph{code}, \emph{SRAM}, and 2 \emph{RAM} regions are executable.

%Unprivileged access to the PPB causes BusFault.

\subsection{Exception, Context Stacking and Unstacking}
\label{sec:ExceptionStacking}

%All Cortex-M processors include a Nested Vectored Interrupt Controller (NVIC). 
When a higher priority interrupt or exception occurs, the processor automatically pushes eight registers (\verb|xPSR|, \verb|PC|, \verb|LR|, \verb|R12|, \verb|R3|, \verb|R2|, \verb|R1|, \verb|R0|; aka state context) to the current stack, which is called context stacking. 
If the Floating Point Unit (FPU) is enabled, the context stacking also pushes FPU related registers (\verb|S0| - \verb|S15| and \verb|FPSCR|; aka FP context).
Then, the processor generates a special exception return value named \verb|EXC_RETURN|, stores it in \verb|LR|, and executes the interrupt service routine (ISR).
%The most significant bits, e.g., 25 bits for Armv8-M processors, of \verb|EXC_RETURN| are reserved and read as 1. 
%As a result, if interpreted as an address, it corresponds to an eXecution-Never address. 
When an ISR exits and \verb|EXC_RETURN| is copied to the \verb|PC|, the processor will automatically perform unstacking, which pops the eight registers off the stack. %and clears corresponding bits in the NVIC registers. 
%The hardware-assisted mechanism of stacking and unstacking makes it possible to develop C language only interrupt handlers.
%PendSV and SysTick are typically used for scheduling the exception context switch when running a RTOS, such as pending the lower priority exceptions until finish the higher one.

\subsection{Fault Handling}
\label{sec:FaultHandling}
% \ziming{what do you meaning by 6 exceptions implemented?}
% There are 6 basic exceptions implemented on the Cortex-M: reset, non-maskable interrupt, HardFault, SVC, PendSV and SysTick. https://interrupt.memfault.com/blog/arm-cortex-m-exceptions-and-nvic
% For more fine-grained fault handling, MemManage, BusFault, and UsageFault can be enabled.
% PendSV and SysTick are typically used for scheduling the exception context switch when running a RTOS, such as pending the lower priority exceptions until finish the higher one.

In the Armv6-M and Armv8-M Baseline architecture, all the fault events trigger the \verb|HardFault| handler.
In the Armv7-M and Armv8-M Mainline, several configurable fault handlers are introduced: \verb|BusFault| (bus returns an error response), \verb|MemManageFault| (memory management fault), \verb|UsageFault| (undefined instructions or other illegal operations), \verb|SecureFault| (security violations in the TrustZone security extension).
These exceptions have programmable priority levels and can be individually enabled or disabled. 
%Fault Status Registers and Fault Address Register are used for debug. MemManage Fault State Register.

\subsection{Memory Protection Unit}
\label{sec:mpu}

Memory Protection Unit (MPU) 
%a programmable unit inside the processor that 
monitors all memory accesses, including instruction fetches and data accesses, over software-designated regions.
Different from a Memory Management Unit (MMU), an MPU does not support virtual memory. 
As shown in Table~\ref{tab:cortexmfamily}, %the number of supported MPU regions on Cortex-M is small.
most devices only support up to 8 MPU regions. %if the MPU is implemented. 
MPU regions on Armv7-M that are larger than 256 bytes can be divided into 8 equally sized subregions, which have the same permissions but can be individually activated.
%MPU registers are mapped into the PPB area, which is privileged access only. 
%When the MPU is enabled, any invalid memory access invokes the \verb|MemManage| handler.
%The MPU is disabled after reset.
%All Cortex-M processors but M0 and M1 can have an MPU.
The permission for an MPU region is determined by the Access Permission field (\verb|AP|) and the eXecute-Never bit (\verb|XN|).
Armv7-M MPUs use 3-bit (\verb|AP[2:0]|) to support six access permissions, while Armv8-M MPUs use 2-bit (\verb|AP[2:1]|) to define four access permissions.
% \verb|AP| has 4 possible values: (i) read-only by any privilege level; (ii) read-only by privileged; iii) read/write by any privilege level; iv) read/write by privileged.
% Therefore, it is not possible to set a region as only accessible by unprivileged but not by privileged.
The \verb|XN| bit determines whether execution is permitted when read is permitted.
%It does not support the eXecution-Only Memory (XOM) permission~\cite{}.
The Cortex-M55 processor introduces a Privileged eXecute Never (\verb|PXN|) bit to prevent the processor from executing the code inside with the privileged level.
It also supports system level use of eXecution-Only Memory (XOM)~\cite{ArmCortexM55}. 
%A limitation of Cortex-M MPU is the small number of regions it can support.

\subsection{Unprivileged Memory Access Instructions}
\label{sec:subsec:STRT}
Cortex-M ISA includes several special store and load instructions (\verb|STR*T|/\verb|LDR*T|) with unprivileged access as shown in Table~\ref{tab:SecInstruction}.
Even when these instructions are executed at the privileged level, they are treated as if they are executed at the unprivileged level.
So the MPU checks the corresponding unprivileged permission bits when executing them~\cite{Armv7MArcRef}.


% shows the instructions that can be used if the current execution mode is unprivileged access only~\cite{Armv7MArcRef} A4-113.
%Including 32-bit word load (\verb|LDRT|) and store (\verb|STRT|), 16-bit halfword store (\verb|STRHT|), 16-bit unsigned halfword load (\verb|LDRHT|), 16-bit signed halfword load (\verb|LDRSHT|), 8-bit byte store (\verb|STRBT|), 8-bit unsigned byte load (\verb|LDRBT|), and 8-bit signed byte load (\verb|LDRSBT|). 

\begin{comment}
\begin{table}[!htpb]
	\center
	\scriptsize
	\caption{Unprivileged Load and Store Instructions}
	\vspace{-0.3cm}
	\label{tab:ls}
	\begin{tabular}{lll}
	\hline
	Data type    				& Load  		& Store         \\ 
								& Unprivileged	& Unprivileged	\\ \hline  \hline
	32-bit word     			& LDRT     		& STRT   		\\
	16-bit halfword    			& -     		& STRHT   		\\
	16-bit unsigned halfword    & LDRHT     	& -   			\\
	16-bit signed halfword   	& LDRSHT    	& -   			\\
	8-bit byte     				& -     		& STRBT   		\\
	8-bit unsigned byte     	& LDRBT     	& -   			\\  
	8-bit signed byte			& LDRSBT		& -				\\
	\hline                                
	\end{tabular}
\end{table}
\end{comment}

\subsection{Debug Units}
\label{sec:debugers}
%Debug authentication Armv8.1
% https://www.sciencedirect.com/topics/engineering/coresight-debug-architecture
%Cortex-M processors implement debug interfaces and features in a separate unit called CoreSight debug architecture~\cite{ArmCoreSightv3}.
%The Debug Access Port (DAP) can be used to access the system bus on those debug units.
As shown in Table~\ref{tab:cortexmfamily}, the Cortex-M architecture comes with debug and trace units that can perform instruction and data tracing, system events profiling, load and store operations counting, etc.
These units are privileged access only by default and support invasive, i.e., control and observe, and non-invasive debugging, i.e., observe without control.
%In invasive debugging, the processor halts when a debug event is triggered, e.g. using the breakpoint (\verb|BKPT|) instruction.
%Non-invasive debugging monitors registers and processor states without interrupting the execution. % arm debugging, nailgun
%~\cite{ArmCortexM0, ArmCortexM0+, ArmCortexM1, ArmCortexM3, ArmCortexM4, ArmCortexM23, ArmCortexM33, ArmCortexM55}. 

% Signals: IAXEN, IAEXSEQ,IAEX[30:0], ATOMIC, EDBGRQ
\subsubsection{Flash Patch and Breakpoint Unit (FPB) and Breakpoint Unit (BPU)}

Both FPB and BPU can be used to configure and enable hardware breakpoints~\cite{Armv7MArcRef, Armv8MArcTech, Armv6MArcRef}. 
The FPB can also be used to patch Flash code and data, such as firmware that cannot be upgraded~\cite{nRF52FP, ArmFBPm3_4}.
Since more IoT devices support full firmware update, this feature is rarely used.
%Flash patch control register (\verb|FP_CTRL|) indicates how many breakpoints the hardware supports and enable the breakpoint.
% Flash patch comparator (\verb|FP_COMPn|) register 

% \subsubsection{Digital Signal Processing (DSP)}

% \subsubsection{Performance Monitoring Unit (PMU)}

\subsubsection{Data Watchpoint and Trace Unit (DWT)}
The DWT provides hardware watchpoints that can halt the execution if the access matches the setting.
%It has up to 4 comparators that support instruction fetch, instruction address (range) and value matching or data address (range) and value matching.
%The comparison is done in parallel with the normal execution flow.
% Functionality: hardware watchpoint, hardware trace packet, cycle counter, instruction address matching, data address matching, data value matching (DWT\_COMP1 or DWT\_COMP3 only), linked/limit matching (DWT\_COMP1 or DWT\_COMP3 only).
For system profiling, %besides the basic processor cycle counting, 
the DWT has several non-invasive counters:  
folded-instruction counting for additional instruction executed in the current cycle; 
load and store instruction counting;
exception overhead counting for total cycles in exception; 
sleep counting for total cycles the processor sleeps; 
and clock per instruction counting for additional cycles when executing multi-cycle instructions.

% Program counter sampling is another non-invasive debug components that can trace PC value packets generated by a DWT comparator matching.

% https://interrupt.memfault.com/blog/cortex-m-watchpoints

% \subsubsection{Instrumentation Trace Macrocell (ITM)}
% ITM gives developer chance to create a debug channel and send messages to the debugger monitor.
% 0xE0001000-0xE0001FFF

\subsubsection{Micro Trace Buffer (MTB)}
The MTB traces non-sequential program counter changes, e.g., branches and exceptions, by storing trace packets to the trace buffer located on the SRAM.
A trace packet is 8 bytes and consists of the source and destination addresses of the control transfer.
%The size and base address of the trace buffer can be configured.
%When the buffer is full, the MTB can either halt the processor or overwrite from the beginning of the buffer.
% The trace history is limited by the size of SRAM.
%MTB supports both invasive and non-invasive mechanisms.
%It can be used to trace instruction execution information~\cite{ArmMTBM23}. 
%When the MTB is enabled, each time the PC changes non-sequentially, e.g. branch or exception, it writes a trace packet which is total of 8 bytes (4 bytes source \verb|PC| + 4 bytes destination \verb|PC|) to the trace buffer.

%User can configure the size and address of the trace buffer in the SRAM.
%The buffer is usually in a circular arrangement to capture the recent instruction executions.
%Also, user can configure the MTB to send halt signals to the processor if the buffer is full.
%This can avoid trace information loss.
%Then the debugger can read the buffer to reconstruct the program flow.

%To configure the MTB in a simple step, three registers are needed.
%\verb|MTB_BASE| register indicates the MTB trace storage starting address in SRAM. 
%\verb|MTB_POSITION| register contains the trace packet write pointer and a wrap bit.
%One trace packet contains a pair of addresses.
%the pointer is the location of the first word of packet which points to the source \verb|PC|. 
%If the trace buffer is full and needs wrap, the wrap bit in \verb|MTB_POSITION| will be set to 1 automatically.
%\verb|MTB_MASTER| register configures the maximum size of SRAM used for tracing and enables the MTB. 
%Or using the TSTART and TSTOP signals can also enable and disable the MTB.
%It also determines the privilege-level accesses to the SRAM (set \verb|MTB_MASTER.RAMPRIV| to 0 means unprivileged accessible, to 1 means privileged access only).

%Trace writing has a higher priority than system writes to AHB.
%If the trace writes frequently, it may cause overhead for high bus load cases.
% Debug authentication interface: DBGEN, NIDEN.

\subsubsection{Embedded Trace Macrocell (ETM)}

% debugging of historical sequences, software profiling, and code coverage analysis.
% ETM has a variety architecture versions and implementations on different Cortex-M processors (Table~\ref{tab:debug-trace}).
The ETM is more powerful than the MTB in that it provides more comprehensive instructions tracing (since M3) and data tracing (M7 only).
The trace packets generated by the ETM have a timestamp from the system clock. %, whereas the counterparts generated by the MTB do not have.
%The trace packets can be exported to a trace port or written to the Embedded Trace Buffer (ETB) on SRAM~\cite{ArmTrace}.
%Table~\ref{tab:cortexmfamily} shows that only M7 supports both instruction and data trace, others support instruction trace only~\cite{ArmETMM4, ArmETMM7, ArmETMM23, ArmETMM33, ArmETMM55}.
% Each trace packet begins with a unique type header (e.g. \verb|0b00000001| for data trace, \verb|0b00101100| for instruction trace) followed by information bytes depends on the packet type.
Instruction tracing can monitor direct and indirect branches, exceptions, e.g., such as \verb|SVC| and \verb|BKPT|, address and context, cycle counting, etc.
% The event packet is 8 bytes that indicates the generated event elements.
%The address and context tracing records the instruction address, the instruction set of the next one, and currently executing instruction, e.g., exception level, security state of the processor.
%This packet has up to 8 bytes including the address value and 1-6 context bytes.
%For more detail, please refer to~\cite{ArmETMv1-3.5, ArmETMv4-4.6}.
% The instruction trace packet  
Data tracing monitors the data accesses, including the addresses of data transfer, data value, and the related load or store instruction.
%ETM and the MTB are exclusive on Cortex-M23 processors.

% \begin{table}[!htpb]
% 	\center
% 	\scriptsize
% 	\caption{Comparison Table for ETM}
% 	\label{tab:etm}
% 	\begin{tabular}{ll}
% 	\hline
% 	Processor	& branches	& conditional instructions	& cycle counts & data address comparison & secure non-invasive debug  			\\ \hline  \hline
% 	M0			&
% 	M33			& instruction trace		 		\\ 
% 	M35P		& v4.2		    	\\
% 	M55			& v4.5				 \\ \hline
% 	\\                                                                    
% 	\end{tabular}
%   \end{table}

% 0xE0041000-0xE0041FFF

% \subsubsection{Cross Trigger Interface (CTI)}

% CTI enables the debug logic, interacting with the MTB, ETM, DWT, and other debug components.

% For example: triggering a hardware breakpoint when a DWT comparator match is detected.

% \subsubsection{Others}

% \begin{table}[!htpb]
% 	\center
% 	\scriptsize
% 	\caption{Debug and Trace Options for Cortex-M Family}
% 	\label{tab:debug-trace}
% 	\begin{tabular}{llllll}
% 	\hline
% 	Processor	&FBP?BPU 	& DWT 			& ETM	 			&  the MTB\\ \hline  \hline
% 	M0 		&BPU		& \checkmark	& $\times$ 			& $\times$ \\
% 	M0+ 	&BPU		& \checkmark 	& $\times$  		& $\times$ \\
% 	M1		&BPU		& DW			& $\times$  		& $\times$ \\
% 	M3		&FBP		& \checkmark	& instruction trace	 		& $\times$\\
% 	M4		&FBP		& \checkmark	& instruction trace		 		& $\times$\\
% 	M7		&FPB		& \checkmark 	& instruction and data trace	& $\times$	\\
% 	M23		&FPB		& \checkmark	& instruction trace x MTB 	& x ETM \\ 
% 	M33		&BPU		& \checkmark	& instruction trace		 		& \checkmark\\ 
% 	M35P	&FPU		& \checkmark	& instruction trace		    & \checkmark\\
% 	M55		&BPU		& \checkmark   	& instruction trace	& \checkmark \\ \hline
% 	\\                                                                    
% 	\end{tabular}
%   \end{table}

%The MPU implementation of the Cortex-M23 or Cortex-M33 processor can define 0, 4, 8, 12, or 16 regions while on Cortex-M0+, Cortex-M3, or Cortex-M4 is either 0 or 8.
%The smallest size of an MPU region is 32 bytes, the maximum size of an MPU region is 4GB.
%All MPU regions are aligned to a multiple of 32 bytes.

%To configure the MPU, we need to set up the starting, ending address of the region, and the secure attributes.
%The secure attributes define the chargeability (shareable, cacheable, or bufferable) and access permissions, including read-only, write-only, read and write, never execute, or privileged access only.
% There are several important registers we use to configure the MPU.
% \begin{itemize}
%   \item \verb|MPU_TYPE| register (bit[15:8]) indicates the numbers of regions the MPU supports for the selected security state.  
%   \item \verb|MPU_CTRL| register provides programmable bit fields for MPU enable features.
%   Bit[2] enable or disable the background region, bit[1] enable for HardFault and NMI (Non-Maskable Interrupt), bit[0] enable or disable the MPU.
%   \item \verb|MPU_RNR| (MPU Region Number Register) indicates the region id that is accessed by the \verb|MPU_RBAR| and \verb|MPU_RLAR|.
%   \item \verb|MPU_RBAR| (MPU Region Base Address Register) defines the starting address (bit[31:5]) of the MPU region and access permissions.
%   Bit[4:3] indicates chargeability for Normal memory, bit[2:1] indicates the read/write access permissions, bit[0] configure the eXecute Never attribute.
%   \item \verb|MPU_RLAR| (MPU Region Limit Address Register) defines the ending address (bit[31:5]) of the MPU region, region enable (bit[0]), and an indirection index to memory attribute array (bit[3:1]).
%   \item \verb|MPU_MAIR0/1| (MPU Attribute Indirection Register 0 and 1) 
% \end{itemize}
%The procedure to configure the MPU always following:

%\begin{enumerate}
%  \item Disable the MPU, check the number of MPU regions this selected security state supports. 
%  \item Select the region id we want to configure.
%  \item Set the starting address and access permissions.
%  \item Set the ending address and memory attribute indirection register.
%  \item Enable the MPU
%  \item Flush the instructions to make it effective immediately.
%\end{enumerate}

%With the enabled MPU, we can prevent stack overflows in one compartment from corrupting memory belonging to another compartment.
%With the execute never secure attribute, we can prevent potentially malicious code execution within unexpected regions.
%Also, we can configure the RAM and SRAM as read-only to prevent accidental corruptions.
%Since all MPU registers are privileged access only, all MPU-assisted secure mechanisms need to elevate to the privilege mode if the current code is at the unprivileged level.
\subsection{Summary of Cortex-M Hardware Features}

The Cortex-M microcontroller architectures do not have many hardware features that are standard on microprocessors, such as MMU, cache, branch prediction, etc.
They, however, offer hardware-assisted automatic stacking and unstacking for exception handling considering its interrupt-driven software model.
Debug units, such as DWT, MTB, and ETM, are widely available on Cortex-M architectures.

%focuses on reducing cost for widespread usage and speedup execution to meet the resource constraints. 
%Most of the processors, as Table~\ref{tab:cortexmfamily} shows, do not integrate with expensive optimization mechanisms such as cache. 
%Instead, the Cortex-M processor has hardware-supported stacking and unstacking for exception context switches.
%Unlike modern systems with MMU that utilize memory virtualization to protect each process, embedded devices rely on privilege separations and an MPU to control the privilege resources access.
%Besides MPU, unprivileged memory access instructions and debug units can also help to build secure design for embedded devices.
%For example, MTB and ETM can help trace and reconstruct the control flow execution.
%DWT can be used to monitor specific data and instruction access.

%We will discuss them in \S\ref{sec:IssueVul} and \S\ref{sec:projects}.
%[So why do we mention those features here? How those can help our research? Explain it.]

==> back_up.tex <==

% INTRO
% and are offering such MCUs with different features~\cite{cmip}.
%dominates the 32-bit MCU market with around 90\% of the market share in 2019~\cite{ArmMarketShare2019}.

%In the 4th quarter of 2020 alone, 4.4 billion Cortex-M processors were shipped~\cite{Armnews2020}. \ZQ{Can 2022 data be shown here?}
%, the Arm Cortex-M family . 
%Today, there are more than 3000 microcontroller parts based on Arm Cortex-M processors. 
%Hardware vendors build a variety of products using Cortex-M processors~\cite{yiu2020definitive}, which include
%(i) consumer devices, e.g., Amazon Dash button, Nest thermostat, Fitbit Flex, Oculus VR;
%(ii) electronic control units in motor vehicles, e.g., real-time motor controls and data acquisitions;
%(iii) data communication subsystems, %in mobile phones, 
%e.g., Bluetooth and ZigBee controllers;
%and (iv) power and peripheral management in complex system-on-chips (SoC), e.g., audio control.

%multicore System-on-Chips (SoC), Application Specific Integrated Circuits (ASIC), Application Specific Standard Products (ASSP), sensors, etc.~\cite{yiu2020definitive}.
%as shown in Table~\ref{tab:cortexmfamily}.
%Some of these devices have a long life cycle, and 
%MCUs play an important role in our daily life, 
%as the devices they power include sensors, medical devices, wearables, smart family gadgets, network cards, SD memory cards, industrial computing units, etc. 
%Notable networked personal devices powered by Cortex-M include Amazon Dash button, Google Nest thermostat, Fitbit Flex, Oculus VR, etc.

%Consequently, only a small group of researchers are familiar with these platform features, and other researchers seeking to study and work on them often need to rediscover the same limitations, tricks, and insights.

%the researchers who are familiar with the security of microprocessors, e.g., x86/64 and Cortex-A, understand the challenges they face in designing secure Cortex-M software.

%We also create a taxonomy of the recent research efforts on securing Cortex-M systems.
%Because the official descriptions of hardware security features~\cite{Armv6MArcRef, Armv7MArcRef, Armv8MArcRef, Armv8MArcTech, Armv8MMPU, ArmCortexM23, ArmCortexM33, ArmCortexM55, Armv8MTZ, ARMpacbti} are hard to digest, %sometimes incomplete and scattered in many documents,
%we develop an open-source test suite that demonstrates their usage.
%\gl{not very clear.}
%In addition, Cortex-M MCUs not only have issues found in Cortex-A microprocessors but also introduce new vulnerabilities. 
%For instance, we report return-to-non-secure (ret2ns) vulnerabilities, which are a confused deputy problem specific to the Cortex-M TrustZone architecture.

%TrustZone-assisted trusted execution environments (TEEs)~\cite{cerdeira2020sok}.
%We analyze which software components are more likely to be affected  %by the vulnerabilities.

%Additionally, due to the hardware limitations and lack of mitigations, the disclosed Cortex-M related bugs exhibit a significantly higher severity compared to all CVE-assigned bugs during the same periods}.
%and privilege escalation through TrustZone.
%on Memory Protection Unit (MPU) and TrustZone assisted isolation environments.
%Because of the monolithic firmware design, even a tiny bug can easily break the functionality or crash the whole system.

%Q4
%We evaluate these efforts based on the protections they offer, deployability, performance, etc.
%The findings will be discussed in .

%Our major observations include that the research community attempts to bring the same defenses from microprocessor-based systems to these systems, e.g., address space layout randomization, and in the meanwhile tackling unique challenges. %most popular secure enhancements on modern desktops and servers are not efficient enough on Cortex-M microcontroller-based systems (e.g., shadow stack~\cite{nyman2017cfi, kawada2020TZmCFI}), which associates with the answer for \textit{Q2}.
%Thus, researchers search for alternative ways or improve known methods via Cortex-M supported hardware features to help secure the resource constraints devices, such as encoding the general-purpose register to protect the integrity of return address~\cite{almakhdhubmurai2020}, leveraging unprivileged instructions to restrict the access to sensitive data from untrusted code~\cite{kwon2019uxom, zhou2020silhouette, du2022kage}, etc.

%discuss the Cortex-M specific hardware issues found by us, e.g., return-to-non-secure vulnerabilities, and others.
%, and their security features are less known. 
%For example, virtual memory management is not available for lack of a Memory Management Unit (MMU), but Cortex-M does offer a Memory Protection Unit (MPU) that provides access control in the physical memory space. 
%Also, Cortex-M has recently introduced its own version of TrustZone, which has different underlying mechanisms from its Cortex-A counterpart.

% Even if Cortex-M offers some security-related features, existing embedded and IoT software systems barely use them and largely lack protection against code injection, control-flow hijack, data corruption, and other attacks.

%We argue that since Cortex-M architecture features more and more security units, such as 
%The main goal is to develop a general and secure scheme.
%because Cortex-M devices provide limited resources for security, most popular secure enhancements on modern desktops and servers are replaced by alternative ways on those systems
%From MPU-assisted privilege separation and isolation to 
%Researchers proposed several solutions to enhance the security of Cortex-M systems.
%However, little of them have been deployed on real-world systems. [Why?]
%We attribute the stagnancy of system and software security on Cortex-M to the following reasons:

%1) 
%As a result, the security of such devices has been largely neglected as both academia and industry made great progress in securing x86/64 and Cortex-A based systems in the last decades.
%However, these devices are no longer in a safe haven since they are connected to the Internet now;

%2) 
% they do provide many security features at the hardware layer. 


%3) It is sometimes difficult to find openly available documents for Cortex-M security features.
%Even when descriptions are available, they may be vague, incomplete, and buried in over tens of thousand pages of technical reference manuals. 
%Additionally, there are not many widely available teaching materials, such as example code.
%There is a big gap in security feature offerings and 

% Due to memory and speed constraints, little key cryptography is absent from such devices.
%In addition, we observe that despite the offering of Cortex-M hardware security primitives, software technologies for security significantly lag behind for several reasons:
%i) mindeset, no need for security;
%i) too many documents hard to start from somewhere;
%ii) no good available start-kit.


%Section \S\ref{sec:methodology} guides the exploration of subsequent sections. 
%Section \S\ref{sec:HardIssueVul} summarizes limitations and issues related to hardware. 
%Section \S\ref{sec:SoftIssueVul} describes the identified Cortex-M software architecture and its associated issues. 
%Section \S\ref{sec:ImpIssueVul} discusses real-world systems' implementation bugs retrieved from CVE database. 
%Section \S\ref{sec:projects} illustrates how existing literature addresses issues at both the hardware and software architectural levels.

%\item We analyze the offerings, limitations, and issues of Cortex-M hardware and software architectures and implementations.
%We report a new confused deputy attack, i.e., ret2ns, that is specific to Cortex-M.
%We perform by far the largest empirical analysis on the adoption of security mechanisms and features on the real-world Cortex-M firmware;

%\item We present a comparative evaluation of the solutions to secure Cortex-M systems.
%Our evaluation framework considers the defenses each solution offers, the hardware units it relies on, and their run-time overhead in terms of memory size, performance, etc.;


%1) We summarize security-related limitations, issues, and vulnerabilities of the Cortex-M based hardware and software.
%We group the findings into three categories: hardware, software architectural, and software implementation, a taxonomy adopted by Cerdeira et al. in studying the security vulnerabilities in Cortex-A TrustZone-assisted TEEs~\cite{cerdeira2020sok}. In particular, we study xxx with the dataset.

%To build background knowledge that leads to better understanding of the security of Cortex-M hardware and software stack, 
%We overview the generic Cortex-M architecture and hardware features, some of which have profound security implications, such as memory protection and debug units (\S\ref{sec:cortexm}); 

%We present a systematic description of Cortex-M hardware security features (\S\ref{sec:trustzone}), %and how to use them at the instruction set architecture layer (ISA), especially TrustZone and other associated controllers (\S\ref{sec:trustzone}). 
%the official descriptions of which are sometimes incomplete and scattered in many documents~\cite{Armv6MArcRef, Armv7MArcRef, Armv8MArcRef, Armv8MArcTech, Armv8MMPU, Armv8MTZ, ArmCortexM23, ArmCortexM33, ArmCortexM55}.
%We developed an open-source code example suite~(\S\ref{sec:codesuite}) that demonstrates how to use the Cortex-M security features
%we overview the dedicated security extensions of Cortex-M;
%to help researchers easily access Cortex-M research;

%3) We present some new attacks at the ISA and ABI layer, architectural deficiencies, which have not been discussed before.  an insightful discussion on the current limitations and open issues in the security of Cortex-M. binary-level backdoors;

%3) We discuss five software architectures of Cortex-M based systems, which are used in production systems and presented in the literature %including the privileged application, monolithic kernel, software-based virtualization/least kernel privilege, dual-world, and multiple trusted execution environment architectures 
%(\S\ref{sec:SoftwareSystem});

%4) We summarize the limitations, issues, and vulnerabilities of the Cortex-M based hardware and software stack (\S\ref{sec:IssueVul}). 
%Additional, we group them into three categories, namely hardware, software architectural, and software implementation;
%, a taxonomy adopted by Cerdeira et al. in studying the security vulnerabilities in TrustZone-assisted TEE systems~\cite{cerdeira2020sok}.

%5) We systematize efforts in securing the software stack on Cortex-M (\S\ref{sec:projects}), which include enforcing isolation and confinement, stack integrity, control flow integrity, etc.
%Also, we evaluate these efforts based on the protections they offer, deployability, performance, etc.;

%Not only do the taxonomy and new findings paint the security landscape of the hardware and software stack of Cortex-M systems, but they also make a rough drawing on the bigger picture of MCU-based embedded and IoT system security.
%We hope this paper will help interested researchers better understand the Cortex-M systems and their security states, point the community to opportunities for improving the security of Cortex-M systems, and inspire security research on embedded and IoT architectures and systems in general.

%6) We discuss future directions in securing Cortex-M systems and beyond (\S\ref{sec:discussion}). 

%7) To help the research community, address this problem, we develop a suite of open source example code (\S Appendix-\ref{sec:codesuite}), for Cortex-M security features exploration.

%Even though there are attempted efforts~\cite{} to explain and educate Cortex-M and TrustZone, they stay at the Application Binary Interface layer.
%We attempt to dive into the Instruction Set Architecture layer and find out design flaws in binary code that compilers which follow ABI will not generate. Show an example here. 


%First of all, there is no good survey or Sok paper on Arm Cortex-M TrustZone.

%The readers do not need background on Cortex-A TrustZone, but procession of which may help understand the features.

%\ziming{Add a figure of all cortex-m devices?}

%The contributions of this paper are summarized as follows:
%\begin{itemize}
%    \item We overview the Cortex-M hardware and architecture
%    \item We
%    \item We        
%\end{itemize}

%The remainder of this paper is organized as follows.
%First, we show the versatility of the basic hardware features for the common Cortex-M processors (Section II).
%Then, we discuss the security extension TrustZone on newly introduced Cortex-M processors since Armv8M architecture (Section III).
%We summarise all possible problems on Cortex-M processors at Section IV and discuss potential attacks at Section V.
%In Section VI, we give a survey about currently used embedded systems.
%To have a better understanding of the hardware support and security properties, we test an IoT example using the Cortex-M33 processor at Section VII and also provide the comprehensive tests at Section VIII.
%Then, we give a comprehensive survey about the projects that enforce the security of the Cortex-M at Section X.

%Compared to Cortex-A and Intel, the security of Cortex-M is not well-known.
%Comparing with their Cortex-A counterparts, which power smartphones, tablets, laptops, servers, etc., the Cortex-M processors have lower maximum frequency, low power, and low interrupt latency.
%Nevertheless, they are powerful enough to run customized deep learning algorithms~\cite{ji2020mcunet}.

%================================================Methodology====================================================

%To get a comprehensive study of Cortex-M processor, we adopt the following methodologies. 

%Our comprehensive study on the security of Arm Cortex-M systems faces several challenges. 
%Obtaining real-world Cortex-M firmware is challenging due to its proprietary nature, as it is often used in commercial products with intellectual property protections. 
%Additionally, the binaries tend to be difficult to analyze because of the lack of documentation and the diversity of firmware interfaces and architectures across different Cortex-M devices. 
%Further complexity is introduced by the wide range of processors supported by the same vendors, as well as by RTOS and libraries, which adds to the difficulty of identifying Cortex-M specific security issues. 
%We address these challenges by adopting the following methodology.

%Apparently, many legacy Cortex-M devices were deeply embedded and isolated from the Internet, and it was believed that the attack surface for them is small.
%Because of their different deployment models, Cortex-M based systems face a variety of threats and attacks.
%For example, consumer devices need to protect the confidentiality of users' sensitive data, while motor controllers must ensure the integrity and availability of the software at run-time.

%\gl{my suggestion: 1. remote attacks via network, 2. nearby wireless attacks via BLE, ZigBee, etc, 3. local attacks through peripherals such as senors, 4. local attacks through debug ports 5. side channel attacks.}

%=======================================threat model
%We do not consider 
% as they are not directly related to the Cortex-M ISA.
%(iv) to obtain secrets from the privileged non-secure state;
%(v) privilege escalation in the non-secure state;
%\gl{what are the differences with (i-iii)? I suppose these are TZ specific. Be more specific. to obtain secrets in the secure world? escalate privilege to secure?}
%the secure state.

%Cortex-M processors powers a variety of devices that face a wide range of adversaries.
%We discuss adversaries and types of attacks based on their attack angles:
%(1) system software adversary aims to control the system's memory to obtain sensitive information, or break the functionalities.
%It usually utilizes software implementation bugs to exploit the system;
%(2) peripheral adversary can control a vulnerable peripheral to access or modify memory or other resources belonging to the victim system;
%(3) microarchitectural adversary monitors the processor's microarchitectures (e.g., CPU state and registers), which allows him to bypass software or hardware level protection techniques.
%All adversaries can access the system on Cortex-M devices in two ways: either directly by physical connection with peripherals or debug connectors, or indirectly from wireless communications such as Bluetooth, or WiFi.
%All codes running on the Cortex-M processor are assumed to be untrusted.

%===============analyzing frimware==============
%The FirmXRay Cortex-M firmware dataset~\cite{wen2020firmxray}, which is collected using a mobile app based approach, includes 790 firmware representing 535 unique devices from two vendors (768 from Nordic~\cite{nordic} and 22 from Texas Instruments~\cite{texasi}). 
%To reduce dataset bias, we used the same mobile app based approach to successfully collect another dataset with firmware from two different vendors (192 from Telink~\cite{telink} and 53 from Dialog~\cite{dialog}).
%We also analyzed the monolithic firmware image dataset from the HAPSTER~\cite{gritti2022heapster}.
%After screening it leaves us with 4 raw binaries from Fitbit and 54 ELF Cortex-M images.
%We perform an empirical analysis on the combined raw binary dataset, which has 1,039 firmware representing 693 unique Cortex-M devices, and 694 additional Nordic firmware without the device info in total.
%The firmware come from the real-world embedded Bluetooth Low Energy (BLE) devices.
%They are collected by crawling and unpacking the mobile apps on the Google Play which have used the BLE relevant APIs.
%Since usually the update process of the BLE embedded devices relies on the mobile apps to transfer the firmware data,
%many vendors directly embedded the firmware image inside the mobile app.
%We cannot confirm the actual device model since they are not provided along with the dataset.

%We notice that some firmware in the dataset have the same filename, but with different hash value.
%After looking into those, we found that they are actually different version of the firmware for the same device,
%so we pre-filter the dataset with device model, and that leave us 431 Nordic and 25 TI firmware for different device models.
%We developed ??? lines of Python code atop Ghidra~\cite{ghidra}.

%To facilitate reverse engineering, 
%we looked into the open-source RTOS code to %locate the task stack overflow error handling function, and 
%find hard-coded error messages,
%~\cite{freertostaskovfchk, rtx5config}.
%Most open-source RTOS distributions will provide the compiler option to enable the task stack overflow checks.
%Thus, we look into their source code to locate the task stack overflow error handling function, which usually prints out a hard-coded error string when triggered.
%We searched the hard-coded message, 
%e.g., ``\verb|Stack overflow|" in CMSIS RTOS2~\cite{cmsisrtos2ovf}, and 
%First, we perform a general search of the \verb|stack| string over the dataset.
%For each result, we manually filter out noisy strings and only look for the fixed error strings that will be printed out when the task stack overflow happens.
%Once found, we also examine its disassembly to ensure the corresponding function is inside a call tree.

%However, the \verb|__stack_chk_fail| function may be overridden by a custom implementation, and in this case, it may not print out the default error string.
%Since the stack canary checks are instrumented in the function prologue and epilogue, we also try to find these specific check patterns in the disassembly code.
%We first compile a simple project using three different prevalent Arm compilers with the stack canaries enabled, and based on the checks in function prologue/epilogue, we create three different pairs of regular expression patterns.
%Then we search the disassembly code to find matches of those patterns.
%If a firmware has used both the prologue and epilogue checks in one of the pattern pairs, we consider stack canaries are deployed.

\begin{comment}
	\verb|CONTROL| register related analysis:
	The \verb|CONTROL| register can be used to specify the current privilege level and current stack pointer.
	%For each \verb|MSR| instruction that changes the \verb|CONTROL| register, we back-trace the instructions that update the source register and calculate the value.
	We create patterns to search for the change of the \verb|CONTROL| register with \verb|MSR| instruction, and get the corresponding source register value.
	Based on the first and second bit of the source value, we are able to determine whether this instruction changes the privilege level, or switches the current stack.
	
	\emph{Stack canary analysis:}
	We consider a generic clue in a given binary to detect the deployment of stack canaries in stripped raw binaries, 
	which is the fixed stack smashing error message string ``\verb|*** stack smashing detected ***|''~\cite{yu2022building}.
	This is the default string that is printed out by the error handling \verb|__stack_chk_fail| function, which is provided by the C library.
	We first search for this string within the dataset. Once found, we check the disassembly code to locate the function and ensure other functions call it.
	If the function is in a valid calling tree, we consider it using stack canaries.
	However, the \verb|__stack_chk_fail| function may be overridden by a custom implementation, and in this case, it may not print out the default error string.
	Since the stack canary checks are instrumented in the function prologue and epilogue, we also try to find these specific check patterns in the disassembly code.
	We first compile a simple project using three different prevalent Arm compilers with the stack canaries enabled, and based on the checks in function prologue/epilogue, we create three different pairs of regular expression patterns.
	Then we search the disassembly code to find matches of those patterns.
	If a firmware has used both the prologue and epilogue checks in one of the pattern pairs, we consider stack canaries are deployed.
\end{comment}

\begin{comment}
	\emph{RTOS identifying and task stack overflow checks analysis:}
	%To identify RTOS in statically-linked, stripped binaries, we use a generic heuristic.
	We observe that, for the firmware that use the open-sourced RTOS distributions, some software development toolkit (SDK) path information will be embedded in the binary after compilation.
	For instance, for a firmware that implements FreeRTOS, the SDK path string like \verb|SDK\external\freertos\source\tasks.c| will be inside the binary.
	These kinds of strings can be found as simple as by performing a \verb|strings| search over the binary.
	To get concrete results, we first perform a string search among popular RTOS distributions such as \verb|freertos|, \verb|mbed-os|, \verb|zeyphyr|, etc.
	Once found a valid result, we disassemble the binary and locate the functions that use this string.
	If the function is located and inside a call tree, we consider that the corresponding RTOS distribution is identified.
	
	We use a similar approach in identifying the RTOS task stack overflow checks.
	Most open-source RTOS distributions will provide the compiler option to enable the task stack overflow checks~\cite{freertostaskovfchk, rtx5config}.
	Thus, we look into their source code to locate the task stack overflow error handling function, which usually prints out a hard-coded error string when triggered.
	First, we perform a general search of the \verb|stack| string over the dataset.
	For each result, we manually filter out noisy strings and only look for the fixed error strings that will be printed out when the task stack overflow happens.
	Once found, we also examine its disassembly to ensure the corresponding function is inside a call tree.
	
	By using this approach, it is possible to miss some positive results. However, with manual checking, the false positive rate is also minimized.
\end{comment}

%\emph{Other analysis:}
%The rest of analysis are based on the fixed instruction or code scheme.
%We search for the \verb|SVC| instructions and if a firmware uses it without any changes of the privilege level, we consider it uses SVC for library call.
%Same approach applies for finding the usage of stack limit registers.
%To find out whether a firmware has properly enforced the instruction synchronization barrier, we look for the \verb|ISB| instruction within 10 instructions after the update of \verb|CONTROL| register.
%The MPU, sMPU, and read back protection are enforced by changing the value of their specific registers which have fixed addresses.
%We search for these addresses in disassembly to see whether they have been modified to determine the usage of those security features.

%===========================CVE============
% Besides ``Arm", we identified the top microcontroller vendors by market sizes~\cite{mcumarkets}, the most popular RTOSes by market growth~\cite{rtosmarket}, and popular used SSL library (Mbed TLS~\cite{Mbedtls}, wolfSSL~\cite{wolf}).
% After confirming a vendor builds Cortex-M based products or an RTOS supports Cortex-M, we retrieved bug reports from 2017 to 2022 in the CVE dataset~\cite{mitrecve} by searching the vendors, products, and RTOSes' names.
% In this step, we retrieved more than 500 bug reports covering hardware and software vulnerabilities.
% Then, we conducted a manual analysis of each report, including verifying the affected chips and inspecting the source code, to confirm the bug indeed affects Cortex-M based systems.
% In addition, two researchers worked together to categorize each bug into a relevant subclass, which is double-checked by a third researcher.

%[Explain the results, why vendor scores are low, RTOSes scores are high.]

\begin{comment}
	%To have a better understanding of threats to current Cortex-M productions, 
	%we analyzed bug reports from the CVE dataset~\cite{mitrecve} that cover hardware designs to software implementations work on Cortex-M processors.
	%In the Arm ecosystem, starting from the Arm license, there are SoC vendors that provide hardware solutions 
	%We followed the top MCU designers list~\cite{mcumarkets} and IoT operating system market trend report~\cite{rtosmarket} to select our keywords for searching relevant CVEs, e.g., the vendor names, ``NXP", or the RTOS names, ``FreeRTOS".
	%We gathered additional CVE reports for Arm company, which related to the Cortex-M architecture, the TrustZone technique for Cortex-M, and a secure firmware implementation named Trusted Firmware-M (TF-M).
	%We also collected the bug reports for Nordic~\cite{nordic} since the firmware dataset covers this vendor.
	Since most of those vendors and RTOSs also support other processors such as Cortex-A, RISC-V, 8-bit microcontrollers, etc.
	We have three groups to identify those bug reports to ensure they are meaningful.
	The first group gathers all CVEs based on keywords.
	The second group inspects the source code and affected boards to confirm if this bug can affect the Cortex-M processor.
	Finally, the third group cross-checks those bug reports and categorizes them into different classes, which we will discuss in \S\ref{sec:ImpIssueVul}.
	
	As Table~\ref{tab:sum} shows, we finally collected bug reports for a total of 9 vendors, including NXP Semiconductors~\cite{NXP}, Microchip Technology~\cite{Microchip}, ST Microelectronics (ST)~\cite{STM}, Texas Instruments (TI)~\cite{texasi}, Cypress Semiconductor~\cite{Infineon}, Silicon Laboratories~\cite{silabs}, Gigadevice~\cite{gigadevice}, and Nordic, 
	and 7 RTOSs, including Mbed OS~\cite{MbedOS}, RIOT-OS~\cite{RIOT}, FreeRTOS~\cite{freertos}, Contiki-ng~\cite{ContikiNG}, CMSIS RTOS2~\cite{cmsisrtos2}, Zephyr~\cite{Zephyr}, and Azure~\cite{copeland2015microsoft}.
	%Nuttx~\cite{nutt2007nuttx}, 
	%Arm official provided solutions such as the Cortex-M TrustZone (TrustZone-M) and Trusted Firmware-M (TF-M), 
	%from top 10 MCU designers~\cite{mcumarkets}
	%and widely adopted RTOSes on embedded devices from system market trend %report~\cite{rtosmarket}.
	%For the RTOSes, we checked 
	%We also collected bug reports of  etc.
	%Still, those MCU designers have other hardware architectures such as RISC-V, we further checked the influenced boards of the bug reports from the vendor's product websites to only collect Cortex-M related ones.
	%Renesas Electronics~\cite{Renesas}, 
	%Infineon Technologies~\cite{Infineon},  Nuvoton~\cite{Nuvoton}, Toshiba~\cite{Toshiba}.
	%Besides RTOSes, there are firmware libraries for IoT net connection, e.g., wolfSSL~\cite{wolf}, Mbed TLS~\cite{Mbedtls}, and software implementation, e.g., STM32 cryptographic firmware library~\cite{stm32cve}).
	%\textit{Classification of disclosed security vulnerabilities:}
	We follow the qualitative ratings of those bugs based on the assigned CVSS attribute score~\cite{cvss}, which represents the severity of a vulnerability into critical (CVSS $\ge$ 9.0), high (CVSS [7.0, 8.9]), medium (CVSS [4.0, 6.9]), and low (CVSS [0.1, 3.9]).
\end{comment}

% means the bug can lead to a complete compromise of the whole system, high (CVSS[]) 


%0.1 – 3.9	Low
%4.0 – 6.9	Medium
%7.0 – 8.9	High
%9.0 – 10.0	Critical

%==================paper=====
%They are
%We review projects in securing Cortex-M based software systems 
%from top venues for academic research in system and security, e.g., IEEE S\&P, USENIX security, CCS, NDSS, DAC, DATE, RTAS, etc.

%=============threat to validity========
\begin{comment}
	Our analysis results may have some biases and imprecisions because of 
	(i) incomplete datasets of Cortex-M based firmware samples.
	Though we collected as many open-source datasets as we can, a huge number of marketing devices are close-source and lack investigations,
	resulting in biased observations in real-world firmware images.
	Therefore, we put extra care to seek generic issues that affect not only the analyzed firmware samples but also others;
	(ii) missing proof-of-concept exploits and vague CVE descriptions for collected vulnerabilities.
	The lack of information leads to inaccurate classifications of vulnerabilities. 
	We analyzed only the reported vulnerabilities that can be retrieved from GitHub, updated patches, etc.
	As a result, there may exist unknown types of vulnerabilities that could introduce additional security issues.
	(iii) over-presentative of an MCU-based system (e.g., FreeRTOS) or vendors.
	Those systems and vendor-specific MCUs report a larger number of bugs than others.
	(iv) over-claim in research projects.
\end{comment}


%========================hardware limitations and issues
%This section presents Cortex-M processors' hardware architectural limitations and issues with respect to security.
%Cortex-M systems are built on top of hardware.
%The correctness of hardware architecture is the foundation of the whole system.

%[should we use this as a takeaway or summary?]
%The relatively simple Cortex-M hardware has a double-edged implication of its security.
%On one hand it lacks hardware support for finer-grained protections,
%but on the other hand the lack of optimization, e.g., no cache, no branch prediction, no speculative execution, etc., makes them immune to some microarchitectural attacks, such as cache side-channel attacks~\cite{lipp2016armageddon, zhang2016truspy, cho2018prime+}, spectre~\cite{kocher2019spectre}, meltdown~\cite{lipp2018meltdown}, etc.

%For performance and cost considerations, Cortex-M does not come with an MMU; thus, 
%To support real-time operation and avoid non-response to interruption when dealing with a virtual memory translation lookup table missing~\cite{yiu2020definitive},

%As discussed in \S\ref{sec:physicalmemory}, the reserved address space for on-chip SRAM is only 512MB. 
%Most devices only have a physical SRAM of several hundred kilo bytes. 
%For example, the STM32F469I-Eval board only has 384KB of SRAM.

%This exposes Cortex-M software systems to ROP attacks~\cite{hristozov2022toctou}.
%ROP attack: Time-Of-Check Time-Of-Use (TOCTOU) attack on DICE-based attestation

%Thus, after compromising a simple bug, an attacker can automatically control the whole system by scanning the physical address space.
% I02. \textbf{Excessively large TCBs:}
% For those systems that do not implement privilege separation, the whole system is considered to be trusted which is not true.
% [check other TCB size]   
%\issue{Absent ASLR implementations:}
%Without memory virtualization, ASLR, which is widely used on desktops and servers to prevent disclosing other variables from attackers, is hard to implement. 
%The entropy is constrained because of the small memory size, 
%And simply randomize the addresses at boot time can be easily compromised since the software systems on Cortex-M devices usually run days, months, or even years.
%From all analyzed software systems, none of them implement the ASLR.

%On the Cortex-A front, Sanctuary~\cite{brasser2019sanctuary} addresses this issue by utilizing the memory access controller to provide multi-domain isolation for sensitive apps, 
%and vTZ~\cite{hua2017vtz} addresses this by utilizing virtualization.
% uTango~\cite{oliveira2021utango}, which will be discussed in \ref{TrustZone-assisted multi-world system:}, attempts to address this issue by re-configuring the SAU at run-time.

% cloc --exclude-lang=CMake,Markdown,JavaScript,XML,CSS,Tcl/Tk,reStructuredText,YAML,XSD,HTML,JSON,make,Python --exclude-dir=target interface bl2 lib platform secure_fw 117732

interfaces for developers to use~\cite{}.
%Thus, the security of remote attestation is weak since it depends on the correctness of related components' implementation.
%As pointed out in~\cite{cerdeira2020sok}, Cortex-A TrustZone lacks a software-independent integrity reporting mechanism.
%Unfortunately, Cortex-M TrustZone has the same limitation. 
%Therefore, some security features, such as remote attestation, need to rely on trusted external hardware.
%For example, eFuses are used to store keys that are the root of trust for reporting, and code that is the root of trust for measurement needs to be stored on a secure ROM.
% Secure boot ensures the authenticity of the software running on a device by security reporting the software integrity measurements to a remote third party.
% The remote attestation will be implemented in software (e.g. TF-M) since TrustZone-M lacks such hardware mechanisms.
% Then the security relies on the correctness of the trust chain running on the highest privileged level.
% This weakens the security as it requires the correctness of all software of the trust chain running in the highest privileged level.

%-----------hardware issues
\begin{comment}
	\issue{Wide interfaces for state switches:}
	
	\ziming{check this one on Monday}
	%Different from Cortex-A TrustZone that only has one entry point (Secure Monitor Call, aka \verb|SMC|) for entering or leaving the secure state, 
	As discussed in \S\ref{sec:cortexm}, Cortex-M TrustZone supports an unlimited number of entries into either state. %(\verb|SG| for entering the secure state; \verb|BLXNS|, \verb|BXNS| for entering the non-secure state). % as discussed in~\S\ref{sec:subsec:stateswithing}.
	Consequently, the secure state software exposes a wide attack surface. %, shown as the secure service in Figure~\ref{fig:overview}(c) and (d).
	%Therefore, it is challenging to implement a secure channel between a non-secure software component and a secure software component, as SeCReT~\cite{jang2015secret} does for the Cortex-A TrustZone.
	%A vulnerability was found is TF-M implementation that an attacker can access secure keys stored in the TrustZone secure state for there is no authentication check between a caller and its associated key owner (CVE-2021-40327).
\end{comment}

\begin{comment}
	\issue{Information leakage through caches:}
	Even though most Cortex-M CPUs do not have a cache, cache side-channel attacks are possible on Cortex-M CPUs with caches.
	For example, a flaw was disclosed that Mbed TLS allows local users to achieve partial plaintext recovery via a cache side-channel attack (CVE-2018-0498).
	%Though the cache-based side-channel attack to obtain the CBC plaintext on Mbed TLS (CVE-2018-0498) was found on other platform, it may be exploitable on Cortex-M, too.
	%FreeRTOS has a use-after-free vulnerability that can write the cache to the file system by flushing cache operation (CVE-2019-18178).
\end{comment}

%A new vulnerability was found in CVE-2021-35465 showing that context stacking with FPU or vector extension may expose secure information in floating-point or vector registers (MVE) to the non-secure state.
%\verb|VLLDM| instruction marks the Floating-point context as active only after restoring all the secure floating-point registers.
%Then the processor knows the floating-point registers are used by the secure state, which is sensitive.
%If the restoring process starts but is abandoned due to an interrupt, the partially restored floating-point register will be present to or even modified by the non-secure state.

%\issue{Attacks through energy management mechanisms:}
%Some hardware devices feature extra cryptographic unit, 
%Power analysis attacks compromise the security of cryptographic devices through analyzing their power consumption.
%ELMO~\cite{mccann2016elmo} utilizes instruction-level power models to capture differential data-dependent effects as neighboring instructions in a sequence way. ELMOEmulating Leaks for the Arm Cortex-M0 without Access to a Side Channel Lab..
%An Efficient Profiling Attack to Real Codes of PIC16F690 and Arm Cortex-M3~\cite{vafa2020efficient}

\begin{comment}
	\issue{Improper access control via cross-state:}
	%TrustZone provides hardware-level isolation but also introduces the semantic gap between two states.
	Because TrustZone does not authenticate the non-secure caller's access permissions, 
	the non-secure malicious application may utilize NSC to access the non-secure sensitive application's code and data.
	More severe, the non-secure application can execute code that is not allowed to run.
\end{comment}

%Because Armv8-M architecture integrates the same inter-processor debugging mechanism as Cortex-A does,
%the non-invasive version of the Nailgun attack is feasible on Cortex-M devices with multiple processors.
%E.g, LPCXpresso55S69 Development Board~\cite{LPC55S69} features dual-core Cortex-M33 processor.
%Arm CoreLink SSE-200 Subsystem for Embedded~\cite{ArmCoreLinkSSE200} features two Cortex-M33 processors.
%Other Cortex-M SoCs may integrate with Cortex-A processors.
%For example, Azure Sphere MT3620 Development Kit~\cite{MT3620} features one Arm Cortex-A7 core and two general purpose Arm Cortex-M4F cores, STM32MP153A~\cite{STM32MP153A} devices embeds a dual-core Cortex-A7 processor and a Cortex-M4 core, etc. 
%Nevertheless, no related CVEs have been assigned to any Cortex-M SoC yet.

\begin{comment}
	To enhance the security of Cortex-M processors, some vendors (ST, TI, NXP) implement their own hardware features, such as ROM patching for bug fixing~\cite{lpc55s6x} and eXecution Only Memory (XOM)~\cite{STxom, TIxom, NXPxom}.
	However, such hardware features introduce new issues~\cite{schink2019taking, CVE202131532, CVE202222819}.
	For example,
	NXP LPC55S6x MCUs include a custom hardware block named ROM Patch Controller, which is similar to FPB to patch the ROM.
	It is accessible from the non-secure state unprivileged level and designed to fix bugs in the ROM after chip fabrication, resulting in potential attacks to access the secure privileged read-only code.
	As shown in CVE-2021-31532, attackers are able to utilize the ROM Patch Controller to modify run-time ROM APIs, which is secure privileged access only, to reconfigure the SAU regions to gain privilege escalation.
	Attackers can also execute code via a crafted unsigned update firmware because NXP LPC55S69 series chips have a buffer overflow bug in parsing ROM patches before the signature is verified.
	To mitigate such an attack, the vendor should lock the ROM Patcher Controller configuration or set up the non-secure MPU to block the access from the non-secure state.
\end{comment}

%Readback protection prevents sensitive information (e.g., protected firmware, user secrets) leakage in internal storage (e.g., flash)~\cite{sultan2020readback}.
%To support this feature, some vendors implement their own hardware units.

%If not properly designed and checked, debugging features and vendor-specific features can lead to severe consequences, e.g., privilege escalation and IP theft.   
%Vendors and developers must be well of all architectural hardware components, such as TrustZone and debugging interface, when utilizing those components to build a secure system to not introduce new attack vectors.

%==============================================software architecture and issues================
%\section{Empirical Analysis of Real-world Cortex-M Systems}
%\label{sec:SoftwareSystem}

%This section summarizes representative Cortex-M software architectures that are discovered in real-world firmware and presented in the literature, %shows these architectures in the ascending order of security protections they provide.
%followed by the software architectural issues we found in real-world firmware.

%We will discuss 
%ShieLD~\cite{khurshid2022shield} and 
%two dual-world systems RT-TEE~\cite{wang2022rt} and SafeTEE~\cite{schonstedt2022safetee} in \ref{Real-time and secure TrustZone-assisted dual-world system:};

%The trusted kernel at the secure privileged level handles non-secure environment switches and resources access control.
%Non-secure state TEEs can only communicate with each other through secure unprivileged services.

\begin{comment}
	In this way, we identified 66 firmware with FreeRTOS (55 from FirmXRay dataset correspond to 5 unique devices, and 11 from other Nordic dataset), and 13 firmware with Mbed OS (6 from FirmXRay dataset correspond to 3 unique devices, and 7 from other Nordic dataset).
\end{comment}

\begin{comment}
	While there are advancing research on Cortex-M software architectures
	no microkernel, The privileged application and monolithic kernel architectures are the most adopted models in today's production systems. 
	%With Cortex-M TrustZone being introduced, the dual-world architecture may find its market in production systems soon. 
	The software-based virtualization and least kernel privilege architectures are presented in recent research papers to address issues of the privileged application and monolithic kernel architectures.
	The multiple trusted execution environment architecture is another new direction being explored recently to extend the dual-world architecture.
\end{comment}

%\subsection{Detailed Implementations}
% We notice that by default the stack on Cortex-M system is executable. 
% We also find that for bare-metal systems, the stack canaries implementation may involve a fixed stack guard value, which is not secure.

% Q: How many firmware have the MPU setting to set the stack non-executable?

% Q: How many of them implement the stack canaries?
% If there is stack canaries, how often it gets updated?

% \textit{Tasks:}
% \begin{itemize}
	% 	\item Read the documents about how to change the MPU to set the non-executable stack, and search the dataset based on that.
	% 	\item (Done) Directly add the stack canaries settings and compile a firmware; check the disassembly code to see how the stack canaries work.
	% 	\begin{itemize}
		% 		\item If we enable the compiler option \verb|-fstack-protector|, the symbols \verb|__stack_chk_guard| and \verb|__stack_chk_fail()| will also be enabled.
		% 		\item In each function's prologue and epilogue, that \verb|__stack_chk_guard| value will be directly loaded from the \verb|.data| section. (There is a pointer after each function, and that pointer points to the \verb|__stack_chk_guard| value)
		% 		\item If we do not define (override) the above two symbols in the program, a default function  \verb|__stack_chk_fail()| will be used and the compiler will also insert another function \verb|__stack_chk_init()| to set the \verb|__stack_chk_guard| to a fixed value \verb|0xff0a0000|.
		% 		\item If we define those two symbols in our program, the \verb|__stack_chk_guard| will be stored at the \verb|.data| section and the \verb|__stack_chk_init()| function won't be added by the compiler.
		% 		\item The (random) guard word can be generated at runtime before \verb|main()| is called. In this case, it will be stored at the \verb|.bss| section. However, after the first generation, the guard word will be fixed during the whole program lifespan.
		% 	\end{itemize}
	% 	\item Check the FreeRTOS implementation: insert stack canaries and see if it behaves the same with the bare-metal one.
	% 	\item Check the dataset to see how many of them have used the stack canaries.
	% 	\begin{itemize}
		% 		\item %The default \verb|__stack_chk_fail()| function uses the "*** stack smashing detected ***: terminated" string as the output. Can we do a string search on the binaries to find out the use of the default stack guard?
		% 	\end{itemize}
	% \end{itemize}

%\finding{Other security features:}

%Keep adding other interesting things we want to know from addressing other questions.

%Q: What are the other possible security features implemented in the firmware?


% Check the memory barrier instructions like \verb|DSB/ISB. After updating the CONTROL register with an MSR instruction, the ISB instruction should be used to ensure the updated configuration is used for subsequent operations.
%\item Check how many have the implementation of \verb|PendSV_Handler|.
%\item Check how many have the implementation of \verb|SysTick_Handler|.

%\finding{Hardware RNG}
%Are they come with TRNG? 

\begin{comment}
	\subsection{Arm Platform Security Architecture (PSA)}
	Arm PSA~\cite {ArmPSA} standardizes the design of programming environment and firmware interfaces with three isolation levels.
	The Root of Trust (RoT)~\cite{rotv1} in PSA contains security services such as cryptography operations and secure storage that are implemented in a secure partition.
	The secure partition is an isolated execution environment (aka. compartment) that has its private resources and access permission along with one or more security services.
	%  to implement and access security services in the device's root of trust (RoT). 
	% It defines three levels of isolation for different security requirements.
	Isolation level 1 requires the hardware features to isolate the Secure Processing Environment (SPE) and the Non-secure Processing Environment (NSPE).
	% For Cortex-M, to protect SPE, can use TrustZone if support, or a dedicated CPU of multi-core processors, or MPU.
	The SPE is further divided into the Application RoT and the PSA RoT.
	Secure Partition Manager (SPM) is provided by PSA RoT to support partition isolation, management, and interaction for software.
	Isolation level 2 additionally isolates those two RoTs.
	Isolation level 3 further isolates the secure partitions inside SPE.
	%If the design of chips, system software, or devices meet the PSA requirements, it passes the PSA certification~\cite{ArmPSACert}.
	
	% \subsubsection{Other IoT Security Standards and Legislation}
	
	% Besides the PSA, there are other standards refer to security in the IoT.
	% % ISO/IEC 30128~\cite{ISO} is more about the network protocols security.
	% ITU-T Recommendation Y.2060~\cite{ITU-T} OneM2M TS-xxx~\cite{m2m} define security capabilities that the IoT should provide authentication, integrity, access control, and etc.
	% NISTIR 8259A~\cite{fagan2020iot} also recommends device cybersecurity capabilities including data protection, device identification and configuration, etc.
	% The detail of those standards are out of our scope in this paper.
	
	% Such as the National Institute of Standards and Technology’s (NIST’s)
	% European Union Agency for Cybersecurity’s (ENISA’s)
	% Internet of Things Global Standards Initiative
	
	% \subsubsection{Conclusion}
	% Those standards aim to provide a guidance to implement the authentication, data integrity and provenance, privacy protection, identify management, 
\end{comment}

\begin{comment}
	\subsection{Common Libraries and Firmware}
	\label{sec:subsec:libandfirmware}
	CMSIS and TF-M are two libraries used in many software projects for Cortex-M. 
	
	\subsubsection{Cortex Microcontroller Software Interface Standard (CMSIS)}
	
	% CMSIS provides a Hardware Abstract Layer (HAL) for Arm Cortex-based microcontrollers.
	CMSIS, a Hardware Abstract Layer (HAL), %hardware sdefines interfaces to help developers to create reusable codes without knowing the details of the Cortex-M hardware.
	% CMSIS is a vendor-independent hardware abstraction layer for Cortex processors.
	has the following main components: 
	(i) CMSIS-Core(M) provides interfaces to access device peripherals, e.g., MPU, SysTick, etc.;
	(ii) CMSIS-Driver implements communication stacks, file systems, or graphic user interfaces;
	% provides generic peripheral driver interfaces for middleware 
	% and connects microcontroller peripherals with middleware that implements for example communication stacks, file systems, or graphic user interfaces;
	(iii) CMSIS-DSP provides signal processing functions.%, such as math, filtering, matrix, statistical, etc.
	It uses the SIMD instruction set if possible;
	%In specific, the intrinsic functions from CMSIS-core are available for Cortex-M4/M7/M33/M35P/M55 SIMD instruction;
	% collection with over 60 Functions for various data types: fixed-point (fractional q7, q15, q31) and single precision floating-point (32-bit). 
	% Implementations optimized for the SIMD instruction set are available for Cortex-M4/M7/M33/M35P;
	(iv) CMSIS-NN~\cite{lai2018cmsis} implements efficient neural networks;
	% Collection of efficient neural network kernels developed to maximize the performance and minimize the memory footprint on Cortex-M processor cores;
	(v) CMSIS-RTOSv1 and CMSIS-RTOSv2 provide API for Real-time Operation System (RTOS) along with a Real Time eXecutive (RTX) implementation, which manages multi-thread;
	%(vi) CMSIS-RTOSv2 extended CMSIS-RTOSv1 to support Armv8-M, dynamic object creation, binary compatible interface, and provisions for multi-core systems;
	%(vii) CMSIS-SVD formalize the system description such as the memory mapped registers of peripherals.
	%It can be used for device-specific debug views of peripherals and to generate CMSIS compliant device header files;
	(vi) CMSIS-DAP interfaces to the DAP;
	(vii) CMSIS-Zone helps partition resources into projects and execution areas. 
	%the management for security partitions which are either the project zone that defines the memory resources and peripherals or the execution zone protected by an MPU.
	It generates the protection code that uses SAU, MPC, PPC and MPU. %linker scripts, and other sub-system resources. 
	
	% CMSIS defines generic tool interfaces and enables consistent device support. 
	% The CMSIS software interfaces simplify software reuse, reduce the learning curve for microcontroller developers, and improve time to market for new devices.
	
	\subsubsection{Secure Communication Libraries}
	Mbed TLS~\cite{Mbedtls} implements Transport Layer Security (SSL/TLS) and Datagram Transport Layer Security (DTLS) protocols to provide secure communications, cryptography, and key management for the embedded environment.
	Mbed TLS has a standalone version for bare-metal systems and an OS version.
	WolfSSL~\cite{wolf} is another SSL library used on Cortex-M software systems. 
	For example, the Zephyr project integrates a modified Mbed TLS, FreeRTOS can integrate either the Mbed TLS module or wolfSSL.
	
	\subsubsection{Embedded Crypto Library}
	Post-quantum crypto library for the Arm Cortex-M4
	
\end{comment}

%similar to Mbed TLS but slightly different in several implementations of crypto algorithms.

%Mbed TLS~\cite{Mbedtls} is a C library that designed mainly target for embedded environment and can also work on other platforms like Win32/64, Linux, Android, iOS, and even the XBox.
%It implements Transport Layer Security (SSL/TLS) and Datagram Transport Layer Security (DTLS) protocols to provide secure communications, cryptography, and key management.
%All those functions are configurable and can be used separately to meet different design requirements.
%Thus, Mbed TLS has the standalone version which is portable for bare-metal systems and the OS version.
% The functionalities of wolfSSL~\cite{wolf} is similar to Mbed TLS but slightly different in several implementations of crypto algorithms.
% wolfSSL supports a wide range of platforms including desktop such as FreeBSD, Windows, embedded software systems such as FreeBSD, TinyOS, .
% embedded and RTOS environment, desktop including Windows, .

%\subsubsection{Trusted Firmware M (TF-M)}
%TFM implements a large number of services and has a TCB of 150+KB.
%To support different Cortex-M devices for variety requirements, TF-M has 3 isolation profiles~\cite{TFMDoc} followed the PSA requirements for 
%i) limited-resources IoT devices that only need weak isolation and light crypto (symmetric);
%ii) cloud connected devices that require complex cipher (both symmetric and asymmetric) and higher isolation;
%iii) and less resource-constrained devices with additional isolation between applications and attestation.
% secure storage, cryptography, attestation, secure boot



%i) \emph{Audio-Playback} reads and plays audio from the SD card; 
%ii) \emph{FatFs\_uSD} implements a FAT filesystem on an SD card;
%iii) \emph{LibJPEG\_Encoding} reads a BMP file from SD card, encodes it to jpeg, then same back to the SD card.
%\emph{LCD\_Animate} can display multiple layers of bitmap images to create animation.
%\emph{Pinlock} compares a hashed pin number with a known hash to decide to lock or unlock a digital lock.
%All those projects have no more than 3 kloc and share the same privilege.

% \begin{table*}[!htpb]
	%   \center
	%   \scriptsize
	%   \caption{Bare-metal Projects}
	%   \label{tab:softpack}
	%   \begin{tabular}{llllll}
		%   \hline
		%   Project   & Company  & Series  & CPU & Toolchain & Code size\\ \hline  \hline
		%   STM32CubeF4 App~\cite{STM32CubeF4}            & STMicrocontroller & STM32    & M4F & EWARM, MDK-ARM, SW4STM32\\
		%   atmel-software-package~\cite{atmelcorp}   & Atmel             & SAM V71 & M7F & GCC-ARM\\
		
		%   \hline
		%   \\                                                                    
		%   \end{tabular}
	% \end{table*}

%How do we know how many systems on Cortex-M are like this?? Any citation to support x\% are bare-metal.
%STM32CubeF4 App~\cite{STM32CubeF4}, atmel-software-package~\cite{atmelcorp}.

%Most of those systems are designed for specific devices, but can be exported to others.
%Table~\ref{tab:stm32cubef4} shows some real world projects~\cite{STM32CubeF4} with ARM-GCC toolchain for STM32 series board.
%For example, \textbf{Audio-Playback} reads and plays audio from the SD card. 
%\textbf{FatFs\_uSD} implements a FAT filesystem on an SD card.
%\textbf{LibJPEG\_Encoding} reads a BMP file from SD card, encodes it to jpeg, then same back to the SD card.
%\textbf{LCD\_Animate} can display multiple layers of bitmap images to create animation.
%\textbf{Pinlock} compares a hashed pin number with a known hash to decide to lock or unlock a digital lock.
%All those projects have no more than 3 kloc and share the same privilege.

%\subsubsection{Operating Systems}
% RTOS is a time constrained system that schedules the thread of execution by examining its priority which is either assigned by users or fixed in the system.
% Almost all RTOSes that support resource constrained devices lack the complete protection.
% The security of RTOS runs on Cortex-M differs on Armv7-M and Armv8-M architectures.
%For example, Tock~\cite{levy2017multiprogramming} runs its kernel at the privileged level and applications at the unprivileged level.
%FreeRTOS~\cite{freertossec} puts the heap memory at the privileged access only area and runs the kernel at the privilege level, then allows tasks to run in either privileged level or unprivileged level. 


\begin{comment}
	%uClinux is different from mainstream Linux in that:
	There is no dynamic heap or stack on uClinux, %cannot increase the size of its available memory at run-time, which means there is no dynamic stack or heap.
	which only supports allocations on stack at compile time. %and implements a global memory pool for extra memory obtain. 
	Applications on uClinux uses \verb|vfork()| instead of \verb|fork()| to spawn a child,
	and both the parent and child share the same memory space including the stack.
	\verb|vfork()| suspends the parent's execution until the child process finishes.
	%iii) It creates a new binary object code format, the flat format, to store executable code and data, and relocations that will be used to load the executable into memory.
	% As for other program loader, such as ELF, will be modified to use absolute references by kernel.
	The \verb|mmap| system call is also modified to guarantee sequential and contiguous mapping for the filesystem. 
	%Then the file can be directly addressable by CPU. Thus, the romfs filesystem is used to store files contiguously.
\end{comment}


%Mbed OS offers two security components: (i) the Secure Partition Manager (SPM) that implements based on TF-M and also works for Armv7-M architecture via the MPU; (ii) the communication protection which can be the Mbed TLS or wolfSSL. 

% Confirm Zephyr no privilege separation: https://docs.zephyrproject.org/latest/security/security-overview.html, but the 
% confirm RIOT OS: https://github.com/RIOT-OS/RIOT/blob/73ccd1e2e721bee38f958f8906ac32e5e1fceb0c/core/init.c
% Confirm NuttX: https://github.com/apache/incubator-nuttx/tree/master/syscall

\begin{comment}
	% Some of them do have other security features.
	OSes provide different levels of support for stack protection. 
	Some support stack cookies for functions.
	For example, RIOT OS provides helper functions to support applications to use GCC's stack smashing protector to detect stack buffer overflow.
	%  by checking if the secret value on the stack is changed.
	% https://doc.riot-os.org/group__sys__ssp.html
	%There are other RTOSes that split the privilege.
	%Tock~\cite{levy2017multiprogramming} runs its kernel at the privileged level and applications at the unprivileged level.
	%FreeRTOS~\cite{freertossec} puts the heap memory at the privilege section and runs the kernel at the privilege level, then allows to create tasks to run in either privileged level or unprivileged level.
	% Tock also writes kernel in Rust that can deal with out-of-bounds pointers and dangling pointers.
	% Confirm FreeRTOS privilege separation: https://www.freertos.org/FreeRTOS-MPU-memory-protection-unit.html
	% Besides TF-M, several RTOSes also provide extra security features.
	% For example, 
	FreeRTOS can detect the stack overflow by setting a stack limit or filling last 20 bytes of the task stack with a known value (\verb|0xee|) when creating the task~\cite{freertoskernel}.
	% FreeRTOS known stack value pattern: https://github.com/FreeRTOS/FreeRTOS-Kernel/blob/a8a9c3ea3e34c10c6818f654883dac3dbdae12d1/portable/MPLAB/PIC32MX/port.c
	Zephyr project protects the stack by either configuring \verb|PSPLIM| if the hardware support or set the MPU-based stack guard.
	%config ARM_STACK_PROTECTION: https://github.com/zephyrproject-rtos/zephyr/blob/16c61ca424d20ca6f3952588dbf6d783f045ce67/arch/arm/core/aarch32/Kconfig
	% mpu guard: https://github.com/zephyrproject-rtos/zephyr/blob/2bed37e534870cabb95766c6b18b1e2c78818ace/arch/arm/core/aarch32/cortex_m/mpu/arm_core_mpu.c
	% https://github.com/zephyrproject-rtos/zephyr/blob/2bed37e534870cabb95766c6b18b1e2c78818ace/arch/arm/core/aarch32/cortex_m/mpu/arm_core_mpu.c
\end{comment}


% Azure Sphere~\cite{stiles2019hardware} is another special IoT solution from Microsoft and works on an Azure Sphere certified chip that provides dependable hardware RoT.
% It has a secure MCU that consists of multiple cores: one Cortex-A7 runs a Linux kernel, and two Cortex-M4 cores run bare-metal applications, or RTOS such as Azure RTOS or FreeRTOS.
% The subsystem runs on Cortex-A core provides crypto engine, remote attestation, and various tampering counter-measures.

% Zephyr later will provide stack protection and privilege separation.

\begin{comment}
	\subsubsection{Mbed OS}
	
	Mbed OS~\cite{MbedOS} is designed for Cortex-M devices that runs both bare-metal systems and RTOS.
	The general architecture has three layers built on the hardware:
	(i) A hardware abstraction layer (HAL) to provide the hardware components such as timers, crypto, and peripheral drivers~\cite{MbedArch};
	(ii) On top of HAL are the OS resources which contain two security blocks: Mbed TLS and Secure Partition Manager (SPM). 
	The Mbed TLS is a comprehensive SSL/TLS solution that includes cryptographic primitives and network protocols to secure the network communication. 
	The SPM meets the PSA to protect the SPE integrated with TF-M (v1.1)~\cite{MbedPSA}.
	Mbed SPM also works on single-core Armv7-M targets via privilege separation;
	(iii) The upper layer are user applications and IoT connectors such as AWS and Google.
	In specific for bare-metal systems, Mbed security only supports the crypto, secure key, and TLS.
	% \subsubsection{Contiki-NG}
	% Contiki-NG~\cite{ContikiNG} 
	
	\subsubsection{FreeRTOS}
	FreeRTOS~\cite{freertos} is a kernel built on top of embedded applications to meet real-time constraints.
	Its security~\cite{freertosesec} benefits from the fully integrated TF-M and only supports Armv8M.
	MPU and TrustZone are configurable to provide privilege separation and physical isolation.
	It also provides a simple security mechanism that can detect the stack overflow by checking the valid stack space or filling a known value at the last 16 bytes of the task stack~\cite{freertoskernel}.
	% It schedules the thread of execution called a task by examining its priority.
	% It supports preemptive or cooperative operation along with basic features including task priority assignment, semaphores, mutexes, queue management, trace recording, and etc~\cite{freertoskernel}.
	% FreeRTOS uses three strategies to allocate the memory: fixed memory allocation, best-fit memory allocation, and custom memory allocation.
	% To minimize the RAM usage and simplifies kernel APIs, the memory of kernel objects are dynamically allocated at run-time and can be freed after deleting a kernel object.
	% Unlike MBed OS, FreeRTOS does not have the HAL so it is hard to port.
	% [FreeRTOS use the term task instead of thread]
	
	% Restrict dynamically allocate the memory at boot time. stack overflow checking
	
	% \subsubsection{Hafnium}
	
	\subsubsection{Azure Sphere}
	
	Azure Sphere~\cite{stiles2019hardware} is an IoT security solution by Microsoft.
	It contains a secured MCU to provide fundamentally secured computing, a custom Linux-based OS, and a cloud-based security service that supports authentication, software update, and error reporting~\cite{AzureSphere}.
	A secure MCU consists multiple cores and each core runs a subsystem with crypto engine, remote attestation, and various tampering counter-measures.
	To develop Azure Sphere, an Azure Sphere Development Kit is needed.
	
	\subsubsection{Tock OS}
	
	Tock~\cite{levy2017multiprogramming} is designed to provide the multiprogramming environment for microcontrollers.
	The kernel is written in Rust which is a memory-safe language that deal with out-of-bounds pointers and dangling pointers.
	
	\subsubsection{Other RTOS}
	The security functionality for other RTOSs mainly on the cryptographic libraries,such as RIOT OS~\cite{RIOT}, Zephyr (v2.5.99)~\cite{Zephyr}, etc.
	Zephyr later will provide stack protection and privilege separation.
	
\end{comment}

% Contiki-NG~\cite{ContikiNG} 
% RT-Thread (v4.0.2)~\cite{RTthread} NANO version is designed for MCU systems. Security???


% Composite
% Djyos
% One os -
% Wombat OS
% Xenomai

\begin{comment}
	\begin{table*}[!htpb]
		\center
		\scriptsize
		\caption{Operating Systems}
		\vspace{-0.3cm}
		\label{tab:os}
		\begin{threeparttable}
			\begin{tabular}{llllllllllllll}
				\hline
				Project                                   & Company   & CPU & \rotatebox{90}{Privilege separation}  & \rotatebox{90}{language}  & \rotatebox{90}{Root of Trust} &  \rotatebox{90}{DEP} &\rotatebox{90}{secure storage}  &\rotatebox{90}{crypto} & \rotatebox{90}{attestation} & \rotatebox{90}{secure boot} & \rotatebox{90}{fault isolation} & \rotatebox{90}{stack protection}\\ \hline  \hline
				Zephyr Project &    &  & \supportlevel{10} &C&\supportlevel{10}&&\supportlevel{10} & &  &\supportlevel{10} &&\supportlevel{10} \\
				Mbed OS full profile~\cite{MbedOS}   & Arm   & All & \supportlevel{10} &C/C++&\supportlevel{10}&& \supportlevel{10} &\supportlevel{10} & \supportlevel{10} & \supportlevel{10} \\
				Mbed OS bare-metal profile   & Arm   & All & \supportlevel{10} &C/C++&&&  &\supportlevel{10} &  & \supportlevel{10} \\
				FreeRTOS~\cite{freertos}  & Amazon   &M23/33 & \supportlevel{10} & C &\supportlevel{10}&\supportlevel{0} & \supportlevel{10} & \supportlevel{10} & \supportlevel{10} & \supportlevel{10} &  & \supportlevel{10}\\
				&         &M3/4/7 & \supportlevel{10} & C &&\supportlevel{0} &  &  &  &  &  & \supportlevel{10} \\
				% Azure Sphere~\cite{stiles2019hardware}  & Microsoft & A7+M4 &\supportlevel{10}&C&\supportlevel{10}&&&\supportlevel{10}&\supportlevel{10}&\supportlevel{10} \\
				% Contiki-NG~\cite{ContikiNG} & Contiki-NG &M0/M0+/M3/M4/M7/M23/M33&& \\
				% Mbed $\mu$Visor~\cite{uVisor}     & Arm   & Separated &&&&  - \\
				OneOS~\cite{oneos}  & & All & \supportlevel{10} &  && &&&&& & \\
				RIOT OS~\cite{RIOT}   & RIOT &M0/0+/3/4 &&C/C++&&&\supportlevel{10} \\
				RT-Thread~\cite{RTthread} & RT-Thread &M33&\supportlevel{10}&C&\supportlevel{10}&&\supportlevel{10}&\supportlevel{10}&\supportlevel{10}&\supportlevel{10}\\
				& &M0/0+/3/4/7/23&-&C&-&&&\supportlevel{10 }&&\\
				TockOS~\cite{levy2017multiprogramming}  & &M0/3/4& \supportlevel{10} & Rust,C/C++ && &&&&&\supportlevel{10} &\supportlevel{10} \\
				\hline
			\end{tabular}
			\begin{tablenotes}    
				\item[] \supportlevel{0}: Not support, \supportlevel{10}: Support
			\end{tablenotes}
		\end{threeparttable}
	\end{table*}
\end{comment}

%\subsection{Summary of software systems on Cortex-M}

%Interestingly, even though some firmware enables MPU, %to configure access permission,
% Even if MPU may be enabled on these systems, 
%such as isolation of privileges, even if the underlying hardware provides corresponding supports.
%the settings can be reverted as everything runs at the privileged level.

%Even though some Cortex-M devices have MPU, % for memory access control, previous research believes that most real-world systems do not use it~\cite{clements2017EPOXY, zhou2019good, clements2018aces}. 
%For the same reason, data execution prevention (DEP) %, a standard feature in modern operating systems, 
%is not enforced on these systems.
%Without memory access control,

\begin{comment}
	\issue{Missing readback protection:}
	As discussed in \ref{Bypassable vendor-specific readback protection:}, Nordic MCUs implement a readback protection mechanism.
	%We The mapped registers to setup the mechanism for different series.
	%By checking the operation on those registers, 
	Notwithstanding, we found that only found 32 out of the 1,458 Nordic samples in our dataset enable this feature. 
	%and 6 of them use the nRF51 flawed readback protection.
	
	\issue{No or weak guards between memory segments:} 
	Guard pages are used on microprocessor-based systems to %usually inserted by operating systems to 
	delimit the boundaries of segments %, such as stack and code, 
	to prevent accidental and intentional overwriting. % from an adjacent segment.
	%Due to the small address space and limited number of MPU regions, it is not efficient to implement guard pages on Cortex-M. 
	%To alleviate this issue, 
	As discussed in \S\ref{sec:cortexm}, Armv8-M also introduces stack limit registers to delimit the boundaries of stacks.
	However, no firmware in our dataset has been used them. %stack limit registers.
	
	\emph{RTOS Implementations:} 
	We found that only a few RTOSs design mechanisms to protect tasks' stacks, and only Zephyr optionally supports using stack limit registers.
	When stack guard is enabled, FreeRTOS~\cite{freertoskernel} and Mbed OS~\cite{rtx5config} insert a predefined delimiter to mark the boundary of each task's stack.
	%a predefined 20-byte delimiter (\verb|0xA5|) to mark the low limit of the stack, which will be checked when a context switch happens.
	Zephyr can use either \verb|PSPLIM| or an MPU-configured memory guard to prevent overwriting beyond a task's stack~\cite{zephyrstackguard}.
	
	\emph{Empirical Analysis on Real-world Firmware:}
	59 of the 66 FreeRTOS-based firmware samples and 7 of the 13 Mbed OS-based firmware samples use task stack overflow guards.
	
\end{comment}

\begin{comment}
	\emph{Compiler and RTOS Implementations:} We found that the GNU Arm Embedded Toolchain (\verb|arm-none-eabi-gcc|, version 10.3.1)~\cite{armgcc}, Arm Compiler 5 (\verb|armcc|, version 5.6u7)~\cite{armcc}, and Arm Compiler 6 (\verb|armclang|, version 6.16)~\cite{armclang} all implement the same canary mechanism as their x86/64 counterparts.
	The feature, however, is disabled by default in all three compilers~\cite{stackarmclang, stackarmcc}.
	%In contrast, it has been a default feature of GCC since Ubuntu 6.10 in 2006~\cite{ubuntucookie}.
	More seriously, different from MMU-enabled systems where \verb|__stack_chk_guard| is a global variable in each process' virtual memory, 
	on Cortex-M there is only one \verb|__stack_chk_guard| in the whole physical address space.
	%As a result, different tasks running on RTOS will have the same canary value.
	RIOT-OS adopts compile-time canary randomization, which ensures each build has a unique canary~\cite{riotstack}.
	Zephyr~\cite{zephyrstackcode} randomly initializes a canary value at boot time.
	%Then the value stays the same until the next reboot.
	Moreover, if the canary value is not initialized explicitly, \verb|arm-none-eabi-gcc| uses a fixed terminator canary (\verb|0xff0a0000|), 
	whereas both \verb|armcc| and \verb|armclang| use \verb|0|.
	In sum, the existing stack canary mechanism designed for process-based OSs is weakened in the single physical address space setting; therefore, a new mechanism with frequent canary updates is needed for Cortex-M and other MCU systems.
\end{comment}
%\emph{Empirical Analysis on Real-world Firmware:}
%Even if the aforementioned compilers offer the canary mechanism, 

%========================================================software implementation bugs====================
%In addition to hardware and software architectural issues, software implementation bugs are also critical. %embedded devices are also influenced by software implementations.
%Given the wide range of Cortex-M system usage scenarios,
%With a variety of usage scenarios on Cortex-M processor powered devices, 
%their software systems also exhibit a variety of structures and have different components.
\begin{comment}
	\begin{table}[!t]
		\center
		\scriptsize
		\caption{Number of disclosed CVEs from 2017 to 2022}
		\vspace{-0.2cm}
		\setlength\tabcolsep{0.55ex}
		\renewcommand{\arraystretch}{1.1}
		\label{tab:sum}
		\scalebox{0.92}{\begin{threeparttable}
				\begin{tabular}{l|c|c|c|c|c}
					\hline
					\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Critical} & \multicolumn{1}{c|}{High} & \multicolumn{1}{c|}{Medium} & \multicolumn{1}{c|}{Low} & \multicolumn{1}{c}{Total} \\ \hline \hline
					\begin{tabular}[c]{@{}l@{}}Arm, Microchip Technology, Silicon Labs,\\NXP Semiconductors, ST Microelectronics,\\Cypress Semiconductor, Gigadevice, Texas\\Instruments, Nordic\end{tabular} & \begin{tabular}[c]{@{}c@{}}4\\ (5.80\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}24\\ (34.78\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}41\\ (59.42\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}-\\		\end{tabular} & 69    \\ \hline
					\begin{tabular}[c]{@{}l@{}}FreeRTOS, CMSIS RTOS2, Mbed OS, Ze-\\phyr, RIOT-OS, Contiki-ng, Azure\end{tabular} & \begin{tabular}[c]{@{}c@{}}45\\ (33.09\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}67\\ (49.26\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}23\\ (16.91\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}1\\ (0.74\%)\end{tabular} & 136   \\ \hline
					\begin{tabular}[c]{@{}l@{}}Mbed TLS, WolfSSL\end{tabular} & \begin{tabular}[c]{@{}c@{}}17\\ (22.67\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}28\\ (37.33\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}30\\ (40.00\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}-\end{tabular} & 75   \\ \hline
					Total & \begin{tabular}[c]{@{}c@{}}66\\ (23.57\%)\end{tabular}& \begin{tabular}[c]{@{}c@{}}119\\ (42.50\%)\end{tabular}& \begin{tabular}[c]{@{}c@{}}94\\ (33.57\%)\end{tabular}& \begin{tabular}[c]{@{}c@{}}1\\ (0.36\%)\end{tabular} & 280\\ \hline                                                             
				\end{tabular}
				%\begin{tablenotes}
				%\item[] The bug reports cover from hardware architecture to software implementation.
				%\end{tablenotes}  
		\end{threeparttable}}
		\vspace{-0.5cm}
	\end{table}
\end{comment}

%This section presents an overview of the hardware and software CVEs on Cortex-M systems from 2017 to 2022 and 
%We are also interested in the nature of these bugs.
%To this end, 

%Figure~\ref{fig:cve_scatters} illustrates the distribution of CVSS scores for Cortex-M related bugs and all bugs~\cite{cve20172023} reported between 2017 and 2023. 
%Due to the factors outlined in \S\ref{sec:HardIssueVul} and \S\ref{sec:SoftIssueVul}, the disclosed Cortex-M related bugs demonstrate noticeably higher severity compared to general bug reports during the same time periods.
%The comprehensive list of bug reports and their detailed classification can be found in our anonymous open-source repository.

\begin{comment} 
	%The score rates the severity of a vulnerability based on its exploitability, affected components, and impact of exploiting this vulnerability.
	It is shown from the table that RTOSs report more security vulnerabilities than vendors.
	In particular, half of the bug reports from vendors are rated as medium, while more than three-quarters of them from RTOSs are rated as critical or high.
	%In particular, 41 of 121 reports (33.88\%) disclosed security vulnerabilities are considered critical.
	However, we cannot conclude that RTOSs are less secure than vendors' implementation. 
	The disparity is due to that (i) most bug reports are from vendors' SDKs, which are used for developers to build chip-specific firmware; 
	(ii) most of the firmwares are bare-metal applications that have fewer system components than an RTOS;
	(iii) RTOS are widely deployed on other platforms and the software implementation vulnerabilities affect not only Cortex-M devices but also other devices powered by Cortex-A, MIPS, etc.
	Nevertheless, these results are useful because they help us understand the security status of current Cortex-M systems, and remind us of how to design a more secure system that avoids vulnerable components.
	
	
	In this section, we focus on the implementation bugs of RTOSs and vendors' IoT solutions, including software development kits (SDK) that help build chip-specific firmware.
	By analyzing related bug reports from public CVE database~\cite{cvss}, we summarize several vulnerable components: (i) wireless communication component supports data transfer between devices or cloud services through network;
	(ii) device driver is required if the system needs to interact with peripherals;
	(iii) dynamic memory management is important to allocate memory for data storage;
	(iv) context switch is necessary if system implements hardware or software assisted isolation (e.g., privilege separation);
	(v) kernel libraries are other functionalities provided by the system.
	%Based on those system components, 
	Table~\ref{tab:CVEs-con} presents the number of bug reports in meaningful categories~\cite{cerdeira2020sok}.
	We will present the details of bug categories below.
\end{comment}

%As the table shows, over half of the reported vulnerabilities are in the communication component (validation bugs in wireless communication and functional bug in protocol implementation) that affect the all analyzed vendors' IoT solutions and RTOSes.
%That is because i) modern embedded systems are network facing and transfer data via wireless communication technology (e.g., Bluetooth, WiFi), which is the most frequently accessed vector by attackers;
%ii) most vendors and RTOSes implement their own communication component to meet different communication requirements. 


%By analyzing our CVE databases, we found most issues come from the wireless communication implementation.
%software implementation causes a lot of vulnerabilities.
%Since embedded devices are used for a variety purpose, 
%This section presents the security issues for existing software systems on Cortex-M processors.
%Following the taxonomy in~\cite{cerdeira2020sok}, those reports are categorized into validation, functional, and extrinsic bugs.
%besides the two known cache side-channel vulnerabilities and one architectural bug, most vulnerabilities are software implementation issues. 
% software implementation introduces the largest number of CVEs with various types.

%That is because IoT devices are network-connected with specifically designed network protocols.
%The vulnerabilities of those protocols leak sensitive information or even allow execution attacks and can influence different versions of software systems.
%For example, the TLS and CoAP library of Mbed and the middleware TCP/IP component of FreeRTOS have buffer overflow and integer overflow vulnerabilities.

%Those CVEs are scored based on their impact on devices ranging from low to critical.
%Over a seventy percent of those vulnerabilities are high or critical, which means they have a severe influence on a large number of devices.

%To have a better understanding of the secure state of software systems for Cortex-M processors, as Table~\ref{tab:sw-CVEs} shows, we manually analyzed bug reports from the CVE database~\cite{mitrecve} that related to some RTOSes and libraries.
%Then those vulnerabilities are categorized based on the different layers.

% Attacks: Smart nest thermostat (blackhat)~\cite{hernandez2014smart},

% \subsubsection{Improper validation of inputs and outputs}

\begin{comment}
	\subsubsection{Memory Safety bugs}
	Memory is safe if and only if the pointer in the program access their intended referents.
	Accessing a memory that is out of bound or accessing a referent that is no longer valid will trigger memory corruptions.
	Those bugs can be the most severe security problems that are frequently used for privilege escalation, arbitrary code execution, information leakage, etc.
	
	% Validation bugs are triggered because the input and/or output values are not handled properly in systems.
	% Including buffer overflows, improper parameter validation, integer overflows, etc.
	% Those bugs are frequently used for 
	
	\issue{Spatial safety bugs:} 
	Accessing a memory that is out of bound constitutes spatial safety bugs.
	Examples like Listing 1 from RIOT-OS (CVE-2021-27697) can copy arbitrary buffer length because it does not check the value of expected\_len, which controls the copy buffer size.
	Or out-of-bounds write from Arm Mbed TLS (CVE-2018-0488) that allow attackers to execute arbitrary code, which may cause Denial-of-Service (DOS).
	An out-of-bounds read on Mbed CoAP lib (CVE-2020-12886) causes a read outside of the intended boundary of the buffer to cause the information leakage.
	Integer overflow (e.g. CVE-2020-10070 on Zephyr Project) also triggers bound errors.
	
	\begin{lstlisting}[label={RIOTcve}, caption={Vulnerability in RIOT-OS~\cite{RIOToscve}. This piece of code utilize buffer copy without checking size of input: expected\_len. Loacated at RIOT/sys/net/gnrc/routing/rpl/gnrc\_rpl\_validation.c}, language=c] 
		case (GNRC_RPL_OPT_PAD1): 
		expected_len += 1; 
		opt = (gnrc_rpl_opt_t *)(((uint8_t *) opt) + 1); 
		continue;  
	\end{lstlisting}
	
	\issue{Temporal safety bugs:} 
	Accessing a referent that is no longer valid triggers the temporal safety bugs.
	Attackers may exploit such bugs to reuse and control the freed region.
	For example, the use after free attack (e.g. CVE-2019-18178) that access a dangling pointer.
	Dereferencing the null pointer from Zephyr Project (CVE-2018-1000800) will cause a CPU page fault, which allows the attacker to call vulnerable kernel APIs.
	
	% \textbf{Bugs in libraries:}
	% Mbed TLS and wolfSSL are lightweight and widely used for RTOSes to provide network communication along with security. 
	% With the bug in those libraries, an attacker is able to crash the library services via DOS attack and steal the sensitive information.
	% Mbed implements TLS and CoAP to help simply the developer's work.
	% I00. \textbf{Vulnerable libraries: information leakage, buffer overflow:}
	
	% \subsubsection{Access level}
	% Vulnerabilities at access level break the access control, authentication, and authorization.
	
	% \subsubsection{Use of Uninitialized Variables}
	
	% \subsubsection{Pointer Type Errors}
	
	\subsubsection{Use of Uninitialized Variables}
	Variables should be initialized to have an indeterminate value.
	The use of uninitialized variables results in undefined behavior.
	
	\issue{Access uninitialized pointer:}
	FreeRTOS frees an uninitialized pointer that can be utilized for remote code execution (CVE-2018-16522).
	Zephyr Project can access uninitialized stack memory (CVE-2020-10060), which may cause a crash, DOS, or information leakage. 
	
	% \begin{lstlisting}[label={FreeRTOScve}, caption={Access uninitialized pointer in FreeRTOS~\cite{RIOToscve}.}, language=c] 
		%   /* Clean-up application protocol array*/
		%   if(Null != pxContext->ppcAlpnProtocols)
		%   {
			%     for(ulprotocl = 0;
			%         ulProtocol < pxContext->ulAlpnProtocolsCount;
			%         ulProtocol++)
			%         {
				%           if(NULL != pxContext->ppcAlpnProtocols[ulProtocl])
				%           {
					%             vPortFree(pxContext->ppcAlpnProtocols[ulProtocol]);
					%           }
				%         }
			%         vPortFree(pxContext->ppcAlpnProtocols);
			%   }
		% \end{lstlisting}
	
\end{comment}

%Validation bugs are further classified depends on different influenced system components.
%We list several bugs below to show the bugs exploited to attack those components.
%We analyzed bugs in different implementation components of production systems.
% Memory is safe if and only if the pointer in the program access their intended referents.
% Accessing a memory that is out of bound or accessing a referent that is no longer valid will trigger memory corruptions.
% Attackers may exploit such bugs to reuse and control the freed region.
% Validation bugs are triggered because the input and/or output values are not handled properly in systems.

\begin{comment}
	\begin{figure}[!t]
		\begin{centering}
			\includegraphics[width=0.48\textwidth]{pics/cve_scatters.pdf}
			%\vspace{-0.8cm}
			\caption{CVSS score distribution of Cortex-M related bugs and all CVE-assigned bugs~\cite{cve20172023} between 2017 to 2023}
			\label{fig:cve_scatters}
		\end{centering}
		\vspace{-0.3cm}	
	\end{figure}
\end{comment}

%By exploiting a bug in communication component, attackers can easy access sensitive information or crash the system.
%Vendors and RTOS implement their own solutions to secure the communication, 
%Those vulnerabilities happen with wireless communication technologies, including Bluetooth low energy, network data parsing, etc.
% \issue{Spatial safety bugs:} 
%Bugs have been discovered in the libraries discussed \S\ref{sec:subsec:libandfirmware}.
%As discussed in , there are libraries for secure communication, which may introduce potential attack surface.

%on vendors' SDKs, 
%including NXP, Microchip, TI, Cypress, and Silicon Labs, 
%have buffer overflow bugs that can trigger denial of services (CVE-2019-19195), 
%allow attackers execute arbitrary remote code (CVE-2018-16986), 
%pair any Bluetooth device (CVE-2019-18614), write arbitrary memory location (CVE-2019-13916), etc.
%Contiki-ng and Zephyr also has buggy Bluetooth implementation that can result in 
%arbitrary code execution (CVE-2020-12140), 
%mory corruption (CVE-2020-10061).
% and denial of services (CVE-2020-10069).
%Besides the Bluetooth, the TCP/IP stack implementation of FreeRTOS, DNS packets handling of FreeRTOS and Contiki-ng also introduce plenty of bugs (e.g., CVE-2021-21281, CVE-2018-16603).

%However, implementation bugs have been reported within the libraries themselves.
%We do not count those bugs in Table~\ref{tab:sum} and Table~\ref{tab:CVEs-con} since these libraries are also used in microprocessor-based systems. 
%, such as personal computers.
%The bug reports database show there are 34 for Mbed TLS and 52 for WolfSSL by the day we check. 


%Contiki-ng has a bug (CVE-2020-14935) to overwrite stack region, including the return address from the vulnerable function, which can redirect the code execution path.
%RIOT-OS (CVE-2021-27697) can copy arbitrary buffer length because it does not check the value of \verb|expected_len|, which controls the copy buffer size.
%The bug (CVE-2019-13120) in FreeRTOS allows attacker to read arbitrary memory when interacting a malformed MQTT publish packet from the attacker.
%RIOT-OS has a buffer overflow bug in its DNS protocol implementation (CVE-2019-1000006).
%FreeRTOS frees an uninitialized pointer in the socket function (CVE-2018-16522).
%Both vulnerabilities can lead to remote code execution.
% Meneghello et al.~\cite{meneghello2019iot} analyzed the security vulnerabilities on real world protocols.
%FreeRTOS also has a bugger overflow bug (CVE-2018-16525) when parsing the DNS/LLVMNR packets that can allow attackers to execute arbitrary code.
%Contiki-NG's SMTP implementation has buffer overflow bugs that can be exploited to overwrite sensitive data (CVE-2020-14934) and hijack control flow (CVE-2020-14935).
%The bluetooth implementation of Cypress WICED BT stack~\cite{WICED} does not restrict link-layer data length on reception~\cite{garbelini2021braktooth}. 
%Zephyr's LwM2M implementation has an infinite loop with malformed input (CVE-2020-13602). 
%Both bugs can cause a denial of service.
%Integer overflow (e.g. CVE-2020-10070 on Zephyr Project) also triggers bound errors.
%FreeRTOS has the integer overflow for a stream buffer (CVE-2021-31572).

\begin{comment}
	Listing 1 from RIOT-OS (CVE-2021-27697) can copy arbitrary buffer length because it does not check the value of expected\_len, which controls the copy buffer size.
	\begin{lstlisting}[label={RIOTcve}, caption={Vulnerability in RIOT-OS~\cite{RIOToscve}. This piece of code utilize buffer copy without checking size of input: expected\_len. Loacated at RIOT/sys/net/gnrc/routing/rpl/gnrc\_rpl\_validation.c}, language=c] 
		case (GNRC_RPL_OPT_PAD1): 
		expected_len += 1; 
		opt = (gnrc_rpl_opt_t *)(((uint8_t *) opt) + 1); 
		continue;  
	\end{lstlisting}
\end{comment}

% ZigBee, Bluetooth Low Energy (BLE), 6LoWPAN and Constrained Application Protocol (CoAP), LoRaWAN.
% \textcolor{blue}{TODO: more details}
% RIOT, Keil RTX, Apache Mynewt, TI-RTOS support wolfSSL.

% \issue{Memory safety bugs within the protocols:}

%Zephyr can elevate privilege when validating syscall numbers with signed integer comparison.
%Zephyr also has a NULL base pointer reference vulnerability in its privileged buffer handling functions, %(CVE-2018-1000800)
%namely \verb|sys_ring_buf_put| and \verb|sys_ring_buf_get|, which can result in memory fault at the privileged level.

%There are other kernel libraries that may crash the system, which are specific for devices or embedded systems.
%This vulnerability can be exploited by malicious applications that trigger such buggy functions.

%TF-M has a bug (CVE-2021-43619) that can overwrite stack memory via the \verb|psa_fwu_write| caller.

% https://github.com/FreeRTOS/FreeRTOS-Kernel/commit/c7a9a01c94987082b223d3e59969ede64363da63


% \begin{lstlisting}[label={FreeRTOScve}, caption={DNS poisoning on FreeRTOS~\cite{RIOToscve}.}, language=c] 
	%   /* Socket listen to the target port */
	%   #if(ipconfigUSE_DNS == 1)
	%   {
		%     if(FreeRIOT_ntoms(pxUDPPacket->xUDPHeader.usSourcePort) == ipDNS_PORT)
		%     {
			%       vARPRefreshCacheEntry(&(pxUDPPacket->xEthernetHeader.xSourceAddress), pxUDPPacket->xIPHeader.ulSourceIPAddress);
			%       xReturn = (Basetype_t)ulDNSHandlePacket(pxNetworkBuffer);
			%     }
		%   }
	%   else ...
	%   #endif
	%   uint32_t ulDNSHandlePacket(NetworkBufferDescriptor_t *pxNetworkBuffer){
		%     uint8_t *pucUDPPayloadBuffer = pxNetworkBuffer->pucEthernetBuffer + sizeof(UDPPacket_t);
		%     DNSMessage_t *pxDNSMessageHeader = (DNSMessage_t *) pucUDPPayloadBuffer;
		%     prvParseDNSReply(pucUDPPayloadBuffer, (uint32_t) pxDNSMessageHeader->usIdentifier);
		%     return pdFAIL;
		%   }
	% \end{lstlisting}

% inadequate encryption strength 


% \textbf{Bugs in libraries:}
% Mbed TLS and wolfSSL are lightweight and widely used for RTOSes to provide network communication along with security. 
% With the bug in those libraries, an attacker is able to crash the library services via DOS attack and steal the sensitive information.

%We identified three types of functional bugs that will break the functionalities of discussed components and lead to security vulnerabilities.
%because the programmer's implementation does not follow the program specification.
%Functional bugs will break the authentication that checks the rights of the code to access the resources, compromise the anonymity that unauthorized users can not read the information, or crash the system.  

%This category targets wireless communication components and focuses on the bugs caused by implementation logistic, showing 18.13\% in .
%When analyzing the bug reports, those are cumbersome
%Similar to the 

%a bug report (CVE-2021-3455) for Zephyr involves a use after free vulnerabilities which leads to device freeze.
% if disconnecting the L2CAP channel right after an invalid ATT request.

%Some systems provide MPU and TrustZone assisted isolation and allow calls between different privilege levels and secure states.
%hardware assisted isolation via MPU or TrustZone, etc

%call 
%the \verb|xPortRaisePrivilege| and \verb|vPortResetPrivilege| 
%the functions that 

% or sensitive information leakage.
%when calling non-secure callable function because unnecessary resources frees . [PLEASE rewrite the TF-M part. Not understandable.]
%TockOS's unprivileged capsule is able to access arbitrary memory (CVE-2018-1000660).
%The bug of Zephyr allows any thread running on the system read and write a socket file descriptor (CVE-2020-10072).
%FreeRTOS MPU platform does not prevent non-kernel code from calling privileged functions to escalate privilege (CVE-2021-43997).
%Besides the memory protection via privilege separation, the file system also faces the risk that the data may be modified.
%For instance, 
%FreeRTOS FAT file system implementation has use after free bug of it (CVE-2019-18178) results in random content written to disk by flushing cache operation.

%[Didn't we say change the title here? security mechanisms are too broad.]

%\gl{I view CVE-2021-32032 as a validation bug.[handled]
	%I'd put CVE-2020-11957 in crypto since it is related to crytpo protocol [The vulnerable function is to generate the Bluetooth pairing key, which belongs to wireless communication, not the crypto key.]
	%}
%that cleans up the crypto context ahead of the lower level clean function, 
%then the latter function cannot locate and free memory, or will access an invalid memory region,
%resulting in system halt or secure data leakage (CVE-2021-32032).
%Zephyr does not check the existing bond with the same identify address during keys distribution phase, resulting possibility to overwrite an existing bond to cause device disconnection (CVE-2021-3436).
%RIOT-OS gnrc\_tcp implementation has infinite loop (CVE-2019-15702).
% TockOS contains an insecure permissions vulnerability in function \verb|get_package_name| in the file \verb|kernel/src/tbfheader.rs|, variable "pub package_name: &'static str," in the file process.rs that can result in A tock capsule (untrusted driver) could access arbitrary memory by using only safe code. This vulnerability appears to have been fixed in commit 42f7f36e74088036068d62253e1d8fb26605feed.
% For those RTOSes who separate the privilege, with improper privilege management, unprivileged users can recover the plaintext of RSA (Mbed TLS: CVE-2018-19608) via the man-in-the-middle attack.

%allowing one to decrypt a ciphertext by making successive queries to the server with the vulnerable library and measuring the server's response time. %, resulting in remote information disclosure.

%\textbf{Functional bugs in peripheral configurations:}

%the improper handling of external factors.
%triggered by possible external factors that the system handles properly.
% They are triggered by the proper handling of external factors that may cause vulnerabilities.
% We categorize them into two classes following with~\cite{cerdeira2020sok}.

% Not related with validation of values or functional correctness of code, but with the proper handling of external factors that might introduce security vulnerabilities.
%The program execution can disclosure undesired information because of the specific implementation components, which are usually encryption units, by analyzing side signals, such as execution time.
%Some cryptography library implementations subject to timing side-channel attacks.

%Mbed TLS was subject to a lucky thirteen timing side-channel attack~\cite{al2013lucky}, which may recover the secret key in CBC mode because the computing time depends on the padding length (CVE-2020-16150).
%The ECC multiplication function in WolfSSL is also vulnerable to this attack, which discloses the private key (CVE-2020-11713).
%WolfSSL mishandles signature generation, which leads to fault injection in RSA cryptography (CVE-2019-19962).
%???Man in the middle attack. CVE-2020-10059.
%Zephyr uses a risky crypto algorithm that does not prevent attackers from influencing the key length (CVE-2019-9506), allowing practical brute-force attacks to decrypt the traffic and inject ciphertext.

%software developers can place a special value \verb|0xFEF5EDA5| above the stack space at reset handle.

% Another cache-based side-channel attack in the Mbed TLS can obtain an RSA private key (CVE-2020-10941).
% For example, the attacker can recover the ECDSA private key with side-channel measurements.
% with precise enough side-channel measurements, the attacker can recover the ECDSA private key (CVE-2020-10932).
% Mbed TLS, side-channel attacks to gain the secret key information: timing based, cache based, etc.
% \textit{Attacks on firmware: }
% Microcontroller's firmware protection vulnerabilities~\cite{206148}.

\begin{comment}
	%[Still do not see how the example is related to physical side channel]
	\issue{Bugs through physical accesses:}
	By leveraging physical access targets, such as a debug interface, one can launch more powerful attackers that even bypass the hardware protection, as discussed in \ref{Bypassable vendor-specific readback protection:}.
	%The physical subjects include debug interface and power pin.
	%Besides the software side-channels, an attacker who have physical access to the devices can also break the protection of systems.
	%It is different from the device drivers that need to connect the device, 
	%Bugs in physical side-channels can happen because of not permanently disabling the debug interface.
	A bug was reported on Gigadevice that allows attackers who have the debug access to redirect the vector table offset register to execute their own code.
	That is because the debugger can write arbitrary flash memory dumping firmware into the SRAM and change the processor's registers~\cite{obermaier2020one}.
	%CVE-2020-13465
	% extract firmware (CVE-2020-13469), or de-obfuscate the observed data.
	%Even if the system restricts flash access by a debugger, STM32L4 device have a bug that the attacker can degrade the access level to access flash by injecting a glitch and power consumption analysis during the boot phase~\cite{schink2021security}.
	
	
	% (CVE-2020-27212)
	
	%The debug interface may also trigger race condition as documented in CVE-2017-18347 for STMicroelectronics STM32F0 device.
	%The race condition happens between the full initialization of the SWD interface and the setup of flash protection, which allows attackers to extract the device's protected firmware.
\end{comment}

%\issue{Concurrency bugs: }
%There are other denial of service attacks triggered by multiple concurrent operations.

%Such bugs are caused by multiple concurrent operations.
% For example, there is a privilege elevation attack on Zephyr project (CVE-2020-10058) because of the insufficient argument validation when multiple syscalls happens in the keyboard scan subsystem. 
%Zephyr suffers from a DoS attack when receiving certain duplicate and back-to-back packets in the Bluetooth subsystem (CVE-2020-10068).
% PASAN: Detecting Peripheral Access Concurrency Bugs within Bare-Metal Embedded Applications~\cite{272140}


% I00. \textbf{Bugs in memory protection:}
% Wrong memory configurations.
% I00. \textbf{Bugs in configuration of peripherals:}

% \textbf{I00. Bugs in security mechanisms:}
% Bugs in the implementation of security algorithms.


% \subsection{Hardware Issues}

% \textbf{I00. Attacks through reconfigurable hardware components:}
% [???]

% \textbf{I00. Attacks through energy management mechanisms:}
% [need to test]

% \subsubsection{Microarchitectural Side-Channels}

% \textbf{I00. Leaking information through caches:}
% [need to test]

% \textbf{I00. Leaking information through branch predictor:}
% [need to test]

% \textbf{I00. Leaking information using Rowhammer:}
% [need to test]

% \subsection{Implementation issues} 

% Find vulnerabilities of Cortex-M; CVEs

% Mbed is an open source OS and development tool for IoT devices.
% Table \ref{tab:CVEs} shows all the vulnerabilities (total 26 by 12/03/2020) reported for Mbed, most of them are related to Mbed TLS library. 

%===================================================secure projects-==============================
%Several projects in our list did not specifically design for Cortex-M, but the idea is generic enough to be applied on Cortex-M. 
%We categorize these projects into several classes based on the specific defenses. %, which address the issues discussed in~\S\ref{sec:IssueVul}.
%We compare the hardware features each project relies on, which has implications on the generalizability, and their overheads in terms of binary size increasement, memory and energy consumption overhead.  %self-reported run-time performance overhead on bare-metal applications, RTOSes, and some benchmarks in different colors. %, where {\color{green} green} represents negligible overhead, {\color{blue} blue} represents quite practical and almost not noticeable, {\color{orange} orange} represents noticeable and {\color{red} red} represents heavy overhead.

%We also evaluate these efforts based on three benefits:
%i) security benefits include the protection granularity, and the security features it provides;
% size of TCB, 
%ii) deployability benefits include usability and generalizability.
%In other words, hardware features these projects need, programmers' involvement, and the generalizability to extend the work to other Cortex-M processors or IoT devices;
%iii) performance benefits include energy usage, memory footprint, and computation performance.

\begin{comment}
	In this section, we review and evaluate the research projects in securing Cortex-M based software systems.
	It is a taxonomy of how academic and industrial projects utilize the security features, such as MPU, TrustZone, DWT,etc.
	We categorize these projects into two parts: one part is a compilation of defense mechanisms, which is targeted to the mitigate the issues we discussed in Section~\S\ref{sec:IssueVul}; another part is the vulnerability discovery.
	Then we evaluate these efforts based on 3 benefits:
	% The benefits encompass 3 categories:
	(i) Security benefits includes .
	(ii) Deployability benefits includes the usability and scalability.
	(1) Usability: rely on what hardware feature? MPU, DWT, TZ?  rely on programmer's notation?  rely on other architecture? such as APEX. (2) scalability: how easy to extend this work to support other processors?
	(iii) Performance benefits includes .
	security, deployability and performance.
	(1) how flexible these approach are. Do they work for all Cortex-M? Do they work for other IoT systems? What are the real requirements of these approaches?
	(2) What attach can it defeats? or what security feature it provides?
	(3) It is practical? performance, energy, memory usage? 
\end{comment}

% The definition of process on Cortex-M processor?
% \subsection{Defenses for Software Systems}
% As described in section (\S\ref{sec:SoftwareSystem}), either real-time operating systems or bare-metal applications can run on Cortex-M processors. 
% Since the bare-metal applications are single-thread, the definition of process only presents in RTOS, which may have multi threads and process switches.
\begin{comment}
	This section describes what issues those projects want to overcome through architectural, implementation, or hardware limitations.
	Each defense addresses partial or more than one single type of issues presented in~\S\ref{sec:IssueVul}.
\end{comment}

%\subsection{Architectural Defenses}

%Isolation, confinement and virtualization protect software modules from being attacked by each other when compromised (see \ref{No memory virtualization:}, \ref{No or weak privilege separation:}, \ref{No or weak memory access control; executable stack:}).

% ~\cite{shu2016study}.
% It constrains the data and control flow into a compartment.
%The confinement is required to constrain the control transfers and sensitive data access.
% The least privilege or privilege separation and TEE are security isolation designs~\cite{saltzer1975protection, shu2016study}.
% \defense{Memory isolation}

%of the privilege and unprivileged code.
%It is natural to utilize the MPU for isolation and confinement by having applications, modules or compartments with different memory permissions run in unprivileged domains and a reference monitor at the privileged level for context switches (including MPU context). 

% before the actual task is executed. 
%application tasks as interrupt handlers and uses interrupt priorities to isolate tasks.
%In addition, to isolate the application tasks and kernel services, it runs the task's code that does not require privileged execution as unprivileged and inlines a system call to trap into the privileged level if needed.
%MPU is used to constrain the current task's write access to kernel's and other tasks' memory at each task schedule.
%Moreover, SAFER SLOTH runs the static analysis on the compiled binary and only allows the kernel system services to run privileged instructions.

% works for both bare-metal applications and RTOS.
%It isolates each software modules (e.g. RTOS kernel, libraries, peripheral drivers) and set access permissions to its own resources (e.g. code, data) based on the programmer-provided configurations, which include the module number, privilege level, entry function, and peripheral access permission. 
% It utilizes MPU to divide the memory for each software module  and set access permissions to its own code, data, and peripheral regions based on the programmer-provided configurations, which include the module number, privilege level, entry function, and peripheral access permission.
%For RTOSes, the uSFI compiler emits unprivileged memory access instructions (\verb|STR*T/LDR*T|) for the kernel's memory access operations so as to remove the kernel out of the TCB. 
% uSFI takes 210 cycles to call cross-module function and 150 cycles to return from the call.
%uSFI incurs 1.1\% performance overhead and 10\% code size overhead.
%running it at the privileged level with unprivileged memory access instructions.
%The uSFI compiler will instrument an entry function and hook interrupt routines for modules and change cross-module procedure calls to \verb|SVC| instructions with the entry function as a parameter.
%The uSFI run-time, which to handle module switches and interrupts, is the only trusted module that runs at a privileged level.

%Thereafter, those approaches need to trap into the higher privileged code to apply its own memory access control whenever switching compartments, which introduces more privilege escalation executions, resulting in higher performance overhead than~\ref{Privilege separation:}.

%It targets both RTOS and bare-metal system and supports dynamic memory allocation and allows flexible mechanisms for resource sharing among different compartments.
%EC offers interfaces for users to define compartments in RTOS and bare-metal systems, incorporating a range of compartment policies, including those from ACES and MINION.
%Instead of using MPU for memory access control or different compartment policies, 

%The MPU-based compartmentalization solutions aforementioned have partially ignored the secure Direct Memory Access (DMA) support,
%which means the DMA controller can write and read any memory location of the MCU without the MPU restriction.

%implements the MPU-assisted RTOS kernel isolation with secure DMA support atop FreeRTOS.
%It defines a capability-based security model for DMA operations.

\begin{comment}
	\defense{MPU-assisted isolation and confinement:}
	% On a Cortex-M processor, privileged access to sensitive resources can be deprived and dynamically re-configured at run-time by an MPU.
	It is natural to utilize the MPU for isolation and confinement by having applications, modules or compartments with different memory permissions run in unprivileged domains and a reference monitor at the privileged level for context switches (including MPU context). 
	%For example, Mbed $\mu$Visor~\cite{uVisor} runs at the privileged level and enforces the least privilege policy by creating independent secure domains for applications.
	%Each security domain has its private data and stack sections, and it has restricted access to selected peripherals.
	
	Research efforts focus on automatic protection of existing bare-metal systems and RTOSs with minimal developer involvements.
	uSFI~\cite{aweke2018usfi} takes source code and developer defined module permissions as input, instruments an entry function for each module, and changes cross-module procedure calls to \verb|SVC| instructions.
	% works for both bare-metal applications and RTOS.
	%It isolates each software modules (e.g. RTOS kernel, libraries, peripheral drivers) and set access permissions to its own resources (e.g. code, data) based on the programmer-provided configurations, which include the module number, privilege level, entry function, and peripheral access permission. 
	% It utilizes MPU to divide the memory for each software module  and set access permissions to its own code, data, and peripheral regions based on the programmer-provided configurations, which include the module number, privilege level, entry function, and peripheral access permission.
	For RTOSs, the uSFI compiler emits unprivileged memory access instructions (\verb|STR*T/LDR*T|) for the kernel's memory access operations so as to remove the kernel out of the TCB. 
	% uSFI takes 210 cycles to call cross-module function and 150 cycles to return from the call.
	uSFI incurs 1.1\% performance overhead and 10\% code size overhead.
	%running it at the privileged level with unprivileged memory access instructions.
	%The uSFI compiler will instrument an entry function and hook interrupt routines for modules and change cross-module procedure calls to \verb|SVC| instructions with the entry function as a parameter.
	%The uSFI run-time, which to handle module switches and interrupts, is the only trusted module that runs at a privileged level.
	
	%Both uSFI and Mbed need manual work to designate the memory regions that belongs to the application based on developer's knowledge.
	% $\mu$Visor also works for MMU-less system via two-tier memory allocation: 
	% It is deprecated after Mbed OS version 5.10, replaced by Mbed SPM, which is the enhancement implementation based on TF-M.
	EPOXY~\cite{clements2017EPOXY} takes the source code of a bare-metal system that runs at the privileged level as input and automatically identifies operations requiring privileged execution.
	It relegates the bare-metal system to the unprivileged level and instruments privilege escalation (\verb|SVC|) and relegation instructions (change \verb|CONTROL[0]| to \verb|1|) around the operations that require privileged execution.
	The run-time average overhead is 0.1\% for the adapted privilege separation in EPOXY and -0.2\% for energy on the BEEBS benchmarks.
	ACES~\cite{clements2018aces} applies the principle
	of least privileges by taking a developer-specified compartmentalization policy and automatically creating an instrumented binary that isolates compartments at run-time to enforce inter-component isolation on bare-metal systems.
	ACES incurs 13\% run-time overhead and 70\% memory overhead.
	MINION~\cite{kim2018securing} automatically identifies the reachable memory regions of processes through offline static analysis on the firmware and conducts run-time memory access control through the MPU.
	MINION incurs 2\% average run-time overhead.
	%hardware-based enforcement.
	%other instructions to . these operations execute inprivileged mode runs the whole bare-metal application at the unprivileged level and defines a restricted operation that only elevates those instructions that require privileged level.
	%Those operations are identified automatically and instrumented with \verb|SVC| instructions to ask the MPU to re-configure the access control.
	%ACES~\cite{clements2018aces} addresses least privilege for bare-metal applications by the automatic compartmentalization at function level.
	% which is identified by static analysis with backend slicing, 
	%MINION aims to secure RTOS to meet real-time requirements.
	%It runs the RTOS at the unprivileged level to avoid frequently privilege switching, leaving only a memory view switcher at the privileged level.
	%It identifies the per-process memory access resources including code, data, and peripheral as a compartment by static analysis.
	% and re-configures the MPU through the memory view switcher when the process context switch happens.
	
	% It allows control-flow transfers as the protected target, using the static or dynamic, or hybrid analysis to trace the control flow;
	% (ii) Separates the privilege and defines constrained operations.
	% The restricted operation is defined by static analysis with backend slicing via LLVM passes.
	% uXOM~\cite{kwon2019uxom} and $\mu$RAI~\cite{almakhdhubmurai2020} also use MPU to restrict access to code and data. 
	% Silhouette~\cite{zhou2020silhouette} uses MPU to restrict the unprivileged code to access the shadow stack. 
	
	As discussed in \ref{Limit on the number of MPU regions and their size:}, the MPU may not provide enough number of regions.
	ACES and MINION address this limitation by merging the compartments.
	ACES supports 3 compartmentalization policies: 
	(i) isolating peripherals from each other; 
	(ii) grouping all functions and global variables that are defined in the same file into the same compartment;
	(iii) merging all code regions with identical data and peripheral dependencies.
	MINION uses the k-means clustering algorithm to group similar objects together and minimizes the number of access control rules and regions. 
	However, these policies are still not sufficient to protect the compartments' small but scattered stacks.  
	To address this issue, ACES emulates writes to a compartment's stack prohibited by the MPU regions. 
	%The micro emulator checks a white-list, which is generated by  static or dynamic analysis, of the areas each compartment is allowed to write.
	%to generate a whitelist to allow stack writings, which provides fine-grained stack access to small regions rather than setting Armv7-M MPU subregions, which only support a smallest size of 32 bytes (see \verb|I02|). 
	
	Tock~\cite{levy2017multiprogramming} is a RTOS written in Rust programming language that provides fault isolation and dynamic memory allocation, and it can take applications written in any language.
	Tock allows each application process to dynamically share its available memory to request kernel services.
	The basic kernel component, which is called capsules, is a Rust struct instance that provides different kernel functionalities and isolates each other.
	Capsules share a single stack.
	The kernel uses an event-driven scheduler to execute capsules cooperatively and provides memory fault isolation. 
	
	%\emph{Peripheral-aware isolation:}
	D-Box~\cite{mera2022d} implements the MPU-assisted RTOS kernel isolation with secure Direct Memory Access (DMA) support atop FreeRTOS.
\end{comment}

%From same group:
%eWASM: Practical Software Fault Isolation for Reliable Embedded Devices.
%Slite: OS Support for Near Zero-Cost, Configurable Scheduling.
%MxU: Towards Predictable, Flexible, and Efficient Memory Access Control for the Secure IoT.

%\subsection{Virtualization}
%Virtualization allows untrusted third party code to run without threatening the security of the privileged kernel.

%Besides, it gives a chance to fully utilize the resources of the devices.
%However, since Cortex-M processor does not have an MMU, it can not support memory virtualization.
%Pan et al.~\cite{pan2018predictable} builds a virtualization framework to execute multiple embedded RTOSes predictably.
%They propose a static memory layout algorithm to dynamically map memory with MPU for effective VM isolation.
%For each RTOS VM, they provide isolation for both the application and system services, including scheduling, memory mapping/access control, and I/O.
%\emph{MPU-assisted multiple TEEs:}
%MultiZone~\cite{pinto2020multi} supports both Cortex-M with MPU and RISC-V with Physical Memory Protection (PMP) to create isolated environments.
%Because Cortex-M does not have a hardware virtualization mechanism, 

%Hermes~\cite{klingensmith2018hermes} is a software-based virtualization system on Cortex-M. %, which is an abstract layer between hardware I/O devices and software.
%It runs at the privileged level with a single interrupt service routine to catch and preprocess all exceptions before dispatching them to the unprivileged guest system.
%MultiZone~\cite{pinto2020multi} presents an exokernel reference implementation on Armv7-M processors.
%It takes the fully-linked binaries of each application and combines them with the dedicated TEE separation kernel running in privileged handler mode.
%During runtime, all the applications run in unprivileged thread mode and the TEE kernel has the ability to trap and emulate the interrupt handlers in unprivileged application threads.
%Though hermes aims to fix the problem that software systems on microcontrollers cannot always respond quickly and deterministically enough to schedule real-time workload, such as I/O events,
%it is portable to support isolated virtual execution environment.

%LTZVisor~\cite{pinto2017ltzvisor} isolates both time and space by utilizing TrustZone for both secure and non-secure states.
%It mainly focuses on Cortex-A TrsutZone but now support Cortex-M TrustZone.
%It helps understand, evaluate, and discuss the benefits and limitations of TurstZone-assisted virtualization.

\begin{comment}
	As the TrustZone technique was introduced, researchers proposed TrustZone-based virtualization and put the hypervisor inside the secure privileged level.
	Such as lLTZVisor~\cite{araujo2018lltzvisor, pinto2019virtualization} and SBIs~\cite{pansbis2022}.
	lLTZVisor is a dual-world virtualization approach to isolate mixed-criticality systems.
	It places the time-constrained software (e.g., RTOS) inside the secure unprivileged level, while the bare-metal application is in the non-secure state.
	In the single-core design, the non-secure software is managed and controlled by a hypervisor, which runs in the secure state and has the same privilege as the secure software.
	In the multi-core design, the hypervisor is split into two parts running in each CPU at the secure state.
	%Each VM handles its own exceptions by configuring the vector table offset register to allocate its own vector table.
	%The hypervisor handles exceptions from the non-secure state that attempt to redirect to the secure state.
	SBIs~\cite{pansbis2022} can support multiple virtual machines (VM).
	It puts the interrupt handlers inside the non-secure privileged level and the VMs in the secure unprivileged level.
	When an interrupt happens, SBIs pauses the VM's execution in the secure state and switches to the corresponding non-secure handler.
	This is done automatically by hardware.
	%Since the hypervisor does not need to trap and emulate the interrupt handlers,
	Then the cost for a context switch depends on the exception latency.
\end{comment}

%unlike virtualization, the dual-world system moves the TCB into the secure state to provide secure services, such as crypto and protected storage.
%A bare-metal application or RTOS runs in the non-secure state and calls NSC APIs to request secure services.
%The design needs to minimize the TCB and maintain real-time availability.

%A recent study shows prevailing security vulnerabilities on TrustZone-assisted dual-world systems~\cite{cerdeira2020sok}.
%Though it targets Cortex-A processors, 
%The solutions discussed in \ref{TrustZone-assisted dual-world system:} may face the same threats.
%Multiple TEEs can mitigate them.

%which is the first attempt to build multiple TEEs on Cortex-M.
%uTango~\cite{oliveira2021utango} is an example of such systems.

%A world scheduler handles the context switch for the isolated non-secure domains by reserving the current context and restoring the next domain's context including its SAU settings. 
%uTango incurs 0.05\% average performance overhead with a 10 ms tick rate and less than 1\% average performance overhead with a 500 $\mu$s tick rate on the Embench benchmark suite~\cite{embench}.
%Utango starts with a configuration file, which defines the memory regions, devices including peripherals and times, and interrupts assigned to each NSVW, to partition the security attributes of platform sources for each NSVW at boot time via SAU.
%The NSVWs communicate with each other via the NSC region.

%directly determining the non-secure state context: access memory regions and permissions.
%assumes the non-secure state configures the MPU.
% without introducing additional communication.
%It assumes the non-secure state already setup the MPU configuration.
%ShieLD~\cite{khurshid2022shield} re-configures the non-secure MPU when the non-secure application requests secure services to access memory.
%It maintains a list of certificated non-secure tasks that need to access the secure services 
%Then it creates a context that contains a unique task ID and requested memory address and size when initializing those tasks.
%Those contexts are used later to configure the non-secure MPU.
%Then it authenticates the context whenever non-secure task tries to call secure services to access the shared memory and configures the non-secure MPU to constrain the resource access if passed authentication.
%However, both are only focus on the confidentiality and integrity, which is insufficient for real-time purpose, e.g., 
% ShieLD reports with a 27x execution overhead.
%Also, they cannot prevent the non-secure from executing sensitive code.
% In conclusion, some projects isolate the memory by depriving the privilege via the MPU but suffer from the limitation of the MPU.
% Cortex-M TrustZone can be an alternative solution.

% Mbed $\mu$Visor is a security component of the Mbed OS, developers need to follow the program rules to enable the $\mu$Visor. 
% $\mu$Visor is superseded by SPM.
% secure Partition Manager (SPM) defined in the Arm Platform Security Architecture (PSA)

% So EPOXY provides the foundation of code integrity, control-flow hijacking defenses, and sensitive IO protection. 
% It can defend the code injection attacks and ROP attacks. 
% EPOXY is application level and does not fix the process isolation or least privilege.
% It also requires programmers to add denotations to announce whether the code or data is sensitive or not.

% MINION~\cite{kim2018securing} creates thread-level compartments to virtually partition the memory space and enforce the access control. 
% To avoid frequently privilege escalation for sensitive instructions, MINION creates an efficient memory view switcher which is the only program runs in privileged level.

% \subsection{Address Space Layout Randomization (ASLR)}
% ASLR is a another security mechanism that randomly positioning the address of libraries, heap, and stack in a process's address space.
% Limited by the small size of memory, Cortex-M processor has few entropy to support a full-featured ASLR.
% [check the RTOS]

% \subsection{Diversification}

% EPOXY implements the software diversity~\cite{jackson2011compiler, homescu2013profile, larsen2014sok} to randomize the data and .bss region to prevent ROP attack.

%Besides isolation solutions in \S\ref{sec:Privilege_Separation_and_Compartment}, \S\ref{sec:Virtualization_and_Multi-world_Systems},
%other projects focus on mitigating memory corruptions attacks (\ref{Validation bugs in wireless communication components:} - \ref{Validation bugs in other components:}),
%~\cite{szekeres2013sok}
%such as control-flow hijackings, which occur through indirect control-flow transfers that divide into forward edges, i.e., function pointers, and backward edges, i.e., return addresses, information leak, etc.
%such as code reuse attacks and code injection.
%This category introduces researches on Cortex-M to defeat those attacks.
%Other memory protections secure memory accesses that are beyond the scope of isolating and confining software modules. %controls the memory access to prevent a program from accessing unintended memory (see \verb|I07, I08|).
%Some projects have optimization or software implementation to mitigate the limitation of hardware.
% \subsection{Software Architectural Defenses}
% Relevant techniques to mitigate the architectural issues are categorized into four types.

%\defense{Data Execution Prevention (DEP):}
%DEP enforces $W \oplus X$ on memory regions.
%For Cortex-M processor, DEP can be achieved by MPU since the MPU provides read/write and execute permissions for regions.
% But without privilege separation, MPU can be easily disabled.
%EPOXY, $\mu$RAI~\cite{almakhdhubmurai2020} and Utango implements DEP by setting the memory regions as execute never via an MPU.

%\ziming{explain (1) stack protections are important; (2) why challenging in implementing these for Cortex-M.}
%Stack is a scratch memory to store information for functions at run-time, such as parameters, return address, local variables, etc.
%Functions are free to push or pop the information from the stack, which exposes the potential risk to allow arbitrarily read, write, and execute (e.g., stack-based buffer overflow).
%Because of the real-time requirements on Cortex-M software systems, performance is the most considerable element when implementing stack protections such as shadow stack, stack canary.
%EPOXY modified the SafeStack by making the stack grow up and placing the .
%EPOXY also 

%Consequently, any overflow on the unsafe stack causes a fault either by accessing beyond the bounds of RAM or trying to access the guard region. 
%The run-time average overhead is 0.1\% for the adapted SafeStack in EPOXY.
% and 0.2\% for energy on the BEEBS benchmarks.

%It usually requires code instrumentation to add inline functions to update and check the return addresses.
%Its security guarantee and performance rely on the mechanism to protect the shadow stack.
%To protect the shadow stack, RECFISH~\cite{walls2019control}, which only protects unprivileged code, maintains shadow stacks at the privileged level and introduces a 30\% overhead.
\begin{comment}
	Silhouette~\cite{zhou2020silhouette} keeps bare-metal applications running at the privileged level but protects them with parallel shadow stacks,
	in which a function's prologue is transformed to save the return address into the regular and shadow stack, 
	and the epilogue is transformed to load the saved return address from the shadow stack.
	To protect the shadow stack, Silhouette deprives the bare-metal application's ability of writing to the shadow stack by transforming regular store instructions to unprivileged ones (\verb|STR*T|).
	%it configures the code region as readable, executable, and non-writable for both privileged and unprivileged accesses, sets the shadow stack as privileged access only, and transforms the privileged store instructions that are not supposed to access the shadow stack to unprivileged ones (\verb|STR*T|).
	%To minimize the instruction transformation, Silhouette inverts the hardware privilege level and changes the access permission of the shadow stack to disallow privileged writes and allow unprivileged writes by either utilizing a reserved bit in \verb|APSR| or setting the reserved \verb|AP| bit (\verb|0xb100|) of \verb|MPU_RASR| register to implement privileged access never.
	%Comparing to the hardware supported privileged separation (MPU) that needs syscall to elevate the privilege (\verb|SVC|), the unprivileged instructions do not require expensive context switches between protection domains.
	Silhouette incurs 1.3\% and 3.4\% performance overhead on the CoreMark-Pro~\cite{coremarkpro2021} and BEEBS~\cite{pallister2013beebs} benchmark suites. 
	Kage~\cite{du2022kage} integrates Silhouette to support CFI enforcement for multi-task systems.
	It incurs 5.2\% average runtime on FreeRTOS.
\end{comment}

%To access the shadow stack,
%CaRE replaces each function call and return with \verb|SVC| instruction to trap into a privileged non-secure module to invoke NSC functions,
%while TZmCFI calls an NSC function directly and addresses multi-tasks in RTOS by associating a separate shadow stack with each task.
%require context switches to access the shadow stack, 

%They keep the target running at the privileged level but protect them with parallel shadow stacks.
%of parallel shadow stacks.
%in which a function's prologue is transformed to save the return address into the regular and shadow stack, 
%and the epilogue is transformed to load the saved return address from the shadow stack.

\begin{comment}
	CaRE~\cite{nyman2017cfi} uses TrustZone and places the shadow stack in a secure memory region. 
	It replaces all direct calls (\verb|BL|) and returns (\verb|BX LR|) with \verb|SVC| instructions to trap into a privileged non-secure module called branch monitor, which invokes NSC functions to update or check the shadow stack in the secure state. 
	In CaRE, each function call or return is replaced by an entry into the privileged level and the secure state; hence, the performance cost is high with a reported 513\% overhead using the Dhrystone benchmark~\cite{weicker1984dhrystone}.
	
	Similar to CaRE, TZmCFI~\cite{kawada2020TZmCFI} uses TrustZone to protect the shadow stack of RTOSs.
	It instruments function's prologue and epilogue to invoke the monitor located in the secure state to push or pop the return address from the shadow stack.
	For handling exception returns, it relocates the exception vector table and updates all entries in the table to point to an exception trampoline, which pushes the current and its parent exception stack frame (a pointer to the exception frame) into the shadow stack.
	At the end of each exception handler, TZmCFI inserts an exception return trampoline to compare the saved and current top exception stack frame.
	To address multi-tasks in RTOS, TZmCFI associates a separate shadow stack with each task.
	Different from CaRE, which uses \verb|SVC| to trap into the privileged level in the non-secure state, TZmCFI calls an NSC function directly.
	%ii) exception handler's prologue and epilogue are replaced by exception return trampoline.
	TZmCFI incurs a performance overhead of 14.14\% on CoreMark~\cite{coremark2021}.
	% smart locks: August [2], Danalock [10],Kevo [20], Okidokeys [30], and Lockitron [25]
\end{comment}

%$\mu$RAI is effective because attackers cannot overwrite the reserved general-purpose register through memory corruption attacks.
%protects the return addresses for bare-metal applications by putting them in the \verb|R+W| only memory.
%It analyzes the call graph to generate hard-coded key for each function and calculate the unique Function ID (FID) via a \verb|XOR| operation, which takes the previous FID and hard-coded key as input.
%Then it inserts a finite list of direct jumps that correspond to possible return target (FID) in the code region of each function.
%It also inserts the same XOR operation before and after each call site, respectively.
%Then at run-time, $\mu$RAI reads the value of \verb|LR| to resolve correct return location, and executes the direct jump where \verb|FID=LR|.
%  via call graph static analysis.

% \emph{Other CFI:}
%Return-Oriented Programming (ROP) is a code reuse attack targeting return address edges.
%Besides maintaining stack and return address integrity, another approach to protect the control-flow backward-edge is to 
%Removing ROP gadgets can also defeat code reuse attacks.

%inserts \verb|NOP| between two 16-bit instructions and str
%uXOM~\cite{kwon2019uxom} replaces the \verb|MOVW| instruction that may generate \verb|STR| instruction by dividing the original immediate value into two numbers, then replacing it with another \verb|MOVW| instruction with an extra \verb|ADDW| instruction, etc. 
%\ziming{use ropgadets and other tools to count how many gadegets we can find in the firmware}

\begin{comment}
	\emph{Hardware-supported stack integrity [TODO]:}
	PA (\S\ref{sec:tz}) introduced in Armv8.3-A and Armv8-M architecture is a low-cost technique to protect pointers against memory vulnerabilities.
	Several projects utilize PA to enforce stack integrity~\cite{liljestrand2019pac, liljestrand2021pacstack, farkhani2021ptauth, li2022pacmem, schilling2022fipac, yoo2022kernel} for Cortex-A.
	%\emph{Other stack protections:}
	% Specifically, it also uses the MPU to restrict the access to code and data, then using the SR to determine the correct return location.
\end{comment}

% Control-flow hijacking attack is the most severe threat because of the C/C++ languages.
% CFI constrains the control flow in an expected control flow graph to protect the forward edge (e.g., indirect calls) and backward edge (e.g.,  return addresses).
%Forward CFI constrains the jump and function call to the valid target.

%which can be enabled with the flag \verb|-fsanitize=cfi|.
\begin{comment}
	Its implementation includes: 
	i) virtual-table verification; 
	ii) indirect function-call checks that maintains a jump table and instruments indirect calls to ensure that it points to a valid jump table entry; 
	iii) indirect-call-check analysis that performs type checking or to identify CFI violations.
\end{comment}

%At run-time, its branch monitor checks if the target matches the record of valid entry points.
%Similar to its shadow stack implementation, its CFI incurs high-performance overhead.

% Kage~\cite{du2020protecting} integrates Silhouette on top of the FreeRTOS to support CFI for multi-task systems.   
% MPU is used to strict the unprivileged level to access the shadow stack. 
% A privileged code scanner is used to detect the privileged instructions before generating the final binary code to make sure there are no potential attacks to disable Silhouette's protection.
% $\mu$RAI's 
% % uses a type-based alias analysis~\cite{lattner2007making} to determine the possible callees from indirect calls.
% implements type-based CFI that considers any function matching the type-signature of any indirect call within the current function as a valid transition in the call graph. [I don't understand the type-signature, also type-based alias analysis. This is the sentence they use. The reference it cites are not the correct paper.]
% The overhead is 10\% on memory.

%Program level diversity includes functions reordering, base addresses randomization (e.g., ASLR), data randomization, etc.
 %adds trap functions to the global function list.
%adding a small function that will jump to a fault handler.
 % diversity is increased by  implements global data randomization, which randomly split unused RAM into different groups that will be later used for data, stack, bss, etc.
 %is only performed at compilation time, so the memory layout of a system stays the same after that. % can be easily circumvented.
 %However, the memory layout of a system stays the same after compilation.
 
 %ASLR has been widely deployed on microprocessor-based systems~\cite{shacham2004effectiveness}.
 %to mitigate memory corruption and code reuse attacks.
 %For example, Linux adopts kernel ASLR to randomize where kernel code is at boot time~\cite{kaslr} and userspace ASLR to randomize the addresses of program segments at load time.
 
 %It incurs runtime overhead of less than 10\% for bare-metal applications.
 \begin{comment}
 	%is a mitigation technique against code reuse attacks~\cite{shacham2004effectiveness}.
 	%The entropy for random offsets, randomization frequency, and randomization process ensure the security guarantees of ASLR.
 	%Microprocessor-based systems utilize MMU and dynamic loader to adopt different randomization policies for kernel-level ASLR, which performs at boot time, and user-level ASLR, which randomizes the address space by the kernel when loading the user application.
 	%Microcontroller-based systems, however, 
 	%are statically linked that lack enough entropy because of \ref{No memory virtualization:} and usually run in the same privilege level.
 	%Solutions in \ref{Compiler-based software diversity:},
 	To address those challenges, 
 	several projects are proposed to provide function-level continuous re-randomization by placing the randomization process inside the secure world, such as HARM~\cite{shi2022harm} and fASLR~\cite{luo2022faslr}.
 	HARM~\cite{shi2022harm} moves non-secure program code from flash to non-secure unused SRAM and shuffles all functions and updates the code/data pointers that refer to them when the randomization is triggered periodically by SysTick exception.
 	%HARM utilizes the TrustZone and puts the HARM runtime system that maintains metadata needed by randomization and periodically invokes the randomization in the secure state.
 	%At the very beginning, HARM moves the non-secure program code from flash to non-secure unused SRAM and keeps a table to store the current address for each function.
 	%When randomization is invoked, HARM run-time system in the secure state shuffles all functions and updates the code/data pointers that refer to them before resuming the execution.
 	%It also supports exceptions by checking whether this is an exception return (\verb|EXC_RETURN|) or not.
 	%University of Georgia Le Guan's paper.
 	However, loading all the application code into the non-secure SRAM requires a large SRAM region and may also hurt the randomization entropy.
 	fASLR
 	%proposes a function-based ASLR scheme implemented in the secure state using MPU, which 
 	only loads functions in use to the SRAM and cleans up finished functions if the unused randomization region space is not enough.
 	%After the non-secure application is compiled, 
 	%At offline analysis phase, it analyzes the compiled binary and profiles a function table and determines randomization regions in unused RAM.
 	% is also determined in this offline analysis.
 	%When the device is booting, 
 	%At run-time, 
 	It uses MPU to configure the non-secure code in the flash as non-executable and sets up the secure HardFault handler to capture the MPU violation exception for all non-secure function calls.
 	%Then when there is a function call in the non-secure state, it will trigger the HardFault exception handler in the secure state, which 
 	%handles invoked functions protected by MPU in the non-secure state.
 	This handler will verify the function entry point and randomly relocate the requested function to SRAM.
 \end{comment}
 
 %Most embedded systems are implemented in C/C++; hence, subject to memory corruption attacks. %(see \ref{Validation bugs in network communication modules:}, \ref{Validation bugs in other privileged code:}, \ref{Implementation bugs in other critical modules:}).
 %Memory-safe programming languages, such as Rust, reduce memory corruption vulnerabilities in software.
 
 
 \begin{comment}
 	The kernel and device drivers of Tock~\cite{levy2017multiprogramming} are developed in Rust. %, which provides memory safety, type safety, and strict aliasing (see \verb|I14, I16|).
 	%Tock~\cite{levy2017multiprogramming} is a RTOS written in Rust programming language that provides fault isolation and dynamic memory allocation, and it can take applications written in any language.
 	Tock allows each application process to dynamically share its available memory to request kernel services.
 	The basic kernel component, which is called capsules, is a Rust struct instance that provides different kernel functionalities and isolates each other.
 	Capsules share a single stack.
 	The kernel uses an event-driven scheduler to execute capsules cooperatively and provides memory fault isolation.
 \end{comment}
 
 
 %In remote code disclosure attacks, attackers exploit 
 %Solutions in \ref{Stack and return address integrity:} and \ref{Forward Control-flow Integrity (CFI):} validate control flows but cannot against attackers utilizing arbitrary memory read vulnerabilities to steal sensitive information, such as intellectual properties.
 %, or find reusable code gadgets for control-flow hijacking.
 %One way to defeat this attack is execution-only memory, which allows instruction execution but forbids memory reads. %prevent information leakage.
 %uXOM~\cite{kwon2019uxom} implements XOM for RIOT-OS~\cite{RIOT} by converting memory access instructions, excluding those that need privilege, into unprivileged ones (\verb|STR*T/LDR*T|) and setting the code region as privileged access only.
 
 %To prevent attacks from exploiting unconverted instructions to turn off the MPU or read code, uXOM defines an atomic verification technique to execute them atomically with the verification routine, which verifies the target addresses and target values.
 % It uses the \verb|SP| as a base register of unconverted load/store to verify whether allow the memory access to code region or re-configure the MPU permissions.
 % It instruments a verification routine before an unconverted instruction, a checking function to check the \verb|SP| value after performing the instruction, and another check routine to validate the \verb|PSP| and \verb|MSP| at the beginning of the exception handlers. 
 %$\mu$XOM incurs 7.3\%, 15.7\%, and 7.5\% for run-time, code size, and energy overhead, on the BEEBS benchmark.
 % For those memory instructions that can not be converted into unprivileged ones such as the memory instructions accessing an interrupt controller, a timer, or an MPU, uXOM devised the atomic verification technique. 
 %\defense{XOM support by DWT unit:}
 %Approach by transforming instructions 
 %(\ref{XOM support by instruction transforming:}) 
 %incurs noticeable overhead since the compile needs to insert additional instructions.
 
 %for bare-metal applications and RTOSes
 %It utilizes the MPU to enforce write protection on code and uses the address range matching capability of the DWT unit to control read access to the code region.
 %The DWT unit generates a debug monitor exception on 
 %A matched read access indicating an illegal code read.
 
 %W$\oplus$X policy on memory by configuring the code region as readable and executable and RAM region as readable and writable.
 %To stop attackers from turning off the MPU protections, the DWT unit also write-protects the MPU registers.
 %After configuring the MPU and DWT, PicoXOM transforms all data in the application to the outside of the code region since the code region is not readable.
 %PicoXOM incurs 0.33\% performance and 5.89\% code size overhead on the BEEBS and CoreMark-Pro benchmark suites. %and five real-time applications.
 % PicoXOM incurs a maximum of 7.48\% performance overhead on BEEBS benchmark, 0.17\% on CoreMark-Pro benchmark, and 0.22\% on real-time applications.
 % The code size increasing for each test is 6.14\%, 4.39\%, and 6.52\% on average.
 
 \begin{comment}
 	\subsection{Formal Verification}
 	Formal verification~\cite{holzmann1995improvement} uses mathematical methods to prove the safety and liveness properties of a system.
 	
 	\defense{Formally-verified software architecture:}
 	\ref{No or weak privilege separation:} - \ref{Missing barrier instructions:}
 	
 	To protect MCU-based systems that lack hardware security features.
 	assembly-level code verification.
 	PISTIS: Trusted Computing Architecture for Low-end Embedded Systems. 
 	MSP430
 	
 	The Security MicroVisor: A Formally-Verified Software-Based Security Architecture for the Internet of Things~\cite{ammar2019s}. 
 	Target to MCUs that do not have the MPU.
 	Virtualization, formal verification, and remote attestation.
 	
 	Design and Verification of the Arm Confidential Compute Architecture.
 	Realms is a new abstraction for confidential computing to protect the data confidentiality and integrity of virtual machines.
 \end{comment}
 
 
 %Integrity checking compares the current state to previous stored state to detect any changes, which can be the %possible attacks (see \verb|I13, I14, I15, I16|).
 %Those projects can prevent more than one single type of bugs in section~\S\ref{sec:IssueVul}.
 
 % at a very low cost.
 % approaches are proposed to attest the firmware, code snippet, data, control flow, data flow, and even data communication integrity for Cortex-M based systems and beyond (see \ref{Validation bugs in wireless communication components:} - \ref{Validation bugs in other components:}).
 
 %\defense{Data integrity attestation:}
 % provides on-device data integrity that
 %Instead of attest the whole system, 
 
 %by linking the transmitted data with an attestation report reflecting the correct generation and processing of the data using control-flow attestation.
 %DIAT reduces the overhead by only attesting modules that process particular data of interest.
 %verifies the correctness of data from one device to another device in autonomous collaborative networks.
 %It decomposes software system into interacting modules and only attests the critical modules that generate and process the data to minimize the attestation complexity. 
 % which are identified by monitoring the data flow between modules' communication (e.g., modules that produce and exchange GPS data in a drone system), to minimize the attestation complexity.
 % DIAT also use multiset hash function~\cite{clarke2003incremental} to reduce the size of attestation reports. 
 % A dispatch instruction is inserted before each integrity-relevant control-flow event.
 % It also monitors data flow to reduce the attestation time, and uses multisets for execution paths to compress attestation reports.
 % DIAT considers software-only attacks.
 % DIAT requires the device to provide run-time isolation, secure storage, and secure boot.
 %Compared with whole system attestation, DIAT entails an overhead reduction of 95\%. 
 %by testing on a flight controller on top of NuttX RTOS. 
 % C-FLAT~\cite{abera2016c} proposes the dynamically remote attestation of the application's control-flow path without source code.
 \begin{comment}
 	C-FLAT~\cite{abera2016c} enables remote hash-based attestation of an application's control-flow path at binary level.
 	It instruments each control-flow instruction in the target application to pass control to a run-time tracer.
 	A trusted measurement engine running in the secure state generates and signs the hash-based attestation report.
 	Because there are unlimited number of legitimate paths in an application (e.g., path explosion introduced by loops), C-FLAT cannot cover all path possibilities.  
 	Since Cortex-M TrustZone was not available then, C-FLAT was implemented on Cortex-A. 
 	The evaluation on open-source syringe pump~\cite{syringepump} indicates 76\% run-time overhead.
 	% But hash-based attestation can not cover all possibilities because of the path explosion.
 	% It is designed for small IoT MCUs and implemented the prototype on Cortex-A TrustZone.
 \end{comment}
 
 %a peripheral-aware control-flow attestation scheme.
 %It compartments the bare-metal application functions into isolated code regions via ACES's peripheral compartmentalization policy, which groups functions that access the same peripheral.
 %It instruments the targeted compartments and continuously monitors
 
 %A trusted and privileged LAPE run-time is protected by the MPU. %, tracks the control-flow path of each compartment by analyzing remote commands that control the peripheral, and periodically pauses and generates the signed attestation report during compartment switching. 
 %LAPE incurs run-time overhead ranging from 0.8\% to 2.2\%.
 
 %a set of tasks or objects that an autonomous system is designed to perform.
 %Compared to LAPE, ARI compartments the system based on different levels of policies and attests the inter and/or intra-compartment levels.
 
 %Securely updating firmware and patching bugs are critical to maintain their security.
 %Transmission encryption, patch authentication, and integrity of updates are required.
 %Thus, updating the devices' firmware remotely and securely is very important to patch . 
 
 % designs a secure and scalable software update framework for IoT devices.
 %Prior update techniques such as the update framework (TUF)~\cite{tuf}, which is an update delivery framework resilient to key compromise for software updating, or Uptane~\cite{karthik2016uptane}, which extends and adapt TUF for automobiles, require direct interaction between manufacture and the devices and do not support update verification.
 %Thus, those frameworks do not suitable and secure for realistic IoT devices that the updates may be delivered via broadcast or from other content delivery networks.
 
 %, which handles the authorization token for each software artifacts created by OEM by extending TUF to embed and sign it or using GlobalPlatform TEE Management Framework (a security model for administration) to deliver it to device encapsulated in the update envelope. 
 % Constraints examples like the signing key OEM use, debug features the software update wants to enable or disable, the regular maintenance time, and different versions of patches, etc.
 % ASSURED requires the secure or authenticated boot, isolated execution, and secure storage, which can be satisfied by TrustZone. 
 %ASSURED outperforms 4.5 times than TUF. 
 % The evaluation shows that ASSURED outperforms TUF (when using full metadata verification) by a factor of 4.5 in terms of total time spent for metadata verification and attestation response generation.
 % [\textcolor{darkblue}{TODO: more details, what kind of constraints? hardware support for key storage.}]
 
 %To maintain the device availability and avoid service downtime, hotpatching can fix minor security issues without interrupting its normal execution.
 %Several firmware patching solutions are proposed and address challenges that where to store the patch code and how to trigger the patch.
 %HERA~\cite{niesler2021hera} first introduces a hotpatching system on real-time embedded systems with negligible overhead.
 %It runs as a low-priority task in RTOS and loads the patch into the RAM first.
 %Then the on-board debugging unit FPB is used to insert a hardware breakpoint at the preconfigured memory location.
 %Once triggering the breakpoint, FPB changes the fetched instruction to the patch address in RAM, which redirects the control flow to hotpatch.
 
 %To generalize the approach to other microcontrollers, RapidPatch ports the Linux extended Berkeley Packet Filter (eBPF), and patches are compiled into ePBF bytecode.
 
 \begin{comment}
 	% allows different MCU vendors to share the same source code patch among different devices.
 	ports the Linux extended Berkeley Packet Filter (eBPF) mechanism to Cortex-M as the hotpatching functionality.
 	To trigger the patch and redirect control flow, it can use (i) the fixed patch points manually inserted by developers; (ii) the hardware debug primitives (e.g., debug monitor exception); or (iii) the built-in patch features (e.g., FPB flash patch like how HERA uses).
 	%The overall system overhead is less than 18.8\% for fixed patch points, and less than 1.5\% for triggering by hardware features.
 \end{comment}
 
 %++++++++++++++++++++++++++vulnerability discovery
 
 %We discuss several projects to discover software vulnerabilities in Cortex-M based systems.
 %As shown in Table~\ref{tab:bug-finding}, 
 %While these solutions use different techniques, such as symbolic execution, static analysis, and fuzzing,
 %much of the effort has been made to emulate firmware execution on a PC, a technique known as rehosting. This facilitates scalable and effective dynamic analysis of MCU firmware.
 
 %, which can be applied to Cortex-M based systems.
 % not necessarily evaluated for Cortex-M software implementations   
 %The vulnerabilities on most Cortex-M software systems are virtually the same as modern OSes in nature.
 %For such systems, peripherals can be the most possible input channels to cause potential attacks.
 % Because of the hardware dependence and peripherals diversities for Cortex-M devices, it is hard to deploy a general framework to discover the vulnerabilities automatically.
 % Standard vulnerability discovery techniques, such as fuzzing, dynamic taint analysis, symbolic and concolic execution, etc., need extra work to deploy on those systems (see \verb|I13, I14, I15, I16|).
 
 %Although it is possible to manually build peripheral models for a particular MCU, as is done in FirmWire~\cite{hernandez2022firmwire},
 %Many solutions try to
 %automatically model the previously unseen peripherals.
 %For example,
 
 %Then, it classifies MMIO registers into four categories.
 %For each category, a heuristic-based method is used to model
 %the behavior of MMIO registers belonging to that category.
 
 %While the aforementioned dynamic methods mainly use fuzzing to find vulnerabilities,
 %We observe more diverse methods being used in works based on static analysis.
 
 %It analyzes the source code to identify the functions and instructions that can be executed concurrently, parses memory layout documents to get the memory-mapped I/O addresses of each peripheral, and extracts peripheral's internal state machines via corresponding device drivers.
 
 %It resolves a stripped raw binary's base address to disassemble the firmware correctly, recognizes Bluetooth-related data structures, and extracts the corresponding configuration values to identify vulnerabilities.
 
 %It identifies memory allocator and de-allocator pairs by dynamically executing selected functions and monitoring their run-time behaviors.
 %Then it performs a bounded model checking and symbolic execution analysis to inspect common classes of heap vulnerabilities.
 
 %With the identified allocator pairs, it will collect more information about their HML prototype and implementation.
 %With the allocator pair information and the firmware image,
 
 \begin{comment}
 	\gl{original ones}
 	
 	\defense{Peripheral-aware vulnerability discovery:}
 	% using static analysis, symbolic execution and/or fuzzing
 	Compared to traditional desktop programs, embedded and IoT software systems have frequent interrupt-driven control flows and more interaction with peripherals (see \ref{Validation bugs in device drivers:}, \ref{Validation bugs in dynamic memory allocations:}, \ref{Functional bugs in memory access control:}).
 	%Consequently, vulnerability discovery needs to take peripherals into account.
 	%Software verification~\cite{wallace1989software} is a mechanism that verifies the implementation to be satisfied by intended requirements, including model checking, symbolic execution, and formal methods, etc.
 	To handle the variety peripherals on different devices for vulnerability discovery, several approaches model the behaviors of peripherals by
 	(i) symbolic and concolic execution.
 	E.g., Inception~\cite{cor2018} run the firmware in the QEMU emulator while redirecting the memory-mapped region to the real peripheral or models the input as symbolic values.
 	$\mu$Emu~\cite{zhou2021automatic} presents unknown peripheral registers as symbols and symbolically executes the firmware to find out the peripheral access points.
 	% which is stored in a knowledge base and used for fuzzing.
 	Laelaps~\cite{cao2020device} takes the binary code as input and utilizes symbolic execution to emulate peripherals to predict the expected behavior of the firmware and generates proper inputs to steer the concrete execution;
 	(ii) access-pattern matching.
 	%Both P$^2$IM~\cite{feng2020p} and DICE~\cite{mera2020dice} propose a fuzzing framework for Cortex-M by emulating peripherals via QEMU. 
 	P$^2$IM abstracts a model that contains register categories, access patterns, interrupts model, and memory layout following the MCU documentation and conventions.
 	DICE identifies DMA input channels when the firmware configures the corresponding DMA controller registers;
 	(iii) static analysis.
 	For instance, PASAN~\cite{kim2021pasan} analyzes the source code to identify the functions and instructions that can be executed concurrently, parses memory layout documents to get the memory-mapped I/O addresses of each peripheral, and extracts peripheral's internal state machines via corresponding device drivers.
 	Most of those approaches integrate with fuzzing technique (Table~\ref{tab:bug-finding}).
 \end{comment}
 
 \begin{comment}
 	PASAN~\cite{kim2021pasan} is a static analysis tool to detect concurrent peripheral access bugs for embedded systems.
 	% It takes the source code, host firmware's memory layout, and the library function list as input to 
 	It analyzes the source code to identify the functions and instructions that can be executed concurrently, parses memory layout documents to get the memory-mapped I/O addresses of each peripheral, and extracts peripheral's internal state machines via corresponding device drivers.
 	PASAN achieves a true positive bug detection rate of 40\% to 100\% at an average of 70\% and discovers 17 bugs on several embedded systems. 
 \end{comment}
 %Deriving IoT Security Configurations via Automated
 %argXtract~\cite{sivakumaran2021argxtract} is an automated static analysis tool that extracts security-relevant configuration information (see \ref{Weak security configuration:}) via supervisor calls (identified using \verb|SVC|) and function calls (identified using function pattern matching) from stripped Cortex-M peripheral firmware binaries. 
 %It is based on the observation that the configuration information, which includes device and protocols or special hardware they use, application repositories, and website interfaces, can indicate the security status and vulnerabilities of the firmware binaries. 
 %It exploits multiple vectors to determine absent information regarding the application code base and locations of inline data within a tripped binary.
 %It provides a generic framework for extracting arguments to a security-relevant supervisor calls and function calls.
 %It employs a template-based approach for defining argument structures.
 %retrieve and process arguments to security-relevant supervisor and function calls, enabling automated bulk analysis of firmware files
 %Deriving IoT Security Configurations via Automated Static Analysis of Stripped ARM Binaries
 \begin{comment}
 	FIE~\cite{davidson2013fie} is a symbolic execution engine specifically designed for embedded systems. 
 	It builds on KLEE~\cite{cadar2008klee} to discover the memory safety vulnerabilities on firmwares. %MSP430 device.
 	FIE comes with a set of default specifications, which returns unconstrained symbolic values to any read from special memory, e.g., peripheral registers.
 	%It models peripheral semantics, and interrupt-driven to generate specifications to address the firmware diversity for MSP430 programs. 
 	%To avoid analyzing a deep or infinite loop, FIE detects and removes the previously analyzed program state and replaces the loop counters with unconstrained symbolic variables.
 	%FIE discovers 21 bugs on 99 open-source firmware programs on MSP430 family.
 	% [the title is for bare-metal application, but test on both RTOS and bare-metal.]
 	% Overall accuracy is 77.05\%.
 	% no developer involvement
 	%\defense{Periperal-aware fuzzing:}
 	%Software testing can check the quality and security of the software.
 	% Such as fuzzing, dynamic taint analysis.
 	% Because of the hardware dependence and diverse peripherals for Cortex-M devices, it is hard to deploy a general framework to test the software automatically.
 	% Standard vulnerability discovery techniques, such as fuzzing, dynamic taint analysis, symbolic and concolic execution, etc., need to be modified to deploy on those devices.
 \end{comment}
 \begin{comment}
 	Inception~\cite{cor2018} % utilizes symbolic execution to detect vulnerabilities for real-world embedded firmware.
 	modifies the symbolic virtual machine to run the LLVM-IR bitcode merged from source code, assembly code, and binary code.
 	To handle the peripheral, it redirects the memory-mapped region to the real peripheral or models the input as symbolic values. 
 	
 	Both P$^2$IM~\cite{feng2020p} and DICE~\cite{mera2020dice} propose a fuzzing framework for Cortex-M by emulating peripherals via QEMU. 
 	P$^2$IM aims to provide a hardware independent and scalable firmware testing framework.
 	It executes a firmware binary in QEMU, handles peripheral accesses, and channels the fuzzing input and feedback between firmware and AFL~\cite{AFLfuzzer}.
 	%It identifies the processor-peripherals except DMA via memory-mapped registers (identify by the address: \verb|0x40000000|-\verb|0x5FFFFFFF|) and identifies interrupts by monitoring the interrupt controller.
 	%P$^2$IM first abstracts a model that contains register categories, access patterns, interrupts model, and memory layout following the MCU documentation and conventions. 
 	%Then it instantiates the abstractions running on QEMU to explore code execution and invoke AFL.
 	P$^2$IM reported 79\% successful execution of sample firmware without manual assistance. %and discovered 7 unique unknown bugs. 
 	To handle firmware that uses DMA, the dynamic analyzer DICE emulates DMA and inputs from peripherals.
 	It identifies DMA input channels when the firmware configures the corresponding DMA controller registers.
 	%DICE detects the firmware access to such resources as a DMA input and invokes the analyzer for further action.
 	%  e.g., feed the fuzzing tool.
 	%DICE evaluated the performance on 83 sample firmware and 11 different MCU SoCs, the accuracy of DMA input channels detection is 89.19\% without false positive.
 	%It also fuzz-tested 7 real-world firmware integrated with P$^2$IM and discovered 5 bugs.
 	% based on the observation that firmware writes the source and destination DMA transfer points into the DMA controller and only the DMA controller can directly access the RAM.
 	% It focuses on the data transfer that targets the RAM and captures the stream by monitoring the memory writes.
 	% DICE: binary
 	
 	Laelaps~\cite{cao2020device} is a concolic execution approach for IoT devices.
 	%proposes a general emulator for Cortex-M processors to run diverse software without knowing a priori knowledge about the target device.
 	It takes the binary code as input and utilizes symbolic execution to emulate peripherals to predict the expected behavior of firmware and generates proper inputs to steer the concrete execution.
 	Laelaps can be used to perform dynamic analysis (e.g., fuzzing).
 	%Unlike P$^2$IM and DICE who model unknown peripherals by observing their access patterns, 
 	$\mu$Emu~\cite{zhou2021automatic} is an automatic firmware analysis tool on top of S2E~\cite{chipounov2011s2e} for Arm MCUs.
 	It presents unknown peripheral registers as symbols and symbolically executes the firmware to find out the peripheral access points, which is stored in a knowledge base and used for fuzzing.
 	%The knowledge base is used for AFL fuzzing.
 \end{comment}
 
 \begin{comment}
 	However, the emulation-based approaches 
 	%face limitations that they 
 	cannot accurately and generally model the peripherals' behavior or handle complex peripherals such as USB.
 	%Other approaches are proposed to address those limitations.
 	%For example, 
 	$\mu$AFL~\cite{li2022mu} supports fully on-device execution and communicates with the host through a debug dongle.
 	%Thus, The peripheral I/O operations can be tested by fuzzing the memory-mapped registers.
 	%To collect the code coverage information, $\mu$AFL 
 	It utilizes the ETM hardware debugging feature to get the instruction trace and capture branch coverage information. %without decoding the raw ETM data.
 	
 	\defense{Wireless communication-aware vulnerability discovery:}
 	Besides the peripheral, wireless communication is another attack vector as discussed in~\ref{Validation bugs in wireless communication components:} and \ref{Functional bugs in protocol implementations:}.
 	FirmXRay~\cite{wen2020firmxray} is a static binary analysis tool that aims to detect Bluetooth link layer vulnerabilities from bare-metal firmware.
 	It resolves a stripped raw binary's base address to disassemble the firmware correctly, recognizes Bluetooth-related data structures, and extracts the corresponding configuration values to identify vulnerabilities.
 	%takes a stripped raw binary and first resolves its base address, which is used for disassembling the firmware correctly.
 	%With the disassembly code, it can recognize Bluetooth-related data structures and extract the corresponding configuration values.
 	%Then FirmXRay identifies vulnerabilities from them.
 	%It uses a mobile app to collect the Cortex-M Bluetooth Low Energy firmware, and we use a similar approach in our empirical analysis.
 	
 	\defense{Dynamic allocator-aware vulnerability discovery:}
 	To address the issue in ~\ref{Functional bugs in memory access control:},
 	%, dynamic memory allocation components also introduce a lot of bugs.
 	HEAPSTER~\cite{gritti2022heapster} is a heap management library analyzer for Cortex-M monolithic firmware images.
 	It identifies memory allocator and de-allocator pairs by dynamically executing selected functions and monitoring their run-time behaviors.
 	%With the identified allocator pairs, it will collect more information about their HML prototype and implementation.
 	%With the allocator pair information and the firmware image,
 	Then it performs a bounded model checking and symbolic execution analysis to inspect common classes of heap vulnerabilities.
 \end{comment}
 
 %The current defense approaches are still in the early stage for many reasons: 
 %(i) lack of hardware support, e.g., MMU and XOM; 
 %(ii) incur noticeable overhead, which could make the applications miss the real-time requirement;
 %(iii) various types of software systems and device peripherals, which require extra effort to keep the robustness and scalability of the defense, etc.
 %As more and more hardware features are introduced to Cortex-M, future research may take advantage of these primitives for more robust and efficient defenses.
 %will be new research utilizing overlooked hardware features
 
 %\subsection{}
 %Some projects may use alternative implementations to provide more secure or efficient functionalities.
 
 \begin{comment}
 	\subsection{Cryptographic primitives, algorithms, and protocols}
 	Due to the limited computational resources and energy budget on Cortex-M, it is important to implement cryptographic primitives, algorithms, and protocols in an inexpensive, fast, and low-power fashion. 
 	
 	\defense{Software-based secure pseudo-random number generation:}
 	Herrewege et al.~\cite{van2014software} implemented a software-based pseudo-random number generator for Cortex-M processors,
 	which uses SRAM startup values as random seeds and the Keccak~\cite{bertoni2013keccak} hash function for entropy extraction and pseudo-random number generation.
 	The approach is lightweight and requires only 496 bytes of ROM and 52 bytes of RAM.
 	%It uses the start-up values of on-chip SRAM as random seed and uses the Keccak hash function for both entropy extraction as well as pseudo-random number generation.
 	
 	\defense{Optimizing cryptographic algorithms and protocols:}
 	%Though the memory access and computation speed are constrained on Cortex-M processors, there are some projects working on optimizing the public-key crypto implementations. 
 	Clercq et al.~\cite{de2014ultra} implemented an efficient and low-power ECC on Cortex-M0+ using an optimized L\'{o}pez-Oahab multiplication with fixed registers, which has a performance improvement of 15\% over the previous fastest optimization. %, which stores the most frequently used words inside a fixed register and stores the least frequently used words inside memory to reduce the memory access. 
 	% Saarinen et al.~\cite{saarinen2018shorter} implements the Round5 ring variants on Cortex-M4 platforms.
 	Seo et al.~\cite{seo2019sike} adopt highly-optimized hand-crafted assembly implementation of finite field arithmetic to implement SIKE round2 on Cortex-M4.
 	Alkim et al.~\cite{alkim2016newhope} implement the post-quantum key exchange protocol NewHope by carefully optimizing the original C implementation in assembly on both Cortex-M0 and Cortex-M4.
 	% It is based on NewHope~\cite{alkim2016post} that can be implemented in constant time.
 	% Wardhani et al.~\cite{wardhani2017fast} implement a fast AES on Cortex-M3 by using lookup tables and storing the instruction and tables on FLASH to accelerate memory access. 
 	% [\textcolor{darkblue}{Comment: this is not a high quality work.}]  
 	% AES    & Cortex-M3 
 	Some Cortex-M processors have the Single instruction Multiple Data (SIMD) instructions that can perform arithmetic operations on two half words or four bytes in parallel.
 	With the help of SIMD, faster cryptographic implementations are possible~\cite{alkim2020cortex, polubelova2020haclxn, seo2016efficient}.  
 	%Efficient arithmetic on ARM-NEON and its application for high-speed RSA implementation~\cite{seo2016efficient}.
 	%This is for Cortex-A.
 	
 	%Cortex-M4 optimizations for {R,M}LWE schemes~\cite{alkim2020cortex}
 	
 	%HACLxN: Verified Generic SIMD Crypto~\cite{polubelova2020haclxn}
 \end{comment}
 
 %\subsection{Other Research}
 
 \begin{comment}
 	\defense{Non-secure caller identification:}
 	As discussed in~\ref{Wide interfaces for state switches:}, a byproduct of Cortex-M TrustZone-based isolation is the confused deputy problem, which is easier to exploit than its Cortex-A counterpart.
 	One way to alleviate this problem is to enforce authentication and authorization between a non-secure software component and a secure software component, as SeCReT~\cite{jang2015secret} does for the Cortex-A TrustZone.
 	On Cortex-M, Secure Informer~\cite{iannillo2022ree} attempts to authenticate a non-secure function by directly determining the non-secure state context without introducing additional communication.
 	
 	%calculates a unique ID for each function that calls secure functions based on the current non-secure MPU configuration.
 	
 	%Refer to~\ref{Return-to-non-secure (ret2ns) vulnerabilities:},
 	%this attack happens because of the semantic problem between secure and non-secure world.
 	%The secure world has trouble to understand how the non-secure world creates and manages callers.
 	%Resulting in confused deputy attacks.
 	%A unique ID for non-secure callers may mitigate such attacks.
 	%TF-M maintains a non-secure world context representation whenever creates a thread.
 	%Secure Informer~\cite{iannillo2022ree} calculates a unique ID for each function that calls secure functions based on the current non-secure MPU configuration.
 \end{comment} 
 
 
 %================================Conclusion====================
 \begin{comment}
 	%The Arm Cortex-M processors are the most popular 32-bit MCUs in the embedded and IoT market. 
 	%However, the security of their hardware and software stack has not been systematically studied. 
 	In hopes of helping interested researchers better understand the Cortex-M systems and their security features, shedding light on the landscape of Cortex-M system and software security, and leading the community to opportunities for improving the security of embedded and IoT devices, in this paper, we presented a systematization study of the hardware and software security of Cortex-M based systems.
 	In particular, we summarized the Cortex-M hardware architectures, security-related hardware features, and their hardware limitations and issues. 
 	%for which we also developed a suite of example code to help researchers easily access Cortex-M research.
 	We systematized representative software architectures on Cortex-M
 	%, which are bare-metal and unikernel architecture, monolithic kernel architecture, exokernel architecture, dual-world architecture, and multi-world architecture.
 	%Those five architectures cover existing and new production software architectures proposed in recent research papers.
 	and performed by far the largest empirical analysis on the compiled real-world Cortex-M firmware dataset. %to learn how the discussed security features are adopted in real.
 	%Besides the empirical analysis, 
 	Our analysis of the publicly disclosed vulnerabilities of Cortex-M based systems revealed what bugs are more likely to occur.
 	%the security of real-world Cortex-M systems.
 	%In total, we discussed 29 hardware, software architectural, and implementation limitations and issues that have serious security implications. %potentially introduce exploitable vulnerabilities from the perspective of .
 	%We find out that the software implementation introduces the most number of vulnerabilities.
 	Additionally, we presented an in-depth study of the state-of-art security research on Cortex-M based systems.
 	%We categorized existing efforts into 22 defenses and evaluated them by analyzing their hardware requirements, generalizability, and overhead.
 	%Based on our analysis, MPU and TrustZone are popular secure techniques utilized to secure the software systems.
 	%Few of those projects pay attention to the debug features.
 	%From our study, we find that it needs a further exploration from both the hardware and software side to build a more secure environment for Cortex-M.
 \end{comment}
 
 
 %====================================appendix====================
 %\ziming{We need to make it clear what contributions are in Sec II and III. When I read the current version, as a reader I can learn something but doesn't mean it make contributions. Maybe summarize some technical highlights? maybe there is a way to formalize thing? Summarize some technical findings?}
 
 %We discuss the Cortex-M architecture, %and security extensions,
 %which are summarized from official documents~\cite{Armv6MArcRef, Armv7MArcRef, Armv8MArcRef, Armv8MArcTech, Armv8MMPU, ArmCortexM23, ArmCortexM33, ArmCortexM55, Armv8MTZ, ARMpacbti}. 
 % and related books~\cite{yiu2020definitive, zhu2015embedded}.
 
 %a brief summary of descriptions are available, they may be vague, incomplete, and buried in over tens of thousand pages of technical reference manuals. 
 %This section does not attempt to cover everything, please refer to official docs~\cite{Armv6MArcRef, Armv7MArcRef, Armv8MArcRef, Armv8MArcTech, Armv8MMPU, ArmCortexM23, ArmCortexM33, ArmCortexM55, Armv8MTZ, ARMpacbti} and books~\cite{yiu2020definitive, zhu2015embedded} if you want to learn more. %, including TrustZone and Pointer Authentication and Branch Target Identification (PACBTI), etc.
 %With TrustZone, many mechanisms, such as exception handling, have been extended.  
 %Figure~\ref{fig:func-blocks} shows the hardware functional blocks of a Cortex-M System-on-Chip (SoC).
 
 %if the MPU is implemented. 
 %The permission for an MPU region is determined by the Access Permission field (\verb|AP|) and the eXecute-Never bit (\verb|XN|).
 %Armv7-M MPUs supports six access permissions, while Armv8-M MPUs defines eight access permissions.
 %The \verb|XN| bit determines whether execution is permitted when read is permitted.
 % Cortex-M55 MPU introduces privileged execute never (\verb|PXN|). %bit. %to prevent the processor from executing the code inside with the privileged level.
 
 %If the processor is running code in the secure memory, the processor is in the secure state. 
 %Otherwise, the processor is in the non-secure state.
 %Each of the interrupts can be assigned as secure or non-secure in the interrupt target non-secure (\verb|NVIC_ITNS|) registers of NVIC.
 %Non-secure interrupts can still be serviced when executing a secure function.
 %\subsubsection{Banked Registers and System Peripherals}
 
 % can have \verb|SG| instructions to enable software to transition from the non-secure state to the secure state. 
 %A non-secure region can be accessed by non-secure and secure software. %, while a secure region can only be access by secure ones.
 %Both secure and non-secure callable belong to secure. regions are further divided into two types: 
 %When \verb|PC| points to an address in a non-secure callable region, the process is in the secure state.
 
 %No every system implements both SAU and IDAU.
 %The SAU should always be present but may have different number of regions.
 %If no SAU regions are defined, or the SAU is disabled, and no IDAU is included in the system then the entire memory address space is defined as secure.
 %The SAU
 %, which is memory-mapped in PPB, 
 %is configurable, %anytime in the secure state. 
 
 %A typical design is to use the IDAU to define a fixed memory partition and use the SAU to change some security attributes at run-time.
 %For instance, in xxx device the IDAU to splits memory into 256MB chunks of alternating secure and non-secure memory.
 %As shown in Table~\ref{tab:idausau},
 %If an address maps to regions defined by both SAU and IDAU, the region of the highest security level is selected.% (see Table~\ref{tab:idausau}).
 
 %Privileged and unprivileged secure software can configure a Memory Protection Controller (MPC), which is included on the path to the memory,
 % SSE-220 2.5.4 SRAM
 %to divide the memory into equal size blocks and to selectively assign each block to its secure or non-secure alias at run-time. 
 %The size of block is determined by the hardware.
 %The MPC provides a single software-configurable bit to define if each block is assigned to secure or non-state world. 
 %Each MPC's configuration interface is mapped to the peripheral region (\verb|0x5800????|).
 %For instance, we assume SAU and IDAU together split the 512MB SRAM region into the non-secure (\verb|0x20000000| - \verb|0x2FFFFFFF|) and secure (\verb|0x30000000| - \verb|0x3FFFFFFF|) parts.
 %A 2MB physical SRAM is mapped at two aliasing 2MB memory regions: (i) a secure region from \verb|0x28200000| - \verb|0x283FFFFF|; and (ii) a non-secure region from \verb|0x38200000| - \verb|0x383FFFFF|.
 %Each block on the SRAM is 64KB, so the MPC provides 32 bits for this SRAM. 
 %For example, the 4MB SRAM can be divided into 32 blocks with 64KB each.
 
 %Non-secure state can not configure the MPC which will trigger the attribution unit violation secure fault.
 %Both Privileged and Unprivileged mode in the secure state can configure the MPC.
 %\subsection{Peripheral Protection Controller}
 %\label{sec:ppc}
 
 %The PPCs perform the task of gating access to the peripherals it protects based on the security settings of each peripheral, and the security attribute of the access. 
 %Each PPC can support up to 16 peripherals.
 % The privileged access only Privilege Control Block (bankedSecure of Non-Secure) is used
 %The configuration interfaces of PPCs are also mapped to the peripheral region.
 %The privileged access only Privilege Control Block (\verb|0x40080000| - \verb|0x40080FFF| in non-secure, \verb|0x50080000| - \verb|0x50080FFF| in secure) is used for PPC to define the access settings for associated peripherals.
 %For SSE200 subsystem~\cite{ArmCoreLinkSSE200}, PPC can configure the access setting of MHU (Message Handling Unit), DUAL TIMER, TIMER, and Watchdog that can raise an interrupt to the processor.
 %Secure PCB can set the peripheral as non-secure access or secure unprivileged access.
 %Non-secure PCB can set non-secure unprivileged access.
 %[Seems only SSE200 subsystem talked about the PPC. The Arm architecture document and reference document did not mention it.]
 % \ziming{need citation for SSE200}
 
 % between the secure and non-secure software.
 %This is achieved by the NSC region and some new instructions.
 
 % Also, the function the non-secure state wants to call must be declared as a non-secure entry.
 % Each call targets to a non-exist entry will trigger an invalid entry point secure error.
 
 %, and the return state (1 for secure, 0 for non-secure) is stored in the least significant bit (LSB) of \verb|LR|.
 % This is because Cortex-M does not support A32 instruction set, so the LSB of an address indicates the security state.
 %After finishing the secure function, this bit will be checked to prevent returning to a fake secure address~\cite{Armv8MTZ}.
 % Then branch to the secure state function.
 
 % to  to a non-secure address.
 %The target security state of those two instructions is indicated by the least significant bit of the target address, 1 means secure, 0 means non-secure~\cite{Armv8mdeveloper}.[need a test]
 %\ziming{Where did you get this sentence? Also need to explain the meaning of least significant bit pf LR and SP.}
 %The \verb|BLXNS| instruction switches the state to non-secure only when the LSB of the target address is 0. 
 %When state switching happens, the processor first automatically pushes a special 32-bit value, namely combined exception Return Program Status Register (\verb|RETPSR|), and the return address with the LSB value 1 onto the current stack.
 %The value of \verb|RETPSR| consists of \verb|IPSR| and other flags.
 %The \verb|LR| is also changed to a special value named \verb|FNC_RETURN| (\verb|0xFEFFFFFF|).
 %The LSB of \verb|FNC_RETURN| indicates which state this function is called from.
 %Since it is only used in the non-secure function return, the value is always \verb|0xFEFFFFFF|.
 %This automatic step is called \verb|FNC_RETURN| stacking.
 %When the \verb|FNC_RETURN| value is loaded to \verb|PC|, the processor will unstack the \verb|RETPSR| value, check the \verb|IPSR|, and clear interruptions, then restore the return address to the secure state.
 %The state switching mechanism for the \verb|BXNS| instruction is much simpler than the \verb|BLXNS| instruction. 
 %If the target address is not \verb|FNC_RETURN| or \verb|EXC_RETURN| and the LSB is 0, \verb|BXNS| branches to non-secure code directly.
 % It clears the \verb|CONTROL.SFPA| value to 0. 
 
 \begin{comment}
 	\textbf{Asynchronous state switching or exception with TrustZone}.
 	\label{sec:subsec:asystateswithing}
 	%\subsubsection{ State Switching}
 	Exceptions and interrupts trigger state switches asynchronously. 
 	%, which extend the exception handling mechanisms discussed in \S\ref{sec:ExceptionStacking}.
 	%Secure privileged software can configure each interrupt, which could happen anytime, as secure or non-secure in the Interrupt Target non-secure (\verb|NVIC_ITNS|) registers.
 	If the exception entry is in the non-secure state,
 	the processor automatically pushes the state context and an additional state context onto the current stack.
 	The additional state context consists of a \verb|Magic Signature|, \verb|R4| - \verb|R11|~\cite{Armv8MArcRef}. 
 	%Different from the \verb|FNC_RETURN| stacking, \verb|RETPSR| is partially used to store the \verb|xPSR| value and other flags.
 	%The additional state context includes \verb|R11|, \verb|R10|, \verb|R9|, \verb|R8|, \verb|R7|, \verb|R6|, \verb|R5|, \verb|R4| along with an integrity signature value (\verb|0xFEFA125B| with Floating-point Extension, \verb|0xFEFA125A| without Floating-point Extension).
 	If the FPU is enabled, the current state is the secure state, the processor pushes additional FP context %(\verb|S16| - \verb|S31|)%, which are \verb|S0| to \verb|S15| and the Floating-point Status and Control Register (\verb|FPSCR|) for the secure state exception, additionally \verb|S16| to \verb|S30| for the non-secure state exception, 
 	onto the current stack. %armv8-m architecture reference p70
 	After context stacking, if the current state is non-secure, all pushed registers will remain unchanged.
 	If the current state is secure, those registers will be set to \verb|UNKNOWN| values or zeros depending on whether the exception happens in the secure state or the non-secure state.
 	To help save and clear the floating-point registers \verb|VLLDM| and \verb|VLSTM| instructions were introduced, which will only work when Floating-point is used in the non-secure state and will be considered as \verb|NOP| if FPU is not present.
 	When \verb|EXC_RETURN| is loaded to the \verb|PC|, the processor automatically unstacks the context stack and checks the return security state.
 	%The process also checks if the 0th bit of signature value matches the \verb|EXC_RETURN[4]|.
 	%If not, the processor generates a \verb|SecureFault| to prevent the non-secure software from using the interrupt return to switch to the secure state illegally.
 	%Since the address starting with \verb|0xF| is non-executable, treating the signature as an address will trigger \verb|MemManageFault|, e.g. replacing the \verb|EXC_RETURN| to \verb|FNC_RETURN| will fail~\cite{Armv8SecureStack}.
 \end{comment}
 
 \begin{comment}
 	\noindent\textbf{Test target instructions}.
 	\label{sec:subsec:TT}
 	The v8-M instruction set introduces the test target (TT) instructions for querying the security state and access permissions of a memory location~\cite{Armv8MArcRef}.
 	There are four variants to query a location for privileged and unprivileged access from the secure or the non-secure state.
 	% for a privileged (\verb|TT|, \verb|TTA| for non-secure) access or unprivileged (\verb|TTT|, \verb|TTAT| for non-secure) access to that location~\cite{Armv8MArcTech} C2.4.247.
 	% These instructions are only valid when executing in the secure state.
 	%The return information is stored in the \verb|TT_RESP| payload format. %, which includes IDAU, SAU, and MPU region number, and access permissions such as non-secure or secure read and writable, non-secure readable, and readable, etc. 
 \end{comment}
 
 %, a similar version of which has been available on Cortex-A since Armv8.3-A, 
 %to mitigate code reuse attacks. %return-oriented programming (ROP) and jump-oriented programming (JOP) attacks.
 %Instructions related to this feature are presented in Table~\ref{tab:SecInstruction}.
 % [should we explain the ROP and JOP here?]
 % Unlike the AArch64 Armv8-A that can use some spare bits in the most significant bit of the pointer to embed security information for validating the pointer
 
 %separate to the pointer and can be enabled for every secure state and privileged level.
 %Creating a PAC is to sign the pointer using a cryptographic mechanism, which takes the pointer, a 32-bit modifier in a general-purpose register, and a 128-bit secret key as inputs.
 %The modifier encodes context information, whereas the key can only be managed at the privileged level.
 %To sign a pointer in a general-purpose register, instruction \verb|PACG| is used.
 %A special instruction \verb|PAC| is used to sign \verb|LR| and use \verb|SP| as the modifier.   
 %To validate a pointer, it follows the same crypto step to generate another PAC called \verb|PACreturn| and compares it with the stored \verb|PACenter|.
 %A \verb|UsageFault| exception is generated if the validation of a pointer fails.
 %Even though this is a new feature on Cortex-M,
 %Different from Cortex-M, AArch64 Armv8-A can use some spare bits in the most significant bit of the pointer to embed security information for validating the pointer.
 % AArch64 Armv8-A is a 64-bit architecture that the pointer authentication information can be stored in the available spare bits in the most significant bits of the pointer. 
 %PTAuth~\cite{farkhani2021ptauth} used 
 %a similar feature on Cortex-A that is used to detect pointer manupilation~\cite{farkhani2021ptauth}.
 %It instruments the code to create a cryptographic authentication code (\verb|AC|) based on a unique ID of each heap object and store the \verb|AC| to the unused bits of the protected pointer.
 %Then authenticate the object during every pointer dereference by re-computing the \verb|AC|.
 %The mismatch of \verb|AC| indicates a temporal memory safety violation.
 %PTAuth incurs 2\% memory overhead and 26\% run-time overhead.
 % BTI mitigates against some JOP via creating an architectural dependency between certain indirect branch instructions and the targeted instructions.
 
 %BTI setting instructions, e.g., \verb|BLX|, set a new \verb|EPSR.B| bit to indicate indirect control flow transfer, and 
 %The target of the transfer must be a BTI clearing instructions, 
 %which include \verb|SG|, \verb|BTI|, and \verb|PACBTI|.
 %A new \verb|EPSR.B| bit is used to record indirect branches. %when BTI is enabled.
 %  for the target security and privilege level.
 %This bit will be set to 1 if BTI setting instruction executes and can only jump to BTI clearing instructions, which will set this bit to 0.
 %Armv8.1-M extends existing indirect branch instructions to support BTI setting and BTI clearing functionality.
 % \subsubsection{Secure Stacking and Unstacking}
 % When the \verb|FNC_RETURN| value loads to \verb|PC|, the processor automatically triggers the unstacking from the secure stack.
 % Similar to exception stacking and unstacking, discuss FNC\_RETURN here.
 %PAC in ARMv8.1-M is similar to Armv8.3-A with implementation differences~\cite{ARMpacbti, armv83A}.
 
 %The hardware handles the key switch for PAC generation or authentication.
 %On authentication failure, Cortex-A sets two bits in embedded PAC with fixed values, which results in a Translation fault when used by a branch.
 %The authentication instruction for cortex-M generates INVSTATE UsageFault on authentication failure.
 %Both ARMv8.1-M and Armv8.3-A use the QARMA algorithm to generate PACs~\cite{QARMA}.
 %Branch Target Identification (BTI) protects indirect branch targets by BTI setting and BTI clearing instructions~\cite{ARMpacbti, armv83A}.
 %A BTI setting instruction sets a bit in the execution program status register (\verb|EPSR|) to record an indirect jump, and a BTI clearing instruction clears the bit.
 %When the bit is set, any instruction fetches except a BTI clearing instruction will result in an exception.
 %BTI setting instructions include \verb|BX|, \verb|BXNS|, \verb|BLX|, \verb|BLXNS|, \verb|BFX|, \verb|BFLX|, \verb|LDR|, \verb|LDM|, \verb|LDMIA|, \verb|LDMFD|, \verb|LDMDB|, and \verb|LDMEA| instructions when used as an indirect branch target.
 %BTI clearing instructions include \verb|BTI|, \verb|SG|, and \verb|PACBTI| instructions which act as a valid landing pad. 
 \begin{comment}
 	\begin{mdframed}[style=remarkstyle,backgroundcolor=blue!10]
 		\textbf{Summary:} The Cortex-M architectures offer several security features, including TrustZone, pointer authentication, branch target identification, etc.
 	\end{mdframed}
 \end{comment}
 
 \begin{comment}
 	\ul{In summary, the Cortex-M architectures offer several security features, including TrustZone, pointer authentication, branch target identification, etc.
 		The Cortex-M TrustZone, which is optimized for faster context switches, has a much different underlying mechanism from the Cortex-A TrustZone. 
 		%The memory map based secure sate mechanism and special branching instructions reduce the world switch latency, resulting more efficient transitions.
 		%TrustZone provides multiple secure function entry points (\verb|SG|) to bridge software between two states.
 		Secure memory partitioning is controlled by IDAU and SAU, and MPCs can control memory aliasing.}
 \end{comment}
 
 %\ziming{Maybe a subsection to explain how the usage scenarios are different from PC and cloud. Maybe a comprehensive table or picture to compare with x86, Cortex-A, RISC-V.}
 
 \begin{comment}
 	\begin{table}[!h]
 		\center
 		\scriptsize
 		\caption{Firmware Sources}
 		\setlength\tabcolsep{0.7ex}
 		\renewcommand{\arraystretch}{1}
 		\rowcolors{2}{gray!15}{white}
 		\label{tab:fw}
 		\scalebox{0.92}{\begin{threeparttable}
 				\begin{tabular}{l|c|c|ccccccccc}
 					\hline
 					\multicolumn{1}{c|}{Source} & Link & \multicolumn{1}{c|}{Total} & Nordic & TI & Telink &Dialog &ST &Others\\ \hline \hline
 					HEAPSTER	&GitHub	&67 &-&-&-&-&4&63\\
 					GalaxyBudsFirmwareDownloader	&GitHub	&19 &-&-&-&-&-&19\\
 					Shannon Baseband Firmware	&GitHub	&19 &-&-&-&-&-&19\\
 					Polypyus Firmware Historian	&GitHub	&10 &-&-&-&-&-&10\\
 					Fuzzware	&GitHub	&50 &-&-&-&-&-&50\\
 					FrimXRay	&GitHub	&794 &769&25&-&-&-&-\\
 					Private Source1	&-	&249 &-&-&196&53&-&-\\
 					Private Source2	&-	&4336 &4336&-&-&-&-&-\\
 					%From Nico (New)	&-	&108& \\
 					Private Source3	&-	&113 &-&-&-&-&-&113\\
 					Private Source4	&-	&1574&-&-&-&-&-&1574\\	\hline
 					%total	&-	&5652 \\
 					%cortex-m&-	&1805\\
 					Total	&-	&7231 &5105&25&196&53&4&1848\\
 					Unique Cortex-M Based Systems&-	&1733 &1462&22&192&53&4&-\\
 					\hline
 				\end{tabular}
 				%\begin{tablenotes}
 				%\item[] The bug reports cover from hardware architecture to software implementation.
 				%\end{tablenotes}  
 		\end{threeparttable}}
 	\end{table}
 \end{comment}

==> background.tex <==
\section{Cortex-M Architecture in a Nutshell}
\label{sec:cortexm}

\begin{table}[!t]
    \center
    \scriptsize
    \renewcommand{\arraystretch}{1}
    \setlength\tabcolsep{0.7ex} 
    %\vspace{-0.4cm} 
    \caption{Cortex-M MCUs and Their Security-related Features}
    \vspace{-0.2cm}
    \label{tab:cortexmfamily}
    \rowcolors{2}{gray!15}{white}
    \begin{threeparttable}
    \begin{tabular}{llcccccccccccccc}
    \hline
    CPU                       & ISA                                 &\rotatebox{90}{Max MPU Regions}  &\rotatebox{90}{TrustZone-M}  &\rotatebox{90}{Max SAU Regions}    &\rotatebox{90}{PACBTI}     &\rotatebox{90}{PXN}&\rotatebox{90}{XOM}&\rotatebox{90}{MSPLIM/PSPLIM}   &\rotatebox{90}{UP Store/Load Ins.}  &\rotatebox{90}{Branch Prediction}  &\rotatebox{90}{ETM} &\rotatebox{90}{MTB} &\rotatebox{90}{DWT}  &\rotatebox{90}{FPB} &\rotatebox{90}{Year Introduced} \Tstrut{18ex}\\ \hline \hline
     M0~\cite{ArmCortexM0}    & v6-M~\cite{Armv6MArcRef}            &                                 &                             &                                   &                           &                   &                   &                                &                                    &                                   &                    &                    &\supportlevel{10}    &\supportlevel{5}    &2009\\ 
     M1~\cite{ArmCortexM1}    & v6-M                                &                                 &                             &                                   &                           &                   &                   &                                &                                    &                                   &                    &                    &\supportlevel{5}     &\supportlevel{5}    &2007 \\ 
     M0+~\cite{ArmCortexM0+}  & v6-M                                &8                                &                             &                                   &                           &                   &                   &                                &                                    &                                   &                    &\supportlevel{10}   &\supportlevel{10}    &\supportlevel{5}    &2012 \\ 
     M3~\cite{ArmCortexM3}    & v7-M~\cite{Armv7MArcRef}            &8                                &                             &                                   &                           &                   &                   &                                &\supportlevel{10}                   &\supportlevel{10}                  &\supportlevel{5}    &                    &\supportlevel{10}    &\supportlevel{10}   &2004 \\ 
     M4~\cite{ArmCortexM4}    & v7-M                                &8                                &                             &                                   &                           &                   &                   &                                &\supportlevel{10}                   &                                   &\supportlevel{5}    &                    &\supportlevel{10}    &\supportlevel{10}   &2010 \\ 
     M7~\cite{ArmCortexM7}    & v7-M                                &16                               &                             &                                   &                           &                   &                   &                                &\supportlevel{10}                   &\supportlevel{10}                  &\supportlevel{10}   &                    &\supportlevel{10}    &\supportlevel{10}   &2014 \\ 
     M23~\cite{ArmCortexM23}  & v8-M Baseline~\cite{Armv8MArcRef}   &16                               &\supportlevel{10}            &8                                  &                           &                   &                   &\supportlevel{10}               &\supportlevel{10}                   &                                   &\supportlevel{5}    &\supportlevel{10}   &\supportlevel{10}    &\supportlevel{10}   &2016 \\ 
     M33~\cite{ArmCortexM33}  & v8-M Mainline~\cite{Armv8MArcRef}   &16                               &\supportlevel{10}            &8                                  &                           &                   &                   &\supportlevel{10}               &\supportlevel{10}                   &                                   &\supportlevel{5}    &\supportlevel{10}   &\supportlevel{10}    &\supportlevel{5}    &2016 \\ 
     M35P~\cite{ArmCortexM35p}& v8-M Mainline                       &16                               &\supportlevel{10}            &8                                  &                           &                   &                   &\supportlevel{10}               &\supportlevel{10}                   &                                   &\supportlevel{5}    &\supportlevel{10}   &\supportlevel{10}    &\supportlevel{10}   &2018 \\ 
     M55~\cite{ArmCortexM55}  & v8.1-M Mainline~\cite{Armv8MArcRef} &16                               &\supportlevel{10}            &8                                  &\supportlevel{10}          &\supportlevel{10}  &\supportlevel{10}  &\supportlevel{10}               &\supportlevel{10}                   &\supportlevel{10}                  &\supportlevel{5}    &                    &\supportlevel{10}    &\supportlevel{5}    &2020 \\  
     M85~\cite{ArmCortexM85}  & v8.1-M Mainline                     &16                               &\supportlevel{10}            &8                                  &\supportlevel{10}          &\supportlevel{10}  &\supportlevel{10}  &\supportlevel{10}               &\supportlevel{10}                   &\supportlevel{10}                  &\supportlevel{5}    &                    &\supportlevel{10}    &\supportlevel{5}    &2022 \\ \hline                    
    \end{tabular}
    \begin{tablenotes}
    %    \item[1] Measured in percentages.
    %    \item[2] Measured in kilobytes (KB).
        \item[] Whitespace: Not support, \supportlevel{10}: Support, \supportlevel{5}: Partially Support. On M23, the ETM and the MTB are exclusive to each other.
     \end{tablenotes}
    \end{threeparttable}
    \vspace{-0.5cm} 
\end{table}
%\ziming{We need to make it clear what contributions are in Sec II and III. When I read the current version, as a reader I can learn something but doesn't mean it make contributions. Maybe summarize some technical highlights? maybe there is a way to formalize thing? Summarize some technical findings?}

%We discuss the Cortex-M architecture, %and security extensions,
%which are summarized from official documents~\cite{Armv6MArcRef, Armv7MArcRef, Armv8MArcRef, Armv8MArcTech, Armv8MMPU, ArmCortexM23, ArmCortexM33, ArmCortexM55, Armv8MTZ, ARMpacbti}. 
% and related books~\cite{yiu2020definitive, zhu2015embedded}.

%a brief summary of descriptions are available, they may be vague, incomplete, and buried in over tens of thousand pages of technical reference manuals. 
%This section does not attempt to cover everything, please refer to official docs~\cite{Armv6MArcRef, Armv7MArcRef, Armv8MArcRef, Armv8MArcTech, Armv8MMPU, ArmCortexM23, ArmCortexM33, ArmCortexM55, Armv8MTZ, ARMpacbti} and books~\cite{yiu2020definitive, zhu2015embedded} if you want to learn more. %, including TrustZone and Pointer Authentication and Branch Target Identification (PACBTI), etc.
%With TrustZone, many mechanisms, such as exception handling, have been extended.  
%Figure~\ref{fig:func-blocks} shows the hardware functional blocks of a Cortex-M System-on-Chip (SoC).

\subsection{General Properties} 

\noindent\textbf{General-purpose registers}.
A Cortex-M MCU has 16 general-purpose registers, i.e., \verb|R0| to \verb|R12|, \verb|R13/SP| (stack pointer), \verb|R14/LR| (link register), and \verb|R15/PC| (program counter).
Depending on the \emph{execution mode} and \verb|CONTROL| register, \verb|SP| shadows the main stack pointer (\verb|MSP|) or the process stack pointer (\verb|PSP|).
In Armv8-M, \verb|MSPLIM| and \verb|PSPLIM| hold the lower limit of the corresponding stack pointer. \verb|LR| holds the return address for a subroutine or a special value \verb|EXC_RETURN| when an interrupt occurs. 
%\gl{(so that the processor knows how to return correctly in the interrupt context)}.

\noindent\textbf{Execution mode, privilege level, and special registers}.
Cortex-M MCUs have thread %(\verb|T|)  
and handler %(\verb|H|) 
execution modes.
They, with the exception of M0/M0+/M1, also have privileged %(\verb|P|) 
and unprivileged 
%(\verb|U|) 
levels. %, which are orthogonal to the execution mode. 
%\gl{Change the preceding sentence to: The privilege level is orthogonal to the execution mode.}
Execution in the thread mode can be either privileged or unprivileged, whereas the handler mode is always privileged.  
%Software at the unprivileged level cannot execute privileged instructions and modify some memory regions, such as the Private Peripheral Bus (PPB).
The current execution mode and privilege level are determined by the combination of the interrupt program status register (\verb|IPSR|) and the \verb|CONTROL| register.
%If \verb|IPSR[8:0]| is 0, the processor is in the thread mode. 
%\verb|CONTROL[0]| determines whether the state is unprivileged,
%whereas \verb|CONTROL[1]| determines whether \verb|SP| shadows \verb|PSP| or \verb|MSP|.
To switch from privileged mode to unprivileged, one can simply set \verb|CONTROL[0]| to 1 using the move-to-system-register (\verb|MSR|) instruction.
To switch from unprivileged to privileged, the software uses the supervisor call (\verb|SVC|) instruction. 

\noindent\textbf{Physical memory map}.
The physical memory space of a Cortex-M MCU is 32-bit, which is equally divided into eight regions. 
%to map different types of memories, devices and system peripherals 
%as shown in Table~\ref{tab:Armv8-system-map}.
%The 4GB address space is sparsely populated due to the limited sizes of the physical devices.
The first region is reserved for \emph{code}. %, and it is mapped to on-chip ROMs or Flash memories. 
%The size of ROMs and Flash range from several KBs to several MBs.
The second region is mapped to on-chip \emph{SRAM}. 
%which together with two \emph{RAM} regions hold mutable run-time data, e.g., stack, heap, and global data.
%The size of SRAM and RAMs also range from several KBs to several MBs.
The \emph{peripheral} and two \emph{device} regions map I/O device registers.
%\gl{not sure the difference between peripheral region and two device regions.}
%which include General Purpose Input and Output (GPIO), Direct memory access (DMA) controller, etc.
The \emph{system} region maps system control registers,
including \emph{private peripheral bus} (PPB) for memory protection unit (MPU), security attribution unit (SAU) in Armv8-M, SysTick timer, etc.
%PPB is further divided into configurations for the secure and the non-secure state if TrustZone is implemented.
%A fixed eXecution Never (XN) attribute is associated with each region in that only \emph{code}, \emph{SRAM}, and 2 \emph{RAM} regions are executable.

\noindent\textbf{Automatic stacking and unstacking}.
When a higher-priority interrupt or exception occurs, the MCU automatically pushes eight registers, i.e., \verb|xPSR|, \verb|PC|, \verb|LR|, \verb|R12|, \verb|R3|, \verb|R2|, \verb|R1|, and \verb|R0|, to the current stack.
%, which is called context stacking. 
%If the Floating Point Unit (FPU) is enabled, the context stacking also pushes FPU related registers (\verb|S0| - \verb|S15| and \verb|FPSCR|; aka FP context).
Then, the MCU stores a special value \verb|EXC_RETURN| to the \verb|LR| register, and executes the interrupt service routine (ISR).
When the ISR returns, the MCU automatically performs unstacking to restore the context.
This is triggered by copying \verb|EXC_RETURN| to the \verb|PC| register.
%, which pops the eight registers off the stack. 

\noindent\textbf{Memory protection}.
The memory protection unit (MPU) regulates access permissions to software-designated physical regions based on the privilege level. Cortex-M55 MPU additionally introduces privileged execute never (\verb|PXN|).
%Different from a Memory Management Unit (MMU), an MPU does not support virtual memory. 
%As shown in Table~\ref{tab:cortexmfamily}, %the number of supported MPU regions on Cortex-M is small.
Most processors only support up to 16 MPU regions. 
%if the MPU is implemented. 
%The permission for an MPU region is determined by the Access Permission field (\verb|AP|) and the eXecute-Never bit (\verb|XN|).
%Armv7-M MPUs supports six access permissions, while Armv8-M MPUs defines eight access permissions.
%The \verb|XN| bit determines whether execution is permitted when read is permitted.
% Cortex-M55 MPU introduces privileged execute never (\verb|PXN|). %bit. %to prevent the processor from executing the code inside with the privileged level.

\noindent\textbf{Unprivileged memory access instructions}.
\label{sec:subsec:STRT}
The v7-M instruction set introduces several special store and load instructions (\verb|STR*T|/\verb|LDR*T|). %with unprivileged access. %as shown in Table~\ref{tab:SecInstruction}.
Even when these instructions are executed at the privileged level, they are treated as if they were executed at the unprivileged level.
%So the MPU checks the corresponding unprivileged permission bits when executing them~\cite{Armv7MArcRef}.

\noindent\textbf{Debug units}.
%As shown in Table~\ref{tab:cortexmfamily}, 
Cortex-M comes with many debug and trace units such as flash patch and breakpoint unit (FPB), data watchpoint and trace unit (DWT), micro trace buffer (MTB), and embedded trace macrocell (ETM). 
These units are restricted to the software at the privileged level and external hardware debug adapters.
They can perform instruction and data tracing, system events profiling, etc. %load and store operations counting, etc.
%These units are privileged access only by default and support invasive, i.e., control and observe, and non-invasive debugging, i.e., observe without control. 

%\ul{In summary, Cortex-M does not have many hardware features that are standard on microprocessors, such as MMU. %, cache, branch prediction, etc.
%It, however, offers hardware-assisted automatic stacking and unstacking for exception handling considering its interrupt-driven software model.
%Debug units, such as DWT, MTB, and ETM, are widely available on Cortex-M architectures.}

\subsection{Security Extensions}
\label{sec:tz}

\noindent\textbf{Secure and non-secure state}.
%TrustZone
%, which is introduced in the Armv8-M architecture, 
%adds an orthogonal partitioning of states to execution modes and privilege levels.
With the Armv8-M TrustZone-M extension (TrustZone-M), the MCU runs either in the secure state or non-secure state.
In the non-secure state, the processor can only access non-secure resources, 
%including memories and memory-mapped peripherals, 
whereas in the secure state, the processor can access all resources.
Different from Cortex-A TrustZone (TrustZone-A)~\cite{AArch64tz} where the selection of the effective execution state is configured in the secure configuration register, 
the division of states in Cortex-M is based on memory regions and the transition between them is regulated by newly introduced instructions (e.g., \verb|SG|). 
%If the processor is running code in the secure memory, the processor is in the secure state. 
%Otherwise, the processor is in the non-secure state.
%Each of the interrupts can be assigned as secure or non-secure in the interrupt target non-secure (\verb|NVIC_ITNS|) registers of NVIC.
%Non-secure interrupts can still be serviced when executing a secure function.
%\subsubsection{Banked Registers and System Peripherals}
Some special registers and system peripherals are banked for different security states, e.g., \verb|MSP|, \verb|PSP|, \verb|CONTROL[1-0]|.
%As shown in Table~\ref{tab:registers}, the general and special registers of \verb|MSP|, \verb|PSP|, \verb|MSPLIM|, \verb|PSPLIM|, \verb|CONTROL[1-0]|, \verb|PRIMASK|, \verb|BASEPRI|, and \verb|FAULTMASK| are banked between two worlds.

\noindent\textbf{Secure memory partitioning}.
A memory region can be secure, non-secure callable (NSC), or non-secure. % in descending order of security.
%A secure region is only accessible by secure software.
An NSC region is a special region that serves as a springboard from non-secure regions to secure regions using the \verb|SG| instruction.
% can have \verb|SG| instructions to enable software to transition from the non-secure state to the secure state. 
%A non-secure region can be accessed by non-secure and secure software. %, while a secure region can only be access by secure ones.
%Both secure and non-secure callable belong to secure. regions are further divided into two types: 
%When \verb|PC| points to an address in a non-secure callable region, the process is in the secure state.
The security assignment of a memory region is controlled by the combination of the internal secure attribution unit (SAU) and a vendor-specific implementation-defined attribution unit (IDAU).
SAU can configure up to 8 regions,
%No every system implements both SAU and IDAU.
%The SAU should always be present but may have different number of regions.
%If no SAU regions are defined, or the SAU is disabled, and no IDAU is included in the system then the entire memory address space is defined as secure.
%The SAU
%, which is memory-mapped in PPB, 
%is configurable, %anytime in the secure state. 
whereas IDAU 
%and they may be configurable or not before boot and 
can't be configured after boot.
%A typical design is to use the IDAU to define a fixed memory partition and use the SAU to change some security attributes at run-time.
%For instance, in xxx device the IDAU to splits memory into 256MB chunks of alternating secure and non-secure memory.
%As shown in Table~\ref{tab:idausau},
%If an address maps to regions defined by both SAU and IDAU, the region of the highest security level is selected.% (see Table~\ref{tab:idausau}).

\noindent\textbf{Memory aliasing, memory protection controller (MPC), and peripheral protection controller (PPC)}.
Memory aliasing, enabled by the MPC, maps shared resources between the secure and non-secure states.
%Privileged and unprivileged secure software can configure a Memory Protection Controller (MPC), which is included on the path to the memory,
% SSE-220 2.5.4 SRAM
%to divide the memory into equal size blocks and to selectively assign each block to its secure or non-secure alias at run-time. 
%The size of block is determined by the hardware.
%The MPC provides a single software-configurable bit to define if each block is assigned to secure or non-state world. 
%Each MPC's configuration interface is mapped to the peripheral region (\verb|0x5800????|).
%For instance, we assume SAU and IDAU together split the 512MB SRAM region into the non-secure (\verb|0x20000000| - \verb|0x2FFFFFFF|) and secure (\verb|0x30000000| - \verb|0x3FFFFFFF|) parts.
%A 2MB physical SRAM is mapped at two aliasing 2MB memory regions: (i) a secure region from \verb|0x28200000| - \verb|0x283FFFFF|; and (ii) a non-secure region from \verb|0x38200000| - \verb|0x383FFFFF|.
%Each block on the SRAM is 64KB, so the MPC provides 32 bits for this SRAM. 
%For example, the 4MB SRAM can be divided into 32 blocks with 64KB each.
Configuring the MPC at run-time can dynamically control which state a memory block is assigned to.
%Non-secure state can not configure the MPC which will trigger the attribution unit violation secure fault.
%Both Privileged and Unprivileged mode in the secure state can configure the MPC.
%\subsection{Peripheral Protection Controller}
%\label{sec:ppc}
Similar to an MPC, a PPC can also be added on paths to peripherals to provide security gating. 
%The PPCs perform the task of gating access to the peripherals it protects based on the security settings of each peripheral, and the security attribute of the access. 
%Each PPC can support up to 16 peripherals.
% The privileged access only Privilege Control Block (bankedSecure of Non-Secure) is used
%The configuration interfaces of PPCs are also mapped to the peripheral region.
%The privileged access only Privilege Control Block (\verb|0x40080000| - \verb|0x40080FFF| in non-secure, \verb|0x50080000| - \verb|0x50080FFF| in secure) is used for PPC to define the access settings for associated peripherals.
%For SSE200 subsystem~\cite{ArmCoreLinkSSE200}, PPC can configure the access setting of MHU (Message Handling Unit), DUAL TIMER, TIMER, and Watchdog that can raise an interrupt to the processor.
%Secure PCB can set the peripheral as non-secure access or secure unprivileged access.
%Non-secure PCB can set non-secure unprivileged access.
%[Seems only SSE200 subsystem talked about the PPC. The Arm architecture document and reference document did not mention it.]
% \ziming{need citation for SSE200}

\noindent\textbf{Synchronous state switching}. 
In contrast with Cortex-A processors, where there is a single entry point, i.e., secure monitor call, for entering or leaving the secure state, Cortex-M supports fast state switches with an unlimited number of entries.
% between the secure and non-secure software.
%This is achieved by the NSC region and some new instructions.
To switch from the non-secure state to the secure state, non-secure software uses the normal branch with link (\verb|BL|) instruction to call into a secure gateway (\verb|SG|) instruction in an NSC region.
% Also, the function the non-secure state wants to call must be declared as a non-secure entry.
% Each call targets to a non-exist entry will trigger an invalid entry point secure error.
Afterwards, the processor state is changed to secure. %, and the return state (1 for secure, 0 for non-secure) is stored in the least significant bit (LSB) of \verb|LR|.
% This is because Cortex-M does not support A32 instruction set, so the LSB of an address indicates the security state.
%After finishing the secure function, this bit will be checked to prevent returning to a fake secure address~\cite{Armv8MTZ}.
% Then branch to the secure state function.
To switch from the secure state to the non-secure state, the software uses the %interstating branch
branch with link and exchange non-secure (\verb|BLXNS|) instruction or branch and exchange non-secure (\verb|BXNS|) instruction.
% to  to a non-secure address.
%The target security state of those two instructions is indicated by the least significant bit of the target address, 1 means secure, 0 means non-secure~\cite{Armv8mdeveloper}.[need a test]
%\ziming{Where did you get this sentence? Also need to explain the meaning of least significant bit pf LR and SP.}
%The \verb|BLXNS| instruction switches the state to non-secure only when the LSB of the target address is 0. 
%When state switching happens, the processor first automatically pushes a special 32-bit value, namely combined exception Return Program Status Register (\verb|RETPSR|), and the return address with the LSB value 1 onto the current stack.
%The value of \verb|RETPSR| consists of \verb|IPSR| and other flags.
%The \verb|LR| is also changed to a special value named \verb|FNC_RETURN| (\verb|0xFEFFFFFF|).
%The LSB of \verb|FNC_RETURN| indicates which state this function is called from.
%Since it is only used in the non-secure function return, the value is always \verb|0xFEFFFFFF|.
%This automatic step is called \verb|FNC_RETURN| stacking.
%When the \verb|FNC_RETURN| value is loaded to \verb|PC|, the processor will unstack the \verb|RETPSR| value, check the \verb|IPSR|, and clear interruptions, then restore the return address to the secure state.
%The state switching mechanism for the \verb|BXNS| instruction is much simpler than the \verb|BLXNS| instruction. 
%If the target address is not \verb|FNC_RETURN| or \verb|EXC_RETURN| and the LSB is 0, \verb|BXNS| branches to non-secure code directly.
% It clears the \verb|CONTROL.SFPA| value to 0. 

\begin{comment}
\textbf{Asynchronous state switching or exception with TrustZone}.
\label{sec:subsec:asystateswithing}
%\subsubsection{ State Switching}
Exceptions and interrupts trigger state switches asynchronously. 
%, which extend the exception handling mechanisms discussed in \S\ref{sec:ExceptionStacking}.
%Secure privileged software can configure each interrupt, which could happen anytime, as secure or non-secure in the Interrupt Target non-secure (\verb|NVIC_ITNS|) registers.
If the exception entry is in the non-secure state,
the processor automatically pushes the state context and an additional state context onto the current stack.
The additional state context consists of a \verb|Magic Signature|, \verb|R4| - \verb|R11|~\cite{Armv8MArcRef}. 
%Different from the \verb|FNC_RETURN| stacking, \verb|RETPSR| is partially used to store the \verb|xPSR| value and other flags.
%The additional state context includes \verb|R11|, \verb|R10|, \verb|R9|, \verb|R8|, \verb|R7|, \verb|R6|, \verb|R5|, \verb|R4| along with an integrity signature value (\verb|0xFEFA125B| with Floating-point Extension, \verb|0xFEFA125A| without Floating-point Extension).
If the FPU is enabled, the current state is the secure state, the processor pushes additional FP context %(\verb|S16| - \verb|S31|)%, which are \verb|S0| to \verb|S15| and the Floating-point Status and Control Register (\verb|FPSCR|) for the secure state exception, additionally \verb|S16| to \verb|S30| for the non-secure state exception, 
onto the current stack. %armv8-m architecture reference p70
After context stacking, if the current state is non-secure, all pushed registers will remain unchanged.
If the current state is secure, those registers will be set to \verb|UNKNOWN| values or zeros depending on whether the exception happens in the secure state or the non-secure state.
To help save and clear the floating-point registers \verb|VLLDM| and \verb|VLSTM| instructions were introduced, which will only work when Floating-point is used in the non-secure state and will be considered as \verb|NOP| if FPU is not present.
When \verb|EXC_RETURN| is loaded to the \verb|PC|, the processor automatically unstacks the context stack and checks the return security state.
%The process also checks if the 0th bit of signature value matches the \verb|EXC_RETURN[4]|.
%If not, the processor generates a \verb|SecureFault| to prevent the non-secure software from using the interrupt return to switch to the secure state illegally.
%Since the address starting with \verb|0xF| is non-executable, treating the signature as an address will trigger \verb|MemManageFault|, e.g. replacing the \verb|EXC_RETURN| to \verb|FNC_RETURN| will fail~\cite{Armv8SecureStack}.
\end{comment}

\begin{comment}
\noindent\textbf{Test target instructions}.
\label{sec:subsec:TT}
The v8-M instruction set introduces the test target (TT) instructions for querying the security state and access permissions of a memory location~\cite{Armv8MArcRef}.
There are four variants to query a location for privileged and unprivileged access from the secure or the non-secure state.
% for a privileged (\verb|TT|, \verb|TTA| for non-secure) access or unprivileged (\verb|TTT|, \verb|TTAT| for non-secure) access to that location~\cite{Armv8MArcTech} C2.4.247.
% These instructions are only valid when executing in the secure state.
%The return information is stored in the \verb|TT_RESP| payload format. %, which includes IDAU, SAU, and MPU region number, and access permissions such as non-secure or secure read and writable, non-secure readable, and readable, etc. 
\end{comment}

\noindent\textbf{Pointer authentication and branch target identification (PACBTI)}.
\label{sec:subsec:PACBTI}
The v8.1-M instruction set introduces the PACBTI extension~\cite{ARMpacbti}. %, which is similar to its Cortex-A counterpart~\cite{armv83A}.
%, a similar version of which has been available on Cortex-A since Armv8.3-A, 
%to mitigate code reuse attacks. %return-oriented programming (ROP) and jump-oriented programming (JOP) attacks.
%Instructions related to this feature are presented in Table~\ref{tab:SecInstruction}.
% [should we explain the ROP and JOP here?]
% Unlike the AArch64 Armv8-A that can use some spare bits in the most significant bit of the pointer to embed security information for validating the pointer
Pointer authentication code (PAC) authenticates pointers at run-time, 
%separate to the pointer and can be enabled for every secure state and privileged level.
%Creating a PAC is to sign the pointer using a cryptographic mechanism, which takes the pointer, a 32-bit modifier in a general-purpose register, and a 128-bit secret key as inputs.
%The modifier encodes context information, whereas the key can only be managed at the privileged level.
%To sign a pointer in a general-purpose register, instruction \verb|PACG| is used.
%A special instruction \verb|PAC| is used to sign \verb|LR| and use \verb|SP| as the modifier.   
%To validate a pointer, it follows the same crypto step to generate another PAC called \verb|PACreturn| and compares it with the stored \verb|PACenter|.
%A \verb|UsageFault| exception is generated if the validation of a pointer fails.
%Even though this is a new feature on Cortex-M,
%Different from Cortex-M, AArch64 Armv8-A can use some spare bits in the most significant bit of the pointer to embed security information for validating the pointer.
% AArch64 Armv8-A is a 64-bit architecture that the pointer authentication information can be stored in the available spare bits in the most significant bits of the pointer. 
%PTAuth~\cite{farkhani2021ptauth} used 
%a similar feature on Cortex-A that is used to detect pointer manupilation~\cite{farkhani2021ptauth}.
%It instruments the code to create a cryptographic authentication code (\verb|AC|) based on a unique ID of each heap object and store the \verb|AC| to the unused bits of the protected pointer.
%Then authenticate the object during every pointer dereference by re-computing the \verb|AC|.
%The mismatch of \verb|AC| indicates a temporal memory safety violation.
%PTAuth incurs 2\% memory overhead and 26\% run-time overhead.
% BTI mitigates against some JOP via creating an architectural dependency between certain indirect branch instructions and the targeted instructions.
and branch target identification (BTI) prevents code reuse attacks 
%to arbitrary memory location 
by constraining indirect branch targets to BTI clearing instructions. % within a select memory region.
%BTI setting instructions, e.g., \verb|BLX|, set a new \verb|EPSR.B| bit to indicate indirect control flow transfer, and 
%The target of the transfer must be a BTI clearing instructions, 
%which include \verb|SG|, \verb|BTI|, and \verb|PACBTI|.
%A new \verb|EPSR.B| bit is used to record indirect branches. %when BTI is enabled.
%  for the target security and privilege level.
%This bit will be set to 1 if BTI setting instruction executes and can only jump to BTI clearing instructions, which will set this bit to 0.
%Armv8.1-M extends existing indirect branch instructions to support BTI setting and BTI clearing functionality.
% \subsubsection{Secure Stacking and Unstacking}
% When the \verb|FNC_RETURN| value loads to \verb|PC|, the processor automatically triggers the unstacking from the secure stack.
% Similar to exception stacking and unstacking, discuss FNC\_RETURN here.
%PAC in ARMv8.1-M is similar to Armv8.3-A with implementation differences~\cite{ARMpacbti, armv83A}.
While Cortex-A adopts the unused most significant bits of a 64-bit pointer to embed the PAC, Cortex-M %has 32-bit memory-mapped address space with no spare bits.
uses a 32-bit PAC and stores it in a general-purpose register.
%Stand-alone general-purpose registers are used to store the 32-bit (fixed) PAC, which leaves the pointer unmodified.
%Cortex-A architecture uses five 128-bit keys: two for data addresses, two for instruction addresses, and one for generic authentication.
Cortex-M has four PAC keys, one for each security state and privilege level.
%The hardware handles the key switch for PAC generation or authentication.
%On authentication failure, Cortex-A sets two bits in embedded PAC with fixed values, which results in a Translation fault when used by a branch.
%The authentication instruction for cortex-M generates INVSTATE UsageFault on authentication failure.
%Both ARMv8.1-M and Armv8.3-A use the QARMA algorithm to generate PACs~\cite{QARMA}.
%Branch Target Identification (BTI) protects indirect branch targets by BTI setting and BTI clearing instructions~\cite{ARMpacbti, armv83A}.
%A BTI setting instruction sets a bit in the execution program status register (\verb|EPSR|) to record an indirect jump, and a BTI clearing instruction clears the bit.
%When the bit is set, any instruction fetches except a BTI clearing instruction will result in an exception.
%BTI setting instructions include \verb|BX|, \verb|BXNS|, \verb|BLX|, \verb|BLXNS|, \verb|BFX|, \verb|BFLX|, \verb|LDR|, \verb|LDM|, \verb|LDMIA|, \verb|LDMFD|, \verb|LDMDB|, and \verb|LDMEA| instructions when used as an indirect branch target.
%BTI clearing instructions include \verb|BTI|, \verb|SG|, and \verb|PACBTI| instructions which act as a valid landing pad. 
\begin{comment}
\begin{mdframed}[style=remarkstyle,backgroundcolor=blue!10]
\textbf{Summary:} The Cortex-M architectures offer several security features, including TrustZone, pointer authentication, branch target identification, etc.
\end{mdframed}
\end{comment}

\begin{comment}
\ul{In summary, the Cortex-M architectures offer several security features, including TrustZone, pointer authentication, branch target identification, etc.
The Cortex-M TrustZone, which is optimized for faster context switches, has a much different underlying mechanism from the Cortex-A TrustZone. 
%The memory map based secure sate mechanism and special branching instructions reduce the world switch latency, resulting more efficient transitions.
%TrustZone provides multiple secure function entry points (\verb|SG|) to bridge software between two states.
Secure memory partitioning is controlled by IDAU and SAU, and MPCs can control memory aliasing.}
\end{comment}

%\ziming{Maybe a subsection to explain how the usage scenarios are different from PC and cloud. Maybe a comprehensive table or picture to compare with x86, Cortex-A, RISC-V.}

==> comments.tex <==
\begin{comment}
\begin{table*}[!htpb]
\center
\scriptsize
\caption{Comparative evaluation of security projects for Cortex-M or other embedded and IoT systems}
\vspace{-0.3cm}
\label{tab:vs-proj}
\scalebox{0.935}{
\begin{threeparttable}
\begin{tabular}{p{12.5ex}|p{0.01ex}p{0.01ex}p{2ex}|p{0.01ex}p{0.01ex}p{0.01ex}p{0.01ex}p{0.01ex}p{0.01ex}p{0.01ex}p{0.01ex}p{0.01ex}p{0.01ex}p{0.01ex}p{0.01ex}p{0.01ex}p{0.01ex}p{0.01ex}p{0.01ex}p{0.01ex}|p{0.01ex}p{0.01ex}p{0.5ex}|p{0.01ex}p{0.01ex}p{0.01ex}p{0.01ex}p{0.5ex}|p{0.5ex}p{0.5ex}p{0.8ex}|p{0.01ex}p{0.8ex}p{0.5ex}p{0.5ex}p{0.5ex}p{0.5ex}p{0.5ex}p{0.5ex}}
\hline
\multicolumn{1}{c}{Project}&\multicolumn{3}{c}{}&\multicolumn{20}{c}{Defenses}&\multicolumn{5}{c}{Hardware}&\multicolumn{3}{c}{}&\multicolumn{8}{c}{Run-time overhead (\%)} \\\hline 

&\rotatebox{90}{Input (C: source code; B: binary)}&\rotatebox{90}{Target (B: bare-metal; R: RTOS; M: Mbed)}&\rotatebox{90}{Prototype implementation (ISA)}&\rotatebox{90}{MPU-assisted isolation and confinement}&\rotatebox{90}{TrustZone-assisted multiple TEEs}&\rotatebox{90}{Software-based virtualization}&\rotatebox{90}{Shadow Stack}&\rotatebox{90}{SafeStack}&\rotatebox{90}{Return address integrity}&\rotatebox{90}{Forward control flow enforcement}&\rotatebox{90}{ROP gadget removal}&\rotatebox{90}{Artificial software diversity}&\rotatebox{90}{Execute only memory}&\rotatebox{90}{Software-based control flow attestation}&\rotatebox{90}{Software-based data integrity attestation}&\rotatebox{90}{Hybrid code integrity attestation}&\rotatebox{90}{Hybrid Proof of Execution}&\rotatebox{90}{Hybrid control flow attestation}&\rotatebox{90}{Hybrid data integrity attestation}&\rotatebox{90}{Secure software update}&\rotatebox{90}{Peripheral-aware static analysis}&\rotatebox{90}{Peripheral-aware symbolic execution}&\rotatebox{90}{Peripheral-aware fuzzing}& \rotatebox{90}{MPU} & \rotatebox{90}{Unprivileged store/load instructions}& \rotatebox{90}{TrustZone} & \rotatebox{90}{DWT} & \rotatebox{90}{Synthesized hardware} & \rotatebox{90}{Code, binary size increasement (Flash \%)}&\rotatebox{90}{Memory overhead (RAM \%)}&\rotatebox{90}{Energy consumption overhead (\%)}&\rotatebox{90}{Bare-metal applications}&\rotatebox{90}{RTOSs}&\rotatebox{90}{BEEBS~\cite{pallister2013beebs}} & \rotatebox{90}{CoreMark~\cite{coremark2021}} & \rotatebox{90}{CoreMark-Pro~\cite{coremarkpro2021}} & \rotatebox{90}{MiBench~\cite{guthaus2001mibench}} &\rotatebox{90}{Dhrystone~\cite{weicker1984dhrystone}} & \rotatebox{90}{BenchIoT~\cite{almakhdhub2019benchiot}}   \\ \hline \hline
% nesCheck~\cite{midi2017memory} &$\circ$ &&&&&&&&&& - & TinyOS applications & - \\

%                                     &C&R &v7 &                Defenses                                  & Hardware     &        performance   &\\

uSFI~\cite{aweke2018usfi}             &C&R &v7 &\supportlevel{10}&  &  &  &  &  &  &\supportlevel{10}&  &   &  &   &  &  &  &  &  &  &  &  &\supportlevel{10}&\supportlevel{10}&  &  &  &\textcolor{darkblue}{10}&  &  &\textcolor{darkblue}{0.7}&\textcolor{darkblue}{9.6}&  &  &  &\textcolor{darkblue}{1.1}&  &\\
$\mu$Visor~\cite{uVisor}              &C&M &v7 &\supportlevel{10}&  &  &  &  &  &  &  &  &   &  &   &  &  &  &  &  &  &  &  &\supportlevel{10}&  &\supportlevel{10}&  &  &  &  &  &  &  &  &  &  &  &  &\\
EPOXY~\cite{clements2017EPOXY}        &C&B &v7 &\supportlevel{10}&  &  &  &\supportlevel{10}&  &  &  &\supportlevel{10}&   &  &   &  &  &  &  &  &  &  &  &\supportlevel{10}&  &  &  &  &\textcolor{darkblue}{8}&  &\textcolor{darkblue}{1.1}&\textcolor{darkblue}{1.8}&  &\textcolor{darkblue}{1.6}&\\
ACES~\cite{clements2018aces}          &C&B &v7 &\supportlevel{10}&  &  &  &  &  &\supportlevel{10}&  &  &   &  &   &  &  &  &  &  &  &  &  &\supportlevel{10}&  &  &  &  &\textcolor{darkorange}{26}&  &  &\textcolor{darkblue}{5.7}&  &  &  &  &  &  &\\
MINION~\cite{kim2018securing}         &C&R &v7 &\supportlevel{10}&  &  &  &  &  &  &  &  &   &  &   &  &  &  &  &  &  &  &  &\supportlevel{10}&  &  &  &  &  &  &  &  &\textcolor{darkblue}{2}&  &  &  &  &  &\\ 
%  Hermes~\cite{klingensmith2018hermes} && & &\supportlevel{10}&  &  &  &  &  &  &  &   &  &   &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &\textcolor{darkblue}{2}&  &  &  &  &  &\\
%  LTZVisor~\cite{pinto2017ltzvisor} && & &\supportlevel{10}&  &  &  &  &  &  &  &   &  &   &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &\textcolor{darkblue}{2}&  &  &  &  &  &\\
Utango~\cite{oliveira2021utango}      &B&R &v8 &  &\supportlevel{10}&  &  &  &  &  &  &  &   &  &   &  &  &  &  &  &  &  &  &\supportlevel{10}&  &\supportlevel{10}&  &  &\textcolor{darkblue}{4.6}&  &  &  &  &  &  &  &  &  &\textcolor{darkgreen}{.05}\\ 
Hermes~\cite{klingensmith2018hermes}&B&R &v7 &  &  &\supportlevel{10}&  &  &  &  &  &  &   &  &   &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ \hline
Silhouette~\cite{zhou2020silhouette}  &C&B &v7 &  &  &  &\supportlevel{10}&  &  &  &  &  &   &  &   &  &  &  &  &  &  &  &  &\supportlevel{10}&\supportlevel{10}&  &  &  &\textcolor{darkblue}{8.9}&  &  &  &  &\textcolor{darkblue}{3.4}&  &\textcolor{darkblue}{1.3}&  & \\ 
CaRE~\cite{nyman2017cfi}              &B&B &v8 &  &  &  &\supportlevel{10}&  &  &&  &  &   &  &   &  &  &  &  &  &  &  &  &\supportlevel{10}&  &\supportlevel{10}&  &  &  &  &  &  &  &  &  &  &  &\textcolor{darkred}{513}&\\ 
TZmCFI~\cite{kawada2020TZmCFI}        &C&R &v8 &  &  &  &\supportlevel{10}&  &  &  &  &  &   &  &   &  &  &  &  &  &  &  &  &\supportlevel{10}&  &  &  &  &  &  &  &  &\textcolor{darkorange}{84}&  &\textcolor{darkorange}{14}&  &  &  &  \\ 
$\mu$RAI~\cite{almakhdhubmurai2020}   &C&B &v7 &  &  &  &  &  &\supportlevel{10}&\supportlevel{10}&  &  &   &  &   &  &  &  &  &  &  &  &  &\supportlevel{10}&  &  &  &  &\textcolor{darkorange}{54.1}&\textcolor{darkblue}{15.2}&  &\textcolor{darkgreen}{.1}&  &  &\textcolor{darkgreen}{.1}&  &  &  &\\ \hline
uXOM~\cite{kwon2019uxom}          &C&R &v7 &  &  &  &  &  &  &  &\supportlevel{10}&  &\supportlevel{10} &  &   &  &  &  &  &  &  &  &  &\supportlevel{10}&\supportlevel{10}&  &  &  &\textcolor{darkblue}{15.7}&  &\textcolor{darkblue}{7.5}&  &  &\textcolor{darkblue}{7.3}&  &  &  &  &\\ 
PicoXOM~\cite{shen2020fast}           &C&R &v7 &  &  &  &  &  &  &  &  &  &\supportlevel{10} &  &   &  &  &  &  &  &  &  &  &\supportlevel{10}&  &  &\supportlevel{10}&  &\textcolor{darkblue}{5.89}&  &  &\textcolor{darkgreen}{.02}&  &\textcolor{darkgreen}{.46}&  &\textcolor{darkgreen}{.11}&  &  &\\ \hline 
C-FLAT~\cite{abera2016c}              &B&B &A  &  &  &  &  &  &  &\supportlevel{10}&  &  &   &\supportlevel{10}&   &  &  &  &  &  &  &  &  &  &  &\supportlevel{10}&  &  &\textcolor{darkorange}{25}&  &  &\textcolor{darkorange}{76}&  &  &  &  &  &  &\\ 
LAPE~\cite{huo2020lape}               &C&B &v7 &\supportlevel{10}&  &  &  &  &  &\supportlevel{10}&  &  &   &\supportlevel{10}&   &  &  &  &  &  &  &  &  &\supportlevel{10}&  &  &  &  &\textcolor{darkorange}{30}&\textcolor{darkblue}{7.5}&  &\textcolor{darkblue}{2.2}&  &  &  &  &  &  &\\ 
% FLASH: 38%, RAM: 8.2%
OAT~\cite{sun2020oat}                 &C&B &A  &  &  &  &  &  &  &\supportlevel{10}&  &  &   &\supportlevel{10}&\supportlevel{10} &  &  &  &  &  &  &  &  &  &  &\supportlevel{10}&  &  &\textcolor{darkblue}{13}&  &  &\textcolor{darkblue}{2.7}&  &  &  &  &  &  & \\ 
DIAT~\cite{abera2019diat}             &C&R &v7 &  &  &  &  &  &  &\supportlevel{10}&  &  &   &\supportlevel{10}&\supportlevel{10} &  &  &  &  &  &  &  &  &  &  &\supportlevel{10}&  &  &  &  &  &  &  &  &  &  &  &  &\\ \hline  
VRASED~\cite{nunes2019vrased}         &C&B &*  &  &  &  &  &  &  &  &  &  &   &  &   &\supportlevel{10}&  &  &  &  &  &  &  &  &  &  &  &\supportlevel{10}&  &\textcolor{darkblue}{3.5}&  &  &  &  &  &  &  &  &\\ 
APEX~\cite{nunes2020apex}             &C&B &*  &  &  &  &  &  &  &  &  &  &   &  &   &  &\supportlevel{10}&  &  &  &  &  &  &  &  &  &  &\supportlevel{10}&  &\textcolor{darkgreen}{.01}&  &  &  &  &  &  &  &  &\\ 
TinyCFA~\cite{nunes2020tiny}          &B&B &*  &  &  &  &  &  &  &\supportlevel{10}&  &  &   &  &   &  &  &\supportlevel{10}&  &  &  &  &  &  &  &  &  &\supportlevel{10}&\textcolor{darkorange}{80}&  &  &\textcolor{darkorange}{50}& \\ 
DIALED~\cite{nunes2021dialed}         &B&B &*  &  &  &  &  &  &  &\supportlevel{10}&  &  &   &  &   &  &  &\supportlevel{10}&\supportlevel{10}&  &  &  &  &  &  &  &  &\supportlevel{10}&  &  &  &  &  &  &  &  &  &  &\\ \hline
% on top of tinyCFA, run-time overhead is 20\%
ASSURED~\cite{asokan2018assured}      &B&R &v8 &  &  &  &  &  &  &  &  &  &   &  &   &  &  &  &  &\supportlevel{10}&  &  &  &  &  &\supportlevel{10}&  &  &\textcolor{darkorange}{67}&  &  &\textcolor{darkblue}{6}&  &  &\\ \hline
PASAN~\cite{kim2021pasan}             &C&R &v7 &  &  &  &  &  &  &  &  &  &   &  &   &  &  &  &  &  &\supportlevel{10}&  &  &  &  &  &  &  &  &  &  &  &  &  &\\
argXtract~\cite{sivakumaran2021argxtract} &B&R &v6/7 &  &  &  &  &  &  &  &  &  &   &  &   &  &  &  &  &  &\supportlevel{10}&  &  &  &  &  &  &  &  &  &  &  &  &  &\\
FIE~\cite{davidson2013fie}            &C&R &*  &  &  &  &  &  &  &  &  &  &   &  &   &  &  &  &  &  &  &\supportlevel{10}&  &  &  &  &  &  &  &  &  &  &  &  &\\
P2IM~\cite{feng2020p}                 &C&R &v7 &  &  &  &  &  &  &  &  &  &   &  &   &  &  &  &  &  &  &  &\supportlevel{10}&  &  &  &  &  &  &  &  &  &  &  &\\
DICE~\cite{mera2020dice}              &C&R &v7 &  &  &  &  &  &  &  &  &  &   &  &   &  &  &  &  &  &  &  &\supportlevel{10}&  &  &  &  &  &  &  &  &  &  &  &\\
Laelaps~\cite{cao2020device}			&B&R &v7 &  &  &  &  &  &  &  &  &  &   &  &   &  &  &  &  &  &  &\supportlevel{10}&\supportlevel{10}&  &  &  &  &  &  &  &  &  &  &  &\\
$\mu$Emu~\cite{zhou2021automatic}     &B&R &v7 &  &  &  &  &  &  &  &  &  &   &  &   &  &  &  &  &  &  &\supportlevel{10}&\supportlevel{10}&  &  &  &  &  &  &  &  &  &  &  &\\
\hline 
\end{tabular}
\begin{tablenotes}
\item[] v7: Armv7-M, v8: Armv8-M, A: Cortex-A, *: TI MSP430~\cite{MSP430}. \supportlevel{10}: Implement a specific security feature or need a specific hardware support. {\color{darkgreen} green}: $\le$1\% negligible overhead, {\color{darkblue} blue}: $<$20\% practical, {\color{darkorange} orange}: $<$100\% noticeable, {\color{darkred} red}: $>$100\% heavy overhead. 
% \item[] Code and memory overhead shows the best case, run-time overhead shows the worst case.
% \item[]: Bare-metal only or RTOSes. Input - source code; binary. Developer involvement - None; annotation; code modification. .
\end{tablenotes}  
\end{threeparttable}
}
\vspace{-0.5cm}
\end{table*}
\end{comment}

\begin{comment}
\subsection{Side channel detection}

\defense{Timing side channel detection}:
Bauer et al.~\cite{bauer2016towards} propose an approach that utilizes cycle-accurate behavioral emulation of relevant CPU behavior such as instruction pipeline flushes and bus connection to detect timing side channels to defense information leakage (see \textbf{I20}).
\end{comment}


%Towards Cycle-Accurate Emulation of Cortex-M Code to Detect Timing Side Channels

%\defense{Lightweight virtualization.} 
%Femto-Containers: DevOps on Microcontrollers with Lightweight Virtualization \& Isolation for IoT Software Modules~\cite{zandberg2021femto}

% \subsubsection{Real-world applications}
\begin{comment}
\begin{table*}[!htpb]
  \center
  \scriptsize
  \caption{Real-world project}
  \vspace{-0.3cm}
  \label{tab:real-app}
  \begin{tabular}{lll}
  \hline
  Project     & Real-world app/Benchmark                            & Source   \\ \hline  \hline
  uSFI        & MiBench~\cite{guthaus2001mibench}   & https://github.com/mageec/beebs\\
              & mbed TLS~\cite{pallister2013beebs}  & https://github.com/ARMmbed/mbedtls\\
  uSFI, TZmCFI& FreeRTOS~\cite{coremark2021}        & https://github.com/FreeRTOS/FreeRTOS\\
  EPOXY, ACES, $\mu$RAI, PicXoM & STM32Cube firmware          & https://github.com/STMicroelectronics/STM32CubeF4\\
  MINION      & 3DR Pixhawk                 & https://github.com/3drobotics/Pixhawk\_OS\_Hardware \\
  uTango      & BenchIoT~\cite{almakhdhub2019benchiot} & https://github.com/embedded-sec/BenchIoT\\
  Silhouette, TZmCFI  & CoreMark~\cite{coremark2021}    & https://github.com/eembc/coremark\\
  Silhouette, PicXoM  & BEEBS~\cite{guthaus2001mibench} & https://github.com/mageec/beebs\\
  CaRE        & OTP, HMAC & \\
              & Dhrystone~\cite{weicker1984dhrystone}&  https://github.com/Keith-S-Thompson/dhrystone \\
  uXOM        & RIOT-OS~\cite{RIOT} & https://github.com/RIOT-OS/RIOT \\
  PicXoM      & CoreMark-Pro~\cite{coremarkpro2021} & https://github.com/eembc/coremark-pro\\
  C-FLAT, OAT, Tiny-CFA, DIALED & Open syringe pump   & https://github.com/naroom/OpenSyringePump/blob/master/syringePump/syringePump.ino\\
  OAT         & House alarm system  & https://github.com/ddrazir/alarm4pi\\
              & Remote movement controller & https://github.com/bskari/pirc/tree/pi2\\
              & Recover controller & http://github.com/Gwaltrip/RoverPi/tree/master/tcpRover\\
              & Light Controller  & https://github.com/Barro/light-controller\\
  DIAT        & Pixhawk (flight controller for drones)           & https://pixhawk.org \\
  VRASED, APEX& original OpenMSP430 core      & openMSP430, 2009\\
  DIALED      & FireSensor      & 
  https://github.com/Seeed-Studio/LaunchPad\_Kit/tree/master/Grove\_Modules/temp\_humi\_senso\\
              & UltrasonicRanger  & https://github.com/Seeed-Studio/LaunchPad\_Kit/tree/master/Grove\_Modules/ultrasonic\_ranger\\
  p$^2$IM     & NuttX, RIOT, and Arduino & \\
              & Self-balancing robot & https://github.com/mbocaneg/Inverted-Pendulum-Robot\\
              & Programmable logic controller & https://github.com/CONTROLLINO-PLC/CONTROLLINO\_Library/tree/master/MAXI\\
              & Gateway & https://github.com/firmata/arduino\\
              & Drone & https://github.com/heethesh/eYSIP-2017\_Control\_and\_Algorithms\_development\_for\_Quadcopter\\
              & CNC & https://github.com/deadsy/grbl\_stm32f4\\
              & Reflow oven & https://github.com/rocketscream/Reflow-Oven-Controller\\
              & RIOT console & https://github.com/RIOTOS/RIOT/tree/master/examples/default\\
              & Steering control & https://github.com/jabelone/car-controller\\
              & Soldering iron & https://github.com/Ralim/ts100\\
              & Heat press & https://en.wikipedia.org/wiki/Heat\_press\\
  DICE        & too much  &\\
  ASSURED     & ?? \\


  % pqm4~\cite{kannwischer2019pqm4} & Cortex-M4 \\
  \hline
  \\                                                                    
  \end{tabular}
\end{table*}
\end{comment}

% \begin{table}[!htpb]
%   \center
%   \scriptsize
%   \caption{Benchmarks}
%   \vspace{-0.3cm}
%   \label{tab:bm}
%   \begin{tabular}{lll}
%   \hline
%   Name                            & Source   \\ \hline  \hline
%   BEEBS~\cite{guthaus2001mibench} & \\
%   MiBench~\cite{pallister2013beebs} & https://github.com/mageec/beebs\\
%   CoreMark~\cite{coremark2021}    & https://github.com/eembc/coremark\\
%   CoreMark-Pro~\cite{coremarkpro2021} & https://github.com/eembc/coremark-pro\\
%   BenchIoT~\cite{almakhdhub2019benchiot}                & https://github.com/embedded-sec/BenchIoT\\
%   MiBench~\cite{guthaus2001mibench}                 & https://github.com/embecosm/mibench\\
%   % pqm4~\cite{kannwischer2019pqm4} & Cortex-M4 \\
%   \hline
%   \\                                                                    
%   \end{tabular}
% \end{table}

\begin{comment}
\subsection{Other IoT Platforms}
Some papers are talking about other embedded devices, not specific for Cortex-M processors.

% TrustLite~\cite{koeberl2014trustlite}  
nesCheck~\cite{midi2017memory} provides a low-overhead spatial memory safety enforcement for TinyOS~\cite{TinyOS}, 
which is a popular embedded OS for wireless sensor network nodes that developed in the nesC language.
It uses static analysis including type tracking to identify memory safety vulnerabilities at compile time.
Then it maintains the metadata for each pointer that contains the memory area where the pointer points to, checks the bounds of the memory address at run-time.
nesCheck is specifically designed for TinyOS applications, which is not support the Cortex-M now.

HART~\cite{du2020hart} proposes an ETM-assisted kernel module on Arm processors.
It reconstructs the program execution by decoding the ETM trace packets.
Built based-on HART, HASAN can detect memory corruptions.
% Hans~\cite{okkerman2020embedded} presents an embedded memory security module to protect the integrity and authenticity of data and applications for IoT devices.
\end{comment}

% \subsection{Machine Learning}

% MCUNet~\cite{lin2020mcunet} is a tiny deep learning model on IoT devices that enable ImageNet-scale inference.
% CMSIS-NN~\cite{lai2018cmsis} optimizes the performance of neural networks on Cortex-M CPUs.

\begin{comment}
\begin{table}[!t]
	\center
	\scriptsize
	\caption{CVEs for Cortex-M Software Systems}
	\vspace{-0.3cm}
	\label{tab:CVEs-con}
	\begin{threeparttable}
		\begin{tabular}{p{19ex}|p{34ex}|p{0.6ex}|p{0.5ex}p{0.5ex}p{0.5ex}p{0.5ex}}
			\hline
			Class                 & Subclass  & \rotatebox{90}{\# Bugs} &\rotatebox{90}{Critical} & \rotatebox{90}{High} & \rotatebox{90}{Medium} \\ \hline  \hline
			Hardware Limitation   & Information leakage though cache  & 2  & &  &2     \\ \hline  
			& Improper stack selection          & 1  & & &1           \\ 
			Architectural Issue   & Unprotected hardware block          & 1  & & &1           \\ 
			& Inf. leakage through state switch         & 1  & & &1           \\ \hline
			\multirow{4}{*}{Software}  & Network communication & 61   &33&19&9     \\ 
			\multirow{4}{*}{Implementation Issue}  & Validation bugs in privileged code     & 28    &4 &20&4     \\ 
			& Vulnerable crypto implementation  &4 &&1&3\\ 
			& Functional implementation bugs & 23    &2&14&7 \\ 
			& Timing side channel              & 15    &1&1&13 \\ 
			% & Concurrency???            & 4     &-&2 (50\%)&2 (50\%)     \\ 
			\hline                                                                   
		\end{tabular}
		\begin{tablenotes}
			\item[] CVEs reports for Mbed, RIOT-OS, TockOS, FreeRTOS, Contiki-ng, Nuttx, Zephyr, wolfSSL, and STM32 from 2015 to 2021 for software implementation issues.
		\end{tablenotes}  
	\end{threeparttable}
	\vspace{-0.5cm}
\end{table}
\end{comment}

\begin{comment}
\begin{table*}[!t]
  \center
  \scriptsize
  \caption{Summary of CVEs for Cortex-M Software}
  \vspace{-0.3cm}
  \label{tab:CVEs-con}
  \begin{tabular}{llc|cccc}
  \hline
  Class                 & Subclass  & \# Bugs     & Critical & High & Medium \\ \hline  \hline
  Hardware Limitation   & Information leakage though cache  & 2  &- &-  &2 (100\%)     \\ \hline  
  Architectural Issue   & Improper stack selection          & 1  &- &- &1 (100\%)           \\ \hline
  \multirow{6}{*}{Implementation Issue}  & Network Communication & 61   &33 (54.10\%)&19 (31.15\%)&9 (14.75\%)      \\ 
                        & Other privileged code     & 28    &4 (14.29\%)&20 (71.43\%)&4 (14.29\%)      \\ 
                        & Vulnerable Crypto Implementation  &4 &-&1 (25\%)&3 (75\%) \\ 
                        & Other implementation bugs & 23    &2 (8.70\%)&14 (60.87\%)&7 (30.43\%)     \\ 
                        & Side channel              & 15    &1 (6.67\%)&1 (6.67\%)&13 (86.67\%)      \\ 
                        % & Concurrency???            & 4     &-&2 (50\%)&2 (50\%)     \\ 
                        \hline                                                                   
  \end{tabular}
\end{table*}
\end{comment}

\begin{comment}
\begin{table*}[!htpb]
  \center
  \scriptsize
  \caption{CVEs}
  \vspace{-0.3cm}
  \label{tab:sw-CVEs}
  \begin{tabular}{lllp{6cm}}
  \hline
  Type                  & OS/App/Hardware           & CVE ID           & Description \\ \hline  \hline
  Access uninitialized pointer& FreeRTOS            & CVE-2018-16522 \\
                        & Zephyr Project  & CVE-2020-10060 \\ \hline
  Buffer overflow       & Mbed TLS                  & CVE-2018-0487 \\ %\cline{2-4}
                        & RIOT-OS                   & CVE-2019-1000006 \\ %\cline{2-4}
                        & FreeRTOS                  & CVE-2018-16526, CVE-2018-16525 \\ %\cline{3-4}
                        & Contiki-NG                & CVE-2020-24336, CVE-2018-19417 \\
                        &                           & CVE-2018-16665, CVE-2018-16664 \\
                        &                           & CVE-2018-1000804 \\ %\cline{2-4}
                        & Mbed TLS                  & CVE-2015-8036, CVE-2015-5291 & Heap-based\\ %\cline{2-4}
                        & Mbed CoAP lib             & CVE-2020-12883, CVE-2019-17212 \\ %\cline{2-4}
                        & RIOT-OS                   & CVE-2021-27698, CVE-2021-27697 & Buffer Copy without Checking Size of Input\\
                        &                           & CVE-2021-27357, CVE-2020-15350  \\ %\cline{2-4}
                        & RIOT-OS                   & CVE-2017-8289 & Stack based \\ 
                        & Zephyr Project            & CVE-2020-10071, CVE-2020-10070 \\ 
                        &                           & CVE-2020-10023, CVE-2020-10022 \\ 
                        &                           & CVE-2020-10019, CVE-2017-14202 \\ 
                        &                           & CVE-2017-14199 \\ \hline
  Confused Deputy       & FreeRTOS                  & CVE-2018-16598 \\ \hline
  Divide by zero        & FreeRTOS                  & CVE-2018-16523 \\ \hline
  Side channel attack   & Mbed TLS                  & CVE-2020-16150, CVE-2020-10941 \\
                        &                           & CVE-2020-10932, CVE-2019-18222 \\
                        &                           & CVE-2019-16910, CVE-2018-0498\\
                        &                           & CVE-2018-0497, \\ \hline
  Out-of-bounds read    & Mbed TLS                  & CVE-2018-9989, CVE-2018-9988	  &  \\ %\cline{2-4} 
                        & Mbed CoAP lib             & CVE-2020-12886, CVE-2020-12884 \\ %\cline{2-4}
                        & FreeRTOS                  & CVE-2019-13120 \\ %\cline{2-4}
                        & Contiki-NG                & CVE-2020-24335, CVE-2020-24334 \\
                        &                           & CVE-2020-14937, CVE-2018-16667 \\ \hline
  Improper privilege management & Mbed TLS          & CVE-2018-19608 \\ \hline
  Out-of-bounds write   & Mbed TLS                  & CVE-2018-0488 & \\ %\cline{2-4}
                        & Mbed CoAP lib             & CVE-2019-17212 \\ %\cline{2-4}
                        & Contiki-NG                & CVE-2020-14937, CVE-2020-14936 \\
                        &                           & CVE-2020-14935, CVE-2020-14934 \\ 
                        &                           & CVE-2019-8359, CVE-2018-20579 \\
                        &                           & CVE-2018-16666, CVE-2018-16663 \\ 
                        & NuttX                     & CVE-2020-17528, CVE-2020-17529 \\ 
                        & wolfSSL                   & CVE-2020-36177\\
                        & Zephyr Project & CVE-2020-10021 \\ \hline
  Improper Certificate Validation & Mbed TLS        & CVE-2017-2784 \\ 
                        & Zephyr Project            & CVE-2020-10059 \\ \hline
  Integer Overflow or wraparound& Mbed OS           & CVE-2021-27435, CVE-2021-27433 \\ \hline
                        & Mbed TLS                  & CVE-2017-18187 & Bound-check bypass\\ %\cline{2-4}
                        & Mbed CoAP lib             & CVE-2019-17211 \\ %\cline{2-4}
                        & FreeRTOS                  & CVE-2021-31572, CVE-2021-31571 \\
                        &                           & CVE-2018-16601 \\ %\cline{2-4}
                        & Contiki-NG                & CVE-2019-9183 \\ 
                        & RIOT OS                   & CVE-2021-27427 \\ 
                        & TI-RTOS                   & CVE-2021-27429, CVE-2021-22636 \\
                        &                           & CVE-2021-27502 \\ 
                        & NuttX                     & CVE-2021-26461 \\ 
                        & Zephyr Project            & CVE-2020-10067, CVE-2020-10063 \\ \hline
  Improper Authentication & Mbed TLS                & CVE-2017-14032 \\ \hline
  Improper Input Validation & Mbed TLS              & CVE-2016-3739 \\ %\cline{2-4}
                        & Mbed MQTT lib             & CVE-2019-17210 \\ %\cline{2-4}
                        & FreeRTOS                  & CVE-2018-16528 \\ 
                        & Zephyr Project            & CVE-2020-10068, CVE-2020-10058 \\
                        &                           & CVE-2020-10028 \\ \hline
  Incorrect comparison  & Zephyr Project            & CVE-2020-10027, CVE-2020-10024 \\ \hline
  Off-by-one Error      & Zephyr Project            & CVE-2020-10062  \\ \hline
  Socket related        & RIOT-OS                   & CVE-2019-17389 \\ \hline
  NULL Pointer Dereference  & RIOT-OS               & CVE-2019-16754 \\ 
                        & NuttX                     & CVE-2020-1939 \\ 
                        & Zephyr Project            & CVE-2018-1000800 \\ \hline
  Infinite loop         & Mbed CoAP lib             & CVE-2020-12885 \\ %\cline{2-4}
                        & RIOT-OS                   & CVE-2019-15702 \\ 
                        & NuttX                     & CVE-2018-20578 \\ \hline
  Memory/data leakage   & Mbed CoAP lib             & CVE-2020-12887 \\ %\cline{2-4}
                        & RIOT-OS                   & CVE-2019-15134 \\ %\cline{2-4}
                        & FreeRTOS  & CVE-2018-16603, CVE-2018-16602 \\
                        &                           & CVE-2018-16600, CVE-2018-16599 \\
                        &                           & CVE-2018-16527, CVE-2018-16524 \\ %\cline{2-4}
                        & TockOS  & CVE-2018-1000660 
                        \\ \hline
  Unknown               & FreeRTOS                  & CVE-2021-32020 \\ \hline
  Use after free        & FreeRTOS                  & CVE-2019-18178 \\ 
                        & Zephyr Project            & CVE-2017-14201 \\ \hline
  Inadequate Encryption Strength & Stm32Cube crypto extension  & CVE-2020-20949 \\ \hline
  Stack underflow       & Armv8-M TrustZone         & CVE-2020-16273  & \\ \hline %https://cve.mitre.org/cgi-bin/cvename.cgi?name=CVE-2020-16273
  \\                                                                    
  \end{tabular}
\end{table*}
\end{comment}

% https://docs.zephyrproject.org/latest/security/vulnerabilities.html#
% https://cve.mitre.org/cgi-bin/cvekey.cgi?keyword=mbed


% 1. Most systems run code at the same privileged level, form baremetal system to the default configuration of Amazon FreeRTOS (v1.4.7)

% Armv8-M Secure Stack Sealing~\cite{Armv8SecureStack}: CVE-2020-16273

\begin{comment}
	OAT~\cite{sun2020oat} formulates the property of \emph{operation} execution integrity, in which an \emph{operation} represents a sub-application code and data for a specific task (e.g.,  moving a robotic arm).
	OAT enables a remote verifier to detect if there is a control-flow or data-only attack on embedded devices.
	% It utilizes Cortex-A TrustZone and puts the measurement engine in the secure state.
	Compared to C-FLAT, OAT enables complete control-flow verification as well as attack flow reconstruction by combining hashes and execution traces in the measurement report. 
	%uses execution hashes for backward-edges and a software-based tracing technique for forward-edges to reduce nondeterministic control paths.
	OAT instruments a trampoline function corresponding to conditional branches and indirect transfers to report the destination information to the trusted measurement engine, which runs in the secure state.
	OAT also instruments load instructions that are supposed to access the control-dependent variables, such as branch/loop condition variables, and compares the variable with the copy recorded in TrustZone to attest the data integrity.
	% OAT can automatically identify those critical variables or check the annotations from programmers.
	%The measurement engine updates the measurement trace, which includes the branch taken (1) / non-taken (0) bit and destination address of indirect call/jump, and the measurement hash that encodes return addresses.
	%Similar to C-FLAT, 
	OAT was evaluated on Cortex-A with 
	% , generate an attestation blob, which is located in the secure state, for further verification.
	a performance overhead of 2.73\% and binary size overhead of 13\%. %tested on five selected embedded programs.
	% and combines hash and tracing-based CFI enforcement~\cite{ge2017griffin}~\cite{van2015practical} to attest both forward- and backward-edges.
\end{comment}

\begin{comment}
	\defense{Hybrid attestation:}
	% Remote attestation enables a verifier to obtain the state of a remote system and detect unauthorized modifications to it.
	%To address the limitation that Remote Attestation (RA) cannot defend itself against malware infection,
	VRASED~\cite{nunes2019vrased} instantiates hardware/software remote attestation co-design aimed at low-end embedded systems, which include Cortex-M devices.
	%introduces a formal verified HW/SW co-designed RA scheme for embedded systems.
	The hardware module enforces access control to the prover's key and secures the execution of the software implementation, which computes the attestation report.
	The security of VRASED is formally verified using linear temporal logic~\cite{cimatti2002nusmv}. %, which includes temporal connectives to enable sequential reasoning, as the formal system, takes a divide-to-conquer approach to verify each HW/SW sub-module via a model checker NuSMV~\cite{cimatti2002nusmv}, and uses a theorem prover Spot~\cite{duret2016spot} to prove RA's soundness and security.
	The hardware module of VRASED requires 122 and 37 additional LUTs and registers respectively, and it takes 0.45 second to attest 4KB of RAM on an 8MHz device.
	A line of work builds on VRASED to support proof of execution, i.e., APEX~\cite{nunes2020apex}, control-flow attestation, i.e., Tiny-CFA~\cite{nunes2020tiny}, and data integrity attestation, i.e., DIALED~\cite{nunes2021dialed}.
	
	
	APEX~\cite{nunes2020apex} provides unforgeable remote proofs of execution based on VRASED.
	
	implements a verified architecture of PoX, which protects the software system even it is fully compromised, on embedded devices.
	It designs a hardware module that allows the verifier to request unforgeable remote proofs to show the successful execution of attested software and produce certain authenticated output additionally. 
	% APEX~\cite{nunes2020apex} proposes a verified remote proofs of execution (PoX) architecture by designing a hardware module that allows the verifier to request unforgeable remote proofs to show the successful execution of attested software and produce certain authenticated output additionally. 
	% PoX protects the software system even it is fully compromised.
	It composes with VRASED~\cite{nunes2019vrased} and monitors a fixed memory region called METADATA to store the information about software execution status, including addresses/pointers to memory boundaries of the executable region, the memory boundaries of expected output, and an EXEC flag that indicates to verifier that the attested code executes successfully.
	APEX uses the same technique as VRASED to verify and prove its implementation.
	Compared with the pure VRASED, APEX incurs extra 2\% registers and 12\% LUTs and takes around 900ms on an 8MHz device.
	
	TinyCFA~\cite{nunes2020tiny} is designed based on APEX~\cite{nunes2020apex}.
	It instruments all control-flow instructions and conditional branches to log the destination to CF-Log, which stores in METADATA memory region.
	% To prevent overwriting CF-Log
	TinyCFA incurs 80\% code size overhead and 50\% run-time overhead on three real-world applications.
	% [\textcolor{darkblue}{TODO: more details.}]
	% \defense{Data flow attestation:}
	% [\textcolor{darkblue}{TODO: more details.}]
	% Those three projects work on TI MSP430~\cite{MSP430} devices, but the idea can also be extended to Cortex-M.
	DIALED~\cite{nunes2021dialed} uses APEX to securely log and authenticate data inputs by instrumenting the TinyCFA enabled program to log all data inputs of the program during execution along with its control-flow to the input log region.
	On top of TinyCFA, DIALED incurs 20\% overhead of code size and run-time.
\end{comment}

\begin{table}[!t]
	\center
	\scriptsize
	\vspace{-0.3cm}
	\caption{Vulnerability discovery for Cortex-M firmware}
	\vspace{-0.3cm}
	\setlength\tabcolsep{0.5ex}
	\rowcolors{2}{white}{gray!15}
	\label{tab:bug-finding}
	\begin{threeparttable}
		\begin{tabular}{l|l|l|ccc|ccc}
			\hline 
			\rowcolor{white}
			& Project & Year& \begin{tabular}[l]{@{}l@{}}\cellcolor{white} \rotatebox[origin=c]{90}{Input} \end{tabular}& \begin{tabular}[l]{@{}l@{}}\cellcolor{white} \rotatebox[origin=c]{90}{Target} \end{tabular}& \begin{tabular}[c]{@{}l@{}}\cellcolor{white} \rotatebox[origin=c]{90}{ISA} \end{tabular}&
			\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\cellcolor{white}Peripheral\\\cellcolor{white}Modeling \end{tabular}}&
			\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\cellcolor{white}I/O\\\cellcolor{white}Interaction\end{tabular}} &\begin{tabular}[c]{@{}c@{}}\cellcolor{white}Support\\\cellcolor{white}Fuzzing \end{tabular} \TBstrut{4ex}{-2.7ex} \\ \hline \hline
			\cellcolor{white}&FirmWare~\cite{firmwire}	&2022&&&&  &&  \\
			\cellcolor{white}&P$^2$IM~\cite{feng2020p}  &2020&C&R &v7 &&&\supportlevel{10}  \\
			\cellcolor{white}&DICE~\cite{mera2020dice}     &2020         &C&R &v7 &  &  &\supportlevel{10}  \\
			\cellcolor{white}&Laelaps~\cite{cao2020device}		&2020	&B&R &v7 &  &&\supportlevel{10}  \\
			\cellcolor{white}&$\mu$Emu~\cite{zhou2021automatic}  &2021   &B&R &v7 &  &&\supportlevel{10}  \\
			\cellcolor{white}&Jetset~\cite{jetset}	&2021&&&&  &&  \\
			\cellcolor{white}&Fuzzware~\cite{fuzzware}	&2022&&&&  &&\supportlevel{10}\\
			\cellcolor{white}&SEmu~\cite{semu}	&2022&&&&  &&  \\
			\multirow{-9}{*}{\cellcolor{white}\ref{Full firmware rehosting:}}&HALucinator~\cite{clements2020halucinator}	&2020&&&&  &&\supportlevel{10}\\
			\hline
			\cellcolor{white}&Avatar~\cite{avatar2}      &2018&&&&  &  &  \\
			\cellcolor{white}&Inception~\cite{cor2018}	&2018		&C&R &v7 &  &&  \\
			\multirow{-3}{*}{\cellcolor{white}\ref{Hardware-in-the-loop rehosting:}}&Frankenstein~\cite{Frankenstein} &2020&&&&  &  &  \\
			\hline
			\cellcolor{white}\ref{On-device fuzzing:}&$\mu$AFL~\cite{li2022mu}	&2022	&B&B&v7 &&&\supportlevel{10}\\ 
			\hline
			\cellcolor{white}&PASAN~\cite{kim2021pasan}      &2021       &C&R &v7 &&  &   \\
			\cellcolor{white}&FirmXRay~\cite{wen2020firmxray}	&2020	&B&B &v7 &&&\\
			\multirow{-3}{*}{\cellcolor{white}\ref{Static methods:}}&HEAPSTER~\cite{gritti2022heapster}	&2022	&B&B &- &&&\\
			%argXtract~\cite{sivakumaran2021argxtract} &B&R &v6/7 &\supportlevel{10}  &  &  \\
			%FIE~\cite{davidson2013fie}            &C&R &*  &  &\supportlevel{10}  &  \\
			\hline 
		\end{tabular}
		\begin{tablenotes}
			\item[] v6: Armv6-M, v7: Armv7-M, A: Cortex-A, R: Cortex-R, M: Cortex-M. \supportlevel{10}: Implement a specific security feature or need specific hardware support. 
			% \item[] Code and memory overhead shows the best case, run-time overhead shows the worst case.
			% \item[]: Bare-metal only or RTOSes. Input - source code; binary. Developer involvement - None; annotation; code modification.
		\end{tablenotes}  
	\end{threeparttable}
	\vspace{-0.5cm}
\end{table}


\begin{table}[!t]
	\center
	\scriptsize
	\renewcommand{\arraystretch}{1}
	\setlength\tabcolsep{0.7ex} 
	%\vspace{-0.4cm} 
	\caption{Cortex-M MCUs and Their Security-related Features}
	\label{tab:family}
	\rowcolors{2}{gray!15}{white}
	\begin{threeparttable}
		\begin{tabular}{llcccccccccccccc}
			\hline
			CPU                       & ISA                                 &\rotatebox{90}{Max MPU Regions}  &\rotatebox{90}{TrustZone-M}  &\rotatebox{90}{Max SAU Regions}    &\rotatebox{90}{PACBTI}     &\rotatebox{90}{PXN}&\rotatebox{90}{XOM}&\rotatebox{90}{MSPLIM/PSPLIM}   &\rotatebox{90}{UP Store/Load Ins.}  &\rotatebox{90}{Branch Prediction}  &\rotatebox{90}{ETM} &\rotatebox{90}{MTB} &\rotatebox{90}{DWT}  &\rotatebox{90}{FPB} &\rotatebox{90}{Year Introduced} \Tstrut{18ex}\\ \hline \hline
			M0    & v6-M            &                                 &                             &                                   &                           &                   &                   &                                &                                    &                                   &                    &                    &\supportlevel{10}    &\supportlevel{5}    &2009\\ 
			M1    & v6-M                                &                                 &                             &                                   &                           &                   &                   &                                &                                    &                                   &                    &                    &\supportlevel{5}     &\supportlevel{5}    &2007 \\ 
			M0+  & v6-M                                &8                                &                             &                                   &                           &                   &                   &                                &                                    &                                   &                    &\supportlevel{10}   &\supportlevel{10}    &\supportlevel{5}    &2012 \\ 
			M3    & v7-M            &8                                &                             &                                   &                           &                   &                   &                                &\supportlevel{10}                   &\supportlevel{10}                  &\supportlevel{5}    &                    &\supportlevel{10}    &\supportlevel{10}   &2004 \\ 
			M4    & v7-M                                &8                                &                             &                                   &                           &                   &                   &                                &\supportlevel{10}                   &                                   &\supportlevel{5}    &                    &\supportlevel{10}    &\supportlevel{10}   &2010 \\ 
			M7    & v7-M                                &16                               &                             &                                   &                           &                   &                   &                                &\supportlevel{10}                   &\supportlevel{10}                  &\supportlevel{10}   &                    &\supportlevel{10}    &\supportlevel{10}   &2014 \\ 
			M23 & v8-M Baseline   &16                               &\supportlevel{10}            &8                                  &                           &                   &                   &\supportlevel{10}               &\supportlevel{10}                   &                                   &\supportlevel{5}    &\supportlevel{10}   &\supportlevel{10}    &\supportlevel{10}   &2016 \\ 
			M33  & v8-M Mainline   &16                               &\supportlevel{10}            &8                                  &                           &                   &                   &\supportlevel{10}               &\supportlevel{10}                   &                                   &\supportlevel{5}    &\supportlevel{10}   &\supportlevel{10}    &\supportlevel{5}    &2016 \\ 
			M35P& v8-M Mainline                       &16                               &\supportlevel{10}            &8                                  &                           &                   &                   &\supportlevel{10}               &\supportlevel{10}                   &                                   &\supportlevel{5}    &\supportlevel{10}   &\supportlevel{10}    &\supportlevel{10}   &2018 \\ 
			M55  & v8.1-M Mainline &16                               &\supportlevel{10}            &8                                  &\supportlevel{10}          &\supportlevel{10}  &\supportlevel{10}  &\supportlevel{10}               &\supportlevel{10}                   &\supportlevel{10}                  &\supportlevel{5}    &                    &\supportlevel{10}    &\supportlevel{5}    &2020 \\  
			M85  & v8.1-M Mainline                     &16                               &\supportlevel{10}            &8                                  &\supportlevel{10}          &\supportlevel{10}  &\supportlevel{10}  &\supportlevel{10}               &\supportlevel{10}                   &\supportlevel{10}                  &\supportlevel{5}    &                    &\supportlevel{10}    &\supportlevel{5}    &2022 \\ \hline                    
		\end{tabular}
		\begin{tablenotes}
			%    \item[1] Measured in percentages.
			%    \item[2] Measured in kilobytes (KB).
			\item[] Whitespace: Not support, \supportlevel{10}: Support, \supportlevel{5}: Partially Support. On M23, the ETM and the MTB are exclusive to each other.
		\end{tablenotes}
	\end{threeparttable}
\end{table} 
 
 \begin{comment}
	\section{Future Directions}
	
	\ziming{A section to point out interesting research directions and difficult level and possible solutions.}
	
	Maybe a table here.
	
	\ziming{Finer-grained stack cookies.}
	
	A future work direction is collecting unbiased Cortex-M firmware dataset.
	
	0. New attacks
	1. Just implement efficient versions of existing mitigations on Cortex-M
	1.1 trace-based control-flow violation 
	2. Redesign existing versions of mitigations for Cortex-M
	3. protect platform-specific asset. PC and mobile may not have such asset.
	4. What issues will we have when we implement it in Rust? performance?
	
	\emph{ret2ns Countermeasures:}
	To mitigate this attack, one feasible way is to let the compiler to instrument checks before the \verb|BXNS| and \verb|BLXNS| instructions.
	The dynamic checks can lookup the non-secure state's MPU to identify code privilege level at destination, and change the \verb|CONTROL_NS.nPRIV| bit accordingly.
	The address masking can be used as static checks with less runtime overhead.
	To facilitate this, the privileged and unprivileged programs in non-secure world need to be reorganized in separate address spaces.
	
	Microkernel.
	
	Would this be a new direction? https://www.cs.columbia.edu/~rgu/publications/osdi22-li.pdf. In general, explore successful strategies on other platform on Cortex-M and IoT. 
	
	PACCTI for cortex-m, how are they different from the Cortex-A counterpart?
	
\end{comment}

 % Future works
	\section{Discussion}
	\label{sec:discussion}
	
	\subsection{What else we can do with existing hardware features?}
	
	Besides those projects we discussed in \S\ref{sec:projects}, which are mainly focusing on utilizing MPU and TrustZone, there are several hardware features on Cortex-M architecture that can be utilized to build other secure designs.
	For example, by learning the functionalities of MTB and ETM, we can trace and reconstruct the control flow execution.
	DWT provides specific data and instruction access checking, which can be used to monitor sensitive information.
	The newly introduced PACBTI also can be used to detect temporal memory safety violation like PTAuth~\cite{farkhani2021ptauth}.
	%PTAuth~\cite{farkhani2021ptauth} instruments the code to create a cryptographic authentication code (\verb|AC|) based on a unique ID of each heap object and store the \verb|AC| to the unused bits of the protected pointer.
	%Then authenticate the object during every pointer dereference by re-computing the \verb|AC|.
	%The mismatch of \verb|AC| indicates a temporal memory safety violation.
	
	\subsection{What else we can do to mitigate the implementation bugs?}
	
	Learn from Table~\ref{tab:CVEs-con}, most vulnerabilities are caused by implementation bugs.
	To mitigate such bugs, there are several discussions.
	
	\subsubsection{Formal verification}
	
	%An application that has been formally verified means it is free of compromise. 
	Formally verified software systems can provide high assurance of isolation between applications, such as sel4~\cite{klein2009sel4}, which does not support Cortex-M processors now.
	%For embedded software systems, there lack of formal verify techniques to prove those programs.
	
	\subsubsection{Bugs finding}
	The most challenge to implement bugs finding techniques of embedded software systems is how to emulate varietal peripherals and different hardware-dependent operations.
	Though there are several pieces of research that are seeking for efficient and accurate peripheral emulation to help firmware dynamic analysis, there still need a long way to meet the fast-growing hardware diversity.
	
	\subsubsection{Software fault isolation} 
	MPU-assisted techniques always suffer from the limitation of configurable region numbers, how to build a pure but efficient software-assisted isolation and confinement is still a worthwhile discussion. 
	Software fault isolation~\cite{tan2017principles} protects program partitions from affecting by the adversary part (see \ref{No memory virtualization:}).
	It has the untrusted fault domain (aka. compartment) and a secure external to manage those domains.
	SFI defines a data and code access policy to constrain the read/write access inside the data region, and a control transfers policy to keep the control-flow stay within the code region or a safe external address.
	But the control transfer policy still exposes to ROP attacks.
	
	\subsubsection{Other artificial software diversity mechanism}
	
	As discussed in \ref{No memory virtualization:}, ASLR used on modern operating systems is hard to deploy on Cortex-M systems because of the low entropy.
	Coarse-grind ASLR is another research direction.
	Besides ASLR, which is program-level diversity, other diversity methods such as instruction-level diversity including instructions reordering, equivalent instruction substitution, and garbage code insertion also show potential security protection.
	
	% iv) Program level diversity includes functions reordering, randomizing the base addresses (e.g., ASLR), program encoding, data, or even library entry point.
	
	\subsubsection{Address or memory sanitizer}
	
	\subsection{Attack prediction}
	
	Some Cortex-M processors (e.g., Cortex-M55) equip cache and branch prediction, which expose the attack surface to Meltdown and Spectre attacks.
	
	
	\future{Formally verified embedded systems:}
	Like sel4~\cite{klein2009sel4}
	
	\future{Software fault isolation:}
	Software fault isolation~\cite{tan2017principles} protects program partitions from affecting by the adversary part (see \verb|I01|).
	It has the untrusted fault domain (aka. compartment) and a secure external to manage those domains.
	SFI defines a data and code access policy to constrain the read/write access inside the data region, and a control transfers policy to keep the control-flow stay within the code region or a safe external address.
	But the control transfer policy still exposes to ROP attacks.
	
	\future{Instruction diversity:}
	Discuss why other diversity does not work.
	%Artificial software diversity~\cite{larsen2014sok} randomizes the programs from different levels to hide the real information from attackers.
	Instruction level diversity includes instruction reordering, equivalent instruction substitution, and garbage code insertion, etc.
	
	\future{Virtualization:}
	
	\future{Hardware Security Enhancement:}
	\section*{Notes}
	
	To-do list: 
	
	(1) Crawl as many cortex-m firmware images as possible. The idea is to generate intelligence of real-world Cortex-M systems.
	
	(2) Also think about crawling Cortex-M projects from GitHub.
	
	(3) May add back the binary trick section ans justify our claim that "document is incomplete". 
	
	To-do list Nov 21st 2002
	
	[] work on the big figure and [3.6]
	
	[X] Rewrite the summary for Section 4.
	
	[X] Exokernel - TrustZone based.
	
	[X] Update Section 6 with new CVEs.
	
	[X] I20 and Table 1 needs to be updated
	
	[] Section 7.7
	
	[] Implement PSPLIM identification in Ghidra
	
	[] All the summary - 


 \subsection{Adversary model}

We consider any thing can be malicious. secure code is malicious. Privileged code is malicious.

$\mathcal{S}_{<U, T, S>}$
Entities: (1) unprivileged software in secure, (2) privileged software in secure (do not need to differentiate handler or thread), (3) unprivileged software in non-secure, (4) privileged software in non-secure (do not need to differentiate handler or thread), (5) peripheral (including DMA).

Potential problems:

1. How difficulty is it to achieve non-executable stack on Cortex-M because we do not have enough MPU regions to do so?

2. Confused deputy. A NSC function can be called by secure and the non-secure state. Then, how does the function know who call it? The origin could be very useful for some cases.

3. Multiple entry kernel by implementing kernel in the secure state privileged instead of non-secure privileged. But, app runs at (U, N).


lack of abstraction, no OS, some bare-metal.

Vendors take compromises on security to reduce footprint. 
For example, commonplace class key usage versus supporting key
provisioning and per-device secrets.

We should have a section to discuss deployed software security defenses in existing OS and compilers. 
We should compare the code generated by different compilers (especial ARMCC).
Use paper [SoK: Eternal War in Memory] as an exhaust list of available software protection approaches.

A comparison table about threats for x86, Cortex-A, and RISC-V. 
Then explain why they are unique for Cortex-M.


\section*{Bug reports}

\textit{Instruction diversity:}
Artificial software diversity~\cite{larsen2014sok} randomizes the programs from different levels to hide the real information from attackers.
(i) Instruction level diversity includes instruction reordering, equivalent instruction substitution, and garbage code insertion, etc.
% For example, uSFI~\cite{aweke2018usfi} inserts \verb|NOP| inside two 32-bit instructions and converts PC-related addressing instructions with equivalent two 32-bit immediate move instructions;
(ii) Basic block level diversity includes basic block reordering, opaque predicate insertion, and branch function insertion;
(iii) Function level diversity includes stack layout randomization, function parameter randomization, and control flow flattening, etc.;
(iv) Program level diversity includes functions reordering, randomizing the base addresses (e.g., ASLR), program encoding, data, or even library entry point;
% EPOXY~\cite{clements2017EPOXY} randomizes the function order after adding a small function that will jump to a fault handler.
% EPOXY also implements global data randomization via an LLVM pass, which randomly split unused RAM into different groups that will be later used for data, stack, bss, etc.;
%v) System level diversity includes the syscall mapping randomization, etc.
% iii）Diversify in function level such as randomize the stack layout, randomize the function parameter, and control flow flattening, etc.
% EPOXY randomize stack. 
% iv) program and system level. 

% \defense{MPU region management:}

% Test cases
\input{tests}

\subsection{Cortex-M projects}
\begin{table*}[!htpb]
	\center
	\scriptsize
	\caption{Projects Based on Cortex-M}
	\vspace{-0.3cm}
	\label{tab:app}
	\begin{tabular}{lll}
		\hline
		Target                  & Project                     & Prototype   \\ \hline  \hline
		Fuzzing                 & P2IM~\cite{feng2020p}       & Cortex-M     \\
		& DICE~\cite{mera2020dice}    & Cortex-M/MIPS M4K/M-Class \\
		Symbolic Execution      & FIE~\cite{davidson2013fie}  & TI MSP430\\
		Deep learning           & MCUNet~\cite{lin2020mcunet} & Cortex-M4, M7   \\
		Neutral network         & CMSIS-NN~\cite{lai2018cmsis} & Cortex-M7 \\
		Secure software         & Keccak-based secure PRNG~\cite{van2014software} &  Cortex-M0(+), M3, and M4(F \\
		& Teaching real-time DSP~\cite{wickert2015using} & Cortex-M4  \\
		& Communications of Smart Meters~\cite{abbasinezhad2017ultra} & Cortex-M3 \\
		& Modular Multiplication~\cite{seo2020memory} & Cortex-M4 \\
		Secure software updating& ASSURED~\cite{asokan2018assured} & HYDRA/Cortex-M33\\
		Cryptography            & ECC~\cite{de2014ultra}  & Cortex-M0+\\
		& NewHope~\cite{alkim2016newhope} & Cortex-M0, M4\\
		& AES~\cite{wardhani2017fast}     & Cortex-M3 \\
		& Round5~\cite{saarinen2018shorter} & Cortex-M4 \\
		& Round2~\cite{seo2019sike} & Cortex-M4 \\
		Benchmark               & BEEBS~\cite{pallister2013beebs} & Cortex-M0 \\
		& CoreMark~\cite{coremark2021}    & \\
		& CoreMark-Pro~\cite{coremarkpro2021} &\\
		& BenchIoT~\cite{} &\\
		& pqm4~\cite{kannwischer2019pqm4} & Cortex-M4 \\
		\hline
		\\                                                                    
	\end{tabular}
\end{table*}

\subsection{Cortex-M TrustZone-enabled Platforms}

Show a complete table of devices that can use Cortex-M TrustZone.
\begin{table*}[!htpb]
	\center
	\scriptsize
	\caption{TrustZone-enabled Platforms}
	\label{tab:platform}
	\begin{tabular}{llllll}
		\hline
		Platform                      & SoC              & Processor  & Multicore & Publicly? & Price   \\ \hline  \hline
		GD32E23x~\cite{}              & GigaDevice       & M23  & single-core  & Yes          &          \\
		GD32E235~\cite{}              & GigaDevice       & M33  & single-core  & Yes          &          \\
		M2351~\cite{}                 & NuMicro          & M23  & single-core  & Yes         &\\
		% SAML10~\cite{}                & Microchip SAML10 & M23 &           &           &  -      \\
		SAML11 Xplained Pro~\cite{}  & Microchip SAML11 & M23  & single-core  & Yes         &         \\
		Renesas S1JA~\cite{}          & Renesas          & M23  &         &           & \\  
		Renesas RA2A1~\cite{}         & Renesas          & M23 &           &           & \\
		Arm MSP2+ FPGA~\cite{}        & Arm              & M23/M33         &           & Yes          &  -      \\
		Arm MSP3 FPGA~\cite{}         & Arm              & M23/M33         &           & Yes          &  -      \\
		&                & Cortex-M33         &           &           &  -      \\
		\hline
		\\                                                                    
	\end{tabular}
\end{table*}

\begin{table}[!htpb]
	\center
	\scriptsize
	\caption{multi-core}
	\label{tab:Multi Core Platforms}
	\begin{tabular}{llllccc}
		\hline
		Company         & Series		& CPU\\ \hline  \hline
		% Altera        	& Cyclone V\\
		STM32			& STM32WB55xx		& M4 + M0+\\
		NXP				& i.MXx				& A9/7/53 + M4/7\\
		& LPC435x/3x/2x/1x	& M4 + M0\\
		Texas Instruments	& OMAP4430, OMAP4460 & A9 + M3\\
		& OMAP5xx			& A15 + M4\\
		Xilinx			& Zynq-7000			& A9 + FPGA (M1/3 soft core)\\
		Microsoft		& MediaTek 3620	chip& A7 + M4 \\
		% Arm				& 
		\hline
		\\                                                                    
	\end{tabular}
\end{table}

\section*{Benchmarks}

% SPEC CPU2000~\cite{henning2000spec} is the most widely used benchmark for modern systems, which characterizes a workload for general-purpose computers by providing self-contained set of programs and data divided into separate integer and floating-pint categories.

Dhrystone~\cite{weicker1984dhrystone} is a synthetic systems programming benchmark to measure processor and compiler performance.
It models the distribution of different types of high-level language statements, operators, operand types and locality sourced from contemporary systems programming statistics to present actual programming practice.
% It reflects actual programming practice in systems languages by modeling the distribution of different types of high-level language statements, operators, operand types and locality sourced from contemporary systems programming statistics.

MiBench~\cite{guthaus2001mibench} is adapted to Arm instruction set to characterize the embedded programs via instruction distribution, memory behavior, and available parallelism.
It contains 35 embedded applications in C language that are divided into six suites, which target to automotive and industrial control, consumer devices, office automation, networking, security, and telecommunications.

BEEBS~\cite{pallister2013beebs} measures the energy consumption of embedded devices.
It can also be used for evaluating performance and code size overhead (see Silhouette~\cite{zhou2020silhouette} and PicoXOM~\cite{shen2020fast}) since it contains a wide range of embedded applications, such as AES, integer and floating-point matrix multiplications, etc.

BenchIoT~\cite{almakhdhub2019benchiot} is designed to evaluate the security, performance, memory usage, and energy consumption for MUCs.
The security evaluation contains minimizing privileged execution (increasing SVC cycles), enforcing memory isolation, and control-flow hijacking protection.
It provides a curated set of five real-world applications that can run on both bare-metal or an OS, which includes smart light, smart locker, etc.
BenchIoT supports Armv7-M now.

CoreMark~\cite{coremark2021} and CoreMark-Pro~\cite{coremarkpro2021} is a processor benchmark suite that supports both high-performance processors and low-end processors.
CoreMark-Pro evaluates the CPU and memory with five integer workload (e.g., JPEG image compression, SHA-256) and four floating-point workload (e.g., neural network and fast Fourier transform).
% One of the workloads is a more memory-intense version of the original CoreMark benchmark.

%pqm4~\cite{kannwischer2019pqm4}

% The SPEC CPU benchmarks in particular have been used in prior CFI literature. 
% However, the SPEC suite is not practical to port to MCUs cores. 

The support library accompanying the Dhrystone benchmark contains both directed indirect subroutine calls, and indirect returns. 



% https://en.wikipedia.org/wiki/Arm_Cortex-M

% multi-processors
% \begin{table*}[!htpb]
	% 	\center
	% 	\scriptsize
	% 	\caption{Arm Multi-caore Processors and Their Security-related Features}
	% 	\label{tab:cortexmfamily}
	% 	\begin{threeparttable}
		% 	\begin{tabular}{llllllllll}
			% 	\hline
			% 	Boards		& Cores									& Frequency & FLASH (kB) & RAM (kB) \\ \hline \hline
			% 	NXP LPC4300 & one Cortex-M4F + one or two Cortex-M0	& 204 MHz	& 0/512/768/1024	& 104/136/168/200/264 \\
			% Texas Instruments SimpleLink Wireless MCUs CC1310 and CC2650 (one programmable Cortex-M3 + one Cortex-M0 network processor + one proprietary Sensor Controller Engine)
			% Cypress PSoC 6200 (one Cortex-M4F + one Cortex-M0+)
			% ST WB (one Cortex-M4F + one Cortex-M0+)
			% Apple A9 (Cortex-M3 as integrated M9 motion co-processor)
			% CSR Quatro 5300 (Cortex-M3 as co-processor)
			% Samsung Exynos 7420 (Cortex-M3 as a DVS microcontroller)[21]
			% Texas Instruments F28, LM3, TMS470, OMAP 4470 (one Cortex-A9 + two Cortex-M3)
			% XMOS XS1-XA (seven xCORE + one Cortex-M3)
			% Cortex-M3 with fpga: Microsemi SmartFusion2 SoC
			% The following vendors support the Cortex-M3 as soft-cores on their FPGA chips:
			% Altera Cyclone-II, Cyclone-III, Stratix-II, Stratix-III
			% Xilinx Spartan-3, Virtex-2, Virtex-3, Virtex-4, Artix-7
			% Cypress PSoC 6200 (one Cortex-M4F + one Cortex-M0+), FM4
			% Microchip (Atmel) SAM4C (Dual core: one Cortex-M4F + one Cortex-M4)
			% NXP LPC4000, LPC4300 (one Cortex-M4F + one Cortex-M0)
			% ST STM32 F3, F4, L4, L4+, WB (one Cortex-M4F + one Cortex-M0+)
			% NXP (Freescale) Vybrid VF6 (one Cortex-A5 + one Cortex-M4F)
			% NXP (Freescale) i.MX 6 SoloX (one Cortex-A9 + one Cortex-M4F)
			% NXP (Freescale) i.MX 7 Solo/Dual (one or two Cortex-A7 + one Cortex-M4F)
			% Texas Instruments OMAP 5 (two Cortex-A15s + two Cortex-M4)
			% Texas Instruments Sitara AM5700 (one or two Cortex-A15s + two Cortex-M4s as image processing units + two Cortex-M4s as general purpose units)
			% \end{tabular}
		% \end{threeparttable}
	% \end{table*}


% M2351 https://www.nuvoton.com/products/microcontrollers/arm-cortex-m23-mcus/m2351-series/?__locale=en

%\subsection{Software Architectures}
%We discuss bare-metal systems and some widely used  with the security for Cortex-M processors.
%Most of those RTOSes listed on table ~\ref{tab:rtos} also work on other platforms like MIPS, x86, and RISC-V.
%To further interest, please check their documents.

\arch{Bare-metal systems and unikernels:}
In the privileged application architecture all codes run at the privileged level, and the non-privileged level of the microcontroller is not utilized as shown in Figure~\ref{fig:overview}(a). 
Both bare-metal applications, which directly run on the hardware without an operating system layer, and RTOSes that execute themselves and applications at the privileged level fall into the category of privileged application architecture. 
These applications are compiled and statically linked with libraries, e.g., libc, Cortex Microcontroller Software Interface Standard (CMSIS), etc., and RTOSes, e.g., Mbed bare-metal profile~\cite{MbedOS}, into one big executable. 
%but is highly risky since a simple vulnerability will compromise the whole system.
%Real-Time Operating Systems (RTOS) run tasks in a tight time boundary and have predictability and determinism operations.
This architecture provides efficient execution and is easy to implement. 
But, it has many security issues, which we discuss in~\ref{No or weak privilege separation:}, \ref{No or weak memory access control; executable stack:}, \ref{No or weak stack separation:}, \ref{Statically linked executables and no dynamic linker:}.

%In most cases, bare-metal applications and RTOSes run at the same privilege level as shown in Figure~\ref{fig:overview}(a).

\arch{Monolithic kernels:}
In the monolithic kernel architecture the RTOSes or privileged services run at the privileged level, whereas applications run at the non-privileged level as shown in Figure~\ref{fig:overview}(b). 
In this architecture, the code base executing at the privileged level, e.g., Hardware Abstraction Layer (HAL), is significantly larger than the non-privileged application, resulting in a monolithic model.
Example RTOSes that adopt this architecture include FreeRTOS with MPU enabled, Tock~\cite{levy2017multiprogramming}, uClinux~\cite{uclinux}, RT-thread~\cite{RTthread}, and Mbed OS~\cite{MbedOS}.
%confirm rt-thread: https://www.rt-thread.io/blog.html
%, execute
%Some designs put the privileged services of Bare-metal applications or RTOS kernel at the privileged level, then untrusted applications call service APIs to communicate with the higher privileged code as shown in Figure~\ref{fig:overview}(b).
%Projects utilize MPU-assisted isolation separate the privilege, which we will discuss in \ref{MPU-assisted isolation and confinement:}.
%For RTOS, Tock~\cite{levy2017multiprogramming} takes advantages of the privilege separation.
%Mbed~\cite{MbedOS} has two profiles: (i) the bare-metal profile with TLS support; (ii) the RTOS profile that supports TLS and privilege separation. 
%uClinux~\cite{uclinux} is a Linux variant designed for microcontrollers without an MMU~\cite{mccullough2004uclinux, durrant2002uclinux}.

\arch{Exokernels:} 
As shown in Figure~\ref{fig:overview}(c), in this architecture the size of the code executing at the privileged level is significantly reduced from~\ref{Monolithic kernel architecture:}. 
Only the sensitive services and a trusted separation kernel have the highest privileged level, 
the unprivileged level is divided into multiple zones to support RTOSes or bare-metal applications, which are managed by the separation kernel.
%Hermes~\cite{klingensmith2018hermes} presents a software-based virtualization for Cortex-M.
We will discuss a software-based virtualization system, namely Hermes~\cite{klingensmith2018hermes}, in \ref{Software-based virtualization:}, a least kernel privilege system, namely EPOXY~\cite{clements2017EPOXY}, and MultiZone~\cite{pinto2020multi} in \ref{MPU-assisted isolation and confinement:}.
% also utilizes MPU to achieve this goal.

%In Hermes, both unchanged RTOSes and bare-metal applications run at unprivileged level, and any privileged operations from them will be trapped and emulated by the hypervisor.
%, hypervisor is an abstract between software and privileged services and isolates the critical core from untrusted code.
%[EPOXY]

%Hermes~\cite{klingensmith2018hermes} implements a thin hypervisor by running itself at the privileged level with a single interrupt service routine to catch and preprocess all exceptions before dispatching them to the unprivileged guest system.


	\arch{Dual-world privileged application architecture:}
	Architecture \textbf{A01} is extended into two worlds if it utilizes TrustZone as shown in Figure~\ref{fig:overview}(d).
	In this architecture, a secure application is loaded first, then gives control to the non-secure application.
	With non-secure callable functions, the non-secure application can access secure services.
	Most startup projects use this architecture to help developers to learn the TrustZone technique, such as the TrustZone Lab on SAM L11 Xplained Pro board~\cite{saml11demo}, TrustZone Blinky project on Arm V2M MPS2+ board~\cite{mps2plusiotkit}, etc.


\arch{Dual-world systems:}
%With TrustZone, the privilege level can be further divided into four levels: non-secure unprivileged and privileged, secure unprivileged and privileged.
%Secure privileged level has the highest privilege and is usually designed to be the root of trust.
As shown in Figure~\ref{fig:overview}(e), it is the extension of architecture \textbf{A02}.
It has more sophisticated isolation levels with privileged separation and Trusted Execution Environment (TEE).
RTOSes and applications run in the non-secure state, whereas the secure services run in the secure state.
%The non-secure code can call secure services through NSC region. 
%As shown in Figure~\ref{fig:overview}(d), the NSC functions can be a secure unprivileged service or trusted privileged service because this kind of state switch does not check the privilege level of either target or source security state.
%This architecture may introduce large TCB size in the secure state.
%Similar to the Arm Trusted Firmware for Cortex-A~\cite{TFA}, 
Arm Trusted Firmware for Cortex-M (TF-M)~\cite{ATFM} provides a HAL to use Cortex-M TrustZone, which is a representation of this architecture. 
%implements the Secure Processing Environment (SPE), where itself runs, and Non Secure Processing Environment (NSPE), where applications and REE OS run, for Cortex-M.
%To this end, it utilizes TrustZone if it is available or a dedicated core to provide physical isolation on multi-core CPUs without TrustZone.
TF-M consists of (i) a secure boot module running at the privileged level to authenticate the integrity of the secure state and non-secure state images;
(ii) a core module running at the secure state privileged level that controls the isolation, communication, and execution;
(iii) other security services running at secure state unprivileged level including crypto, internal trusted storage, protected storage, and attestation~\cite{TFMtech}.
Keil RTX5~\cite{rtx5}, Mbed OS~\cite{MbedOS}, FreeRTOS~\cite{freertoskernel}, RT-Thread~\cite{RTthread}, Zephyr~\cite{Zephyr}, etc., integrate ATF-M~\cite{ATFM}. %example RTOSes.
%Other RTOSes such as Kinibi-M~\cite{KinibiM}, ProvenCore-M~\cite{ProvenCoreM} are also this architecture.
\textbf{A05} can be an advance design to build a secure software system.
However, it only supports one TEE and suffers from the increasing size of TEE TCBs, which promote itself more prone to vulnerabilities~\cite{van2019tale}.

\arch{Multi-world systems:}
As shown in Figure~\ref{fig:overview}(f), this architecture extends the dual-world design into multiple equally-secure TEEs within the non-secure state.
The trusted kernel at the secure privileged level handles non-secure environment switches and resources access control.
%Non-secure state TEEs can only communicate with each other through secure unprivileged services.
We will discuss uTango~\cite{oliveira2021utango}, one example to build multiple TEEs by utilizing Cortex-M TrustZone, in \ref{TrustZone-assisted multiple TEEs:}.

\subsubsection(SVC misuse)
%1,469 samples . % when the whole firmware executes at the privileged level.
%In particular, the Nordic nRF5 series firmware call the SoftDevice~\cite{nordicsoftdevice} APIs using \verb|SVC|.

%The Supervisor Calls (SVC) are widely used to escalate the privilege level, which can be handy to quickly switch between different privilege modes.
%However, some vendors like the Nordic may define their own SVC handler, not to separate the privilege level, but to generate interrupts implementing special Application Program Interface (API) calls~\cite{cmsissvc}.
%On the Nordic nRF5 series, there is a firmware module identified as SoftDevice~\cite{nordicsoftdevice}, 
%which is a pre-compiled and linked binary to be used as the wireless protocol stack that complements a corresponding SoC.
%The application can use the SoftDevice API as a high-level programming language interface, and this API is implemented using thread-safe SVC interrupts.
%If a bare-metal program running at the single privileged level enables the SoftDevice,
%the SVC function call will be directly made in the privileged mode,
%and there will be no privilege switches since everything running in the privileged execution mode.
%In this case, the SVC call acts only as a normal interruption,
%and the application side of this program can have a chance to take control the SoftDevice by altering the control flow.
%(For the programs with single privilege level, the use of the SVC API function call is not enough to provide a robust privilege separation.)

\issue{No or weak stack separation:}
RTOSs, including FreeRTOS~\cite{freertosstack} and Zephyr~\cite{zephyrstack}, support multi-tasking, so each task has its own stack.
%FreeRTOS uses a hardcoded 20-byte delimiter (\verb|0xA5|s) to mark the limit of a stack, which is checked when a context switch happens.
%Zephyr uses \verb|PSPLIM| to prevent overwriting.
%For each task, they split the current stack into different regions to store the corresponding task stack, 
%and the context switching will use the current stack pointer to locate different tasks.
However, stack separation between the kernel and application is rarely used in bare-metal firmware.
10 samples that adopt privilege separation (discussed in~\ref{No or weak privilege separation:}) leverage both the \verb|MPS-| and \verb|PSP-|based stacks.
In addition, another 124 samples in our dataset use both the \verb|MPS-| and \verb|PSP-|based stacks without privilege separation.
%Even without enforcing the privilege separation, the program can still choose to use different stacks for different tasks,
%ensuring the corruption of one task does not spread to others.
%The bit 1 of the \verb|CONTROL| register determines the current activate stack.
%In our analyzed dataset, we found 52 out of 1035 firmware, which is 35 of the 689 devices, have switched to use the PSP as the current stack.
All other samples (1,663; 92.54\%) only adopt a single \verb|MSP|-based stack.
%and execute at a single privileged level all the time.
%As we discussed previously, the 8 firmware which carry out privilege separation also use multiple stacks,
%so there are only 44 firmware (30 devices) have used both main and process stacks without changing the privilege level.
%\ziming{no one uses multiple PSP. Different task on FreeRTOS/Zephyr will PSP/MSP?}

\issue{No or weak memory access control; executable stack:}
% Execution protection stops the execution within arbitrary memory regions.
Even though some Cortex-M devices have MPU, % for memory access control, 
previous research believes that most real-world systems do not use it~\cite{clements2017EPOXY, zhou2019good, clements2018aces}. 
We confirm that 1,773 of the 1,797 firmware in our dataset do not use MPU, %, whose registers are memory-mapped at fixed addresses.
which means the address space in \emph{code}, \emph{SRAM}, and \emph{RAM} is executable. 
For the same reason, data execution prevention (DEP) %, a standard feature in modern operating systems, 
is not enforced on these systems.
Without memory access control,
malicious code can also read and write arbitrary memory. %(see Figure~\ref{fig:overview} (a)).
%For example, there is no  since MPU is not enabled.
%DEP is used to prevent executing code from non-executable memory space.
%Cortex-M processors do define a memory region that address starting with \verb|0xF| is non executable.
%And MPU provides \verb|XN| bit to configure a memory region as execute never.
%Since MPU is seldom enabled for most software systems, the DEP implementation is weak.
%The MPU registers are used to define the MPU regions and their attributes,
%and they reside in the Secure System Control Space (SCS) memory region.
Out of the 24 firmware samples that use MPU in our dataset, 5 samples use the MPU defined by Arm. The remaining 19 samples use a vendor-specific implementation (i.e., Nordic's simplified MPU (sMPU)~\cite{nordicmpu}), which only supports
a subset of features defined by Arm.
Specifically, sMPU only supports read and write permissions and can only divide memory into two protection domains.

% , which are different versions for the same series of Nordic Cortex-M0 devices, use Nordic' simplified MPU (sMPU)~\cite{nordicmpu} since Cortex-M0 does not have an MPU.
% The sMPU only supports the read and write permissions, and it can only divide memory into two protection domains. 
%, namely region 0 and region 1.
%Region 0 is occupied by the SoftDevice~\cite{nordicsoftdevice} (precompiled SDK binary file region) while region 1 is available to the application.
%SoftDevice program and data memory are sandboxed to prevent SoftDevice program corruption by the application ensuring robust and predictable performance.
%When memory protection is enabled, these regions will be used by the Memory Protection Unit to enforce runtime protection and readback protection of resources classified as region 0. 
%While region 0 \emph{code} has full access to the address space, it cannot be read or written by region 1.
%Region 0 \emph{SRAM} is also not writable to region 1 programs.
% NVM protection blocks (below) is complimentary and optional to the region 0 sandboxing mentioned above
%The program memory region (including \ziming{region 1 and region 2}), which is the non-volatile memory (flash), can be protected from erases or writes depending on settings in the \verb|PROTENSET| registers. 
%while the Armbuilt-in one can also set the execution permission, to prevent the memory from being executed in a protected region.
%One bit in a \verb|PROTENSET| register represents one protected block. 
%There are two \verb|PROTENSET| registers of 32 bits which means there are 64 protection blocks in total.
%The protection block size can be configured by the \verb|PROTBLOCKSIZE| register and is default 4KB.

%Since the Nordic includes the application program interface and libraries, which is called SoftDevice, into a pre-compiled and linked binary,
%they provides a runtime separation on the code memory, RAM and peripherals to isolate the SoftDevice program and the applications.
%The SoftDevice code region cannot be read, written, or erased at runtime by the application code region, and the SoftDevice RAM region cannot be written to by an application at runtime.
%The SoftDevice code region will always have full access to the system.
%Besides the separation on the code memory, the entire code region can also be divided into 64 protectable blocks with independent setting of the erase/write permission.
%Another major difference is that the Nordic MPU implementation can only control the memory read and write accesses,
%while the Arm built-in one can also set the execution permission, to prevent the memory from being executed in a protected region.

%\ziming{I do not understand here. Is the MPU configuration divides the memory or the MPU divides the memory?? How did you find the name 0 and 1? Is this from some materials or just reverse engineering? Do they use a single privileged level? If Region 1 has a code injection vulnerability, can region 1 code change the settings of MPU?}
%The Nordic customized MPU divides the code memory, RAM and peripherals into two regions: region 0 and region 1.
%Region 0 is occupied by the SoftDevice~\cite{nordicsoftdevice} (precompiled SDK binary file region) while region 1 is available to the application.
%SoftDevice program and data memory are sandboxed to prevent SoftDevice program corruption by the application ensuring robust and predictable performance.
%When memory protection is enabled, these regions will be used by the Memory Protection Unit to enforce runtime protection and readback protection of resources classified as region 0. 
%Region 0 program memory cannot be read, written, or erased at runtime.
%Region 0 RAM cannot be written to by an application at runtime.
% NVM protection blocks (below) is complimentary and optional to the region 0 sandboxing mentioned above
%The program memory region (including region 1 and region 2), which is the non-volatile memory (flash), can be protected from erases or writes depending on settings in the \verb|PROTENSET| registers. 
%One bit in a \verb|PROTENSET| register represents one protected block. 
%There are two \verb|PROTENSET| registers of 32 bits which means there are 64 protection blocks in total.
%The protection block size can be configured by the \verb|PROTBLOCKSIZE| register and is default 4KB.

%For the CPUs without native hardware MPU support, e.g., Cortex-M0, the chip vendor may provide their customized implementation of memory protection unit~\cite{nordicmpu}.
%The customized MPU registers are defined in the peripheral memory region, and serves the same functionality as the Arm native MPU.
%The MPU register addresses for the Arm native implementation stay same among different supported CPUs.
%To see whether a firmware has used the MPU or not, we can directly look for the operations on the \verb|MPU_CTRL| register, which has a fixed address of \verb|0xE000ED94|.
%We find that no firmware in the dataset has enabled the Arm native MPU.
%However, since all the firmware in dataset come from the same vendor Nordic, 
%we also use the customized MPU register address from the Nordic to filter the dataset, and found only one of the device has implemented the Nordic-defined MPU.

\begin{comment}
	\issue{Weak readback protection:}
	Readback protection 
	%is an important security feature that can 
	prevents the leakage of data on the memory and flash through the debugging interface.
	%\ziming{Does Arm come with build-in readback protection?} (Need to have a deeper look at the Arm CoreSight)
	%The Arm supports different debug-related features~\cite{Armv7MArcRef}. 
	%However, securing those features using readback protection and other methods depends on the chip vendors' implementation.
	%With this protection, the program can restrict the attackers from being able to extract data from flash memory even if they have physical access to the device.
	%The MPU can be configured to protect the memory ranges, however the read/write/execute permissions set by the MPU can be simply bypassed by the external debugger since the MPU is implemented within the CPU core and relies on the CPU-initiated bus transactions.
	%The debugger uses the other bus masters such as the system memory debug Test Access Port (TAP) and DMA.
	%There are many ways to prevent the debugger from accessing the protected regions of flash, including partial restrictions and 
	Besides completely disabling the hardware debug interface~\cite{sultan2020readback}, some systems include specific features for readback protection. 
	%However, these partial restrictions may leave potential logic holes to the attackers, which can be used to circumvent the restriction.
	For example, sMPU can disable the debugger access to the flash memory region.
	However, it still allows register access and single stepping of the processor, which was exploited to dump the full flash content~\cite{kris2015dumping}.
	This flaw was addressed in the new processors~\cite{nordicnrf52}.
	But for the Nordic firmware in our dataset, only 34 out of 1462 firmware have enabled the readback protection.
	%And 6 of them use the nRF51 flawed readback protection.
\end{comment}

%\emph{RIOT-OS Implementations:}
%The RIOT-OS has the implementation of the stack canaries based on the compiler built-in support~\cite{riotstack}.
%It has a canary value randomization mechanism which will ensure the stack canary has a different value on each build.
%The canary value is generated by the build system randomly and passed to the protection module using the \verb|-D| compiler flag. 
%The protection module object file is marked as \verb|PHONY|, which will make sure it gets rebuilt on each make invocation, and thereby ensuring that each build has a different random canary value.

%\emph{Zephyr Project Implementations:}
%The Zephyr Project has an configuration option \verb|CONFIG_STACK_CANARIES| to enable the compiler stack protection with canaries~\cite{zephyrstack}.
%This option is disabled by default, since enabling it can result in a significant increase in footprint and an associated decrease in performance.
%During the initialization at boot-time, it generates a random canary value assigned to the global canary variable~\cite{zephyrstackcode}.
%The random value generation is based on the device driver; on some constrained devices (e.g. devices without random number generator), 
%the produced canary value is not considered as a cryptographically secure random value.

%The GNU Arm Embedded Toolchain, \verb|armclang| (Arm Compiler 6), \verb|armcc| (Arm Compiler 5) provide built-in supports for the stack canaries, which can be enabled with several compiler options.
%A guard variable that is overwritten indicates a buffer overflow, and the checking code alerts the run-time environment.

%For the GNU Arm Embedded Toolchain version 10.3-2021.10, 
%we tested the compiler built-in stack canaries by compiling a single file using the \verb|arm-none-eabi-gcc| compiler, with the flag \verb|-fstack-protector-all|.
%When a function is called with stack canary enabled, 
%the initial value of its canary variable is taken from a global variable \verb|__stack_chk_guard|, 
%and the program should provide a stack overflow hook function \verb|__stack_chk_fail()| to handle the fallback.
%A suitable implementation can set the canary variable \verb|__stack_chk_guard| to a random value when the program is loaded, and before the first protected function is executed.
%If no definition of the canary variable and the fallback function is provided in the program code,
%the compiler will generate a function \verb|__stack_chk_init()| to set a fix value \verb|0xff0a0000| to the canary variable, and a default implementation of \verb|__stack_chk_fail()| will be used.

%For the \verb|armclang| and \verb|armcc|, we tested this built-in stack canaries on a FreeRTOS demo project with five different tasks.
%Those tasks are created to be run infinitely, with the label \verb|__noreturn|.
%We also define a simple print value function that does return to compare the compiler behavior on different function types.

%Arm Compiler 5 uses the \verb|armcc| as the compiler tool.
%We use the Arm Keil IDE with \verb|armcc| V5.06 update 7 (build 960) to test the stack canaries behavior.
%Different from the GCC compiler, The \verb|armcc| uses the flag \verb|--protect_stack_all| to enable the stack canaries.
%Once enabled, we must provide a declaration in the program code for the global variable \verb|__stack_chk_guard| and the fallback function \verb|__stack_chk_fail()|, 
%otherwise the compiler will give out an undefined symbol error.
%If we do not provide any initial value to the canary variable, the compiler will use 0 to initialize the \verb|__stack_chk_guard| when the program gets loaded.
%And before the linking process of the linker, the \verb|__stack_chk_guard| is loaded from the \verb|.data| section.
%For the non-return task functions, the compiler will only instrument the canary insert operation in the function prologue, and do not add checks in the function epilogue.

%Arm Compiler 6 uses the compiler tool \verb|armclang| instead of \verb|armcc|.
%We use the Arm Keil IDE with \verb|armclang| V6.16, and set the compiler flag \verb|-fstack-protector-all| to enable the stack canaries.
%The compiler requirements of the global variable \verb|__stack_chk_guard| and the fallback function \verb|__stack_chk_fail()| are similar to the \verb|armcc|.
%However, before the lining process, the stack canary value address in each protected function only points to zero.
%And in the \verb|armclang|, the compiler do not touch the non-return task functions.

%As described above, those kinds of stack canaries protection may not secure.
%Even if we can give a random canary value during the program initialization, the canary word must remain unchanged during the life of the program. 
%Since there is no process separation as the X86 platform, that canary value is global and same to each function in the program.
%It should also be mentioned that the canary word is stored in a writable memory region, which means it could be easily modified by other malicious functions.

\emph{Empirical Analysis on Real-world Firmware:}
%Since all the firmware in our dataset are real-world raw binaries, it is hard to identify the stack canaries implementation by function or variable symbols.
%For this reason, we move the focus to the relatively invariant canary insert and check operations at the function prologue and epilogue.
%For each Arm compiler in each optimization level, we recognize its instruction pattern which is related to the stack canaries in the function prologue and epilogue,
%and create the corresponding regular expression to match the disassembled firmware dataset.
% Comment: right now we only have regex for one optimization level
%There are four regular expressions for each compiler, matching the canary operations in the function prologue and epilogue in two optimization levels.
Even if the aforementioned compilers offer the canary mechanism, only \emph{one} of the 1,797 firmware samples in our dataset adopts it.
%It is probably because the option is by default disabled. 
%used has enabled the compiler built-in stack canaries support.
% Possible reasons:
%We surmise that the reason for not enabling the compiler stack protection is the performance overhead introduced by the extra checks in each function.

%We found 13 firmware in our dataset use Mbed-OS, and ??? of them enabled the thread stack overflow check.
%By the time of our analysis, Ghidra does not support identifying the instructions to access the stack limit registers.

\begin{comment}
	On FreeRTOS, each task has its own stack. It has a compiler option \verb|configCHECK_FOR_STACK_OVERFLOW| to enable the task stack overflow checking~\cite{freertostaskovfchk}.
	When switching the tasks, the RTOS kernel can check that either the processor stack pointer remains within the valid stack space,
	or the last 16 bytes within the valid stack range remains same when the stack was first created by the task.
	The latter method is stronger however less efficient than the former one.
	
	
	Mbed-OS uses the Keil-RTX5 RTOS kernel, which implements a software stack overflow checking that can be enabled with defining \verb|OS_STACK_CHECK|~\cite{rtx5config}.
	During the thread switch, the kernel will check both that the current running thread stack pointer is within the stack space,
	and the stack magic word at bottom of the stack is intact. 
	The stack magic word is a fixed value that defined in the kernel header file.
	% RTX5 Header File: https://www.keil.com/pack/doc/CMSIS_Dev/RTOS2/html/theory_of_operation.html
\end{comment}

%erflow by setting a stack limit or filling the last 20 bytes of the stack with a known value (\verb|0xa5|) when a task is created.
%  for checking the remained unused space for tasks.
% FreeRTOS known stack value pattern: https://github.com/FreeRTOS/FreeRTOS-Kernel/blob/ac2c383bc14b2577101cad238c8779f4d9c14d6c/tasks.c#L844
% https://github.com/FreeRTOS/FreeRTOS-Kernel/blob/ac2c383bc14b2577101cad238c8779f4d9c14d6c/tasks.c#L3052
%Since the value is fixed, it can be very easily exploited.
%Even though GCC provides a stack cookie mechanism by instrumenting a function's prologue and epilogue~\cite{gccssp}, %with a failure handler to check if the value is changed.
%this mechanism needs run-time support from the OS to provide a unique cookie and a failure handler function,
%which only a few OS, including RIOT OS and Zephyr, implement.
% Mbed OS, RT-thread, TockOS, etc. miss such implementation. 
% Weidler et al.~\cite{weidler2017return} showed that arbitrary code can be executed via return-oriented programming on the Cortex-M processor.
% RIOT OS: https://github.com/RIOT-OS/RIOT/blob/73ccd1e2e721bee38f958f8906ac32e5e1fceb0c/sys/ssp/ssp.c
% https://github.com/zephyrproject-rtos/zephyr/blob/be0f5fe0b0be7d095419ee90d23c8831cf8de9c1/kernel/compiler_stack_protect.c#L49-L53  __stack_chk_guard

%The detail of vulnerability is presented in~\cite{}, for example, 
%When \verb|EXC_RETURN| is loaded to \verb|PC|, it will check the \verb|EXC_RETURN.SPSEL| bit to choose which stack pointer to use.
%But when handling \verb|FNC_RETURN|, there is no such bit. 
%Programmers can manipulate the code to choose \verb|MSP_S|, which may cause the unintended memory access from the secure main stack.
%For example, when a processor running in secure thread mode with the \verb|PSP_S|, a non-secure function call happens, the \verb|PSP_S| changes to \verb|PSP_NS|.
%Then in the non secure function, it transits to a non secure \verb|SVC| handler with \verb|MSP_NS| when an \verb|SVC| instruction executes.
%At the \verb|SVC| handler, attacker executes \verb|BX <FNC_RETURN>| to change the stack to \verb|MSP_S|, then trigger the processor to pop out invalid return address (CVE-2020-16273).
%Thus, the non secure code can jump to arbitrary secure address space.

\subsubsection{Missing barrial instructions}
%Arm architectures allow the design of processors to reorder memory access, which mostly happens in high-end processors and multiprocessor systems.
%The memory barrier instructions can be used to enforce ordering between memory accesses~\cite{yiu2020definitive}.
%On the Cortex-M processors that have relatively simple pipelines, the processor does not reorder any memory accesses, and most applications work without any memory barrier instructions.
%However, there are some cases that the aforementioned barrier instructions are still needed to ensure the effect of the a system configuration change takes place before subsequent operations.
%For example, After updating the \verb|CONTROL| register with an \verb|MSR| instruction, the \verb|ISB| instruction should be used to ensure the updated configuration is used for subsequent operations~\cite{yiu2020definitive}.

\begin{comment}
	\issue{Statically linked executables and no dynamic linker:}
	Most software systems on Cortex-M are statically linked into one big executable, namely the firmware, 
	and no dynamic linker is available in most RTOSs.
	Therefore, a load-time ASLR, which has been another standard feature in modern operating systems for more than a decade, cannot be implemented.
	Even if boot time ASLR is possible, many IoT devices will not reboot for a very long time.
\end{comment}


\begin{comment}
	(1) Cortex-M processors do not support some techniques we take for granted on x86/64 or Cortex-A, and their security features are less known.
	For example, virtual memory management is not available for lack of a Memory Management Unit (MMU), but Cortex-M does offer a Memory Protection Unit (MPU) that provides access control in the physical memory space.
	Also, Cortex-M has recently introduced its own version of TrustZone, which has different underlying mechanisms from its Cortex-A counterpart;
	(2) Even if Cortex-M offers some security-related features, existing embedded and IoT software systems barely use them and largely lack protection against code injection, control-flow hijack, data corruption, and other attacks. 
	In other words, software technologies for security on such devices significantly lag behind the development of not only mobile and personal computer security but also their own hardware security offerings;
	
	In other words, software technologies for security on such devices significantly lag behind the development of not only mobile and personal computer security but also their own hardware security offerings.
\end{comment}

\begin{comment}
	\issue{Weak security configuration:}
	As discussed in argXtract~\cite{sivakumaran2021argxtract}, configuration information that includes device and protocols or special hardware they use, application repositories, and website interfaces, can indicate the security status and introduce vulnerabilities of the firmware binaries. 
	For example, the man in the middle attack because the Bluetooth communication is not encrypted or authenticated~\cite{hackerbluetooth}.
	Default root password configuration~\cite{2880} exposes root privilege to attackers.
\end{comment}


% \subsubsection{Lack of basic security features}
% No hardware random number generators or standard encryption units.
% \textcolor{blue}{TODO: more features}

% \textit{Attacks on protocols: }
% Internet of Threats~\cite{meneghello2019iot}.
% \textcolor{blue}{TODO: more details}

% \textcolor{blue}{TODO: more details}

% \textit{Other attacks: }
% Laser fault injection~\cite{selmke2018locked}.

==> cortexmtz.tex <==
\section*{Cortex-M Security Extensions}
\label{sec:trustzone}

In this section, we discuss Cortex-M security extensions, including TrustZone and Pointer Authentication and Branch Target Identification (PACBTI), etc.
With TrustZone, many mechanisms, such as exception handling, have been extended.  
Figure~\ref{fig:ModePLSecure} shows a complete execution mode, privilege level, and security state transition diagram with TrustZone. 
%, and it provides a system-wide approach to security by splitting system-on-chip resources into the secure and non-secure states. 

\subsection{Secure and Non-secure State}

TrustZone
%, which is introduced in the Armv8-M architecture, 
adds an orthogonal partitioning of states to execution modes and privilege levels.
With TrustZone, the processor has the secure (\verb|S|) and non-secure (\verb|N|) state.
Non-secure software can only access non-secure resources including memories and memory-mapped peripherals, whereas secure software can access both secure and non-secure resources.
Different from Cortex-A TrustZone~\cite{AArch64tz} that uses the \verb|NS| bit in the Secure Configuration Register (\verb|SCR|) to indicate the operation state of the processor, the division of secure and non-secure in Cortex-M is memory map based and transitions between states take place automatically. 
If the processor is running code in the secure memory, the processor is in the secure state. 
Otherwise, the processor is in the non-secure state.
Each of the interrupts can be assigned as secure or non-secure in the interrupt target non-secure (\verb|NVIC_ITNS|) registers of NVIC.
%Non-secure interrupts can still be serviced when executing a secure function.

\subsubsection{Banked Registers and System Peripherals}

Some special registers/bits and memory-mapped system peripherals/registers are banked between security states.
As shown in Table~\ref{tab:registers}, the general and special registers of \verb|MSP|, \verb|PSP|, \verb|MSPLIM|, \verb|PSPLIM|, \verb|CONTROL[1-0]|, \verb|PRIMASK|, \verb|BASEPRI|, and \verb|FAULTMASK| are banked between two worlds.
%As shown in Table~\ref{tab:peripherals}, 
%Some registers in controllers, such as MPU and NVIC, are also banked.

%Armv8M with the secure extension enabled provides two kinds of MPUs, secure MPU and non-secure MPU.
%Secure code can access secure MPU registers and follows the secure MPU configurations.
%Non-secure code can access non-secure MPU registers and follows the non-secure MPU configurations.
%All MPU registers are privileged access only, any unprivileged access will trigger a fault exception.

% \verb|IDAU| region number (\verb|IREGION|), and access permission non-secure read and writable (\verb|NSRW|), non-secure readable (\verb|NSR|), read and writable (\verb|RW|), readable (\verb|R|), SAU region valid flag (\verb|SRVALID|) and SAU region number (\verb|SREGION|), MPU region valid flag (\verb|MRVALID|) and MPU region number (\verb|MREGION|).

%\subsection{Memory Infrastructure}

% To configure the TrustZone security features, Cortex-M processor introduced the memory partitioning  

\begin{figure}[!tbp]
  \begin{centering}
  \includegraphics[width = .47\textwidth]{pics/ns-s-transition.pdf}
  \vspace{-0.2cm}
  \caption{Execution Mode, Privilege Level, and Security State Transition Diagram}
  \label{fig:ModePLSecure}
  \end{centering}
  \vspace{-0.5cm}
\end{figure}

\subsection{Secure Memory Partitioning and Attribution Units}
\label{sec:sau}
A continuous memory region can be secure, non-secure callable (NSC), or non-secure. % in descending order of security.
A secure region is only accessible by secure software.
An NSC region can have \verb|SG| instructions to enable software to transition from the non-secure state to the secure state. 
A non-secure region can be accessed by non-secure and secure software. %, while a secure region can only be access by secure ones.
%Both secure and non-secure callable belong to secure. regions are further divided into two types: 
%When \verb|PC| points to an address in a non-secure callable region, the process is in the secure state.
Whether a memory region is secure, NSC or non-secure is controlled by the combination of the internal Secure Attribution Unit (SAU) and an external Implementation Defined Attribution Unit (IDAU).
%No every system implements both SAU and IDAU.
%The SAU should always be present but may have different number of regions.
%If no SAU regions are defined, or the SAU is disabled, and no IDAU is included in the system then the entire memory address space is defined as secure.
The SAU
%, which is memory-mapped in PPB, 
is programmable anytime in the secure state. 
IDAU is implementation defined, 
and they may be configurable or not before boot and usually can't be reprogrammed after boot.
%A typical design is to use the IDAU to define a fixed memory partition and use the SAU to change some security attributes at run-time.
%For instance, in xxx device the IDAU to splits memory into 256MB chunks of alternating secure and non-secure memory.
%As shown in Table~\ref{tab:idausau},
If an address maps to regions defined by both SAU and IDAU, the region of the highest security level is selected.% (see Table~\ref{tab:idausau}).

\begin{comment}
Both IDAU and SAU can configure the region as secure, non-secure, or NSC~\cite{ArmSNS}.
But there are several principles the processor follows: 
(i) The region configured as secure by IDAU can not be changed by SAU;
(ii) SAU can configure a non-secure region defined by IDAU to secure or NSC;
(iii) SAU can also configure a non-secure region or NSC region defined by IDAU to non-secure region.
%If the secure configuration does not follow the upper principles, it will be ignored by the processor.


\begin{table}[!htpb]
  \center
  \scriptsize
  \caption{Final Result Combined with IDAU and SAU}
  \label{tab:idausau}
  \begin{tabular}{lll}
  \hline
  IDAU        & SAU           & Final result          \\ \hline \hline
  Secure      & Secure        & Secure                \\
  Secure      & Non-secure    & Secure                \\ 
  Secure      & NSC           & Secure                \\
  NSC         & Secure        & Secure                \\
  NSC         & Non-secure    & NSC                   \\
  NSC         & NSC           & NSC                   \\
  Non-secure  & Secure        & Secure                \\ 
  Non-secure  & Non-secure    & Non-secure            \\ 
  Non-secure  & NSC           & NSC   
  \\ \hline                                                                    
  \end{tabular}
\end{table}

\end{comment}
% secure      & secure or non-secure     & secure        \\ 
% secure or non-secure  & secure      & secure        \\ 
% secure NSC or NS      & S-NSC         & S-NSC        \\ 
% non-secure  & NS         & NS           \\ 
% NCS         & NS         & NS

%The IDAU security value does not define privileged or unprivileged accessibility.
%There are several limitations of the SAU and IDAU-based memory partition:
%ii) software can only make a region to a higher security level by overwriting IDAU settings in the SAU. 
%As a result, software cannot release more regions to the non-secure state after boot.
%To overcome these limitations, some system supports memory aliasing and gating for memory and peripherals with Memory Protection Controller and Peripheral Protection Controller, which will be discussed in Section~\ref{sec:memalias}.

\begin{comment} 
\begin{table*}[!htpb]
\center
\scriptsize
\caption{Acronyms and descriptions of security-related peripherals and controllers}
\label{tab:peripherals}
\begin{tabular}{lllll}
\hline
Acronym & Full name & Banked in TZ? & Description & Access?                                                                                                                                                                                                             \\
\hline
\hline
NVIC & Nested Vectored Interrupt Controller & Some registers\\
MPU & Memory Protection Unit & Yes & Since Armv6-M\\
SAU & Security Attribution Unit & No & Since Armv8-M & secure Privileged\\
IDAU & Implementation Defined Attribution Unit & No & & Implementation Defined \\
MPC & Memory Protection Controller & x. \\ 
PPC & Peripheral Protection Controller & x. \\                                                                
 \hline                                                                
\end{tabular}
\end{table*}
\end{comment}

%\subsection{Memory Access Management}

\subsection{Memory Aliasing, Memory Protection Controller, and Peripheral Protection Controller}
\label{sec:memalias}

Memory aliasing maps share resources between the secure and non-secure states.
Privileged and unprivileged secure software can configure a Memory Protection Controller (MPC), which is included on the path to the memory,
% SSE-220 2.5.4 SRAM
to divide the memory into equal size blocks and to selectively assign each block to its secure or non-secure alias at run-time. 
%The size of block is determined by the hardware.
%The MPC provides a single software-configurable bit to define if each block is assigned to secure or non-state world. 
%Each MPC's configuration interface is mapped to the peripheral region (\verb|0x5800????|).
%For instance, we assume SAU and IDAU together split the 512MB SRAM region into the non-secure (\verb|0x20000000| - \verb|0x2FFFFFFF|) and secure (\verb|0x30000000| - \verb|0x3FFFFFFF|) parts.
%A 2MB physical SRAM is mapped at two aliasing 2MB memory regions: (i) a secure region from \verb|0x28200000| - \verb|0x283FFFFF|; and (ii) a non-secure region from \verb|0x38200000| - \verb|0x383FFFFF|.
%Each block on the SRAM is 64KB, so the MPC provides 32 bits for this SRAM. 
%For example, the 4MB SRAM can be divided into 32 blocks with 64KB each.
By configuring and changing the corresponding bit in the MPC at run-time, secure software can dynamically control which world a block is assigned to.
%Non-secure state can not configure the MPC which will trigger the attribution unit violation secure fault.
%Both Privileged and Unprivileged mode in the secure state can configure the MPC.
%\subsection{Peripheral Protection Controller}
%\label{sec:ppc}
Similar to an MPC, a Peripheral Protection Controller (PPC) can also be added on paths to peripherals to provide security gating. 
%The PPCs perform the task of gating access to the peripherals it protects based on the security settings of each peripheral, and the security attribute of the access. 
%Each PPC can support up to 16 peripherals.
% The privileged access only Privilege Control Block (bankedSecure of Non-Secure) is used
%The configuration interfaces of PPCs are also mapped to the peripheral region.
%The privileged access only Privilege Control Block (\verb|0x40080000| - \verb|0x40080FFF| in non-secure, \verb|0x50080000| - \verb|0x50080FFF| in secure) is used for PPC to define the access settings for associated peripherals.
%For SSE200 subsystem~\cite{ArmCoreLinkSSE200}, PPC can configure the access setting of MHU (Message Handling Unit), DUAL TIMER, TIMER, and Watchdog that can raise an interrupt to the processor.
%Secure PCB can set the peripheral as non-secure access or secure unprivileged access.
%Non-secure PCB can set non-secure unprivileged access.
%[Seems only SSE200 subsystem talked about the PPC. The Arm architecture document and reference document did not mention it.]
% \ziming{need citation for SSE200}

\subsection{Synchronous State Switching}
\label{sec:subsec:stateswithing}
%Different from Cortex-A TrustZone that uses the \verb|SMC| instruction and secure monitor handler as the sole entry point for synchronous state switching, 

Cortex-M supports an unlimited number of entries for direct calling between the secure and non-secure software.
This is achieved with the non-secure callable region and a special secure gate instruction (\verb|SG|).
To switch from the non-secure state to the secure state, non-secure software uses the \verb|BL| instruction to call into an \verb|SG| instruction in an NSC region.
% Also, the function the non-secure state wants to call must be declared as a non-secure entry.
% Each call targets to a non-exist entry will trigger an invalid entry point secure error.
After executing the \verb|SG| instruction, the processor state changes to secure. %, and the return state (1 for secure, 0 for non-secure) is stored in the least significant bit (LSB) of \verb|LR|.
% This is because Cortex-M does not support A32 instruction set, so the LSB of an address indicates the security state.
%After finishing the secure function, this bit will be checked to prevent returning to a fake secure address~\cite{Armv8MTZ}.
% Then branch to the secure state function.
To switch from the secure state to the non-secure state, secure software uses the interstating branch
instruction \verb|BLXNS| or \verb|BXNS| to call or branch to a non-secure address.
%The target security state of those two instructions is indicated by the least significant bit of the target address, 1 means secure, 0 means non-secure~\cite{Armv8mdeveloper}.[need a test]
%\ziming{Where did you get this sentence? Also need to explain the meaning of least significant bit pf LR and SP.}
%The \verb|BLXNS| instruction switches the state to non-secure only when the LSB of the target address is 0. 
When state switching happens, the processor first automatically pushes a special 32-bit value, namely combined exception Return Program Status Register (\verb|RETPSR|), and the return address with the LSB value 1 onto the current stack.
The value of \verb|RETPSR| consists of \verb|IPSR| and other flags.
The \verb|LR| is also changed to a special value named \verb|FNC_RETURN| (\verb|0xFEFFFFFF|).
%The LSB of \verb|FNC_RETURN| indicates which state this function is called from.
%Since it is only used in the non-secure function return, the value is always \verb|0xFEFFFFFF|.
This automatic step is called \verb|FNC_RETURN| stacking.
When the \verb|FNC_RETURN| value is loaded to \verb|PC|, the processor will unstack the \verb|RETPSR| value, check the \verb|IPSR|, and clear interruptions, then restore the return address to the secure state.
The state switching mechanism for the \verb|BXNS| instruction is much simpler than the \verb|BLXNS| instruction. 
If the target address is not \verb|FNC_RETURN| or \verb|EXC_RETURN| and the LSB is 0, \verb|BXNS| branches to non-secure code directly.
% It clears the \verb|CONTROL.SFPA| value to 0. 

\subsection{Asynchronous State Switching or Exception with TrustZone}
\label{sec:subsec:asystateswithing}
%\subsubsection{ State Switching}
Exceptions and interrupts trigger state switches asynchronously, which extend the exception handling mechanisms discussed in \S\ref{sec:ExceptionStacking}.
%Secure privileged software can configure each interrupt, which could happen anytime, as secure or non-secure in the Interrupt Target non-secure (\verb|NVIC_ITNS|) registers.
If the exception entry is in the non-secure state,
the processor automatically pushes the state context and an additional state context onto the current stack.
The additional state context consists of a \verb|Magic Signature|, \verb|R4| - \verb|R11|~\cite{Armv8MArcRef}. 
%Different from the \verb|FNC_RETURN| stacking, \verb|RETPSR| is partially used to store the \verb|xPSR| value and other flags.
%The additional state context includes \verb|R11|, \verb|R10|, \verb|R9|, \verb|R8|, \verb|R7|, \verb|R6|, \verb|R5|, \verb|R4| along with an integrity signature value (\verb|0xFEFA125B| with Floating-point Extension, \verb|0xFEFA125A| without Floating-point Extension).
If the FPU is enabled, the current state is the secure state, the processor pushes additional FP context %(\verb|S16| - \verb|S31|)%, which are \verb|S0| to \verb|S15| and the Floating-point Status and Control Register (\verb|FPSCR|) for the secure state exception, additionally \verb|S16| to \verb|S30| for the non-secure state exception, 
onto the current stack. %armv8-m architecture reference p70
After context stacking, if the current state is non-secure, all pushed registers will remain unchanged.
If the current state is secure, those registers will be set to \verb|UNKNOWN| values or zeros depending on whether the exception happens in the secure state or the non-secure state.
To help save and clear the floating-point registers \verb|VLLDM| and \verb|VLSTM| instructions were introduced, which will only work when Floating-point is used in the non-secure state and will be considered as \verb|NOP| if FPU is not present.
When \verb|EXC_RETURN| is loaded to the \verb|PC|, the processor automatically unstacks the context stack and checks the return security state.
%The process also checks if the 0th bit of signature value matches the \verb|EXC_RETURN[4]|.
%If not, the processor generates a \verb|SecureFault| to prevent the non-secure software from using the interrupt return to switch to the secure state illegally.
%Since the address starting with \verb|0xF| is non-executable, treating the signature as an address will trigger \verb|MemManageFault|, e.g. replacing the \verb|EXC_RETURN| to \verb|FNC_RETURN| will fail~\cite{Armv8SecureStack}.

\subsection{Test Target Instruction Variants}
\label{sec:subsec:TT}
Armv8-M introduces the Test Target (TT) instruction variants for querying the security state and access permissions of a memory location~\cite{Armv8MArcTech}.
There are four variants to query a location for privileged and unprivileged access from the secure or the non-secure state.
% for a privileged (\verb|TT|, \verb|TTA| for non-secure) access or unprivileged (\verb|TTT|, \verb|TTAT| for non-secure) access to that location~\cite{Armv8MArcTech} C2.4.247.
% These instructions are only valid when executing in the secure state.
%The return information is stored in the \verb|TT_RESP| payload format. %, which includes IDAU, SAU, and MPU region number, and access permissions such as non-secure or secure read and writable, non-secure readable, and readable, etc. 

\subsection{Pointer Authentication and Branch Target Identification}
\label{sec:subsec:PACBTI}
Armv8.1-M introduces the Pointer Authentication and Branch Target Identification (PACBTI) extension~\cite{ARMpacbti}, a similar version of which has been available on Cortex-A since Armv8.3-A, to mitigate Return-Oriented Programming (ROP) and Jump-Oriented Programming (JOP) attacks.
%Instructions related to this feature are presented in Table~\ref{tab:SecInstruction}.
% [should we explain the ROP and JOP here?]
% Unlike the AArch64 Armv8-A that can use some spare bits in the most significant bit of the pointer to embed security information for validating the pointer

Pointer authentication uses a 32-bit Pointer Authentication Code (PAC) stored in a general-purpose register to authenticate a pointer at run-time. 
%separate to the pointer and can be enabled for every secure state and privileged level.
Creating a PAC is to sign the pointer using a cryptographic mechanism, which takes the pointer, a 32-bit modifier in a general-purpose register, and a 128-bit secret key as inputs.
The modifier encodes context information, whereas the key can only be managed at the privileged level.
To sign a pointer in a general-purpose register, instruction \verb|PACG| is used.
A special instruction \verb|PAC| is used to sign \verb|LR| and use \verb|SP| as the modifier.   
%To validate a pointer, it follows the same crypto step to generate another PAC called \verb|PACreturn| and compares it with the stored \verb|PACenter|.
%A \verb|UsageFault| exception is generated if the validation of a pointer fails.
%Even though this is a new feature on Cortex-M,
%Different from Cortex-M, AArch64 Armv8-A can use some spare bits in the most significant bit of the pointer to embed security information for validating the pointer.
% AArch64 Armv8-A is a 64-bit architecture that the pointer authentication information can be stored in the available spare bits in the most significant bits of the pointer. 
PTAuth~\cite{farkhani2021ptauth} used a similar feature on Cortex-A to detect heap-based temporal memory corruption.
%It instruments the code to create a cryptographic authentication code (\verb|AC|) based on a unique ID of each heap object and store the \verb|AC| to the unused bits of the protected pointer.
%Then authenticate the object during every pointer dereference by re-computing the \verb|AC|.
%The mismatch of \verb|AC| indicates a temporal memory safety violation.
%PTAuth incurs 2\% memory overhead and 26\% run-time overhead.
% BTI mitigates against some JOP via creating an architectural dependency between certain indirect branch instructions and the targeted instructions.
Branch Target Identification (BTI) prevents JOP 
%to arbitrary memory location 
by extending existing indirect branch instructions to constrain the target to a BTI clearing instruction within a select memory region.
%BTI setting instructions, e.g., \verb|BLX|, set a new \verb|EPSR.B| bit to indicate indirect control flow transfer, and 
%The target of the transfer must be a BTI clearing instructions, 
%which include \verb|SG|, \verb|BTI|, and \verb|PACBTI|.
%A new \verb|EPSR.B| bit is used to record indirect branches. %when BTI is enabled.
%  for the target security and privilege level.
%This bit will be set to 1 if BTI setting instruction executes and can only jump to BTI clearing instructions, which will set this bit to 0.
%Armv8.1-M extends existing indirect branch instructions to support BTI setting and BTI clearing functionality.


% \subsubsection{Secure Stacking and Unstacking}

% When the \verb|FNC_RETURN| value loads to \verb|PC|, the processor automatically triggers the unstacking from the secure stack.
% Similar to exception stacking and unstacking, discuss FNC\_RETURN here.

\begin{comment}
\subsection{Mode, Level, and State Transitions}
\label{sec:modelevelstate}

As figure \ref{fig:ModePLSecure} shows, the Cortex-M processor with TrustZone has two privilege levels (Privileged and Unprivileged) and four modes (Secure Thread, secure Handler, non-secure Thread, and non-secure Handler). 
We already discussed most transition routines in previous sections.  

The transition between secure and the non-secure state does not care about which privilege level they are.
That is to say, the non-secure state can access either the secure Privileged or secure Unprivileged with the help of the NCS function (\verb|SG|).
This will introduce a potential software attack. 

NSC cam implement multiple secure code entry points, where as in Cortex-A TrustZone the secure monitor mode handler is the sole entry point.
\end{comment}

% \begin{figure}[!htbp]
%   \begin{centering}
%   \includegraphics[width = .45\textwidth]{pics/IDAU-SAU-MPC-MPU.pdf}
%   \caption{IDAU, SAU, MPC, MPU}
%   \label{fig:Secure}
%   \end{centering}
% \end{figure}

% \begin{figure}[!htbp]
%   \begin{centering}
%   \includegraphics[width = .47\textwidth]{pics/memory.jpg}
%   \caption{memory}
%   \label{fig:}
%   \end{centering}
% \end{figure}

\subsection{Summary of Cortex-M Security Extensions}

The Cortex-M architectures offer several security features, including TrustZone, pointer authentication, branch target identification, etc.
The Cortex-M TrustZone, which is optimized for faster context switches, has a much different underlying mechanism from the Cortex-A TrustZone. 
%The memory map based secure sate mechanism and special branching instructions reduce the world switch latency, resulting more efficient transitions.
%TrustZone provides multiple secure function entry points (\verb|SG|) to bridge software between two states.
Secure memory partitioning is controlled by IDAU and SAU, and MPCs can control memory aliasing.
%Even though the security state of the processor is determined by what code it executes, 
%The security state is configurable via SAU and MPC at run-time, which makes the memory partition more flexible.

%As most of the registers are shared between secure and non-secure state, besides the hardware supported exception stacking and unstacking, developer should carefully manipulate the value in those registers to prevent information leakage, which we will discuss in \S\ref{sec:IssueVul}.

%The newly introduced PACBTI also can be used to detect temporal memory safety violation like PTAuth~\cite{farkhani2021ptauth}.

%\ref{Information leakage to the non-secure state due to state switches:} .

%memory alias, dynamically remapping to secure or the non-secure state at run-time...

==> related.tex <==
\begin{comment}
    \issue{Information leakage through power consumption:}
    The power consumption can leak implementation details, mainly targeting the cryptographic unit, in a subtle way.
    %is used to spot subtle leaks in implementations 
    The reason is that the power consumption of the target instruction is affected by the previously executed one~\cite{tiwari1996instruction}.
    %shows a more severe issue that can leak the instruction execution.
    Thus, power consumption is often utilized for instruction reverse engineering and code-breaking, which allows attackers to recover secret keys and even retrieve sensitive program code or algorithms.
    For instance,
    ELMO~\cite{mccann2016elmo} simulates instruction-level power models for Cortex-M0 to identify leaky instructions.
    The experiments of leakage detection tests for unprotected AES implementation of Mbed TLS~\cite{Mbedtls} and a masked AES show that ELMO is able to produce leakage trace for arbitrary program code.
    Another example is that Vafa et. al~\cite{vafa2020efficient} attach efficient profiling attack on Cortex-M3 processor to recover real boards' instructions.
    
    
    \section{Related Work}
    
    % Li et al.~\cite{li2019research} Research on arm trustzone.
    
    % Demystifying Arm TrustZone: A Comprehensive Survey
    To the best of our knowledge, a complete systematization of knowledge of the security of Cortex-M hardware and software is absent at the time of this writing.
    Several recent papers discussed the features of Cortex-A TrustZone, the software vulnerabilities in Cortex-A TrustZone-assisted TEEs, and the security of communication techniques on Cortex-M. 
    Pinto et al.~\cite{pinto2019demystifying} presented an in-depth study of Arm TrustZone with a focus on the Cortex-A TrustZone.
    They discussed a variety of architectures of using Cortex-A TrustZone to build TEEs on computer platforms and enable virtualization in mobile and embedded devices.
    Cerdeira et al.~\cite{cerdeira2020sok} studied the prevailing security vulnerabilities in Cortex-A TrustZone-assisted TEE systems
    by analyzing 207 bugs on five major commercially successful TEEs, i.e., Qualcomm, Trustonic, Huawei, Nvidia, and Linaro.
    They also presented a survey of defense techniques that can help overcome the security issues prevalent in the TEE systems.
    Meneghello et al.~\cite{meneghello2019iot} presented a broad overview of the security risks in low-end IoT devices and discussed the security of the design and implementation of popular transmission technologies used in the IoT domain, namely ZigBee, BLE, 6LoWPAN, and LoRaWAN on Cortex-M.
    
    On runtime software security of trustzone-m based iot devices~\cite{luo2020runtime}.
    On Security of TrustZone-M Based IoT Systems~\cite{luo2022security}.
    
    Sok: Security evaluation of home-based iot deployments~\cite{alrawi2019sok}.  
    
    \end{comment}
    % HEAPSTER paper.
    % present a vulnerability study to understand the types of vulnerabilities and limitations that affecting existing TrustZone-assisted (targeting Cortex-A) TEE systems by analyzing 207 TEE bugs on five major commercial TEEs (i.e., Qualcomm, Trustonic, Huawei, Nvidia, and Linaro), which are categorized into architectural, critical implementation, and hardware issues.
    %They also highlight several research-relevant techniques learning from respective papers that can be employed to overcome those issues.
    
    % provide a comprehensive survey about researches based on TrustZone technology from both academia and industry.
    %They studied existing TrustZone-based systems and categorizing them into TEEs and hardware-assisted virtualization, which mainly focus on Cortex-A TrustZone.
    
    % SoK: Understanding the prevailing security vulnerabilities in TrustZone-assisted TEE systems
    
    % point out the main challenge to build correct TEEs is 
    % the main challenges to build them correctly, and what contributions can be borrowed from the research community.
    %  them into to understand the vulnerabilities and limitations types that affect existing TrustZone-assisted TEES and point out the main challenges to build correct TEEs.
    
    % Good Motive but Bad Design: Why Arm MPU Has Become anOutcast in Embedded Systems
    %Zhou et al.~\cite{zhou2019good} discuss the outcast of utilizing an MPU after analyzing the performance, showing the issues of MPU that face bypass attacking and configurable number limitations.
    
    %The security of low-end IoT devices 
    
    
    %which mainly focuses on the communication protocols in IoT networks.
    %They categorize the security requirements for IoT system into information level, access level, and functional level and discuss specific security mechanisms for common used communication protocols, including encrypt mechanism, cryptography, random number generator, secure hardware, and intrusion detection system.
    %By analyzing real IoT attack reports, they conclude the weakness of current IoT protocols.
    %Lu~\cite{lu2021survey} analyzes the RISC-V security technologies from the hardware and architecture perspectives.
    %A Survey and Analysis on SoC Platform Security in ARM, Intel and RISC-V Architecture~\cite{nicholas2020survey}
    %Aly et al.~\cite{aly2019enforcing} list and discuss works related to security threats and challenges across different layers of IoT connected network architecture, such as network management layer and data center layer.
    %There are other literature that review different aspects of IoT devices including operating systems~\cite{qutqut2018comprehensive}, specific communication protocols~\cite{iglesias2019analysis}, machine learning at the network edge~\cite{murshed2019machine}.
    
    
    % Luo et al.~\cite{luo2020runtime} On Run-time Software Security of TrustZone-M based IoT Devices.
    
    % Challenges in designing exploit mitigations for deeply embedded systems  uArmor
    % Abbasi et al.~\cite{abbasi2019challenges} Challenges in designing exploit mitigations for deeply embedded systems.
    
    % Microcontroller Based IoT System Firmware Security: Case Studies
    % Gao et al.~\cite{gao2019microcontroller} 
    
    % Sensaoui et al.~\cite{sensaoui2020depth} An In-Depth Study and Implementation of Protection Mechanisms For Embedded Devices Running Multiple Applications
    
    %\subsection{Systematization}
    
    %\cite{cerdeira2020sok, clements2018aces, kwon2019uxom, almakhdhubmurai, zhou2020silhouette, salehi2019microguard, clements2017EPOXY, clements2020halucinator, jung2020secure, ji2020mcunet, shen2020fast}

==> sec.tex <==
\section{Hardware Limitations and Issues}
\label{sec:HardIssueVul}

%This section presents Cortex-M processors' hardware architectural limitations and issues with respect to security.
%Cortex-M systems are built on top of hardware.
%The correctness of hardware architecture is the foundation of the whole system.

%[should we use this as a takeaway or summary?]
%The relatively simple Cortex-M hardware has a double-edged implication of its security.
%On one hand it lacks hardware support for finer-grained protections,
%but on the other hand the lack of optimization, e.g., no cache, no branch prediction, no speculative execution, etc., makes them immune to some microarchitectural attacks, such as cache side-channel attacks~\cite{lipp2016armageddon, zhang2016truspy, cho2018prime+}, spectre~\cite{kocher2019spectre}, meltdown~\cite{lipp2018meltdown}, etc.

\subsection{Hardware Limitations}

Hardware limitations are missing or constrained hardware features to support security, which is typically non-patchable.

\vspace{.2cm}\centerline{\ul{Limitations of Memory Protection Mechanisms}}

\limitation{No memory virtualization:} 
%For performance and cost considerations, Cortex-M does not come with an MMU; thus, 
%To support real-time operation and avoid non-response to interruption when dealing with a virtual memory translation lookup table missing~\cite{yiu2020definitive},
No hardware-supported memory virtualization is available on Cortex-M processors due to the absence of an MMU. 
Instead, software modules share the same physical address space. %and are aware of the existence of each other. 
Such lack of memory virtualization also implies a small address space (4GB),
%As discussed in \S\ref{sec:physicalmemory}, the reserved address space for on-chip SRAM is only 512MB. 
%Most devices only have a physical SRAM of several hundred kilo bytes. 
%For example, the STM32F469I-Eval board only has 384KB of SRAM.
which presents additional challenges to effective address space layout randomization (ASLR) 
% scheme is challenging 
due to the low entropy. %in the physical address space layout.
%This exposes Cortex-M software systems to ROP attacks~\cite{hristozov2022toctou}.
%ROP attack: Time-Of-Check Time-Of-Use (TOCTOU) attack on DICE-based attestation

%Thus, after compromising a simple bug, an attacker can automatically control the whole system by scanning the physical address space.
% I02. \textbf{Excessively large TCBs:}
% For those systems that do not implement privilege separation, the whole system is considered to be trusted which is not true.
% [check other TCB size]   
%\issue{Absent ASLR implementations:}
%Without memory virtualization, ASLR, which is widely used on desktops and servers to prevent disclosing other variables from attackers, is hard to implement. 
%The entropy is constrained because of the small memory size, 
%And simply randomize the addresses at boot time can be easily compromised since the software systems on Cortex-M devices usually run days, months, or even years.
%From all analyzed software systems, none of them implement the ASLR.

\limitation{No input-output memory management unit:}
Besides MMU, input-output memory management unit (IOMMU) or its equivalents, i.e., IOMPU, that provide memory protection from malicious direct memory access (DMA)-capable peripherals are also missing on Cortex-M.
Some hardware vendors implement their own IOMPU, i.e., the resource domain controller on NXP i.MX RT~\cite{nxprt, nxpxrdc},
but they are only found in some of the latest devices.

\limitation{A small number of MPU regions and limited sizes:} 
%As discussed in \S\ref{sec:mpu}, 
Cortex-M only supports a small number of MPU regions (e.g., 8 or 16), and the size of regions must be a multiple of 32 bytes.
Compared to the page-based memory access control offered on microprocessors, the granularity of the MPU-based access control is coarse-grained, and it is not sufficient to implement fine-grained isolation schemes that require a large number of separate regions. 
%Projects, such as ACES~\cite{clements2018aces}, use an emulator to allow selective reads and writes to regions to bypass this limitation.

\vspace{.2cm}\centerline{\ul{Limitations of Security Extensions}}

\limitation{A small number of SAU Regions:} %As shown in %Table~\ref{tab:cortexmfamily}, 
The number of regions supported by SAU is small, e.g., up to 8 regions on Cortex-M33, 
resulting in limited design choices in splitting the secure and non-secure address space.
To alleviate this issue, hardware vendors use the IDAU to create the partitioning, which supports up to 256 regions.
But if the software design needs more partitions or if a device has many peripherals, even 256 regions may not be enough~\cite{sauidaumpcppc}.

% \issue{Limited types of access permission supported by MPU:}

% \issue{Weak firmware protection:}
% Microcontroller's firmware protection vulnerabilities~\cite{johannes2017firmware}.

\limitation{No intrinsic encryption to protect the secure state memory:}
TrustZone-M does not %provide a hardware-supported mechanism to 
encrypt the secure state memory.
Consequently, cold boot attacks~\cite{halderman2009lest} can dump the secure state memory.
There could also be information leakage when a memory protection controller (MPC) assigns a memory region from the secure state to the non-secure state at run-time, which we will discuss in \ref{Information leakage to the non-secure state due to state switches:}.

\limitation{Lack of intrinsic support for multiple trusted execution environments:}
%Same as Cortex-A TrustZone, 
TrustZone-M only provides \emph{one} isolated execution environment, namely the secure state, in which the trusted firmware and core services execute, resulting in a large software trusted computing base (TCB). 
For instance, TF-M~\cite{TFMsrc} has over 117K lines of %C/C++ and assembly
code.
%On the Cortex-A front, Sanctuary~\cite{brasser2019sanctuary} addresses this issue by utilizing the memory access controller to provide multi-domain isolation for sensitive apps, 
%and vTZ~\cite{hua2017vtz} addresses this by utilizing virtualization.
% uTango~\cite{oliveira2021utango}, which will be discussed in \ref{TrustZone-assisted multi-world system:}, attempts to address this issue by re-configuring the SAU at run-time.

% cloc --exclude-lang=CMake,Markdown,JavaScript,XML,CSS,Tcl/Tk,reStructuredText,YAML,XSD,HTML,JSON,make,Python --exclude-dir=target interface bl2 lib platform secure_fw 117732

\limitation{Lack of hardware-based remote attestation in TrustZone-M:}
Same as Cortex-A~\cite{cerdeira2020sok}, Cortex-M TrustZone lacks a hardware-based integrity reporting mechanism,
so it cannot provide a hardware-based remote attestation as Intel software guard extensions (SGX) does.
For example, the Arm platform security architecture (PSA) introduces a weakened software-based attestation method~\cite{ArmPSASM, ArmPSAattestation}. %and defines software interfaces for developers to use~\cite{}.
%Thus, the security of remote attestation is weak since it depends on the correctness of related components' implementation.
%As pointed out in~\cite{cerdeira2020sok}, Cortex-A TrustZone lacks a software-independent integrity reporting mechanism.
%Unfortunately, Cortex-M TrustZone has the same limitation. 
%Therefore, some security features, such as remote attestation, need to rely on trusted external hardware.
%For example, eFuses are used to store keys that are the root of trust for reporting, and code that is the root of trust for measurement needs to be stored on a secure ROM.
% Secure boot ensures the authenticity of the software running on a device by security reporting the software integrity measurements to a remote third party.
% The remote attestation will be implemented in software (e.g. TF-M) since TrustZone-M lacks such hardware mechanisms.
% Then the security relies on the correctness of the trust chain running on the highest privileged level.
% This weakens the security as it requires the correctness of all software of the trust chain running in the highest privileged level.

\begin{mdframed}[style=remarkstyle,backgroundcolor=blue!10]
\centerline{\textbf{Key Findings}}

\begin{itemize}[noitemsep,topsep=0pt,leftmargin=*]

\item The Cortex-M architecture offers weaker memory management interfaces than popular microprocessors, creating challenges to enforce memory isolation and safety.

\item TrustZone-M inherits the same hardware limitations of TrustZone-A and introduces more constraints.

\end{itemize}
%1. Limited memory management interface.
%1. its TZ inherit Cortex-A TZ limitation.
%Cortex-M processor is designed for a low-end device that is resource constrained, requiring power saving and real-time.
%Consequently, many security features, such as Memory Management Unit (MMU), which is on x86/64 and Cortex-A, are missing.
%This urges researchers propose software based approaches to protect systems on Cortex-M.
\end{mdframed}

\begin{figure*}[hbt!]
	\begin{centering}
		\includegraphics[width=\textwidth]{pics/overview.pdf}
		\vspace{-0.5cm}
		\caption{Identified Cortex-M software architectures in the collected dataset and in the literature. 
%			(a) bare-metal systems and unikernels; 
%			(b) monolithic kernels;
%			(c) exokernels;
%			(d) dual-world systems; and (e) multi-world systems.
			NS-UP: non-secure unprivileged, NS-P: non-secure privileged, S-UP: secure unprivileged, S-P: secure privileged.}
		\label{fig:overview}
	\end{centering}
	\vspace{-0.3cm}
\end{figure*}

\subsection{Hardware Issues}

Hardware issues discuss vulnerable hardware components and hardware-supported operations, encompassing general and vendor-specific issues. 

\vspace{.2cm}\centerline{\ul{Vendor-Agnostic Hardware Issues}}

\begin{comment}
\issue{Wide interfaces for state switches:}
\ziming{check this one on Monday}
%Different from Cortex-A TrustZone that only has one entry point (Secure Monitor Call, aka \verb|SMC|) for entering or leaving the secure state, 
As discussed in \S\ref{sec:cortexm}, Cortex-M TrustZone supports an unlimited number of entries into either state. %(\verb|SG| for entering the secure state; \verb|BLXNS|, \verb|BXNS| for entering the non-secure state). % as discussed in~\S\ref{sec:subsec:stateswithing}.
Consequently, the secure state software exposes a wide attack surface. %, shown as the secure service in Figure~\ref{fig:overview}(c) and (d).
%Therefore, it is challenging to implement a secure channel between a non-secure software component and a secure software component, as SeCReT~\cite{jang2015secret} does for the Cortex-A TrustZone.
%A vulnerability was found is TF-M implementation that an attacker can access secure keys stored in the TrustZone secure state for there is no authentication check between a caller and its associated key owner (CVE-2021-40327).
\end{comment}

\begin{comment}
\issue{Information leakage through caches:}
Even though most Cortex-M CPUs do not have a cache, cache side-channel attacks are possible on Cortex-M CPUs with caches.
For example, a flaw was disclosed that Mbed TLS allows local users to achieve partial plaintext recovery via a cache side-channel attack (CVE-2018-0498).
%Though the cache-based side-channel attack to obtain the CBC plaintext on Mbed TLS (CVE-2018-0498) was found on other platform, it may be exploitable on Cortex-M, too.
%FreeRTOS has a use-after-free vulnerability that can write the cache to the file system by flushing cache operation (CVE-2019-18178).
\end{comment}

\issue{Fast state switch mechanism exploitable for privilege escalation:}
The fast state switch mechanism of TrustZone-M can be exploited for arbitrary code execution with escalated privilege in the non-secure state, namely the ret2ns attack~\cite{ma2023dac}.
The wide state transition surface on TrustZone-M also makes the exploitation of this issue easier than exploiting ret2usr~\cite{kemerlis2012kguard, kemerlis2014ret2dir} on x86 or boomerang~\cite{machiry2017boomerang} on Cortex-A.

\issue{Information leakage to the non-secure state due to state switches:} 
\label{issue:informationleakSW}
Information leakage to the non-secure state could happen through memory, general-purpose and special registers:
(i) MPC can map a memory region into either the secure or non-secure state at run-time.
If a region used by the secure state is re-mapped into the non-secure state without proper sanitization, 
%and the content is not cleared by secure software,
sensitive information will be leaked to the non-secure state;
(ii) information leakage could also happen if the general-purpose registers are not cleared when switching to the non-secure state. 
To address this issue, Arm recommends general-purpose registers that are not used to pass arguments should be set to zero before state switches~\cite{Armv8MArcRef};
(iii) CVE-2021-35465 reports an implementation issue of the floating-point lazy load multiple (\verb|VLLDM|) instruction, which allows the non-secure handler to access and modify the secure state floating-point unit register values. 

%A new vulnerability was found in CVE-2021-35465 showing that context stacking with FPU or vector extension may expose secure information in floating-point or vector registers (MVE) to the non-secure state.
%\verb|VLLDM| instruction marks the Floating-point context as active only after restoring all the secure floating-point registers.
%Then the processor knows the floating-point registers are used by the secure state, which is sensitive.
%If the restoring process starts but is abandoned due to an interrupt, the partially restored floating-point register will be present to or even modified by the non-secure state.

%\issue{Attacks through energy management mechanisms:}
%Some hardware devices feature extra cryptographic unit, 
%Power analysis attacks compromise the security of cryptographic devices through analyzing their power consumption.
%ELMO~\cite{mccann2016elmo} utilizes instruction-level power models to capture differential data-dependent effects as neighboring instructions in a sequence way. ELMOEmulating Leaks for the Arm Cortex-M0 without Access to a Side Channel Lab..
%An Efficient Profiling Attack to Real Codes of PIC16F690 and Arm Cortex-M3~\cite{vafa2020efficient}

\begin{comment}
\issue{Improper access control via cross-state:}
%TrustZone provides hardware-level isolation but also introduces the semantic gap between two states.
Because TrustZone does not authenticate the non-secure caller's access permissions, 
the non-secure malicious application may utilize NSC to access the non-secure sensitive application's code and data.
More severe, the non-secure application can execute code that is not allowed to run.
\end{comment}

\issue{Improper privilege management for inter-processor debugging:}
CVE-2018-18068 reports 
%Ning et al.~\cite{ning2019understanding} discovered 
that in both Cortex-M and Cortex-A processors with TrustZone support, the debugging host's privilege level is ignored in the inter-processor debugging mode, allowing the non-secure state to gain access to the secure state resources via the ETM and performance monitor unit (PMU)~\cite{ning2019understanding, ning2021revisiting}.
%Because Armv8-M architecture integrates the same inter-processor debugging mechanism as Cortex-A does,
%the non-invasive version of the Nailgun attack is feasible on Cortex-M devices with multiple processors.
%E.g, LPCXpresso55S69 Development Board~\cite{LPC55S69} features dual-core Cortex-M33 processor.
%Arm CoreLink SSE-200 Subsystem for Embedded~\cite{ArmCoreLinkSSE200} features two Cortex-M33 processors.
%Other Cortex-M SoCs may integrate with Cortex-A processors.
%For example, Azure Sphere MT3620 Development Kit~\cite{MT3620} features one Arm Cortex-A7 core and two general purpose Arm Cortex-M4F cores, STM32MP153A~\cite{STM32MP153A} devices embeds a dual-core Cortex-A7 processor and a Cortex-M4 core, etc. 
%Nevertheless, no related CVEs have been assigned to any Cortex-M SoC yet.

\vspace{.2cm}\centerline{\ul{Vendor-specific Hardware Issues}}

\issue{Improper privilege management in vendor-specific hardware features:}
Some hardware vendors introduce over-powerful hardware features that can be exploited to gain full control of the system.
For example, NXP LPC55S6x MCUs include a ROM patch controller to fix bugs in the ROM after fabrication.
%which is accessible from the non-secure state unprivileged level and designed , resulting in potential attacks to access the secure privileged read-only code.
CVE-2021-31532 reports that even attackers in the non-secure state and unprivileged level can utilize the ROM patch controller to reconfigure the SAU regions to gain privilege escalation.
CVE-2022-22819 shows that the ROM patch controller firmware also has a buffer overflow bug that can lead to arbitrary code execution at the privileged level.

\begin{comment}
To enhance the security of Cortex-M processors, some vendors (ST, TI, NXP) implement their own hardware features, such as ROM patching for bug fixing~\cite{lpc55s6x} and eXecution Only Memory (XOM)~\cite{STxom, TIxom, NXPxom}.
However, such hardware features introduce new issues~\cite{schink2019taking, CVE202131532, CVE202222819}.
For example,
NXP LPC55S6x MCUs include a custom hardware block named ROM Patch Controller, which is similar to FPB to patch the ROM.
It is accessible from the non-secure state unprivileged level and designed to fix bugs in the ROM after chip fabrication, resulting in potential attacks to access the secure privileged read-only code.
As shown in CVE-2021-31532, attackers are able to utilize the ROM Patch Controller to modify run-time ROM APIs, which is secure privileged access only, to reconfigure the SAU regions to gain privilege escalation.
Attackers can also execute code via a crafted unsigned update firmware because NXP LPC55S69 series chips have a buffer overflow bug in parsing ROM patches before the signature is verified.
To mitigate such an attack, the vendor should lock the ROM Patcher Controller configuration or set up the non-secure MPU to block the access from the non-secure state.
\end{comment}

\issue{Bypassable vendor-specific readback protection:}
Only Cortex-M55 and M85 have the execute-only memory (XOM) feature, which prevents software running on the processor (a.k.a software-based code disclosure attack) or a hardware debugger from reading memory (including flash) that is designated as execute-only~\cite{sultan2020readback}.
To protect the IP and cryptographic keys on systems before M55, some hardware vendors implement their own hardware units to prevent reading from the debug interface, a feature known as readback protection.
%Readback protection prevents sensitive information (e.g., protected firmware, user secrets) leakage in internal storage (e.g., flash)~\cite{sultan2020readback}.
%To support this feature, some vendors implement their own hardware units.
For instance, the Nordic nRF51 series implement a mechanism to prevent debuggers from directly accessing flash and RAM address ranges. 
This protection, however, can be easily bypassed through arbitrary register read and write and single stepping in debugging~\cite{kris2015dumping}.
Though the mechanism was improved in the nRF52 series~\cite{nordicnrf52}, 
CVE-2020-27211 reports that a voltage glitch attack can still bypass it~\cite{schink2021security}.
Similar mechanisms implemented by ST~\cite{STxom}, NXP~\cite{NXPxom}, and TI~\cite{TIxom} %implement the eXecute-Only Memory (XOM) since only the version after Cortex-M55 processor features XOM.
%However, similar to Nordic nRF51 series devices, they allow single-stepping inside the XOM.
are also bypassable by inferring instructions from the observed state transitions~\cite{schink2019taking}.
%Thus, the XOM can be defeated~\cite{schink2019taking} by observing CPU registers and the effect of code/instruction execution %(CVE-2019-14236, CVE-2019-14239, CVE-2019-14237, CVE-2019-14238) 
%through the debug probe.
%Disabling the debug interface or restricting any privileged code execution on the device can mitigate such an issue.
%Moreover, executing the protected firmware inside the TrustZone protected environment would also mitigate this issue.

\begin{mdframed}[style=remarkstyle,backgroundcolor=blue!10]
\centerline{\textbf{Key Findings}}

\begin{itemize}[noitemsep,topsep=0pt,leftmargin=*]

\item The state switch mechanism introduced in TrustZone-M leads to new privilege management vulnerabilities and information leakage.

\item The fragmentation of the Cortex-M ecosystem has brought in new security challenges: vendors aggressively introduce over-powerful hardware features, which can undermine Cortex-M systems security if not properly designed.
%If not properly designed and checked, debugging features and vendor-specific features can lead to severe consequences, e.g., privilege escalation and IP theft.   
%Vendors and developers must be well of all architectural hardware components, such as TrustZone and debugging interface, when utilizing those components to build a secure system to not introduce new attack vectors.
\end{itemize}
\end{mdframed}

\section{Software Architectural Issues}
\label{sec:SoftIssueVul}

\input{platforms}

\subsection{Architectural Issues}

\begin{table*}[!t]
	\center
	\scriptsize
	\caption{Empirical Analysis of Security Features Adopted in Real-world Firmware}
	\label{tab:bin_anal}	
	%\vspace{-0.2cm}
	\renewcommand{\arraystretch}{1}
	\setlength\tabcolsep{0.38ex}
	\rowcolors{2}{gray!15}{white}
	%\scalebox{1}
	\begin{threeparttable}
		\begin{tabular}{l|cccc|cc|cccc|cccc|cccc|cc|cc|cc|cc}
			\hline
			\rowcolor{white}\multicolumn{1}{c|}{Hardware Vendor}                                     & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Nordic\\ \cellcolor{white}(FirmXRay)\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Other\\ \cellcolor{white}Nordic\end{tabular}} & \multicolumn{4}{c|}{TI}                                    & \multicolumn{4}{c|}{Telink}                                 & \multicolumn{4}{c|}{Dialog}                                & \multicolumn{2}{c|}{NXP}  & \multicolumn{2}{c|}{Cypress}  & \multicolumn{2}{c|}{ST}  & \multicolumn{2}{c}{Total} \\ \cline{2-23} \hline
			\rowcolor{white}
			Security Feature                                                                         & \multicolumn{2}{c|}{\#F}                           & \multicolumn{2}{c|}{\#D}                     & \multicolumn{2}{c|}{\#F}                                                                     & \multicolumn{2}{c|}{\#F}        & \multicolumn{2}{c|}{\#D} & \multicolumn{2}{c|}{\#F}         & \multicolumn{2}{c|}{\#D} & \multicolumn{2}{c|}{\#F}        & \multicolumn{2}{c|}{\#D} & \multicolumn{2}{c|}{\#F}  & \multicolumn{2}{c|}{\#F}      & \multicolumn{2}{c|}{\#F} & \multicolumn{2}{c}{\#F}   \\ \hline \hline
			Privilege Separation~(\ref{No or weak privilege separation:})                            & 8           & \multicolumn{1}{c|}{1.04\%}          & 5                     & 0.97\%               & 2                                                    & 0.29\%                                & 0 & \multicolumn{1}{c|}{0\%}    & 0          & 0\%         & 0  & \multicolumn{1}{c|}{0\%}    & 0        & 0\%           & 0 & \multicolumn{1}{c|}{0\%}    & 0        & 0\%           & 0           & 0\%         & 0           & 0\%             & 0           & 0\%        & 10         & 0.56\%       \\ 
			SVC for Library Call~(\ref{SVC misuse:})                                                 & 753         & \multicolumn{1}{c|}{98.04\%}         & 500                   & 97.47\%              & 690                                                  & 100\%                                 & 2 & \multicolumn{1}{c|}{9.09\%} & 1          & 5\%         & 17 & \multicolumn{1}{c|}{8.85\%} & 17       & 14.17\%       & 0 & \multicolumn{1}{c|}{0\%}    & 0        & 0\%           & 0           & 0\%         & 2           & 2.99\%          & 2           & 50\%       & 1,466      & 81.58\%      \\
			Stack Separation~(\ref{No or weak stack separation:})                                    & 49          & \multicolumn{1}{c|}{6.38\%}          & 34                    & 6.63\%               & 82                                                   & 11.88\%                               & 0 & \multicolumn{1}{c|}{0\%}    & 0          & 0\%         & 0  & \multicolumn{1}{c|}{0\%}    & 0        & 0\%           & 3 & \multicolumn{1}{c|}{5.66\%} & 1        & 2.78\%        & 0           & 0\%         & 0           & 0\%             & 0           & 0\%        & 134        & 7.46\%       \\
			Memory Access Control (MPU)~(\ref{No or weak memory access control; executable stack:})  & 0           & \multicolumn{1}{c|}{0\%}             & 0                     & 0\%                  & 4                                                    & 0.58\%                                & 0 & \multicolumn{1}{c|}{0\%}    & 0          & 0\%         & 0  & \multicolumn{1}{c|}{0\%}    & 0        & 0\%           & 0 & \multicolumn{1}{c|}{0\%}    & 0        & 0\%           & 1           & 100\%       & 0           & 0\%             & 0           & 0\%        & 5          & 0.28\%       \\
			Memory Access Control (sMPU)~(\ref{No or weak memory access control; executable stack:}) & 19          & \multicolumn{1}{c|}{2.47\%}          & 17                    & 3.31\%               & 0                                                    & 0\%                                   & \multicolumn{2}{c|}{-}          & \multicolumn{2}{c|}{-}   & \multicolumn{2}{c|}{-}           & \multicolumn{2}{c|}{-}   & \multicolumn{2}{c|}{-}          & \multicolumn{2}{c|}{-}   & \multicolumn{2}{c|}{-}    & \multicolumn{2}{c|}{-}        & \multicolumn{2}{c|}{-}   & 19         & 1.10\%       \\
			Missing Readback Protection~(\ref{Missing readback protection:})                         & 17          & \multicolumn{1}{c|}{2.21\%}          & 9                     & 1.75\%               & 15                                                   & 2.17\%                                & \multicolumn{2}{c|}{-}          & \multicolumn{2}{c|}{-}   & \multicolumn{2}{c|}{-}           & \multicolumn{2}{c|}{-}   & \multicolumn{2}{c|}{-}          & \multicolumn{2}{c|}{-}   & \multicolumn{2}{c|}{-}    & \multicolumn{2}{c|}{-}        & \multicolumn{2}{c|}{-}   & 32         & 1.78\%       \\
			Stack Canaries~(\ref{No or weak stack canary:})                                          & 0           & \multicolumn{1}{c|}{0\%}             & 0                     & 0\%                  & 1                                                    & 0.14\%                                & 0 & \multicolumn{1}{c|}{0\%}    & 0          & 0\%         & 0  & \multicolumn{1}{c|}{0\%}    & 0        & 0\%           & 0 & \multicolumn{1}{c|}{0\%}    & 0        & 0\%           & 0           & 0\%         & 0           & 0\%             & 0           & 0\%        & 1          & 0.06\%       \\
			Stack Limit Register Usage~(\ref{No or weak guards between memory segments:})            & 0           & \multicolumn{1}{c|}{0\%}             & 0                     & 0\%                  & 0                                                    & 0\%                                   & 0 & \multicolumn{1}{c|}{0\%}    & 0          & 0\%         & 0  & \multicolumn{1}{c|}{0\%}    & 0        & 0\%           & 0 & \multicolumn{1}{c|}{0\%}    & 0        & 0\%           & 0           & 0\%         & 0           & 0\%             & 0           & 0\%        & 0          & 0\%          \\
			Task Stack Ovf. Guard*~(\ref{No or weak guards between memory segments:})                & 59          & \multicolumn{1}{c|}{96.72\%}         & 4                     & 80\%                 & 9                                                    & 32.14\%                               & \multicolumn{2}{c|}{-}          & \multicolumn{2}{c|}{-}   & \multicolumn{2}{c|}{-}           & \multicolumn{2}{c|}{-}   & \multicolumn{2}{c|}{-}          & \multicolumn{2}{c|}{-}   & \multicolumn{2}{c|}{-}    & \multicolumn{2}{c|}{-}        & \multicolumn{2}{c|}{-}   & 68         & 76.40\%      \\
			Proper Instruction Sync. Barriers†~(\ref{Missing barrier instructions:})                 & 30          & \multicolumn{1}{c|}{36.59\%}         & 16                    & 27.12\%              & 68                                                   & 40\%                                  & \multicolumn{2}{c|}{-}          & \multicolumn{2}{c|}{-}   & \multicolumn{2}{c|}{-}           & \multicolumn{2}{c|}{-}   & 0 & \multicolumn{1}{c|}{0\%}    & 0        & 0\%           & \multicolumn{2}{c|}{-}    & \multicolumn{2}{c|}{-}        & \multicolumn{2}{c|}{-}   & 98         & 34.88\%       \\ \hline
			%\rowcolor{white}
			%Total                     & \multicolumn{2}{c|}{768}                           & \multicolumn{2}{c|}{513}    & \multicolumn{2}{c|}{694}                                                  & \multicolumn{2}{c|}{22}         & \multicolumn{2}{c|}{20}  & \multicolumn{2}{c|}{192}         & \multicolumn{2}{c|}{120} & \multicolumn{2}{c|}{53}         & \multicolumn{2}{c|}{36}  & \multicolumn{2}{c|}{4}      & \multicolumn{2}{c}{1,733}  \\ \hline
		\end{tabular}
		\begin{tablenotes}
			\item[] \#F: Number of firmware, \#D: Number of devices, -: Not applicable, *: The percentage is only based on firmware that use RTOS, †: The percentage is only based on firmware that update \verb|CONTROL| with the \verb|MSR| instruction.
		\end{tablenotes}  
	\end{threeparttable}
	\vspace{-0.5cm}
\end{table*}


%Software architectural issues refer to misuse of 
Software architectural issues refer to common limitations and flaws we found in real-world firmware.

%in the design of the Cortex-M production software systems mainly in the architectural models of A1, A2, and A3.
%Some of these issues can be avoided by redesigning or modifying the software, but it is usually at the cost of performance.
%\ziming{need to explain some of these issues can be simply solved by using existing hardware features. Some of them cannot and need new mechanism.}
%We refer those issues to Figure~\ref{fig:overview}, which presents the specific architecture details of different software applications.


\issue{No or weak privilege separation:}
As shown in Table~\ref{tab:bin_anal}, only 10 out of 1,797 samples in our dataset execute some code at the unprivileged level, and the others execute entirely at the privileged level.
%As shown in Figure~\ref{fig:overview}(a),
%not only bare-metal programs but also applications on some RTOSes execute at the privileged level and have unrestricted access to the physical memory space including system controllers and peripherals.
Interestingly, even though some firmware enables
MPU, %to configure access permission,
% Even if MPU may be enabled on these systems, 
%such as isolation of privileges, even if the underlying hardware provides corresponding supports.
the settings can be reverted as everything runs at the privileged level.
Due to the lack of fault isolation and privilege separation, 
a bug anywhere may compromise the whole system.
% lead to a crash or full control by an attacker.
%The bit 0 of the \verb|CONTROL| register determines the current privilege level.
%We found 81 of the 790 firmware, which is 32 of the 535 devices, in the FirmXRay dataset have changed the \verb|CONTROL| register.
%which infers they have employed the privilege separation in their system.

\issue{SVC misuse:}
The \verb|SVC| instruction is designed to escalate the execution level; %, same as the \verb|syscall| instruction on x64.
however, executing this instruction at the privileged level also transfers the control to the SVC handler. 
Surprisingly, we find that 1,443 (98.97\%) Nordic samples run everything at the privileged level and misuse this feature to call library APIs, e.g., Nordic SoftDevice~\cite{nordicsoftdevice},
instead of privilege escalation.
Similar behaviors are also observed on some TI, Telink, Cypress, and ST systems.

%1,469 samples . % when the whole firmware executes at the privileged level.
%In particular, the Nordic nRF5 series firmware call the SoftDevice~\cite{nordicsoftdevice} APIs using \verb|SVC|.

%The Supervisor Calls (SVC) are widely used to escalate the privilege level, which can be handy to quickly switch between different privilege modes.
%However, some vendors like the Nordic may define their own SVC handler, not to separate the privilege level, but to generate interrupts implementing special Application Program Interface (API) calls~\cite{cmsissvc}.
%On the Nordic nRF5 series, there is a firmware module identified as SoftDevice~\cite{nordicsoftdevice}, 
%which is a pre-compiled and linked binary to be used as the wireless protocol stack that complements a corresponding SoC.
%The application can use the SoftDevice API as a high-level programming language interface, and this API is implemented using thread-safe SVC interrupts.
%If a bare-metal program running at the single privileged level enables the SoftDevice,
%the SVC function call will be directly made in the privileged mode,
%and there will be no privilege switches since everything running in the privileged execution mode.
%In this case, the SVC call acts only as a normal interruption,
%and the application side of this program can have a chance to take control the SoftDevice by altering the control flow.
%(For the programs with single privilege level, the use of the SVC API function call is not enough to provide a robust privilege separation.)

\issue{No or weak stack separation:}
RTOSs, including FreeRTOS~\cite{freertosstack} and Zephyr~\cite{zephyrstack}, support multi-tasking, so each task has its own stack.
%FreeRTOS uses a hardcoded 20-byte delimiter (\verb|0xA5|s) to mark the limit of a stack, which is checked when a context switch happens.
%Zephyr uses \verb|PSPLIM| to prevent overwriting.
%For each task, they split the current stack into different regions to store the corresponding task stack, 
%and the context switching will use the current stack pointer to locate different tasks.
However, stack separation between the kernel and application is rarely used in bare-metal firmware.
10 samples that adopt privilege separation (discussed in~\ref{No or weak privilege separation:}) leverage both the \verb|MPS-| and \verb|PSP-|based stacks.
In addition, another 124 samples in our dataset use both the \verb|MPS-| and \verb|PSP-|based stacks without privilege separation.
%Even without enforcing the privilege separation, the program can still choose to use different stacks for different tasks,
%ensuring the corruption of one task does not spread to others.
%The bit 1 of the \verb|CONTROL| register determines the current activate stack.
%In our analyzed dataset, we found 52 out of 1035 firmware, which is 35 of the 689 devices, have switched to use the PSP as the current stack.
All other samples (1,663; 92.54\%) only adopt a single \verb|MSP|-based stack.
%and execute at a single privileged level all the time.
%As we discussed previously, the 8 firmware which carry out privilege separation also use multiple stacks,
%so there are only 44 firmware (30 devices) have used both main and process stacks without changing the privilege level.
%\ziming{no one uses multiple PSP. Different task on FreeRTOS/Zephyr will PSP/MSP?}

\issue{Secure state exception stack frame manipulation:}
For TrustZone-M enabled processors,
CVE-2020-16273 shows that the non-secure state software may manipulate the secure stacks and hijack the secure control flow
if the secure software does not properly initialize the secure stacks. % when the stacks are created. % or when performing non-standard transitioning between states or modes.
To this end, an attacker creates a fake exception return stack frame to deprivilege an interrupt.
To mitigate this attack, Arm recommends adding an integrity signature to the bottom of the secure exception stack frame~\cite{ARMsecurestack}.
%[Why are we talking about attacks??? This section is about limitation or issues]

\issue{No or weak memory access control; executable stack:}
% Execution protection stops the execution within arbitrary memory regions.
Even though some Cortex-M devices have MPU, % for memory access control, 
previous research believes that most real-world systems do not use it~\cite{clements2017EPOXY, zhou2019good, clements2018aces}. 
We confirm that 1,773 of the 1,797 firmware in our dataset do not use MPU, %, whose registers are memory-mapped at fixed addresses.
which means the address space in \emph{code}, \emph{SRAM}, and \emph{RAM} is executable. 
For the same reason, data execution prevention (DEP) %, a standard feature in modern operating systems, 
is not enforced on these systems.
Without memory access control,
malicious code can also read and write arbitrary memory. %(see Figure~\ref{fig:overview} (a)).
%For example, there is no  since MPU is not enabled.
%DEP is used to prevent executing code from non-executable memory space.
%Cortex-M processors do define a memory region that address starting with \verb|0xF| is non executable.
%And MPU provides \verb|XN| bit to configure a memory region as execute never.
%Since MPU is seldom enabled for most software systems, the DEP implementation is weak.
%The MPU registers are used to define the MPU regions and their attributes,
%and they reside in the Secure System Control Space (SCS) memory region.
Out of the 24 firmware samples that use MPU in our dataset, 5 samples use the MPU defined by Arm. The remaining 19 samples use a vendor-specific implementation (i.e., Nordic's simplified MPU (sMPU)~\cite{nordicmpu}), which only supports
a subset of features defined by Arm.
Specifically, sMPU only supports read and write permissions and can only divide memory into two protection domains.

% , which are different versions for the same series of Nordic Cortex-M0 devices, use Nordic' simplified MPU (sMPU)~\cite{nordicmpu} since Cortex-M0 does not have an MPU.
% The sMPU only supports the read and write permissions, and it can only divide memory into two protection domains. 
%, namely region 0 and region 1.
%Region 0 is occupied by the SoftDevice~\cite{nordicsoftdevice} (precompiled SDK binary file region) while region 1 is available to the application.
%SoftDevice program and data memory are sandboxed to prevent SoftDevice program corruption by the application ensuring robust and predictable performance.
%When memory protection is enabled, these regions will be used by the Memory Protection Unit to enforce runtime protection and readback protection of resources classified as region 0. 
%While region 0 \emph{code} has full access to the address space, it cannot be read or written by region 1.
%Region 0 \emph{SRAM} is also not writable to region 1 programs.
% NVM protection blocks (below) is complimentary and optional to the region 0 sandboxing mentioned above
%The program memory region (including \ziming{region 1 and region 2}), which is the non-volatile memory (flash), can be protected from erases or writes depending on settings in the \verb|PROTENSET| registers. 
%while the Armbuilt-in one can also set the execution permission, to prevent the memory from being executed in a protected region.
%One bit in a \verb|PROTENSET| register represents one protected block. 
%There are two \verb|PROTENSET| registers of 32 bits which means there are 64 protection blocks in total.
%The protection block size can be configured by the \verb|PROTBLOCKSIZE| register and is default 4KB.

%Since the Nordic includes the application program interface and libraries, which is called SoftDevice, into a pre-compiled and linked binary,
%they provides a runtime separation on the code memory, RAM and peripherals to isolate the SoftDevice program and the applications.
%The SoftDevice code region cannot be read, written, or erased at runtime by the application code region, and the SoftDevice RAM region cannot be written to by an application at runtime.
%The SoftDevice code region will always have full access to the system.
%Besides the separation on the code memory, the entire code region can also be divided into 64 protectable blocks with independent setting of the erase/write permission.
%Another major difference is that the Nordic MPU implementation can only control the memory read and write accesses,
%while the Arm built-in one can also set the execution permission, to prevent the memory from being executed in a protected region.

%\ziming{I do not understand here. Is the MPU configuration divides the memory or the MPU divides the memory?? How did you find the name 0 and 1? Is this from some materials or just reverse engineering? Do they use a single privileged level? If Region 1 has a code injection vulnerability, can region 1 code change the settings of MPU?}
%The Nordic customized MPU divides the code memory, RAM and peripherals into two regions: region 0 and region 1.
%Region 0 is occupied by the SoftDevice~\cite{nordicsoftdevice} (precompiled SDK binary file region) while region 1 is available to the application.
%SoftDevice program and data memory are sandboxed to prevent SoftDevice program corruption by the application ensuring robust and predictable performance.
%When memory protection is enabled, these regions will be used by the Memory Protection Unit to enforce runtime protection and readback protection of resources classified as region 0. 
%Region 0 program memory cannot be read, written, or erased at runtime.
%Region 0 RAM cannot be written to by an application at runtime.
% NVM protection blocks (below) is complimentary and optional to the region 0 sandboxing mentioned above
%The program memory region (including region 1 and region 2), which is the non-volatile memory (flash), can be protected from erases or writes depending on settings in the \verb|PROTENSET| registers. 
%One bit in a \verb|PROTENSET| register represents one protected block. 
%There are two \verb|PROTENSET| registers of 32 bits which means there are 64 protection blocks in total.
%The protection block size can be configured by the \verb|PROTBLOCKSIZE| register and is default 4KB.

%For the CPUs without native hardware MPU support, e.g., Cortex-M0, the chip vendor may provide their customized implementation of memory protection unit~\cite{nordicmpu}.
%The customized MPU registers are defined in the peripheral memory region, and serves the same functionality as the Arm native MPU.
%The MPU register addresses for the Arm native implementation stay same among different supported CPUs.
%To see whether a firmware has used the MPU or not, we can directly look for the operations on the \verb|MPU_CTRL| register, which has a fixed address of \verb|0xE000ED94|.
%We find that no firmware in the dataset has enabled the Arm native MPU.
%However, since all the firmware in dataset come from the same vendor Nordic, 
%we also use the customized MPU register address from the Nordic to filter the dataset, and found only one of the device has implemented the Nordic-defined MPU.

\issue{Missing readback protection:}
As discussed in \ref{Bypassable vendor-specific readback protection:}, Nordic MCUs implement a readback protection mechanism.
%We The mapped registers to setup the mechanism for different series.
%By checking the operation on those registers, 
Notwithstanding, we found that only found 32 out of the 1,458 Nordic samples in our dataset enable this feature. 
%and 6 of them use the nRF51 flawed readback protection.

\begin{comment}
\issue{Weak readback protection:}
Readback protection 
%is an important security feature that can 
prevents the leakage of data on the memory and flash through the debugging interface.
%\ziming{Does Arm come with build-in readback protection?} (Need to have a deeper look at the Arm CoreSight)
%The Arm supports different debug-related features~\cite{Armv7MArcRef}. 
%However, securing those features using readback protection and other methods depends on the chip vendors' implementation.
%With this protection, the program can restrict the attackers from being able to extract data from flash memory even if they have physical access to the device.
%The MPU can be configured to protect the memory ranges, however the read/write/execute permissions set by the MPU can be simply bypassed by the external debugger since the MPU is implemented within the CPU core and relies on the CPU-initiated bus transactions.
%The debugger uses the other bus masters such as the system memory debug Test Access Port (TAP) and DMA.
%There are many ways to prevent the debugger from accessing the protected regions of flash, including partial restrictions and 
Besides completely disabling the hardware debug interface~\cite{sultan2020readback}, some systems include specific features for readback protection. 
%However, these partial restrictions may leave potential logic holes to the attackers, which can be used to circumvent the restriction.
For example, sMPU can disable the debugger access to the flash memory region.
However, it still allows register access and single stepping of the processor, which was exploited to dump the full flash content~\cite{kris2015dumping}.
This flaw was addressed in the new processors~\cite{nordicnrf52}.
But for the Nordic firmware in our dataset, only 34 out of 1462 firmware have enabled the readback protection.
%And 6 of them use the nRF51 flawed readback protection.
\end{comment}

\issue{No or weak stack canary:} 
%Stack canary is a compiler-based approach to prevent the stack frames of functions from being overwritten~\cite{cowan1998stackguard}.
%To this end, a compiler instruments code in the protected function's prologue to place a canary onto the stack frame and the epilogue to check if the canary is overwritten. 
In the standard C libraries (libc),
the value of stack canary is taken from a global variable \verb|__stack_chk_guard|, which stays the same during a process' life cycle. %and when a process is forked. 
In modern OSes, the value is randomly initialized when a process is created, so different processes have different canary values. 
If a canary is found tampered with, the function \verb|__stack_chk_fail()| is called to terminate the program.

\emph{Compiler and RTOS Implementations:} We found that the GNU Arm Embedded Toolchain (\verb|arm-none-eabi-gcc|, version 10.3.1)~\cite{armgcc}, Arm Compiler 5 (\verb|armcc|, version 5.6u7)~\cite{armcc}, and Arm Compiler 6 (\verb|armclang|, version 6.16)~\cite{armclang} all implement the same canary mechanism as their x86/64 counterparts.
The feature, however, is disabled by default in all three compilers~\cite{stackarmclang, stackarmcc}.
In contrast, it has been a default feature
of GCC since Ubuntu 6.10 in 2006~\cite{ubuntucookie}.
% whereas GCC on Ubuntu has enabled it by default since Ubuntu 6.10 in 2006~\cite{ubuntucookie}.
%i.e., \verb|-fno-stack-protector|, 
%and needs be enabled with compiler options explicitly, e.g., \verb|-fstack-protector|, etc.
More seriously, different from MMU-enabled systems where \verb|__stack_chk_guard| is a global variable in each process' virtual memory, 
on Cortex-M there is only one \verb|__stack_chk_guard| in the whole physical address space.
As a result, different tasks running on FreeRTOS will have the same canary value.
RIOT-OS adopts compile-time canary randomization, which ensures each build has a unique canary~\cite{riotstack}.
Zephyr~\cite{zephyrstackcode} randomly initializes a canary value at boot time.
Then the value stays the same until the next reboot.
Moreover, if the canary value is not initialized explicitly, \verb|arm-none-eabi-gcc| uses a fixed terminator canary value (\verb|0xff0a0000|), 
whereas both \verb|armcc| and \verb|armclang| use \verb|0|.
The existing stack canary mechanism designed for process-based OSes is weakened in the single physical address space setting; therefore, a new mechanism that updates the canary value more frequently is needed for Cortex-M and other MCU software systems.

%\emph{RIOT-OS Implementations:}
%The RIOT-OS has the implementation of the stack canaries based on the compiler built-in support~\cite{riotstack}.
%It has a canary value randomization mechanism which will ensure the stack canary has a different value on each build.
%The canary value is generated by the build system randomly and passed to the protection module using the \verb|-D| compiler flag. 
%The protection module object file is marked as \verb|PHONY|, which will make sure it gets rebuilt on each make invocation, and thereby ensuring that each build has a different random canary value.

%\emph{Zephyr Project Implementations:}
%The Zephyr Project has an configuration option \verb|CONFIG_STACK_CANARIES| to enable the compiler stack protection with canaries~\cite{zephyrstack}.
%This option is disabled by default, since enabling it can result in a significant increase in footprint and an associated decrease in performance.
%During the initialization at boot-time, it generates a random canary value assigned to the global canary variable~\cite{zephyrstackcode}.
%The random value generation is based on the device driver; on some constrained devices (e.g. devices without random number generator), 
%the produced canary value is not considered as a cryptographically secure random value.


%The GNU Arm Embedded Toolchain, \verb|armclang| (Arm Compiler 6), \verb|armcc| (Arm Compiler 5) provide built-in supports for the stack canaries, which can be enabled with several compiler options.
%A guard variable that is overwritten indicates a buffer overflow, and the checking code alerts the run-time environment.

%For the GNU Arm Embedded Toolchain version 10.3-2021.10, 
%we tested the compiler built-in stack canaries by compiling a single file using the \verb|arm-none-eabi-gcc| compiler, with the flag \verb|-fstack-protector-all|.
%When a function is called with stack canary enabled, 
%the initial value of its canary variable is taken from a global variable \verb|__stack_chk_guard|, 
%and the program should provide a stack overflow hook function \verb|__stack_chk_fail()| to handle the fallback.
%A suitable implementation can set the canary variable \verb|__stack_chk_guard| to a random value when the program is loaded, and before the first protected function is executed.
%If no definition of the canary variable and the fallback function is provided in the program code,
%the compiler will generate a function \verb|__stack_chk_init()| to set a fix value \verb|0xff0a0000| to the canary variable, and a default implementation of \verb|__stack_chk_fail()| will be used.

%For the \verb|armclang| and \verb|armcc|, we tested this built-in stack canaries on a FreeRTOS demo project with five different tasks.
%Those tasks are created to be run infinitely, with the label \verb|__noreturn|.
%We also define a simple print value function that does return to compare the compiler behavior on different function types.

%Arm Compiler 5 uses the \verb|armcc| as the compiler tool.
%We use the Arm Keil IDE with \verb|armcc| V5.06 update 7 (build 960) to test the stack canaries behavior.
%Different from the GCC compiler, The \verb|armcc| uses the flag \verb|--protect_stack_all| to enable the stack canaries.
%Once enabled, we must provide a declaration in the program code for the global variable \verb|__stack_chk_guard| and the fallback function \verb|__stack_chk_fail()|, 
%otherwise the compiler will give out an undefined symbol error.
%If we do not provide any initial value to the canary variable, the compiler will use 0 to initialize the \verb|__stack_chk_guard| when the program gets loaded.
%And before the linking process of the linker, the \verb|__stack_chk_guard| is loaded from the \verb|.data| section.
%For the non-return task functions, the compiler will only instrument the canary insert operation in the function prologue, and do not add checks in the function epilogue.

%Arm Compiler 6 uses the compiler tool \verb|armclang| instead of \verb|armcc|.
%We use the Arm Keil IDE with \verb|armclang| V6.16, and set the compiler flag \verb|-fstack-protector-all| to enable the stack canaries.
%The compiler requirements of the global variable \verb|__stack_chk_guard| and the fallback function \verb|__stack_chk_fail()| are similar to the \verb|armcc|.
%However, before the lining process, the stack canary value address in each protected function only points to zero.
%And in the \verb|armclang|, the compiler do not touch the non-return task functions.

%As described above, those kinds of stack canaries protection may not secure.
%Even if we can give a random canary value during the program initialization, the canary word must remain unchanged during the life of the program. 
%Since there is no process separation as the X86 platform, that canary value is global and same to each function in the program.
%It should also be mentioned that the canary word is stored in a writable memory region, which means it could be easily modified by other malicious functions.


\emph{Empirical Analysis on Real-world Firmware:}
%Since all the firmware in our dataset are real-world raw binaries, it is hard to identify the stack canaries implementation by function or variable symbols.
%For this reason, we move the focus to the relatively invariant canary insert and check operations at the function prologue and epilogue.
%For each Arm compiler in each optimization level, we recognize its instruction pattern which is related to the stack canaries in the function prologue and epilogue,
%and create the corresponding regular expression to match the disassembled firmware dataset.
% Comment: right now we only have regex for one optimization level
%There are four regular expressions for each compiler, matching the canary operations in the function prologue and epilogue in two optimization levels.
Even if the aforementioned compilers offer the canary mechanism, only \emph{one} of the 1,797 firmware samples in our dataset adopts it.
%It is probably because the option is by default disabled. 
%used has enabled the compiler built-in stack canaries support.
% Possible reasons:
%We surmise that the reason for not enabling the compiler stack protection is the performance overhead introduced by the extra checks in each function.

\issue{No or weak guards between memory segments:} 
Guard pages are used to %usually inserted by operating systems to 
delimit the boundaries of segments, such as stack and code, to prevent accidental and intentional overwriting from an adjacent segment.
%Due to the small address space and limited number of MPU regions, it is not efficient to implement guard pages on Cortex-M. 
%To alleviate this issue, 
As discussed in \S\ref{sec:cortexm}, Armv8-M also introduces stack limit registers (\verb|PSPLIM|, \verb|MSPLIM|) to delimit the boundaries of stacks.
No firmware in our dataset has used the stack limit registers.

\emph{RTOS Implementations:} 
However, we found that only a few RTOSs design mechanisms to protect tasks' stacks, and only Zephyr optionally supports using stack limit registers.
When stack guard is enabled, FreeRTOS~\cite{freertoskernel} and Mbed OS~\cite{rtx5config} insert a predefined delimiter to mark the boundary of each task's stack.
%a predefined 20-byte delimiter (\verb|0xA5|) to mark the low limit of the stack, which will be checked when a context switch happens.
Zephyr can use either \verb|PSPLIM| or an MPU-configured memory guard to prevent overwriting beyond a task's stack~\cite{zephyrstackguard}.

\emph{Empirical Analysis on Real-world Firmware:}
59 of the 66 FreeRTOS-based firmware samples and 7 of the 13 Mbed OS-based firmware samples use task stack overflow guards.
%We found 13 firmware in our dataset use Mbed-OS, and ??? of them enabled the thread stack overflow check.
%By the time of our analysis, Ghidra does not support identifying the instructions to access the stack limit registers.

\begin{comment}
On FreeRTOS, each task has its own stack. It has a compiler option \verb|configCHECK_FOR_STACK_OVERFLOW| to enable the task stack overflow checking~\cite{freertostaskovfchk}.
When switching the tasks, the RTOS kernel can check that either the processor stack pointer remains within the valid stack space,
or the last 16 bytes within the valid stack range remains same when the stack was first created by the task.
The latter method is stronger however less efficient than the former one.


Mbed-OS uses the Keil-RTX5 RTOS kernel, which implements a software stack overflow checking that can be enabled with defining \verb|OS_STACK_CHECK|~\cite{rtx5config}.
During the thread switch, the kernel will check both that the current running thread stack pointer is within the stack space,
and the stack magic word at bottom of the stack is intact. 
The stack magic word is a fixed value that defined in the kernel header file.
% RTX5 Header File: https://www.keil.com/pack/doc/CMSIS_Dev/RTOS2/html/theory_of_operation.html
\end{comment}

%erflow by setting a stack limit or filling the last 20 bytes of the stack with a known value (\verb|0xa5|) when a task is created.
%  for checking the remained unused space for tasks.
% FreeRTOS known stack value pattern: https://github.com/FreeRTOS/FreeRTOS-Kernel/blob/ac2c383bc14b2577101cad238c8779f4d9c14d6c/tasks.c#L844
% https://github.com/FreeRTOS/FreeRTOS-Kernel/blob/ac2c383bc14b2577101cad238c8779f4d9c14d6c/tasks.c#L3052
%Since the value is fixed, it can be very easily exploited.
%Even though GCC provides a stack cookie mechanism by instrumenting a function's prologue and epilogue~\cite{gccssp}, %with a failure handler to check if the value is changed.
%this mechanism needs run-time support from the OS to provide a unique cookie and a failure handler function,
%which only a few OS, including RIOT OS and Zephyr, implement.
% Mbed OS, RT-thread, TockOS, etc. miss such implementation. 
% Weidler et al.~\cite{weidler2017return} showed that arbitrary code can be executed via return-oriented programming on the Cortex-M processor.
% RIOT OS: https://github.com/RIOT-OS/RIOT/blob/73ccd1e2e721bee38f958f8906ac32e5e1fceb0c/sys/ssp/ssp.c
% https://github.com/zephyrproject-rtos/zephyr/blob/be0f5fe0b0be7d095419ee90d23c8831cf8de9c1/kernel/compiler_stack_protect.c#L49-L53  __stack_chk_guard

%The detail of vulnerability is presented in~\cite{}, for example, 
%When \verb|EXC_RETURN| is loaded to \verb|PC|, it will check the \verb|EXC_RETURN.SPSEL| bit to choose which stack pointer to use.
%But when handling \verb|FNC_RETURN|, there is no such bit. 
%Programmers can manipulate the code to choose \verb|MSP_S|, which may cause the unintended memory access from the secure main stack.
%For example, when a processor running in secure thread mode with the \verb|PSP_S|, a non-secure function call happens, the \verb|PSP_S| changes to \verb|PSP_NS|.
%Then in the non secure function, it transits to a non secure \verb|SVC| handler with \verb|MSP_NS| when an \verb|SVC| instruction executes.
%At the \verb|SVC| handler, attacker executes \verb|BX <FNC_RETURN>| to change the stack to \verb|MSP_S|, then trigger the processor to pop out invalid return address (CVE-2020-16273).
%Thus, the non secure code can jump to arbitrary secure address space.

\issue{Missing barrier instructions:}
Barrier instructions, including data memory barrier (\verb|DMB|), data synchronization barrier (\verb|DSB|), and instruction synchronization barrier (\verb|ISB|), can enforce ordering between memory accesses and system configurations, which makes sure that a system configuration
takes effect before any memory operations~\cite{membarrier}.
The omission of memory barrier instructions is unlikely to cause any issues on most Cortex-M MCUs because they do not have out-of-order execution and branch prediction capabilities.
For the Cortex-M devices that do have such capabilities, this may lead to similar vulnerabilities that were discovered on microprocessors~\cite{lipp2018meltdown, kocher2018spectre, ravichandran2022pacman}.
To check if barriers are set in firmware, for any \verb|CONTROL| register update, we verify if there is an \verb|ISB| instruction in its ten subsequent instructions. 
%To find out whether a firmware has properly enforced the instruction synchronization barrier, we look for the \verb|ISB| instruction within 10 instructions after the update of \verb|CONTROL| register.
Our analysis shows that only 98 of the 281 firmware samples (34.88\%) that update the \verb|CONTROL| register use the \verb|ISB| instruction thereafter.
Note that we do not claim the other 183 firmware samples are vulnerable because we do not know which MCUs they target.

%Arm architectures allow the design of processors to reorder memory access, which mostly happens in high-end processors and multiprocessor systems.
%The memory barrier instructions can be used to enforce ordering between memory accesses~\cite{yiu2020definitive}.
%On the Cortex-M processors that have relatively simple pipelines, the processor does not reorder any memory accesses, and most applications work without any memory barrier instructions.
%However, there are some cases that the aforementioned barrier instructions are still needed to ensure the effect of the a system configuration change takes place before subsequent operations.
%For example, After updating the \verb|CONTROL| register with an \verb|MSR| instruction, the \verb|ISB| instruction should be used to ensure the updated configuration is used for subsequent operations~\cite{yiu2020definitive}.

\begin{comment}
\issue{Statically linked executables and no dynamic linker:}
Most software systems on Cortex-M are statically linked into one big executable, namely the firmware, 
and no dynamic linker is available in most RTOSs.
Therefore, a load-time ASLR, which has been another standard feature in modern operating systems for more than a decade, cannot be implemented.
Even if boot time ASLR is possible, many IoT devices will not reboot for a very long time.
\end{comment}

\begin{mdframed}[style=remarkstyle,backgroundcolor=blue!10]
\textbf{Key Findings:} 
Even if Cortex-M offers some security features in its ISA, the real-world firmware samples in our dataset barely use them and largely lack the software security mitigations that are widely deployed on modern microprocessor-based systems.
In addition, some mitigations, e.g., stack canaries, are less effective on MCU-based systems and should be redesigned.
\end{mdframed}

\begin{comment}
(1) Cortex-M processors do not support some techniques we take for granted on x86/64 or Cortex-A, and their security features are less known.
For example, virtual memory management is not available for lack of a Memory Management Unit (MMU), but Cortex-M does offer a Memory Protection Unit (MPU) that provides access control in the physical memory space.
Also, Cortex-M has recently introduced its own version of TrustZone, which has different underlying mechanisms from its Cortex-A counterpart;
(2) Even if Cortex-M offers some security-related features, existing embedded and IoT software systems barely use them and largely lack protection against code injection, control-flow hijack, data corruption, and other attacks. 
In other words, software technologies for security on such devices significantly lag behind the development of not only mobile and personal computer security but also their own hardware security offerings;

In other words, software technologies for security on such devices significantly lag behind the development of not only mobile and personal computer security but also their own hardware security offerings.
\end{comment}

\begin{comment}
\issue{Weak security configuration:}
As discussed in argXtract~\cite{sivakumaran2021argxtract}, configuration information that includes device and protocols or special hardware they use, application repositories, and website interfaces, can indicate the security status and introduce vulnerabilities of the firmware binaries. 
For example, the man in the middle attack because the Bluetooth communication is not encrypted or authenticated~\cite{hackerbluetooth}.
Default root password configuration~\cite{2880} exposes root privilege to attackers.
\end{comment}


% \subsubsection{Lack of basic security features}
% No hardware random number generators or standard encryption units.
% \textcolor{blue}{TODO: more features}

% \textit{Attacks on protocols: }
% Internet of Threats~\cite{meneghello2019iot}.
% \textcolor{blue}{TODO: more details}

% \textcolor{blue}{TODO: more details}

% \textit{Other attacks: }
% Laser fault injection~\cite{selmke2018locked}.

\section{Bug Reports on Real-world Systems}
\label{sec:ImpIssueVul}
%In addition to hardware and software architectural issues, software implementation bugs are also critical. %embedded devices are also influenced by software implementations.
%Given the wide range of Cortex-M system usage scenarios,
%With a variety of usage scenarios on Cortex-M processor powered devices, 
%their software systems also exhibit a variety of structures and have different components.
\begin{comment}
\begin{table}[!t]
	\center
	\scriptsize
	\caption{Number of disclosed CVEs from 2017 to 2022}
	\vspace{-0.2cm}
	\setlength\tabcolsep{0.55ex}
	\renewcommand{\arraystretch}{1.1}
	\label{tab:sum}
	\scalebox{0.92}{\begin{threeparttable}
		\begin{tabular}{l|c|c|c|c|c}
			\hline
			\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Critical} & \multicolumn{1}{c|}{High} & \multicolumn{1}{c|}{Medium} & \multicolumn{1}{c|}{Low} & \multicolumn{1}{c}{Total} \\ \hline \hline
			\begin{tabular}[c]{@{}l@{}}Arm, Microchip Technology, Silicon Labs,\\NXP Semiconductors, ST Microelectronics,\\Cypress Semiconductor, Gigadevice, Texas\\Instruments, Nordic\end{tabular} & \begin{tabular}[c]{@{}c@{}}4\\ (5.80\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}24\\ (34.78\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}41\\ (59.42\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}-\\		\end{tabular} & 69    \\ \hline
			\begin{tabular}[c]{@{}l@{}}FreeRTOS, CMSIS RTOS2, Mbed OS, Ze-\\phyr, RIOT-OS, Contiki-ng, Azure\end{tabular} & \begin{tabular}[c]{@{}c@{}}45\\ (33.09\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}67\\ (49.26\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}23\\ (16.91\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}1\\ (0.74\%)\end{tabular} & 136   \\ \hline
			\begin{tabular}[c]{@{}l@{}}Mbed TLS, WolfSSL\end{tabular} & \begin{tabular}[c]{@{}c@{}}17\\ (22.67\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}28\\ (37.33\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}30\\ (40.00\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}-\end{tabular} & 75   \\ \hline
			Total & \begin{tabular}[c]{@{}c@{}}66\\ (23.57\%)\end{tabular}& \begin{tabular}[c]{@{}c@{}}119\\ (42.50\%)\end{tabular}& \begin{tabular}[c]{@{}c@{}}94\\ (33.57\%)\end{tabular}& \begin{tabular}[c]{@{}c@{}}1\\ (0.36\%)\end{tabular} & 280\\ \hline                                                             
		\end{tabular}
		%\begin{tablenotes}
			%\item[] The bug reports cover from hardware architecture to software implementation.
		%\end{tablenotes}  
	\end{threeparttable}}
	\vspace{-0.5cm}
\end{table}
\end{comment}

\begin{table}[!t]
	\center
	\scriptsize
	\caption{Distribution of disclosed Cortex-M related CVEs (2017 - 2023)}
	%\vspace{-0.2cm}
	\setlength\tabcolsep{0.5ex}
	\renewcommand{\arraystretch}{1}
	\rowcolors{2}{gray!15}{white}
	\label{tab:sum}
	\scalebox{0.92}{\begin{threeparttable}
			\begin{tabular}{l|cc|cc|cc|cc|cc}
				\hline
				\multicolumn{1}{c|}{HW Vendor/RTOS/Lib} & \multicolumn{2}{c|}{Critical} & \multicolumn{2}{c|}{High} & \multicolumn{2}{c|}{Medium} & \multicolumn{2}{c|}{Low} & \multicolumn{2}{c}{Total} \\ \hline \hline
				Arm                                     & 0          & 0\%              & 3         & 50.00\%       & 2          & 33.33\%        & 1        & 16.67\%       & 6         & 1.94\%        \\
				Microchip Technology                    & 1          & 14.29\%          & 2         & 28.57\%       & 4          & 57.14\%        & 0        & 0\%           & 7         & 2.26\%        \\
				Silicon Labs                            & 2          & 33.33\%          & 1         & 16.67\%       & 3          & 50.00\%        & 0        & 0\%           & 6         & 1.94\%        \\
				NXP Semiconductors                      & 1          & 8.33\%           & 5         & 41.67\%       & 6          & 50.00\%        & 0        & 0\%           & 12        & 3.87\%        \\
				ST Microelectronics                     & 2          & 12.50\%          & 2         & 12.50\%       & 12         & 75.00\%        & 0        & 0\%           & 16        & 5.16\%        \\
				Cypress Semiconductor                   & 0          & 0\%              & 6         & 50.00\%       & 6          & 50.00\%        & 0        & 0\%           & 12        & 3.87\%        \\
				Gigadevice                              & 0          & 0\%              & 0         & 0\%           & 6          & 100.00\%       & 0        & 0\%           & 6         & 1.94\%        \\
				Texas Instruments                       & 0          & 0\%              & 6         & 54.55\%       & 5          & 45.45\%        & 0        & 0\%           & 11        & 3.55\%        \\
				Nordic                                  & 0          & 0\%              & 2         & 50.00\%       & 2          & 50.00\%        & 0        & 0\%           & 3         & 1.29\%        \\ \hline
				Subtotal (HW vendors)                   & 6          & 7.50\%           & 27        & 33.75\%       & 46         & 57.50\%        & 1        & 1.25\%        & 80        & 25.81\%       \\ \hline \hline
				FreeRTOS                                & 3          & 15.79\%          & 9         & 47.39\%       & 7          & 36.84\%        & 0        & 0\%           & 19        & 6.13\%        \\
				CMSIS RTOS2                             & 1          & 100.00\%         & 0         & 0\%           & 0          & 0\%            & 0        & 0\%           & 1         & 0.32\%        \\
				Mbed OS                                 & 6          & 60.00\%          & 4         & 40.00\%       & 0          & 0\%            & 0        & 0\%           & 10        & 3.23\%        \\
				Zephyr                                  & 12         & 21.82\%          & 28        & 50.91\%       & 14         & 25.45\%        & 1        & 1.82\%        & 55        & 17.74\%       \\
				RIOT-OS                                 & 8          & 34.78\%          & 14        & 60.87\%       & 1          & 4.35\%         & 0        & 0\%           & 23        & 7.42\%        \\
				Contiki-ng                              & 15         & 40.54\%          & 18        & 48.65\%       & 4          & 10.81\%        & 0        & 0\%           & 37        & 11.94\%       \\
				Azure                                   & 5          & 38.46\%          & 2         & 15.38\%       & 5          & 38.46\%        & 1        & 7.69\%        & 13        & 4.19\%        \\ \hline
				Subtotal (RTOSs)                       & 50         & 31.65\%          & 75        & 47.47\%       & 31         & 19.62\%        & 2        & 1.27\%        & 158       & 50.97\%       \\ \hline \hline
				Mbed TLS                                & 6          & 20.69\%          & 12        & 41.38\%       & 11         & 37.93\%        & 0        & 0\%           & 29        & 9.35\%       \\
				WolfSSL                                 & 10         & 23.26\%          & 13        & 30.23\%       & 20         & 46.51\%        & 0        & 0\%           & 43        & 13.87\%       \\ \hline
				Subtotal (Libs)                         & 16         & 22.22\%          & 25        & 34.72\%       & 31         & 43.01\%        & 0        & 0\%           & 72        & 23.23\%       \\ \hline \hline
				Total                                   & 72         & 23.23\%          & 127       & 40.97\%       & 108        & 34.84\%        & 3        & 0.97\%        & \multicolumn{2}{c}{310}   \\ \hline
			\end{tabular}
			%\begin{tablenotes}
			%\item[] The bug reports cover from hardware architecture to software implementation.
			%\end{tablenotes}  
	\end{threeparttable}}
	\vspace{-0.5cm}
\end{table}

%\gl{try to use chip vendors instead of vendors. A vendor can also provide RTOSes.}

%In this section, we discuss the bug reports on Cortex-M systems.
Table~\ref{tab:sum} presents the numbers of Cortex-M related CVEs affecting nine hardware vendors, seven RTOSs, and two TLS libraries.
For each hardware vendor, we break down the number based
on their CVSS scores~\cite{cvss}.
As shown in the table, the majority of CVEs (57.50\%) affecting
hardware vendors are classified as ``medium'' severity, while the majority of CVEs affecting RTOSs (79.12\%) are categorized as either ``critical'' or ``high''.
%This section presents an overview of the hardware and software CVEs on Cortex-M systems from 2017 to 2022 and 
%We are also interested in the nature of these bugs.
%To this end, 
We use a bug classification system proposed in~\cite{cerdeira2020sok} to characterize them into three major classes, validation, functional, and extrinsic.
We summarize the results in Table~\ref{tab:CVEs-con}, where
we further provide a breakdown of bugs based on their functions and the software components affected by them.
The comprehensive list of bug reports and their detailed classification can be found in our anonymous open-source repository.

\begin{comment} 
%The score rates the severity of a vulnerability based on its exploitability, affected components, and impact of exploiting this vulnerability.
It is shown from the table that RTOSs report more security vulnerabilities than vendors.
In particular, half of the bug reports from vendors are rated as medium, while more than three-quarters of them from RTOSs are rated as critical or high.
%In particular, 41 of 121 reports (33.88\%) disclosed security vulnerabilities are considered critical.
However, we cannot conclude that RTOSs are less secure than vendors' implementation. 
The disparity is due to that (i) most bug reports are from vendors' SDKs, which are used for developers to build chip-specific firmware; 
(ii) most of the firmwares are bare-metal applications that have fewer system components than an RTOS;
(iii) RTOS are widely deployed on other platforms and the software implementation vulnerabilities affect not only Cortex-M devices but also other devices powered by Cortex-A, MIPS, etc.
Nevertheless, these results are useful because they help us understand the security status of current Cortex-M systems, and remind us of how to design a more secure system that avoids vulnerable components.


In this section, we focus on the implementation bugs of RTOSs and vendors' IoT solutions, including software development kits (SDK) that help build chip-specific firmware.
By analyzing related bug reports from public CVE database~\cite{cvss}, we summarize several vulnerable components: (i) wireless communication component supports data transfer between devices or cloud services through network;
(ii) device driver is required if the system needs to interact with peripherals;
(iii) dynamic memory management is important to allocate memory for data storage;
(iv) context switch is necessary if system implements hardware or software assisted isolation (e.g., privilege separation);
(v) kernel libraries are other functionalities provided by the system.
%Based on those system components, 
Table~\ref{tab:CVEs-con} presents the number of bug reports in meaningful categories~\cite{cerdeira2020sok}.
We will present the details of bug categories below.
\end{comment}

%As the table shows, over half of the reported vulnerabilities are in the communication component (validation bugs in wireless communication and functional bug in protocol implementation) that affect the all analyzed vendors' IoT solutions and RTOSes.
%That is because i) modern embedded systems are network facing and transfer data via wireless communication technology (e.g., Bluetooth, WiFi), which is the most frequently accessed vector by attackers;
%ii) most vendors and RTOSes implement their own communication component to meet different communication requirements. 


%By analyzing our CVE databases, we found most issues come from the wireless communication implementation.
%software implementation causes a lot of vulnerabilities.
%Since embedded devices are used for a variety purpose, 
%This section presents the security issues for existing software systems on Cortex-M processors.
%Following the taxonomy in~\cite{cerdeira2020sok}, those reports are categorized into validation, functional, and extrinsic bugs.
%besides the two known cache side-channel vulnerabilities and one architectural bug, most vulnerabilities are software implementation issues. 
% software implementation introduces the largest number of CVEs with various types.

%That is because IoT devices are network-connected with specifically designed network protocols.
%The vulnerabilities of those protocols leak sensitive information or even allow execution attacks and can influence different versions of software systems.
%For example, the TLS and CoAP library of Mbed and the middleware TCP/IP component of FreeRTOS have buffer overflow and integer overflow vulnerabilities.

%Those CVEs are scored based on their impact on devices ranging from low to critical.
%Over a seventy percent of those vulnerabilities are high or critical, which means they have a severe influence on a large number of devices.

%To have a better understanding of the secure state of software systems for Cortex-M processors, as Table~\ref{tab:sw-CVEs} shows, we manually analyzed bug reports from the CVE database~\cite{mitrecve} that related to some RTOSes and libraries.
%Then those vulnerabilities are categorized based on the different layers.

% Attacks: Smart nest thermostat (blackhat)~\cite{hernandez2014smart},

% \subsubsection{Improper validation of inputs and outputs}

\begin{table*}[!ht]
	\center
	\scriptsize
	\caption{Distribution of Cortex-M software CVEs in different classes}
	\vspace{0.1cm}
	\setlength\tabcolsep{0.8ex}
	\renewcommand{\arraystretch}{1}
	\rowcolors{2}{gray!15}{white}
	\label{tab:CVEs-con}	
	\begin{tabular}{l|l|l|l|l|cc}
		\hline
		\rowcolor{white}
		Bug Class         & Functions & Affected HW Vendors' SDKs  & Affected RTOSs & Affected TLS libs & \multicolumn{2}{c}{\#Bugs}        \\ \hline \hline
		\cellcolor{white} & Communication      & \begin{tabular}[c]{@{}l@{}}\cellcolor{white}NXP (2), Microchip (3), ST (1), TI (2),\\Cypress (8), Silicon Libs (5), Nordic (3)\end{tabular} & \begin{tabular}[c]{@{}l@{}}\cellcolor{white}FreeRTOS (11), RIOT-OS (12), Mbed OS (7),\\Zephyr (20), Contiki-ng (29)\end{tabular} & Mbed TLS (15), wolfSSL (22) & 142 & 49.65\%  \\
		\cellcolor{white} & Device Driver               & NXP (4), ST (5)                                               & Zephyr (5), Azure (5)                                                &- & 19 & 6.64\%  \\
		\cellcolor{white} & Memory Allocation   & NXP  (1)                                                      & \begin{tabular}[c]{@{}l@{}}\cellcolor{white}FreeRTOS (3), RIOT-OS (1), Mbed OS (2),\\CMSIS RTOS2 (1), Zephyr (1)\end{tabular}  & - & 9 & 3.15\%   \\
		\cellcolor{white} & Context Switch              & TF-M (1)                                                      & Zephyr (4)                                                        &  -  & 5 & 1.75\%   \\
		\multirow{-7}{*}{\cellcolor{white}Validation} & Others      & NXP (1), TF-M (1), Microchip (1)                              & RIOT-OS (4), Contiki-ng (7), Zephy (5)                             &  - & 19 & 6.64\% \\ \hline
		\cellcolor{white} & Protocol Implementation     &
		\begin{tabular}[c]{@{}l@{}}\cellcolor{gray!15}ST (2), Microchip (2), TI (8), Cypress (2),\\Silicon Labs (1) \end{tabular}
		& \begin{tabular}[c]{@{}l@{}}\cellcolor{gray!15}FreeRTOS (3), RIOT-OS (4), Zephyr (15),\\Mbed OS (1)\end{tabular} & Mbed TLS (7), wolfSSL (14) & 61 & 21.32\% \\
		\cellcolor{white} & Memory Access Control      & TF-M (1)   & FreeRTOS (2), Zephyr (4), Contiki-ng (1)                                             &- & 8 & 2.80\%   \\
		\multirow{-4}{*}{\cellcolor{white}Functional} & Cryptography Primitive         & TF-M (1)                                                       & RIOT-OS (2), Zephyr (1)                               & - & 4 &1.40\%    \\ \hline
		\cellcolor{white}Extrinsic & Software Side-Channel      & Microchip (1), ST (2)                                         & -                                                                     & Mbed TLS (9), wolfSSL (7) &  19 &6.64\%    \\ \hline
		%Total & - & 57 & 135 & 75 & 266\\ \hline
	\end{tabular}
	\vspace{-0.3cm}
\end{table*}

\begin{comment}
\subsubsection{Memory Safety bugs}
Memory is safe if and only if the pointer in the program access their intended referents.
Accessing a memory that is out of bound or accessing a referent that is no longer valid will trigger memory corruptions.
Those bugs can be the most severe security problems that are frequently used for privilege escalation, arbitrary code execution, information leakage, etc.

% Validation bugs are triggered because the input and/or output values are not handled properly in systems.
% Including buffer overflows, improper parameter validation, integer overflows, etc.
% Those bugs are frequently used for 

\issue{Spatial safety bugs:} 
Accessing a memory that is out of bound constitutes spatial safety bugs.
Examples like Listing 1 from RIOT-OS (CVE-2021-27697) can copy arbitrary buffer length because it does not check the value of expected\_len, which controls the copy buffer size.
Or out-of-bounds write from Arm Mbed TLS (CVE-2018-0488) that allow attackers to execute arbitrary code, which may cause Denial-of-Service (DOS).
An out-of-bounds read on Mbed CoAP lib (CVE-2020-12886) causes a read outside of the intended boundary of the buffer to cause the information leakage.
Integer overflow (e.g. CVE-2020-10070 on Zephyr Project) also triggers bound errors.

\begin{lstlisting}[label={RIOTcve}, caption={Vulnerability in RIOT-OS~\cite{RIOToscve}. This piece of code utilize buffer copy without checking size of input: expected\_len. Loacated at RIOT/sys/net/gnrc/routing/rpl/gnrc\_rpl\_validation.c}, language=c] 
  case (GNRC_RPL_OPT_PAD1): 
    expected_len += 1; 
    opt = (gnrc_rpl_opt_t *)(((uint8_t *) opt) + 1); 
  continue;  
\end{lstlisting}

\issue{Temporal safety bugs:} 
Accessing a referent that is no longer valid triggers the temporal safety bugs.
Attackers may exploit such bugs to reuse and control the freed region.
For example, the use after free attack (e.g. CVE-2019-18178) that access a dangling pointer.
Dereferencing the null pointer from Zephyr Project (CVE-2018-1000800) will cause a CPU page fault, which allows the attacker to call vulnerable kernel APIs.

% \textbf{Bugs in libraries:}
% Mbed TLS and wolfSSL are lightweight and widely used for RTOSes to provide network communication along with security. 
% With the bug in those libraries, an attacker is able to crash the library services via DOS attack and steal the sensitive information.
% Mbed implements TLS and CoAP to help simply the developer's work.
% I00. \textbf{Vulnerable libraries: information leakage, buffer overflow:}

% \subsubsection{Access level}
% Vulnerabilities at access level break the access control, authentication, and authorization.

% \subsubsection{Use of Uninitialized Variables}

% \subsubsection{Pointer Type Errors}

\subsubsection{Use of Uninitialized Variables}
Variables should be initialized to have an indeterminate value.
The use of uninitialized variables results in undefined behavior.

\issue{Access uninitialized pointer:}
FreeRTOS frees an uninitialized pointer that can be utilized for remote code execution (CVE-2018-16522).
Zephyr Project can access uninitialized stack memory (CVE-2020-10060), which may cause a crash, DOS, or information leakage. 

% \begin{lstlisting}[label={FreeRTOScve}, caption={Access uninitialized pointer in FreeRTOS~\cite{RIOToscve}.}, language=c] 
%   /* Clean-up application protocol array*/
%   if(Null != pxContext->ppcAlpnProtocols)
%   {
%     for(ulprotocl = 0;
%         ulProtocol < pxContext->ulAlpnProtocolsCount;
%         ulProtocol++)
%         {
%           if(NULL != pxContext->ppcAlpnProtocols[ulProtocl])
%           {
%             vPortFree(pxContext->ppcAlpnProtocols[ulProtocol]);
%           }
%         }
%         vPortFree(pxContext->ppcAlpnProtocols);
%   }
% \end{lstlisting}

\end{comment}

\subsection{Validation bugs}
Validation bugs refer to bugs that mishandle or improperly validate input and output data.
Examples are out-of-bounds read and write, improper parameter validation, etc.
They are frequently used for arbitrary write and read, allowing attackers to steal/overwrite sensitive information, execute remote code, or cause a denial of service.
%Validation bugs are further classified depends on different influenced system components.
%We list several bugs below to show the bugs exploited to attack those components.
%We analyzed bugs in different implementation components of production systems.
% Memory is safe if and only if the pointer in the program access their intended referents.
% Accessing a memory that is out of bound or accessing a referent that is no longer valid will trigger memory corruptions.
% Attackers may exploit such bugs to reuse and control the freed region.
% Validation bugs are triggered because the input and/or output values are not handled properly in systems.

\issue{Validation bugs in communication components:}
IoT systems are interconnected using the networking technologies, such as wireless communications.
%By exploiting a bug in communication component, attackers can easy access sensitive information or crash the system.
%Vendors and RTOS implement their own solutions to secure the communication, 
%Those vulnerabilities happen with wireless communication technologies, including Bluetooth low energy, network data parsing, etc.
% \issue{Spatial safety bugs:} 
%Bugs have been discovered in the libraries discussed \S\ref{sec:subsec:libandfirmware}.
%As discussed in , there are libraries for secure communication, which may introduce potential attack surface.
Table~\ref{tab:CVEs-con},
shows that 49.65\% of validation bugs affect communication stacks, e.g., Bluetooth and TCP/IP implementations.
For instance, 
%on vendors' SDKs, 
%including NXP, Microchip, TI, Cypress, and Silicon Labs, 
%have buffer overflow bugs that can trigger denial of services (CVE-2019-19195), 
%allow attackers execute arbitrary remote code (CVE-2018-16986), 
%pair any Bluetooth device (CVE-2019-18614), write arbitrary memory location (CVE-2019-13916), etc.
%Contiki-ng and Zephyr also has buggy Bluetooth implementation that can result in 
%arbitrary code execution (CVE-2020-12140), 
%mory corruption (CVE-2020-10061).
% and denial of services (CVE-2020-10069).
%Besides the Bluetooth, the TCP/IP stack implementation of FreeRTOS, DNS packets handling of FreeRTOS and Contiki-ng also introduce plenty of bugs (e.g., CVE-2021-21281, CVE-2018-16603).
FreeRTOS has a DNS poisoning bug that does not check if a DNS answer matches an outgoing query (CVE-2018-16598).
%To reduce the number of critical bugs, 
Some Cortex-M based systems use open-source libraries, such as Mbed TLS or WolfSSL, which also have validation bugs (39 bugs as of Nov. 2022).
%However, implementation bugs have been reported within the libraries themselves.
%We do not count those bugs in Table~\ref{tab:sum} and Table~\ref{tab:CVEs-con} since these libraries are also used in microprocessor-based systems. 
%, such as personal computers.
%The bug reports database show there are 34 for Mbed TLS and 52 for WolfSSL by the day we check. 


%Contiki-ng has a bug (CVE-2020-14935) to overwrite stack region, including the return address from the vulnerable function, which can redirect the code execution path.
%RIOT-OS (CVE-2021-27697) can copy arbitrary buffer length because it does not check the value of \verb|expected_len|, which controls the copy buffer size.
%The bug (CVE-2019-13120) in FreeRTOS allows attacker to read arbitrary memory when interacting a malformed MQTT publish packet from the attacker.
%RIOT-OS has a buffer overflow bug in its DNS protocol implementation (CVE-2019-1000006).
%FreeRTOS frees an uninitialized pointer in the socket function (CVE-2018-16522).
%Both vulnerabilities can lead to remote code execution.
% Meneghello et al.~\cite{meneghello2019iot} analyzed the security vulnerabilities on real world protocols.
%FreeRTOS also has a bugger overflow bug (CVE-2018-16525) when parsing the DNS/LLVMNR packets that can allow attackers to execute arbitrary code.
%Contiki-NG's SMTP implementation has buffer overflow bugs that can be exploited to overwrite sensitive data (CVE-2020-14934) and hijack control flow (CVE-2020-14935).
%The bluetooth implementation of Cypress WICED BT stack~\cite{WICED} does not restrict link-layer data length on reception~\cite{garbelini2021braktooth}. 
%Zephyr's LwM2M implementation has an infinite loop with malformed input (CVE-2020-13602). 
%Both bugs can cause a denial of service.
%Integer overflow (e.g. CVE-2020-10070 on Zephyr Project) also triggers bound errors.
%FreeRTOS has the integer overflow for a stream buffer (CVE-2021-31572).

\begin{comment}
Listing 1 from RIOT-OS (CVE-2021-27697) can copy arbitrary buffer length because it does not check the value of expected\_len, which controls the copy buffer size.
\begin{lstlisting}[label={RIOTcve}, caption={Vulnerability in RIOT-OS~\cite{RIOToscve}. This piece of code utilize buffer copy without checking size of input: expected\_len. Loacated at RIOT/sys/net/gnrc/routing/rpl/gnrc\_rpl\_validation.c}, language=c] 
  case (GNRC_RPL_OPT_PAD1): 
    expected_len += 1; 
    opt = (gnrc_rpl_opt_t *)(((uint8_t *) opt) + 1); 
  continue;  
\end{lstlisting}
\end{comment}

% ZigBee, Bluetooth Low Energy (BLE), 6LoWPAN and Constrained Application Protocol (CoAP), LoRaWAN.
% \textcolor{blue}{TODO: more details}
% RIOT, Keil RTX, Apache Mynewt, TI-RTOS support wolfSSL.

% \issue{Memory safety bugs within the protocols:}

\issue{Validation bugs in device drivers:}
%Besides wireless communication, 
Device drivers are exposed to attackers through physically-accessible peripherals, e.g., the USB interface.
%Different from bugs in communication component, attackers need physical access to exploit such bugs, and can even bypass hardware protections.
We found 19 bugs that affect two hardware vendors and two RTOSs in this category.
For instance, 
%There are several bug reports corresponding to validation in device drivers.
the buffer overread bug of the NXP Kinetis K82 USB driver can be leveraged to access the flash (CVE-2021-44479).
The USB driver in the Zephyr also has a buffer overflow bug that allows a USB-connected host to cause possible remote code execution (CVE-2020-10019). 
%The USB driver in the ST SDK does not validate message headers, which can lead to 
%denial of services (CVE-2021-34268), and 
%arbitrary code execution (CVE-2021-34262).

\issue{Validation bugs in dynamic memory allocations:}
%To handle different memory requirements on different devices, 
Embedded systems commonly implement custom allocators rather than using the standard heap implementations in the Libc~\cite{gritti2022heapster}.
%The valuable dynamic allocator implementation 
%Vulnerable heap implementation: HEAPSTER identifies the heap implementation of current Cortex-M software systems. 
Bugs in heap management can result in a system crash or arbitrary code execution.
%Zephyr
For example,
%FreeRTOS has insufficient bounds checking in its malloc function (CVE-2021-32020).
NXP's SDK, RIOT-OS, Mbed OS, and CMSIS RTOS are vulnerable to integer overflows in their allocator functions~\cite{integercve}.

\issue{Validation bugs in context switch components:}
%For some embedded systems that provide system services need to properly handle the context switch.
Bugs in these components have been exploited for privilege escalation.
%that separate privileges and the handling of different tasks is important to secure the system isolation.
Zephyr uses signed integer comparison to validate the syscall number, so a negative number leads to privilege escalation (CVE-2020-10027).
%Zephyr can elevate privilege when validating syscall numbers with signed integer comparison.
%Zephyr also has a NULL base pointer reference vulnerability in its privileged buffer handling functions, %(CVE-2018-1000800)
%namely \verb|sys_ring_buf_put| and \verb|sys_ring_buf_get|, which can result in memory fault at the privileged level.
TF-M has a bug allowing for out-of-bounds write in an NSC function, 
%calling secure functions under the non-secure handler mode 
which can lead to data leakage from the secure state (CVE-2021-27562).

\issue{Validation bugs in other components:}
As discussed in~\ref{No or weak privilege separation:},
many systems execute entirely at the privileged level, and bugs in any component could lead to severe consequences.
%There are other kernel libraries that may crash the system, which are specific for devices or embedded systems.
%This vulnerability can be exploited by malicious applications that trigger such buggy functions.
For example, a buffer overflow in FreeRTOS' shell implementation can cause privileged code execution (CVE-2020-10023).
The flash-related functions of Microchip's SDK have integer overflows that can be leveraged to access flash memory (CVE-2019-16127).
%TF-M has a bug (CVE-2021-43619) that can overwrite stack memory via the \verb|psa_fwu_write| caller.

% https://github.com/FreeRTOS/FreeRTOS-Kernel/commit/c7a9a01c94987082b223d3e59969ede64363da63


% \begin{lstlisting}[label={FreeRTOScve}, caption={DNS poisoning on FreeRTOS~\cite{RIOToscve}.}, language=c] 
%   /* Socket listen to the target port */
%   #if(ipconfigUSE_DNS == 1)
%   {
%     if(FreeRIOT_ntoms(pxUDPPacket->xUDPHeader.usSourcePort) == ipDNS_PORT)
%     {
%       vARPRefreshCacheEntry(&(pxUDPPacket->xEthernetHeader.xSourceAddress), pxUDPPacket->xIPHeader.ulSourceIPAddress);
%       xReturn = (Basetype_t)ulDNSHandlePacket(pxNetworkBuffer);
%     }
%   }
%   else ...
%   #endif
%   uint32_t ulDNSHandlePacket(NetworkBufferDescriptor_t *pxNetworkBuffer){
%     uint8_t *pucUDPPayloadBuffer = pxNetworkBuffer->pucEthernetBuffer + sizeof(UDPPacket_t);
%     DNSMessage_t *pxDNSMessageHeader = (DNSMessage_t *) pucUDPPayloadBuffer;
%     prvParseDNSReply(pucUDPPayloadBuffer, (uint32_t) pxDNSMessageHeader->usIdentifier);
%     return pdFAIL;
%   }
% \end{lstlisting}

% inadequate encryption strength 


% \textbf{Bugs in libraries:}
% Mbed TLS and wolfSSL are lightweight and widely used for RTOSes to provide network communication along with security. 
% With the bug in those libraries, an attacker is able to crash the library services via DOS attack and steal the sensitive information.

\subsection{Functional bugs}
Functional bugs 
%are not introduced by validating input or output, but
refer to programming errors that do not correctly implement the intended design.
%We identified three types of functional bugs that will break the functionalities of discussed components and lead to security vulnerabilities.
%because the programmer's implementation does not follow the program specification.
%Functional bugs will break the authentication that checks the rights of the code to access the resources, compromise the anonymity that unauthorized users can not read the information, or crash the system.  

\issue{Functional bugs in protocol implementations:}
%Some functional bugs may break the protocol functionality that crash the system or leak information.
21.32\% of the functional bugs are related to protocol implementations.
%This category targets wireless communication components and focuses on the bugs caused by implementation logistic, showing 18.13\% in .
%When analyzing the bug reports, those are cumbersome
%Similar to the 
For instance,
%a bug report (CVE-2021-3455) for Zephyr involves a use after free vulnerabilities which leads to device freeze.
% if disconnecting the L2CAP channel right after an invalid ATT request.
the Bluetooth controller in the Cypress SDK uses
a much shorter random number (than 128 bits) as the paring number, allowing the brute force of the random number to perform a man-in-the-middle attack during BLE pairing (CVE-2020-11957).
%Some bugs in the system kernel will elevate its privileges or break the system's functionality.

\issue{Functional bugs in memory access control:}
%Some systems provide MPU and TrustZone assisted isolation and allow calls between different privilege levels and secure states.
%hardware assisted isolation via MPU or TrustZone, etc
Incorrect memory access control configurations, including MPU- and TrustZone-based, sabotage the intended isolation.
We found eight bugs affecting one hardware vendor and two RTOSs in this category.
For example, FreeRTOS has a bug that allows unprivileged code to call 
%the \verb|xPortRaisePrivilege| and \verb|vPortResetPrivilege| 
the functions that set privilege (CVE-2021-43997). %, which causes privilege escalation.
% or sensitive information leakage.
%when calling non-secure callable function because unnecessary resources frees . [PLEASE rewrite the TF-M part. Not understandable.]
%TockOS's unprivileged capsule is able to access arbitrary memory (CVE-2018-1000660).
%The bug of Zephyr allows any thread running on the system read and write a socket file descriptor (CVE-2020-10072).
%FreeRTOS MPU platform does not prevent non-kernel code from calling privileged functions to escalate privilege (CVE-2021-43997).
%Besides the memory protection via privilege separation, the file system also faces the risk that the data may be modified.
%For instance, 
%FreeRTOS FAT file system implementation has use after free bug of it (CVE-2019-18178) results in random content written to disk by flushing cache operation.

%[Didn't we say change the title here? security mechanisms are too broad.]
\issue{Functional bugs in cryptography primitives:}
%Embedded systems implement several security mechanisms, such as cryptography primitives.
%Another potential source of vulnerabilities.
We found four bug reports in this category. %the insufficient of those mechanisms.
For instance,
RIOT-OS has a nonce reuse bug in its encryption function (CVE-2021-41061), and
TF-M has a functional bug when cleaning up the memory allocated for a multi-part cryptographic operation, resulting in
a memory leak 
%in its cryptographic library 
(CVE-2021-32032).
%\gl{I view CVE-2021-32032 as a validation bug.[handled]
%I'd put CVE-2020-11957 in crypto since it is related to crytpo protocol [The vulnerable function is to generate the Bluetooth pairing key, which belongs to wireless communication, not the crypto key.]
%}
%that cleans up the crypto context ahead of the lower level clean function, 
%then the latter function cannot locate and free memory, or will access an invalid memory region,
%resulting in system halt or secure data leakage (CVE-2021-32032).
%Zephyr does not check the existing bond with the same identify address during keys distribution phase, resulting possibility to overwrite an existing bond to cause device disconnection (CVE-2021-3436).
%RIOT-OS gnrc\_tcp implementation has infinite loop (CVE-2019-15702).
% TockOS contains an insecure permissions vulnerability in function \verb|get_package_name| in the file \verb|kernel/src/tbfheader.rs|, variable "pub package_name: &'static str," in the file process.rs that can result in A tock capsule (untrusted driver) could access arbitrary memory by using only safe code. This vulnerability appears to have been fixed in commit 42f7f36e74088036068d62253e1d8fb26605feed.
% For those RTOSes who separate the privilege, with improper privilege management, unprivileged users can recover the plaintext of RSA (Mbed TLS: CVE-2018-19608) via the man-in-the-middle attack.


\subsection{Extrinsic bugs}
Extrinsic bugs refer to defects that do not belong to validation bugs nor functional errors, for example,
the improper handling of external factors.
%triggered by possible external factors that the system handles properly.
% They are triggered by the proper handling of external factors that may cause vulnerabilities.
% We categorize them into two classes following with~\cite{cerdeira2020sok}.

\issue{Software side-channels:}
% Not related with validation of values or functional correctness of code, but with the proper handling of external factors that might introduce security vulnerabilities.
%The program execution can disclosure undesired information because of the specific implementation components, which are usually encryption units, by analyzing side signals, such as execution time.
%Some cryptography library implementations subject to timing side-channel attacks.
The implementations of PKCS \#1 v1.5 padding for RSA in the ST (CVE-2020-20949) and Microchip (CVE-2020-20950) SDKs are vulnerable to Bleichenbacher attack~\cite{bleichenbacher1998chosen}, a timing side-channel attack that 
%~\cite{timingRSA}
% This attack 
allows one to decrypt a ciphertext by making successive queries to the server with the vulnerable library and measuring the server's response time. %, resulting in remote information disclosure.
%Mbed TLS was subject to a lucky thirteen timing side-channel attack~\cite{al2013lucky}, which may recover the secret key in CBC mode because the computing time depends on the padding length (CVE-2020-16150).
%The ECC multiplication function in WolfSSL is also vulnerable to this attack, which discloses the private key (CVE-2020-11713).
%WolfSSL mishandles signature generation, which leads to fault injection in RSA cryptography (CVE-2019-19962).
%???Man in the middle attack. CVE-2020-10059.
%Zephyr uses a risky crypto algorithm that does not prevent attackers from influencing the key length (CVE-2019-9506), allowing practical brute-force attacks to decrypt the traffic and inject ciphertext.

%software developers can place a special value \verb|0xFEF5EDA5| above the stack space at reset handle.

% Another cache-based side-channel attack in the Mbed TLS can obtain an RSA private key (CVE-2020-10941).
% For example, the attacker can recover the ECDSA private key with side-channel measurements.
% with precise enough side-channel measurements, the attacker can recover the ECDSA private key (CVE-2020-10932).
% Mbed TLS, side-channel attacks to gain the secret key information: timing based, cache based, etc.
% \textit{Attacks on firmware: }
% Microcontroller's firmware protection vulnerabilities~\cite{206148}.

\begin{comment}
%[Still do not see how the example is related to physical side channel]
\issue{Bugs through physical accesses:}
By leveraging physical access targets, such as a debug interface, one can launch more powerful attackers that even bypass the hardware protection, as discussed in \ref{Bypassable vendor-specific readback protection:}.
%The physical subjects include debug interface and power pin.
%Besides the software side-channels, an attacker who have physical access to the devices can also break the protection of systems.
%It is different from the device drivers that need to connect the device, 
%Bugs in physical side-channels can happen because of not permanently disabling the debug interface.
A bug was reported on Gigadevice that allows attackers who have the debug access to redirect the vector table offset register to execute their own code.
That is because the debugger can write arbitrary flash memory dumping firmware into the SRAM and change the processor's registers~\cite{obermaier2020one}.
%CVE-2020-13465
% extract firmware (CVE-2020-13469), or de-obfuscate the observed data.
%Even if the system restricts flash access by a debugger, STM32L4 device have a bug that the attacker can degrade the access level to access flash by injecting a glitch and power consumption analysis during the boot phase~\cite{schink2021security}.


% (CVE-2020-27212)

%The debug interface may also trigger race condition as documented in CVE-2017-18347 for STMicroelectronics STM32F0 device.
%The race condition happens between the full initialization of the SWD interface and the setup of flash protection, which allows attackers to extract the device's protected firmware.
\end{comment}

\begin{mdframed}[style=remarkstyle,backgroundcolor=blue!10]
\textbf{Key Findings:} 
Most Cortex-M based production systems, e.g., bare-metal firmware and RTOSs, are written in memory-unsafe languages, e.g., C/C++,
and the number of discovered bugs shows a growing trend in the last several years.
%, increasing the risk of introducing memory corruption bugs.
% whose lack of safety leads to memory corruption bugs.
% Besides that, 
%Furthermore, programming errors and extrinsic bugs also present additional challenges to the security of real-world Cortex-M systems.
%Real-world Cortex-M based systems suffer from all kinds of intended (e.g., attacker-manipulated inputs) and unintended (e.g., programming errors) implementation bugs, of which most are input validation bugs.
%Securing those systems requires not only a security design but also correct implementations.
\end{mdframed}

%\issue{Concurrency bugs: }
%There are other denial of service attacks triggered by multiple concurrent operations.

%Such bugs are caused by multiple concurrent operations.
% For example, there is a privilege elevation attack on Zephyr project (CVE-2020-10058) because of the insufficient argument validation when multiple syscalls happens in the keyboard scan subsystem. 
%Zephyr suffers from a DoS attack when receiving certain duplicate and back-to-back packets in the Bluetooth subsystem (CVE-2020-10068).
% PASAN: Detecting Peripheral Access Concurrency Bugs within Bare-Metal Embedded Applications~\cite{272140}


% I00. \textbf{Bugs in memory protection:}
% Wrong memory configurations.
% I00. \textbf{Bugs in configuration of peripherals:}

% \textbf{I00. Bugs in security mechanisms:}
% Bugs in the implementation of security algorithms.


% \subsection{Hardware Issues}

% \textbf{I00. Attacks through reconfigurable hardware components:}
% [???]

% \textbf{I00. Attacks through energy management mechanisms:}
% [need to test]

% \subsubsection{Microarchitectural Side-Channels}

% \textbf{I00. Leaking information through caches:}
% [need to test]

% \textbf{I00. Leaking information through branch predictor:}
% [need to test]

% \textbf{I00. Leaking information using Rowhammer:}
% [need to test]

% \subsection{Implementation issues} 

% Find vulnerabilities of Cortex-M; CVEs

% Mbed is an open source OS and development tool for IoT devices.
% Table \ref{tab:CVEs} shows all the vulnerabilities (total 26 by 12/03/2020) reported for Mbed, most of them are related to Mbed TLS library. 

==> table.tex <==
\begin{table*}[!ht]
	\center
	\scriptsize
	\caption{Comparative evaluation of system isolation and attack mitigation projects for Cortex-M (\S\ref{subsec:Privilege_Separation_and_Compartment} - \S\ref{subsec:firmware-update}). The first column of the table lists the major defense mechanism proposed or adopted in a project.}
	%\vspace{-0.2cm}
	\label{tab:vs-proj}
	\setlength\tabcolsep{0.43ex}
	%\renewcommand{\arraystretch}{1}
	\rowcolors{2}{white}{gray!15}
	\begin{threeparttable}
		\begin{tabular}{l|l|c|l|ccc|cccccc|cccccc|cc|c|ccccc|ccc|cc|ccccc}
			\hline
			\rowcolor{white}
			\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{}&\multicolumn{3}{c}{}&\multicolumn{15}{c}{Defenses}&\multicolumn{5}{c}{Hardware}&\multicolumn{10}{c}{Self-reported average or worst case overhead (\%)} \\\hline
			\rowcolor{white}
			\multicolumn{1}{c|}{\rotatebox{90}{}}                                                                                             & \multicolumn{1}{l|}{Project}                                  & {Year} & \multicolumn{1}{l|}{Venue} & \rotatebox{90}{Input (S: source code; B: binary)} & \rotatebox{90}{Target (B: bare-metal; R: RTOS)} & \rotatebox{90}{Prototype Implementation (ISA)} & \rotatebox{90}{Privilege Separation} & \rotatebox{90}{Compartmentalization} & \rotatebox{90}{DMA-enabled Compartmentalization} & \rotatebox{90}{Software-based Virtualization} & \rotatebox{90}{TrustZone-based Virtualization} & \multicolumn{1}{c}{\rotatebox{90}{TrustZone-assisted Dual/Multi-world}}        & \rotatebox{90}{Shadow Stack} & \rotatebox{90}{Return Address Integrity} & \rotatebox{90}{Forward-edge Control Flow Integrity} & \rotatebox{90}{Compiler-based Software Diversity} & \rotatebox{90}{Address Space Layout Randomization} & \multicolumn{1}{c}{\rotatebox{90}{ROP Gadget Removal (\ref{ROP gadget removal:})}} & \rotatebox{90}{Software-based Execute Only Memory} & \multicolumn{1}{c}{\rotatebox{90}{SW-based Control-flow and Data Attes.}}  & \rotatebox{90}{Firmware Update} & \rotatebox{90}{MPU} & \rotatebox{90}{Unprivileged Store/Load Instructions} & \rotatebox{90}{TrustZone} & \rotatebox{90}{DWT} & \rotatebox{90}{FPB} & \rotatebox{90}{Code, Binary Size Increasement} & \rotatebox{90}{Memory Overhead} & \multicolumn{1}{c}{\rotatebox{90}{Energy Consumption Overhead}} & \rotatebox{90}{Bare-metal Applications} & \multicolumn{1}{c}{\rotatebox{90}{RTOSs}} & \rotatebox{90}{BEEBS~\cite{pallister2013beebs}}   & \rotatebox{90}{CoreMark~\cite{coremark2021}} & \rotatebox{90}{CoreMark-Pro~\cite{coremarkpro2021}} & \rotatebox{90}{Dhrystone~\cite{weicker1984dhrystone}} & \rotatebox{90}{Embench~\cite{embench}} \\ \hline \hline
			\cellcolor{white}                                                                                                                 & SAFER SLOTH~\cite{danner2014safer}                            & 2014   & RTAS                       & S                                                 & R                                               & v7                                             & \supportlevel{10}                    &                                      &                                                  &                                               &                                                &                                                                                &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 & \supportlevel{10}   &                                                      &                           &                     &                     & \cellcolor{white}                              & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{white}                       & \cellcolor{deepred}{$>$100}               & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\
			\multirow{-2}{*}{\cellcolor{white}\ref{Privilege separation:}}\tikzmark{d01}                                                      & EPOXY~\cite{clements2017EPOXY}                                & 2017   & S\&P                       & S                                                 & B                                               & v7                                             & \supportlevel{10}                    &                                      &                                                  &                                               &                                                &                                                                                &                              &                                          &                                                     & \supportlevel{10}                                 &                                                    &                                                                                    &                                                    &                                                                            &                                 & \supportlevel{10}   &                                                      &                           &                     &                     & \cellcolor{red}{29}                            & \cellcolor{red}{29}             & \cellcolor{lightgreen}{2.6}                                     & \cellcolor{lightgreen}{2.4}             & \cellcolor{white}                         & \cellcolor{lightgreen}{1.6}                       & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\ \hline
			\cellcolor{white}                                                                                                                 & uSFI~\cite{aweke2018usfi}                                     & 2018   & DATE                       & S                                                 & R                                               & v7                                             & \supportlevel{10}                    & \supportlevel{10}                    &                                                  &                                               &                                                &                                                                                & \supportlevel{5}             &                                          & \supportlevel{10}                                   &                                                   &                                                    & \supportlevel{10}                                                                  &                                                    &                                                                            &                                 & \supportlevel{10}   & \supportlevel{10}                                    &                           &                     &                     & \cellcolor{lightred}{10}                       & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{white}                       & \cellcolor{green}{1.1}                    & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\
			\cellcolor{white}\tikzmark{d02i}                                                                                                  & ACES~\cite{clements2018aces}                                  & 2018   & USENIX                     & S                                                 & B                                               & v7                                             & \supportlevel{10}                    & \supportlevel{10}                    &                                                  &                                               &                                                &                                                                                & \supportlevel{5}             &                                          & \supportlevel{10}                                   &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 & \supportlevel{10}   &                                                      &                           &                     &                     & \cellcolor{red}{70}                            & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{lightred}{13}                & \cellcolor{white}                         & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\
			\multirow{-3}{*}{\cellcolor{white}\ref{Compartmentalization with heavy context switches:}}\tikzmark{d02o}                         & MINION~\cite{kim2018securing}                                 & 2018   & NDSS                       & S                                                 & R                                               & v7                                             & \supportlevel{10}                    & \supportlevel{10}                    &                                                  &                                               &                                                &                                                                                & \supportlevel{5}             &                                          & \supportlevel{10}                                   &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 & \supportlevel{10}   &                                                      &                           &                     &                     & \cellcolor{green}{-71.3}                       & \cellcolor{green}{-98.86}       & \cellcolor{white}                                               & \cellcolor{white}                       & \cellcolor{lightgreen}{6.13}              & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\ \hline
			\cellcolor{white}                                                                                                                 & OPEC~\cite{zhou2022opec}                                      & 2022   & EuroSys                    & S                                                 & B                                               & v7                                             & \supportlevel{10}                    & \supportlevel{10}                    &                                                  &                                               &                                                &                                                                                &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 & \supportlevel{10}   &                                                      &                           &                     &                     & \cellcolor{lightgreen}{1.79}                   & \cellcolor{lightgreen}{5.53}    & \cellcolor{white}                                               & \cellcolor{green}{.23}                  & \cellcolor{white}{}                       & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\
			\cellcolor{white}\tikzmark{d03i}                                                                                                  & EC~\cite{khan2023ec}                                          & 2023   & S\&P                       & S                                                 & B/R                                             & v7                                             & \supportlevel{10}                    & \supportlevel{10}                    &                                                  &                                               &                                                &                                                                                &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 & \supportlevel{10}   &                                                      &                           & \supportlevel{10}   &                     & \cellcolor{white}                              & \cellcolor{lightgreen}{2.57}    & \cellcolor{white}                                               & \cellcolor{white}{}                     & \cellcolor{white}{}                       & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\
			\multirow{-3}{*}{\cellcolor{white}\ref{Compartmentalization with reduced context switches:}}\tikzmark{d03o}                       & CRT-C~\cite{khan2023low}                                      & 2023   & S\&P                       & S                                                 & R                                               & v7                                             &                                      & \supportlevel{10}                    &                                                  &                                               &                                                &                                                                                &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 &                     &                                                      &                           &                     &                     & \cellcolor{white}                              & \cellcolor{lightgreen}{1.75}    & \cellcolor{white}                                               & \cellcolor{white}                       & \cellcolor{lightgreen}{2.63}              & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\ \hline
			\multirow{1}{*}{\cellcolor{white}\tikzmark{d04i}\ref{DMA-enabled compartmentalization:}}\tikzmark{d04o}                           & D-Box~\cite{mera2022d}                                        & 2022   & NDSS                       & S                                                 & R                                               & v7                                             & \supportlevel{10}                    &                                      & \supportlevel{10}                                &                                               &                                                &                                                                                &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 & \supportlevel{10}   &                                                      &                           &                     &                     & \cellcolor{green}{-.12}                        & \cellcolor{green}{-.07}         & \cellcolor{green}{-18.2}                                        & \cellcolor{white}                       & \cellcolor{lightgreen}{2}                 & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\ \hline \hline
			\cellcolor{white}\tikzmark{d05i}                                                                                                  & Hermes~\cite{klingensmith2018hermes}                          & 2018   & MCSA                       & S                                                 & B/R                                             & v7                                             & \supportlevel{10}                    &                                      &                                                  & \supportlevel{10}                             &                                                &                                                                                &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 & \supportlevel{10}   &                                                      &                           &                     &                     & \cellcolor{white}                              & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{white}                       & \cellcolor{white}                         & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\
			\multirow{-2}{*}{\cellcolor{white}\ref{Software-based virtualization:}}\tikzmark{d05o}                                            & MultiZone~\cite{pinto2020multi}                               & 2020   & EW                         & B                                                 & B                                               & v7                                             & \supportlevel{10}                    &                                      &                                                  & \supportlevel{10}                             &                                                &                                                                                &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 & \supportlevel{10}   &                                                      &                           &                     &                     & \cellcolor{white}                              & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{green}{.01}                  & \cellcolor{white}                         & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\ \hline
			\cellcolor{white}\tikzmark{d06i}                                                                                                  & lLTZVisor~\cite{araujo2018lltzvisor, pinto2019virtualization} & 2018   & RTAS                       & S                                                 & B/R                                             & v8                                             & \supportlevel{10}                    &                                      &                                                  &                                               & \supportlevel{10}                              &                                                                                &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 &                     &                                                      & \supportlevel{10}         &                     &                     & \cellcolor{white}                              & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{white}                       & \cellcolor{green}{.6}                     & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\
			\multirow{-2}{*}{\cellcolor{white}\ref{TrustZone-based virtualization:}}\tikzmark{d06o}                                           & SBIs~\cite{pansbis2022}                                       & 2022   & RTAS                       & S                                                 & B/R                                             & v8                                             & \supportlevel{10}                    &                                      &                                                  &                                               & \supportlevel{10}                              &                                                                                &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 & \supportlevel{10}   &                                                      & \supportlevel{10}         &                     &                     & \cellcolor{white}                              & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{white}                       & \cellcolor{white}                         & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\ \hline
			\cellcolor{white}                                                                                                                 & RT-TEE~\cite{wang2022rt}                                      & 2022   & S\&P                       & S                                                 & R                                               & v8                                             & \supportlevel{10}                    &                                      &                                                  &                                               &                                                & \supportlevel{10}                                                              &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 &                     &                                                      & \supportlevel{10}         &                     &                     & \cellcolor{white}                              & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{white}                       & \cellcolor{white}                         & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\
			\multirow{-2}{*}{\cellcolor{white}\tikzmark{d07i}\ref{Real-time and secure TrustZone-assisted dual-world system:}}\tikzmark{d07o} & SafeTEE~\cite{schonstedt2022safetee}                          & 2022   & DATE                       & S                                                 & R                                               & v8                                             & \supportlevel{10}                    &                                      &                                                  &                                               &                                                & \supportlevel{10}                                                              &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 &                     &                                                      & \supportlevel{10}         &                     &                     & \cellcolor{white}                              & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{white}                       & \cellcolor{white}                         & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{lightgreen}{2.5}            \\ \hline
			\multirow{1}{*}{\cellcolor{white}\tikzmark{d08i}\ref{TrustZone-assisted multi-world system:}}\tikzmark{d08o}                      & uTango~\cite{oliveira2021utango}                              & 2022   & Access                     & B                                                 & B/R                                             & v8                                             &                                      &                                      &                                                  &                                               &                                                & \supportlevel{10}                                                              &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 & \supportlevel{10}   &                                                      & \supportlevel{10}         &                     &                     & \cellcolor{lightgreen}{4.6}                    & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{white}                       & \cellcolor{white}                         & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{green}{.05}                 \\ \hline
			\cellcolor{white}                                                                                                                 & Secure Informer~\cite{iannillo2022ree}                        & 2022   & CPSS                       & S                                                 & R                                               & v8                                             &                                      &                                      &                                                  &                                               &                                                & \supportlevel{10}                                                              &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 & \supportlevel{10}   &                                                      & \supportlevel{10}         &                     &                     & \cellcolor{green}{$<$.01}                      & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{white}                       & \cellcolor{lightgreen}{3.5}               & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\
			\multirow{-2}{*}{\cellcolor{white}\tikzmark{d09i}\ref{Secure cross-state communication:}}\tikzmark{d09o}                          & ShieLD~\cite{khurshid2022shield}                              & 2022   & TDSC                       & S                                                 & R                                               & v8                                             &                                      &                                      &                                                  &                                               &                                                & \supportlevel{10}                                                              &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 & \supportlevel{10}   &                                                      & \supportlevel{10}         &                     &                     & \cellcolor{green}{.04}                         & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{white}                       & \cellcolor{deepred}{2600}                 & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\ \hline \hline
			\cellcolor{white}                                                                                                                 & CaRE~\cite{nyman2017cfi}                                      & 2017   & RAID                       & B                                                 & B                                               & v8                                             &                                      &                                      &                                                  &                                               &                                                &                                                                                & \supportlevel{10}            &                                          & \supportlevel{10}                                   &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 & \supportlevel{10}   &                                                      & \supportlevel{10}         &                     &                     & \cellcolor{lightred}{14.5}                     & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{deepred}{369}                & \cellcolor{white}                         & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{deepred}{513}                              & \cellcolor{white}                      \\
			\cellcolor{white}                                                                                                                 & Silhouette~\cite{zhou2020silhouette}                          & 2020   & USENIX                     & S                                                 & B                                               & v7                                             &                                      &                                      &                                                  &                                               &                                                &                                                                                & \supportlevel{10}            &                                          & \supportlevel{10}                                   &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 & \supportlevel{10}   & \supportlevel{10}                                    &                           &                     &                     & \cellcolor{lightgreen}{8.9}                    & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{white}                       & \cellcolor{white}                         & \cellcolor{green}{3.4}                            & \cellcolor{white}                            & \cellcolor{green}{1.3}                              & \cellcolor{white}                                     & \cellcolor{white}                      \\
			& TZmCFI~\cite{kawada2020TZmCFI}                                & 2020   & IJPP                       & S                                                 & R                                               & v8                                             &                                      &                                      &                                                  &                                               &                                                &                                                                                & \supportlevel{10}            &                                          & \supportlevel{10}                                   &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 & \supportlevel{10}   &                                                      & \supportlevel{10}         &                     &                     & \cellcolor{white}                              & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{white}                       & \cellcolor{red}{84}                       & \cellcolor{white}                                 & \cellcolor{lightred}{14.14}                  & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\
			\multirow{-2}{*}{\cellcolor{white}\ref{Stack and return address integrity:}}
			\cellcolor{white}& Kage~\cite{du2022kage}                                        & 2022   & USENIX                     & S                                                 & R                                               & v7                                             &                                      &                                      &                                                  &                                               &                                                &                                                                                & \supportlevel{10}            &                                          & \supportlevel{10}                                   &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 & \supportlevel{10}   & \supportlevel{10}                                    &                           &                     &                     & \cellcolor{red}{49.8}                          & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{white}                       & \cellcolor{lightred}{5.2}                 & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\
			& SUM~\cite{choi2023sum}                           & 2023   & C\&S                       & S                                                 & B                                               & v7                                             &                                      &                                      &                                                  &                                               &                                                &                                                                                & \supportlevel{10} &                         &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 & \supportlevel{10}   &                                                      &                           &                     &                     & \cellcolor{lightgreen}{8.33}                          & \cellcolor{white}      & \cellcolor{white}                                               & \cellcolor{green}{2.77}                   & \cellcolor{green}{2.63}                         & \cellcolor{white}                                 & \cellcolor{white}                       & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\
			\cellcolor{white}                                                                                                                 & SHERLOC~\cite{tan2023sherloc}                                        & 2023   & CCS                     & S                                                 & B/R                                               & v8                                             &                                      &                                      &                                                  &                                               &                                                &                                                                                &             & \supportlevel{10}                                   & \supportlevel{10}                                   &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 &   &   &    \supportlevel{10}     &   \supportlevel{10}  &                     &   & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{deepred}{123}   & \cellcolor{deepred}{1106}                 & \cellcolor{white} \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\
			& $\mu$RAI~\cite{almakhdhubmurai2020}                           & 2020   & NDSS                       & S                                                 & B                                               & v7                                             &                                      &                                      &                                                  &                                               &                                                &                                                                                &                              & \supportlevel{10}                        &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 & \supportlevel{10}   &                                                      &                           &                     &                     & \cellcolor{red}{54.1}                          & \cellcolor{lightred}{15.2}      & \cellcolor{white}                                               & \cellcolor{green}{.1}                   & \cellcolor{white}                         & \cellcolor{white}                                 & \cellcolor{lightgreen}{8.1}                       & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\
			\multirow{-5}{*}{\cellcolor{white}\ref{Forward-edge control-flow integrity (CFI):}}\tikzmark{d10o}                                & RIO~\cite{kim2023rio}                           & 2023   & NDSS                       & S                                                 & B                                               & v8                                             &                                      &                                      &                                                  &                                               &                                                &                                                                                &                              & \supportlevel{10}                        &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 &    &                                                      & \supportlevel{10}   &                     &                     & \cellcolor{red}{29.9}                          & \cellcolor{white}      & \cellcolor{white}                                               & \cellcolor{lightred}{16.83}                   & \cellcolor{white}                         & \cellcolor{white}                                 & \cellcolor{white}                       & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\ \hline
			\multirow{1}{*}{\cellcolor{white}\tikzmark{d12i}\ref{Compiler-based software diversity:}}\tikzmark{d12o}                          & Randezvous~\cite{shen2022randezvous}                          & 2022   & EuroS\&P                  & S                                                 & B                                               & v7/8                                           &                                      &                                      &                                                  &                                               &                                                &                                                                                & \supportlevel{10}            &                                          &                                                     & \supportlevel{10}                                 &                                                    &                                                                                    & \supportlevel{10}                                  &                                                                            &                                 & \supportlevel{10}   &                                                      &                           &  \supportlevel{10}  &                     & \cellcolor{lightred}{13.6}                     & \cellcolor{red}{24.5}           & \cellcolor{white}                                               & \cellcolor{green}{0.6}                  & \cellcolor{white}                         & \cellcolor{lightgreen}{6.9}                       & \cellcolor{white}                            & \cellcolor{lightgreen}{7.0}                         & \cellcolor{white}                                     & \cellcolor{white}                      \\ \hline
			\cellcolor{white}                                                                                                                 & HARM~\cite{shi2022harm}                                       & 2022   & EuroS\&P                  & B                                                 & B/R                                             & v8                                             &                                      &                                      &                                                  &                                               &                                                &                                                                                &                              &                                          &                                                     &                                                   & \supportlevel{10}                                  &                                                                                    &                                                    &                                                                            &                                 & \supportlevel{10}   &                                                      & \supportlevel{10}         &                     &                     & \cellcolor{lightred}{15.49}                    & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{lightred}{5.8}               & \cellcolor{red}{21}                       & \cellcolor{red}{28}                               & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\
			\multirow{-2}{*}{\cellcolor{white}\tikzmark{d13i}\ref{Address space layout randomization (ASLR):}}\tikzmark{d13o}                 & fASLR~\cite{luo2022faslr,shao2022faslr}                       & 2022   & ESORICS                    & S                                                 & B                                               & v8                                             &                                      &                                      &                                                  &                                               &                                                &                                                                                &                              &                                          &                                                     &                                                   & \supportlevel{10}                                  &                                                                                    &                                                    &                                                                            &                                 & \supportlevel{10}   &                                                      & \supportlevel{10}         &                     &                     & \cellcolor{white}                              & \cellcolor{lightgreen}{4.73}    & \cellcolor{white}                                               & \cellcolor{lightred}{9.65}              & \cellcolor{white}                         & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\ \hline 
			\cellcolor{white}\tikzmark{d15i}\ref{Secure multiprogramming with memory-safe languages:}\tikzmark{d15o}                                         & Tock~\cite{levy2017multiprogramming}                          & 2017   & SOSP                       & S                                                 & R                                               & v7                                             & \supportlevel{10}                    &                                      &                                                  &                                               &                                                &                                                                                &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 & \supportlevel{10}   &                                                      &                           &                     &                     & \cellcolor{white}                              & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{white}                       & \cellcolor{white}                         & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\ \hline
			\ref{Formal verification:}                                         & Pip-MPU~\cite{dejon2023pip}                          & 2023   & IJESA                       & S                                                 & B/R                                               & v7/8                                             & \supportlevel{10}                    &                                      &                                                  &                                               &                                                &                                                                                &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            &                                 & \supportlevel{10}   &                                                      &                           &                     &                     & \cellcolor{white}                              & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{white}                       & \cellcolor{white}                         & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\ \hline \hline
			& uXOM~\cite{kwon2019uxom}                                      & 2019   & USENIX                     & S                                                 & R                                               & v7                                             &                                      &                                      &                                                  &                                               &                                                &                                                                                &                              &                                          &                                                     &                                                   &                                                    & \supportlevel{10}                                                                  & \supportlevel{10}                                  &                                                                            &                                 & \supportlevel{10}   & \supportlevel{10}                                    &                           &                     &                     & \cellcolor{lightred}{15.7}                     & \cellcolor{white}               & \cellcolor{lightred}{7.5}                                       & \cellcolor{white}                       & \cellcolor{white}                         & \cellcolor{red}{7.3}                              & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\
			\multirow{-2}{*}{\cellcolor{white}\tikzmark{d15i}\ref{Software-based XOM:}}\tikzmark{d15o}                                        & PicoXOM~\cite{shen2020fast}                                   & 2020   & SecDev                     & S                                                 & B/R                                             & v7                                             &                                      &                                      &                                                  &                                               &                                                &                                                                                &                              &                                          &                                                     &                                                   &                                                    &                                                                                    & \supportlevel{10}                                  &                                                                            &                                 & \supportlevel{10}   &                                                      &                           & \supportlevel{10}   &                     & \cellcolor{lightred}{5.89}                     & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{green}{.02}                  & \cellcolor{white}                         & \cellcolor{green}{0.46}                           & \cellcolor{white}                            & \cellcolor{green}{-.11}                             & \cellcolor{white}                                     & \cellcolor{white}                      \\ \hline \hline
			\cellcolor{white}                                                                                                                 & DIAT~\cite{abera2019diat}                                     & 2019   & NDSS                       & S                                                 & R                                               & v7                                             &                                      &                                      &                                                  &                                               &                                                &                                                                                &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    & \supportlevel{10}                                                          &                                 &                     &                                                      &                           &                     &                     & \cellcolor{white}                              & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{white}                       & \cellcolor{deepred}{400}                  & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\
			\cellcolor{white}                                                                                                                 & LAPE~\cite{huo2020lape}                                       & 2020   & HPCC                       & S                                                 & B                                               & v7                                             & \supportlevel{10}                    &                                      &                                                  &                                               &                                                &                                                                                &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    & \supportlevel{5}                                                           &                                 & \supportlevel{10}   &                                                      &                           &                     &                     & \cellcolor{red}{38}                            & \cellcolor{lightred}{8.2}       & \cellcolor{white}                                               & \cellcolor{lightgreen}{2.2}             & \cellcolor{white}                         & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\
			\cellcolor{white}                              & ISC-FLAT~\cite{neto2023isc}                                     & 2023   & RTAS                     & S                                                 & B                                               & v8                                             &                                      &                                      &                                                  &                                               &                                                &                                                                                &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    &  \supportlevel{10}                                                         &                                 & \supportlevel{10}   &                                                      & \supportlevel{10}         &                     &                     & \cellcolor{white}                              & \cellcolor{white}      & \cellcolor{lightred}{17.5}                                               & \cellcolor{red}{35.1}              & \cellcolor{white}                         & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\ 
			\multirow{-4}{*}{\cellcolor{white}\ref{Software-based control-flow and data integrity attestation:}}                              & ARI~\cite{wangari2023ari}                                     & 2023   & USENIX                     & S                                                 & R                                               & v7                                             &                                      &                                      &                                                  &                                               &                                                &                                                                                &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    &  \supportlevel{10}                                                         &                                 & \supportlevel{10}   &                                                      & \supportlevel{10}         &                     &                     & \cellcolor{white}                              & \cellcolor{lightred}{12.5}      & \cellcolor{white}                                               & \cellcolor{lightred}{10.7}              & \cellcolor{white}                         & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\
			\hline \hline
			& ASSURED~\cite{asokan2018assured}                              & 2018   & TCAD                       & B                                                 & R                                               & v8                                             &                                      &                                      &                                                  &                                               &                                                &                                                                                &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            & \supportlevel{10}               &                     &                                                      & \supportlevel{10}         &                     &                     & \cellcolor{red}{80}                            & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{white}                       & \cellcolor{white}                         & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\
			& DisPatch~\cite{kim2022reverse}                              & 2022   & MobiSys                       & B                                                 & R                                               & v7                                             &                                      &                                      &                                                  &                                               &                                                &                                                                                &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            & \supportlevel{10}               &                     &                                                      &        &                     &                     & \cellcolor{green}{.53}                            & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{white}                       & \cellcolor{green}{1.48}                         & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\
			\multirow{-3}{*}{\cellcolor{white}\ref{Secure software update:}\tikzmark{d17o}}                                                                    
			& Shimware~\cite{gustafson2023shimware}                              & 2023   & RAID                       & B                                                 & B/R                                               & v7                                             &                                      &                                      &                                                  &                                               &                                                &                                                                                &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            & \supportlevel{10}               &                     &                                                      &         &                     &                     & \cellcolor{white}                            & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{white}                       & \cellcolor{white}                         & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\
			\hline
			\cellcolor{white}                                                                                                                 & HERA~\cite{niesler2021hera}                                   & 2021   & NDSS                       & S                                                 & R                                               & v7                                             &                                      &                                      &                                                  &                                               &                                                &                                                                                &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            & \supportlevel{10}               &                     &                                                      &                           &                     & \supportlevel{10}   & \cellcolor{white}                              & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{white}                       & \cellcolor{white}                         & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\
			\multirow{-2}{*}{\cellcolor{white}\tikzmark{d18i}\ref{Firmware hotpatching:}}                                                     & RapidPatch~\cite{he2022rapidpatch}                            & 2022   & USENIX                     & S                                                 & B/R                                             & v7                                             &                                      &                                      &                                                  &                                               &                                                &                                                                                &                              &                                          &                                                     &                                                   &                                                    &                                                                                    &                                                    &                                                                            & \supportlevel{10}               &                     &                                                      &                           &                     & \supportlevel{10}   & \cellcolor{white}                              & \cellcolor{white}               & \cellcolor{white}                                               & \cellcolor{white}                       & \cellcolor{green}{1.5}               & \cellcolor{white}                                 & \cellcolor{white}                            & \cellcolor{white}                                   & \cellcolor{white}                                     & \cellcolor{white}                      \\ \hline
			%\cellcolor{white}&OAT~\cite{sun2020oat}&2020                 &C&B &A  &  &  &  &  &  &  &  &&  &  &\supportlevel{10}&  &  &   &\supportlevel{10}&\supportlevel{10} &  &  &  &\supportlevel{10}&  &  &\textcolor{darkblue}{13}&  &  &\textcolor{darkblue}{2.7}&  &  &  &  &  &  & \\ 
			%\cellcolor{white}&Pan et al.~\cite{pan2018predictable}&2018&C&R &v7 &  &  &  &\supportlevel{10}&  &  &  &  &  &  &  &  &  &  &  &  &\supportlevel{10}&  &  &  &  &  &  &  &  &&&  &  &  &  &  & \\
			%\cellcolor{white}&C-FLAT~\cite{abera2016c}&2016              &B&B &A  &  &  &  &  &  &&  &  &  &  &\supportlevel{10}&  &  &   &\supportlevel{10}&  &  &  &  &\supportlevel{10}&  &  &\textcolor{darkorange}{25}&  &  &\textcolor{darkorange}{76}&  &  &  &  &  &  &\\
			%VRASED~\cite{nunes2019vrased}         &C&B &*  &  &  &  &  &  &  &  &  &  &   &  &   &\supportlevel{10}&  &  &  &  &  &  &  &  &\supportlevel{10}&  &\textcolor{darkblue}{3.5}&  &  &  &  &  &  &  &  &\\ 
			%APEX~\cite{nunes2020apex}             &C&B &*  &  &  &  &  &  &  &  &  &  &   &  &   &  &\supportlevel{10}&  &  &  &  &  &  &  &\supportlevel{10}&  &\textcolor{darkgreen}{.01}&  &  &  &  &  &  &  &  &\\ 
			%Tiny-CFA~\cite{nunes2020tiny}          &B&B &*  &  &  &  &  &  &  &\supportlevel{10}&  &  &   &  &   &  &  &\supportlevel{10}&  &  &  &  &  &  &\supportlevel{10}&\textcolor{darkorange}{80}&  &  &\textcolor{darkorange}{50}& \\ 
			%DIALED~\cite{nunes2021dialed}         &B&B &*  &  &  &  &  &  &  &\supportlevel{10}&  &  &   &  &   &  &  &\supportlevel{10}&\supportlevel{10}&  &  &  &  &  &\supportlevel{10}&  &  &  &  &  &  &  &  &  &  &\\ \hline
		\end{tabular}
		\begin{tikzpicture}[overlay,remember picture]
			\draw[-{Classical TikZ Rightarrow[length=2.5pt]},line width=1pt, color=black] ($(pic cs:d01)+(-6pt,1ex)$) to ($(pic cs:d02i)+(6pt,1.8ex)$);
			\draw[-{Classical TikZ Rightarrow[length=2.5pt]},line width=1pt, color=black] ($(pic cs:d02o)+(-6pt,2.2ex)$) to ($(pic cs:d03i)+(6pt,2ex)$);
			\draw[-{Classical TikZ Rightarrow[length=2.5pt]},line width=1pt, color=black] ($(pic cs:d03o)+(-6pt,2.4ex)$) to ($(pic cs:d04i)+(6pt,1.6ex)$);
			\draw[-{Implies},double,line width=1pt, color=black] ($(pic cs:d04o)+(-6pt,-.2ex)$) to ($(pic cs:d05i)+(6pt,.5ex)$);
			\draw[-{Classical TikZ Rightarrow[length=2.5pt]},line width=1pt, color=black] ($(pic cs:d05o)+(-6pt,1.2ex)$) to ($(pic cs:d06i)+(6pt,0.6ex)$);
			\draw[-{Classical TikZ Rightarrow[length=2.5pt]},line width=1pt, color=black] ($(pic cs:d06o)+(-6pt,1.2ex)$) to ($(pic cs:d07i)+(6pt,2ex)$);
			\draw[-{Classical TikZ Rightarrow[length=2.5pt]},line width=1pt, color=black] ($(pic cs:d07o)+(-6pt,1.2ex)$) to ($(pic cs:d08i)+(6pt,1.6ex)$);
			%\draw[-stealth,double,line width=1pt, color=black] ($(pic cs:d07o)+(-6pt,-.2ex)$) to ($(pic cs:d08i)+(6pt,2ex)$);
			\draw[-{Classical TikZ Rightarrow[length=2.5pt]},line width=1pt, color=black] ($(pic cs:d10o)+(-6pt,3.6ex)$) to ($(pic cs:d12i)+(6pt,1.6ex)$);
			\draw[-{Classical TikZ Rightarrow[length=2.5pt]},line width=1pt, color=black] ($(pic cs:d12o)+(-6pt,-.2ex)$) to ($(pic cs:d13i)+(6pt,1.6ex)$);
			\draw[-{Implies},double,line width=1pt, color=black] ($(pic cs:d13o)+(-6pt,1ex)$) to ($(pic cs:d15i)+(6pt,8.6ex)$);
			\draw[-{Classical TikZ Rightarrow[length=2.5pt]},line width=1pt, color=black] ($(pic cs:d17o)+(-6pt,-.2ex)$) to ($(pic cs:d18i)+(6pt,2ex)$);
			
		\end{tikzpicture}
		\vspace{-0.3cm}
		\begin{tablenotes}
			\item[] 
			%USENIX: USENIX Security.
			%EW: Embedded World Conference.
			%IJPP: International Journal of Parallel Programming. 
			v7: Armv7-M, v8: Armv8-M. 
			\supportlevel{5}: Partially implementation of a security feature.
			\supportlevel{10}: Implement a security feature or need specific hardware support.
			\contour{black}{$\downarrow$} and \contour{black}{$\Downarrow$} represent small and big steps towards a similar goal, respectively. 
			%{\color{darkgreen} green}: $\le$1\% negligible overhead, {\color{darkblue} blue}: $<$20\% practical, {\color{darkorange} orange}: $<$100\% noticeable, {\color{darkred} red}: $>$100\% heavy overhead. 
			%*: $\mu$Visor is deprecated and being replaced by the secure partition manager after Mbed OS v5.10.
			% \item[] Code and memory overhead shows the best case, run-time overhead shows the worst case.
			% \item[]: Bare-metal only or RTOSes. Input - source code; binary. Developer involvement - None; annotation; code modification. . *: TI MSP430~\cite{MSP430}
		\end{tablenotes}
	\end{threeparttable}
	\vspace{-0.3cm}
\end{table*}

==> tests.tex <==
\section{Test Cases}

\subsection{Our Test Cases}

A table of all test cases and how they map to different sections in the paper.

\ziming{Where to output? only to LCD? some devices may not have LCD. Can we set to serial port/JTAG debug as well?}
To check the output from the debugging view (Keil IDE windows), we can use printf() via the ITM (debug and trace feature of Cortex-M, may need more description about ITM).
Some processors did not implement ITM, we can retargeting the I/O to UART, and use the series windows via serios port.
But the interrupt of UART has a lower priority than HardFault\_handler or other exceptions which we want to print out the stack or register information while at the handler mode.
The I/O retargeting to UART can not work when a hardware fault happens.
One possible solution is to use the UART without the interrupt, such as DMA.
Another solution is to change the UART interrupt priority higher than fault handlers.
The later solution may have a potential security problem.  
Or if the device supports the LCD screen, we can also utilize the LCD to print out the debug information.

\ziming{we should redesign to code to run a ton of tests in one image. If a test generates a fault and the tests cannot continue, we software reset the system.}

\ziming{The beginning of the test case suite should read system registers and print out the hardware configurations of the system: 1) CPU Model, frequency, SRAM/SSRAM. Also print out a banner that CactiLab developed this tool.}

\ziming{Each test case should print out the purpose of the test, test number, the expected outcome.}




==> testsuite.tex <==
In the appendix, we first provide a detail walk-through of Cortex-M architectures and security features. Then, we describe our test code.
 
\section*{A Suite of Example Cortex-M Code}
\label{sec:codesuite}

We developed a suite of example Cortex-M code to help researchers easily access Cortex-M research.
The suite is tested on the Cortex-M33 based Armv8 IoT Kit FVP~\cite{M33IoTKit}, which can be used on the Cortex-M Prototyping System (MPS2+)-based Field Programmable Gate Array (FPGA)~\cite{mps2} prototype board.
We will open-source and keep developing the suite after the paper is accepted.
To show the good faith of open-source, we put an anonymized copy of the source code online for artifact evaluations\footnote{\url{https://anonymous.4open.science/r/cortex-m-test-suite-v1}}.
The example code suite includes the following components:

(1) Helper and configuration functions.
These functions provide a C language interface to configure the system and peripheral registers. 
The current version includes:
(i) exception handlers that retrieve detailed fault information;
(ii) functions to enable and disable data and instruction cache;
(iii) stack dump function that prints out regular stack and exception stack contents;
helper functions to configure and control (iv) MPU;
(v) SAU; (vi) MPC; (vii) DWT; (viii) MTB.

(2) Test cases to demonstrate how to use hardware features.
The current version includes the following test cases:
(i) change \verb|xPSR|;
(ii) legal and illegal memory accesses;
(iii) \verb|TT| instruction examples;
(iv) stacking and unstacking with and without TrustZone;
(v) instruction tracing with MTB;
(vi) performance measurement and data access monitor with DWT;
(vii) state transition tests and performance measurement.


\begin{comment}
To run the prototype, we use Cortex-M33 Armv8 IoT Kit FVP~\cite{M33IoTKit}, which is intended to be implemented on the Cortex-M Prototyping System (MPS2+)-based system Field Programmable Gate Array (FPGA)~\cite{mps2}, on Keil IDE~\cite{keil}.
Each example functions has either \verb|_s| or \verb|_ns| suffix to indicate whether it executes in the secure or the non-secure state.
\end{comment}

\begin{comment}
Table~\ref{tab:Bare-metalApps} shows some bare-metal system examples that come with development boards, e.g., STM32F479I-Eval~\cite{stm324feval} and STM32F4-Discovery~\cite{stm324fdisc}.
These examples represent real-world IoT applications that use different peripherals, e.g., SD card, LCD screen, digital lock. 

\begin{table}[!ht]      
	\centering
	\scriptsize  
	\caption{Example Bare-metal Systems}  
	\vspace{-0.3cm}
	\begin{threeparttable}   
		\begin{tabular}{p{2cm}p{0.6cm}p{4cm}ll|} \hline
			Application   & KLOC   & Description \\ \hline\hline
			Audio-Playback$^1$     & 2.98   & Read and play audio from SD card \\ 
			FatFs\_uSD$^1$         & 1.29   & Fat file system on SD card  \\ 
			LibJPEG\_Encoding$^1$  & 1.58   & Read .bmp from SD, encode to jpeg\\ 
			LibJPEG\_Decoding$^1$  & 1.53   & Read jpeg from SD, display on LCD \\ 
			%LCD\_Display       & 1.48  & Read .bmp from SD, display on LCD \\ 
			LCD\_Animate$^1$       & 1.58  & Display .bmp images\\ 
			SSL\_Client$^1$        & 2.30  & An SSL client  \\
			PinLock$^2$            & 1.20  & Digital lock with Pin  \\ \hline
		\end{tabular}
		\begin{tablenotes}
			\item[] $^1$STM32F469I-Eval, $^2$STM32F4-Discovery
		\end{tablenotes}
	\end{threeparttable}  
	\label{tab:Bare-metalApps}
\end{table}
\end{comment}

% \subsection{Example: Cortex-M33 Armv8 IoT Kit FVP}

\begin{comment}
This memory map is divided into secure and non-secure regions. In general, the memory alternates between secure and non-secure regions in 256MB steps, with only a few address areas that are exempted from security mapping because they are related to debug
functionality.

To provide memory and peripherals that can be mapped as secure or non-secure using software, several address regions are aliased as shown in the table.

For a row where the column Alias with row ID is not empty, the column indicates which other row entry it is aliased to in the memory map within the same table for that entry.
\end{comment}

% \begin{table*}[!ht]      
% 	\centering
% 	\scriptsize  
% 	\caption{Test Cases}  
% 	\vspace{-0.3cm}
% 	\begin{threeparttable}   
% 	\begin{tabular}{lp{6cm}llll} \hline
% 	Test case    	& Test case description   & Test data & Expected result & Actual result & Status\\ \hline\hline
% 	Configuration	& Configure SAU to split memory\\
% 					& Configure MPC to map memory\\
% 					& Configure MPU to protect memory\\ 
% 					\hline
% 	Secure instructions& \verb|TT, TTT, TTA, TTAT| \\ 
% 					& \verb|SVC| \\
% 					& \verb|SG| \\
% 					\hline
% 	Memory access	& S-UP accesses NS-P \\
% 					& NS-UP accesses S-P \\
% 					\hline
% 	Special register&xPSR \\ \hline
% 	Branches 		& Comprehensive branches\\
% 					& Unintended transition between NS and S \\
% 					\hline
% 	Exceptions 		& Fake \verb|EXC_RETURN|m \verb|RNC_RETURN| \\
% 					& \verb|EXC_RETURN| With and without TZ \\
% 	\hline
% 	\end{tabular}
%    \end{threeparttable}  
% 	\label{tab:Bare-metalApps}
% \end{table*}

%  I. Example code for configuration.

%\test{Existing cases}

%\ziming{Make sure CMSIS does not have these examples or code.  May create a table for this as well.}

\begin{comment}
\subsection{Abstract libraries}
Abstract libraries provide basic functionality to support our test cases, including:
(i) rewritten exception handlers: \verb|HardFault_Handler| handles each type of faults (e.g., \verb|MemoryManagementFault| in \S\ref{sec:FaultHandling}) to fetch specific sub-type faults from \verb|SCB|;
(ii) privilege escalation and other privileged functions are implemented in the \verb|SVC_Handler|;
(iii) dump function that prints out exception stack information; 
(iv) \verb|DWT| related functions to do CPU cycle count measurement and install data access watchpoint;
(iii) \verb|MTB| configuration that enable/disable/pause/resume the trace unit;
(iv) \verb|SwitchStackPointer_s| changes stack pointer from MSP to PSP;
(vi) security state configuration: \verb|test_config_mpu_s/ns| provides dynamically MPU configuration at run-time. 
\verb|test_config_sau_s| configures SAU (see~\S\ref{sec:sau}) to dynamically partition the memory security state.
\verb|test_config_mpc_s| configures MPC (see~\S\ref{sec:memalias}) to release memory to non-secure;
(v) \verb|sys_reset/recover| resets or recovers the state of the CPU when exception finishes, etc.

\subsection{Test cases}
Those test cases can be linked back to previous sections.

\test{Check the special register xPSR in \S\ref{sec:mode}.}
Malicious xPSR value may change the CPU state.
As document~\cite{Armv8MArcRef} describes, \verb|APSR| is read-write and provides both privileged and unprivileged access.
\verb|EPSR| and \verb|IPSR| is read-only by \verb|MRS| instruction.
\verb|EPSR| reads as zero.
Any writes to \verb|IPSR| and \verb|EPSR| will be ignored by the processor (\verb|test_ipsr_s|). 
%Since xPSR already indicates the mode the CPU is from, why need the MODE bit to indicate to return to thread to handler again?? what if they do not match??.

\test{Example code to test MPU functionality.}
\verb|arm_mpu_config_s/ns| configures default MPU in secure and the non-secure state (see~\S\ref{sec:mpu}) to separate the privilege level and assign access permissions to each region. 
\verb|test_mpu_ns| gives several examples to test how MPU work.

% II. Example code for triggering intended behaviors including faults.

\test{Explore special instructions: TT, SVC, and SG.}
%\verb|TT|, \verb|SVC|, \verb|STR*T/LDR*T|) instructions, we developed 
\verb|test_tt_s/ns| shows how \verb|TTA?T?| (see~\S\ref{sec:subsec:TT}) instructions work with and without MPU configuration.
 
In normal case, thread mode will run \verb|SVC| (see~\S\ref{sec:mode}) instruction to enter the handler mode.
\verb|test_svc_s| tries to run \verb|SVC| in the handler mode, which will trigger \verb|HardFault|.

%\verb|test_up_ins_s| tests unprivileged memory access instructions  (see~\S\ref{sec:subsec:STRT}). [TODO]
 
By observing the epilogue of function calls between secure and the non-secure state, \verb|SG| (See~\S\ref{sec:trustzone}) instruction should be placed in the NSC region and usually followed with the \verb|B| instruction, which branch targets to secure code, to provide a secure entry for non-secure code.
\verb|test_sg_s| puts \verb|SG| in the secure memory, showing that it works as normal in the secure state while non-secure code cannot access it.
\verb|test_sg_ns| puts \verb|SG| in non-secure memory, which will be ignored by the CPU.
\verb|test_sg_s| also tests to run \verb|BL|, \verb|BX|, and \verb|BLX| instructions after \verb|SG|.
\verb|test_sg_2_ns_s| branches (\verb|BX|) to non-secure target after \verb|SG|.
Any attempt to switch from secure to the non-secure state without \verb|BXNS, BXLNS| instruction will trigger invalid transition \verb|SecureFault|. 

\test{Observe the hardware stacking and unstacking (see~\S\ref{sec:ExceptionStacking} and~\S\ref{sec:subsec:stateswithing}):}
Check the stack of \verb|EXC_RETURN| with and without TrustZone.
The additional stack context is stacked if this is a transition from the secure state to the non-secure state. [-]

The stack of \verb|FNC_RETURN| can be observed when the secure state finish initialization and call \verb|NonSecure_ResetHandler|, which will use \verb|BLXNS| instruction. [-]

\test{Explore the debug units in \S\ref{sec:debugers}).}
\verb|test_mtb_s| traces branches and stores the address pairs in an allocated SRAM region. 
It observes the control-flow path for different cases, including infinite loop (\verb|test_mtb_s_infinite_loop|), stack overflow (\verb|test_mtb_s_stack_overflow|), and bad \verb|ASM| instructions (\verb|test_mtb_s_memory_corrup|).   
DWT can be used to measure the CPU cycles (see \textbf{T08}) and monitor data access (\verb|test_dwt_s| and \verb|test_dwt_ns|).
%\verb|test_etm_s| [TODO].

\test{Example code for transitions, including normal and unintended transitions in \S\ref{sec:subsec:stateswithing}.}
A comprehensive branch test cases based on Figure~\ref{fig:ModePLSecure} show in example code \verb|test_b_s| and \verb|test_b_ns|. 
The memory access between the secure state and the non-secure state does not check the privilege level of either source or destination address.

%Secure state unprivileged code can access SRAM that is configured as privileged read-only in the non-secure state.
%S-P, S-UP \verb|BL| to NSC.
Secure state code (P and UP) \verb|BL, BLX| to the non-secure state (P or UP) triggers invalid transition \verb|SecureFault|.
%S-P, S-UP \verb|BLXNS/BXNS| to S/NS (P/UP).
%NS-UP code can also access the memory region configured as secure privileged read-only via NSC functions (\verb|test_cases_ns|).
Non-secure code (P and UP) directly \verb|BL/BLX| the secure state memory (P or UP) directly will generate invalid entry point \verb|SecureFault|.
%NS-P/NS-UP  to S/NSC triggers invalid entry point \verb|SecureFault|. 
Non-secure (P and UP) \verb|BLXNS/BXNS| to S/NS/NSC triggers invalid transition \verb|SecureFault|.

The target security state of those two instructions is indicated by the least significant bit of the target address, 1 means secure, 0 means non-secure~\cite{Armv8mdeveloper}. 
Show the LSB of the address used by \verb|BLXNS| and \verb|BXNS|. 
These instructions are only supposed to switch from S to NS.

%Observe how \verb|BXNS| works (\verb|test_bxns_s|).

%Check the epilogue of NSC function. Since it is callable from the secure state as well, how does \verb|BXNS| works. (B3.14 On transition from Secure to Non-secure state, if the least significant bit of an interstating branch is set to one the execution of the next instruction will generate a fault. ??)

\test{Performance measurement for privilege escalation and the secure state transition.}
%\ziming{Xi: Could you please put your test results here?}
To measure the cost of the context switching, we used DWT to collect the CPU cycles without interrupting the processor.
The time measurement of state switching checks the time as soon as the state changes from non-secure to secure.
\end{comment}

\begin{comment}
As for privilege switching, the last bit of the \verb|CONTROL| register indicates the current privilege mode.
1 means non-privilege mode, 0 means privilege mode.
Writing 1 to \verb|CONTROL| register will disable the privilege.
If we want to enable the privilege, the SVC handler is used and the mode will be elevated to privilege temporarily.
Then write 0 to the \verb|CONTROL| register to enable the privilege.
\end{comment}

\begin{comment}
Since DWT is memory-mapped to PPB which is privileged access only, we created two types of tests for the privilege switching may not very precise but can still show what we want to know:

\begin{itemize}
	\item Time measurement starts after jumping into the \verb|SVC| handler.
	It actually missed the time cycles for triggering the \verb|SVC| handler.
	\item Time measurement starts before dropping privilege (MSR CONTROL, 1), then trigger SVC immediately.
	It actually added the time cycles to run the privilege dropping instruction.
\end{itemize}

\begin{comment}
All those tests ran 500 times to get the minimum, maximum, and average time cycles.
Since the second test for privilege switching contains the time cycles of writing to the \verb|CONTROL| register, we also measured this instruction.
\end{comment}


\begin{comment}
\begin{table}[!htpb]
	\center
	\scriptsize
	\caption{Overhead of State Switching and Privilege Switching}
	\label{tab:Overhead-ss-ps}
	\begin{tabular}{llcp{1cm}}
		\hline
		Context Switch & Min & Max & Average \\ \hline  \hline
		Non-secure $\rightarrow$ Secure & 34 &  34 & 34 \\
		Secure $\rightarrow$ Non-secure & 37 &  38 & 37.0020 \\
		Unprivileged $\rightarrow$ Privileged (missed cycles) & 55 & 55 & 55 \\
		Unprivileged $\rightarrow$ Privileged (added cycles)  & 78 & 145 & 79.0415 \\
		Write to CONTROL  & 19 & 84 & 19.1139 \\ \hline                      
	\end{tabular}
\end{table}
\end{comment}
%\ziming{Check Cortex-M for beginner 5.2. The measurement is not consistent with your.}

%By learning from the table \ref{tab:Overhead-ss-ps}, we observe that even with missing time cycles, the time cost of context switch for unprivileged to privileged level is 61\% higher than TrustZone state switching.


\subsection{Binary tricks}

%\test{Explore the ABI level secure compile flag.} 
To help developer, compiler provides compile flags to support TrustZone project (e.g., \verb|-cmse| in Keil IDE).
A function is declared as non-secure callable with attribute  (\verb|__attribute__((cmse_nonsecure_entry))|).
Comparing with other secure functions, the compiler will automatically generate \verb|SG| instruction in the NSC region and branch to this function in secure state.
The prologue will check and clear floating-point registers since the state transition automatically has stacking as discussed in \S\ref{sec:subsec:asystateswithing}.[add floating-point register in this section]
The epilogue instruction is \verb|BXNS LR| instead of \verb|BX LR|.
%The float-point registers \verb|s0| to \verb|s15| will be changed to \verb|LR|.

\test{Arbitrary NSC functions in \textbf{I14}.}
Besides those compile attributes, developer can also insert arbitrary NSC function in the NSC region.
%A \verb|SG| instruction provides an entry point to switch from non-secure to the secure state.
\verb|test_sg_s| writes arbitrary instructions in the NSC region after \verb|SG|.
Then \verb|test_sg_ns| will \verb|BX| directly to this address to run \verb|SG| and change the non-secure state the secure state, then executes secure code. 

\test{Privilege escalation.} To escalate the privilege level of the current execution mode in the non-secure state, we can either call \verb|SVC|, which can be other syscalls, or configure \verb|CONTROL_NS| in the secure state (\verb|test_p_ns|)*. 

% III. Example code for ABI attacks.

\subsection{ABI/ISA level attacks}
	
\test{SG ROP.} 
\verb|SG| is a 4-byte instruction, which is actually a duplicated 2-byte hex value. 
Jump to the middle of 4-byte instruction to generate unintended instructions. \verb|test_malicious_sg_s|). [$\times$]
	% \ziming{SG is 4 bytes, so it can not pretend to be part of another instruction.
	% Hold on, we can have two 4 bytes instructions, 2 bytes from the first 4 and 2 bytes from the second 4 to pretend to be SG. Then, build a ROP chain from there?}
	 
\test{Ret-to-secure state attack.} An NS function has buffer overflow. The return address is overwritten to a legit NSC stub. In this attack, the attacker will be able to call any exposed the secure state function. 
	
\test{Secure stack pointer vulnerability.}
with an empty stack, put a fake \verb|EXC_RETURN| or \verb|FNC_RETURN| to trigger unstacking~\cite{Armv8SecureStackSealing}.
	 
\test{Stack information leakage.}
an unprivileged program can change state context which was saved during context stacking. Because context stacking uses current stack, PSP may be used. Also, a malicious kernel can change \verb|EXC_RETURN| to use the wrong stack.

\subsection{Others}
\begin{enumerate}
	\item Speculative execution? Spectra? Meltdown? 
	\item Cache side channel attack?
	\item Check if all compilers with generate code to clear general-purpose registers when switch from secure to NS. Is there a more efficient way to clear registers. 
	\item Check if clearing registers are required in ABI. [CVE-2021-35465]
	\item To switch from non-secure to secure, does compilers generate code to clear general-purpose registers as well?
	\item Why do not need secure anyway? why not putting everything in non-secure callable?
\end{enumerate}


\begin{figure}[!t]
	\begin{centering}
		\includegraphics[width=.5\textwidth]{pics/arch.pdf}
		\vspace{-0.4cm}
		\caption{Software architecture of production systems} %Some processors do not support flash patching, so the star means a partially implemented FPB.}
	\label{fig:arch}
\end{centering}
\vspace{-0.5cm}
\end{figure}

\begin{comment}
\subsection{System IP}

\url{https://developer.arm.com/ip-products/subsystem/corstone/corstone-201}

Corstone SSE-200 subsystem

Arm Cortex-M33 processor

Arm CoreLink SIE-200

Instruction caches with Arm TrustZone support

Power infrastructure components

CoreSight SoC-400M

Arm CryptoCell

Potential titles:

1. SoK: Understanding Trusted Execution Environments on IoT Devices

2. SoK: All You wanted to Know about Cortex-M Security Features

3. SoK: Demystifying Security Related Hardware Features on IoT Devices

4. SoK: Demystifying the Security of Arm Cortex-M based Internet-of-Things Systems

Products:

https://www.eletimes.com/renesas-extends-arm-cortex-based-mcu-family-for-industrial-and-iot-applications

\end{comment}

%\section{Notes}

%\ziming{The same function $F$ in the secure state. Compile it as a regular function and \_\_attribute\_\_((cmse\_nonsecure\_entry)), compare the differences in the generated binary code.
%I think the function itself will be the same. 
%The only difference is for nsc, the NSC stub is generated,
%which means at ISA level we can actually call any function in the secure state from NS.}

%\ziming{Why are there no BNS or BLNS instructions?}	

%\ziming{So should we run kernel in handler mode or $<$T, P$>$? What are the difference? Benefits and disadvantages of each? Where does Mbed and RTOS put the kernel?} 

%\ziming{Somehow formally model Cortex-M operations, and formally verify if there is any vulnerabilities. Operational semantics.}

%\ziming{Like the Quest to replace passwd paper, we evaluate these schemes based on deployability, security, performance, etc.} [\checkmark]

%\ziming{Do MBed, FreeRTOS have a filesystem? How is write and read persistent storage abstracted in such systems? Do MBed, FreeRTOS provide heap support? Can we use malloc, free() or new when we develop program?} [FreeRTOS manages heap]

%\ziming{Explain EXCRETURN. LAGO attack possible? a malicious kernel module manipulate the stack and triggers unstacking.} [Secure Stack sealing]

%\ziming{Defense techniques: (1) Code integrity (W xor E, Remote Attestation); (2) Code pointer integrity; (3) instruction set randomization; (4) ASLR; (5) CFI; (6) non-executable data; (7) execution-only memory; (8) data space randomization; (9) data flow integrity} [defense section: \checkmark]

%\ziming{a figure showing the configuration relations of all controllers: MPU, SAU, IDAU, MPC, PPC} [\checkmark]

%\ziming{Draw a ring figure for default Cortex-M privileged and unprivileged operations. The ring should consider secure and NS as well.} [\checkmark]

%\ziming{What is the status of the the following defenses on Cortex-M and compilers? (0) data execution prevention (1) stack cookies, (2) exception handler validation, (3) data execution prevention; do we have enough MPU to support this? 4) ASLR.} [maybe: \checkmark]



% SAML10, 11, the MSP2+ FPGA.

\begin{comment}
\begin{table}[!htpb]
\center
\scriptsize
\caption{Access Permissions}
\vspace{-0.3cm}
\label{tab:ap}
\begin{threeparttable}
\begin{tabular}{llcc}
\hline
Privileged    & Unprivileged  & Armv7-M              & Armv8-M          \\ \hline  \hline
No access     & No access     & \supportlevel{10}   & \supportlevel{0} \\
Read/Write    & No access     & \supportlevel{10}   & \supportlevel{10} \\
Read/Write    & Read-only     & \supportlevel{10}   & \supportlevel{0} \\
Read/Write    & Read/Write    & \supportlevel{10}   & \supportlevel{10} \\
Read-only     & No access     & \supportlevel{10}   & \supportlevel{10} \\
Read-only     & Read-only     & \supportlevel{10}   & \supportlevel{10}\\  
\hline                                
\end{tabular}
\begin{tablenotes}
\item[] \supportlevel{0}: Not support, \supportlevel{10}: Support
\end{tablenotes}
\end{threeparttable}
\end{table}

\end{comment}

\begin{comment}
\begin{table}[!htpb]
	\center
	\scriptsize
	\caption{RTOS}
	\label{tab:rtos}
	\begin{tabular}{llllccc}
		\hline
		Project               & \rotatebox{90}{Open-source?} & CPU & Version & \rotatebox{90}{Privilege Separation}& \rotatebox{90}{Crypto} & \rotatebox{90}{RoT}\\ \hline  \hline
		% Abassi~\cite{}        &$\times$&M0/3/4&\\
		Apache Mynewt~\cite{} &\checkmark&M0/3/4/7&v1.9.0\\	
		% Azure Sphere~\cite{stiles2019hardware}  &\checkmark&M4&v21.04&\supportlevel{0}&\supportlevel{10}&\supportlevel{10}\\
		BRTOS~\cite{}         &\checkmark&M0/3/4&v1.9.0\\
		BeRTOS                &\checkmark&M3&\\
		ChibiOS/RT~\cite{}    &\checkmark&M0/3/4&v20.3.3&-&-&-\\ 
		Contiki-NG~\cite{ContikiNG} &\checkmark&&&\checkmark\\
		distortos~\cite{}     &\checkmark&M0/0+/1/4/7&&-&-&-\\
		dnx RTOS~\cite{}      &\checkmark&M3&v2.4.0&-&-&-\\
		eChronos~\cite{}      &\checkmark&M3-7&&\\
		eCosPro~\cite{}       &$\times$&M3/4/7&&\\
		embOS~\cite{}         &$\times$&M&&\\
		Embkernel~\cite{}     &\checkmark&M&&\\
		ERIKA Enterprise~\cite{} &\checkmark&M4/7&&\\
		EUROS~\cite{}         &$\times$&M3&&\\
		Flexible Safety RTOS  &$\times$&M&&\\
		FreeOSEK~\cite{}      &\checkmark&M4&&\\
		FreeRTOS~\cite{freertos}  &\checkmark&M3/4/7&v10.4.0&\checkmark&&\supportlevel{10}\\
		Frosted~\cite{}       &\checkmark&M&&\\
		FunkOS~\cite{}        &\checkmark&M3&&\\
		FX-RTOS               &\checkmark&M0/1/3&&\\
		hyperCOS              &$\times$&M3/4&&\\
		IntrOS                &\checkmark&M&&\\
		ISIX                  &\checkmark&M3&&\\
		Keil RTX5			  &\checkmark&M&&\checkmark\\
		Lepton                &\checkmark&M3/4&&\\
		Mbed OS~\cite{MbedOS} &\checkmark&All&v6.10&\checkmark&\supportlevel{10} \\
		MicroC/OS-III         &\checkmark&M1/3/4&&\\
		Milos                 &\checkmark&M3&&\\
		miosix                &\checkmark&STM32&&\\
		mipOS                 &\checkmark&M3&&\\
		nOS                   &\checkmark&M0/3/4&&\\
		Nucleus RTOS          &\checkmark&M3/4&&\\
		NUFR                  &\checkmark&M0/3/4&&\\
		NuttX~\cite{nutt2007nuttx}&\checkmark&M0/3/4/7 &&\supportlevel{0}\\
		OneOS~\cite{oneos}				  &\checkmark&STM32&v1.2&&\supportlevel{10}\\
		picoOS                &\checkmark&M&&\\
		Piko/RT               &\checkmark&M3/4&&\\
		Pharos                &\checkmark&M4&&\\
		QP                    &\checkmark&M0-7 &&\\
		RIOT OS~\cite{RIOT}   &\checkmark&All&v5.00&\supportlevel{0}&\supportlevel{10}\\
		RODOS                 &\checkmark&M3&&\\
		RT-Thread NANO~\cite{RTthread} &\checkmark&M0/0+/3/4/7/23&v4.0.3&\checkmark&\supportlevel{10}\\
		SCIOPTA               &$\times$&M0/3/4&&\\
		scmRTOS               &\checkmark&M3&&\\
		SDPOS                 &\checkmark&M3&&\\
		silRTOS               &\checkmark&M&&\\
		StateOS               &\checkmark&M&&\\
		Stratify OS           &\checkmark&M3/4&&\\
		TencentOS Tiny		  &\checkmark&M0/3/4/7 \\
		TI-RTOS               &\checkmark&M3/4&&\\
		TockOS~\cite{levy2017multiprogramming}  &\checkmark&M3/4 &&\checkmark\\
		TNKKernle             &\checkmark&M3&&\\
		TNeo                  &\checkmark&M0/0+/1/3/4&&\\
		uKOS~\cite{}          &\checkmark&M3/4/7&\\
		Huawei LiteOS         &\checkmark&M0/3/4/7&&\\
		Zephyr                &\checkmark&M0/3/4/23/33&v2.5.0&\checkmark&\supportlevel{10}\\
		
		\hline
		\\                                                                    
	\end{tabular}
	\begin{tablenotes}
		\item[] \supportlevel{0}: Not support, \checkmark/\supportlevel{10}: Support, \supportlevel{5}: Partially Support
	\end{tablenotes}
\end{table}


\begin{table*}[!htpb]
\center
\scriptsize
\caption{Bug reports}
\vspace{-0.3cm}
\label{tab:CVEs}
\begin{tabular}{c|p{4cm}|c|p{10cm}}
\hline
Class             & Subclass              & \# Bugs & Type - OS/App/Hardware [CVE ID]         \\ \hline  \hline
\multirow{3}{*}{Architectural Issue} & \textbf{Improper stack selection} & 1 &   Stack underflow - Armv8-M TrustZone [CVE-2020-16273]  \\ 
 & \textbf{Unprotected hardware block} & 1 &  NXP LPC55S6x ROM Patch Controller   [CVE-2021-31532]  \\
 & \textbf{Inf. leakage through state switch} & 1 &  VLLDM instruction Security Vulnerability [CVE-2021-35465]  \\
  \hline
Hardware Issue    & \textbf{Information leakage though cache}  & 2  & Cache side channel - Mbed TLS [CVE-2018-0498], wolfSSL [CVE-2018-12436] \\ \hline
\multirow{50}{*}{Implementation}  & \multirow{18}{*}{\textit{Validation bugs - }} & 61 & Access uninitialized pointer (1h) - FreeRTOS [CVE-2018-16522] \\ \cline{4-4}
\multirow{50}{*}{Issue}           & \multirow{18}{*}{\textbf{Network Communication}} &  & MQTT-SN (1h) - RIOT-OS [CVE-2019-17389] \\ \cline{4-4}
&&& Buffer overflow (20,15c3h2m) - Mbed TLS [CVE-2018-0487-c, CVE-2015-8036-m, CVE-2015-5291-m], RIOT-OS [CVE-2019-1000006-c, CVE-2021-27698-c, CVE-2021-27697-c, CVE-2021-27357-c, CVE-2017-8289-c], FreeRTOS[CVE-2018-16526-h, CVE-2018-16525-h], Contiki-NG [CVE-2020-24336-c, CVE-2018-19417-c], Mbed CoAP lib [CVE-2020-12887-h, CVE-2020-12883-c, CVE-2019-17212-c], Zephyr  [CVE-2020-10071-c, CVE-2020-10070-c, CVE-2017-14199-c], wolfSSL [CVE-2019-64390-c, CVE-2019-11873-c], TockOS  [CVE-2018-1000660-h] \\ \cline{4-4}
&&&  Out-of-bounds read (16,5c5h6m) - Mbed TLS[CVE-2018-9989-h, CVE-2018-9988-h], Mbed CoAP lib [CVE-2020-12886-c, CVE-2020-12884-c], FreeRTOS[CVE-2019-13120-h, CVE-2018-16603-m, CVE-2018-16602-m, CVE-2018-16600-m, CVE-2018-16599-m, CVE-2018-16527-m, CVE-2018-16524-m], Contiki-NG [CVE-2020-24335-h, CVE-2020-24334-h, CVE-2020-14937-c], wolfSSL [CVE-2019-16748-c, CVE-2019-15651-c] \\\cline{4-4}
&&&  Out-of-bounds write (11,10c1h) - Mbed TLS[CVE-2018-0488-c], Mbed CoAP lib [CVE-2019-17212-c], Contiki-NG [CVE-2020-14936-c, CVE-2020-14935-c, CVE-2020-14934-c, CVE-2019-8359-c], NuttX [CVE-2020-17528-c, CVE-2020-17529-c], wolfSSL [CVE-2020-36177-c, CVE-2019-18840-h, CVE-2017-2800-c] \\ \cline{4-4}
&&&  Integer Overflow (5,2c3h)    - Mbed TLS[CVE-2017-18187-c], Mbed CoAP lib [CVE-2019-17211-c], FreeRTOS[CVE-2018-16601-h], Contiki-NG [CVE-2019-9183-h], Zephyr [CVE-2020-10063-h] \\ \cline{4-4}
&&&  NULL Pointer Dereference (2,1c1h) - RIOT-OS [CVE-2019-16754-h], NuttX [CVE-2020-1939-c]\\ \cline{4-4}
&&&  Use after free (1h)           - Zephyr [CVE-2017-14201] \\ \cline{4-4}
&&&  Improper Input Validation (3,2h1m) - Mbed TLS [CVE-2016-3739-m], Mbed MQTT lib [CVE-2019-17210-h],  FreeRTOS[CVE-2018-16528-h] \\ \cline{4-4}
&&&  Invalid pointer free (1h) - Mbed TLS [CVE-2017-2784-h] \\  \cline{2-4}
& \multirow{13}{*}{\textit{Validation bugs - }} & 28 & Access uninitialized pointer (1m) - Zephyr[CVE-2020-10060-m] \\ \cline{4-4} 
& \multirow{13}{*}{\textbf{Other privileged code}} && Buffer overflow (9,3c4h2m) - RIOT-OS [CVE-2020-15350-c], Contiki-NG [CVE-2018-1000804-c, CVE-2018-16664-h, CVE-2018-16665-m], Zephyr [CVE-2020-10023-m (shell), CVE-2017-14202-h (shell), CVE-2020-10022-c, CVE-2020-10019-h (USB), CVE-2017-8854-h (DH file)] \\ \cline{4-4}
&&                                & Out-of-bounds read (1h) - Zephyr [CVE-2018-16667-h] \\ \cline{4-4}
&&                                & Out-of-bounds write (4h) - Contiki-NG [CVE-2018-20579-h, CVE-2018-16666-h, CVE-2018-16663-h], Zephyr [CVE-2020-10021-h (USB)]\\ \cline{4-4}
&&                                & Integer overflow (10h) - Mbed OS [CVE-2021-27435-h, CVE-2021-27433-h], FreeRTOS [CVE-2021-31572-h, CVE-2021-31571-h], RIOT OS [CVE-2021-27427-h], TI-RTOS [CVE-2021-27429-h, CVE-2021-2263-h, CVE-2021-27502-h], NuttX [CVE-2021-26461-h], Zephyr [CVE-2020-10067-h]\\ \cline{4-4}
&&                                & Null pointer dereference (1c) - Zephyr [CVE-2018-1000800-c] \\ \cline{4-4}
&&                                &  UpdageHub module (1m)    - Zephyr [CVE-2020-10059-m] \\ \cline{4-4}
&&                                & Use after free (1h) - FreeRTOS[CVE-2019-18178-h] \\\cline{2-4}
& \textit{Functional bugs - } & 4 & Stm32Cube crypto extension [CVE-2020-20949] \\
& \textbf{Vulnerable Crypto Implementation}  & & wolfSSL[CVE-2019-19962, CVE-2018-16870, CVE-2017-13099] \\ \cline{2-4}
& \multirow{12}{*}{\textit{Functional bugs - }} & 23 &  Infinite loop (3h)       - Mbed CoAP lib[CVE-2020-12885-h], RIOT-OS [CVE-2019-15702-h], NuttX [CVE-2018-20578-h] \\ \cline{4-4}
& \multirow{12}{*}{\textbf{Other implementation bugs}} &&  Divide by zero (1h)       - FreeRTOS[CVE-2018-16523] \\ \cline{4-4}
&&&  Incorrect comparison (2h) - Zephyr [CVE-2020-10027-h, CVE-2020-10024-h] \\ \cline{4-4}
&&&  Off-by-one Error (1c)     - Zephyr [CVE-2020-10062]  \\ \cline{4-4}
&&&  Multi-syscalls (3,2h1m)    - Zephyr [CVE-2020-10068-m (Bluetooth), CVE-2020-10058-h (Kscan), CVE-2020-10028-h] \\ \cline{4-4}
&&&  Improper privilege management (1m) - Mbed TLS[CVE-2018-19608] \\ \cline{4-4}
&&&  Improper Authentication (1h)       - Mbed TLS      [CVE-2017-14032] \\ \cline{4-4}
&&&  Buggy heap management (1c)    - FreeRTOS[CVE-2021-32020] \\ \cline{4-4}
&&&  Buggy functions (9,5h4m)          - wolfSSL [Improper certification: CVE-2021-3336-h, DTLS message clearance: CVE-2020-24585-m, Mishandle CCS message: CVE-2020-12457-h, Miss encryption of sensitive data: CVE-2019-14317-m, Mishandle CRT process: CVE-2015-7744-m, Resource management errors: CVE-2015-6925-h, Malicious user can access cache: CVE-2017-6076-m, Accept malformed DH key: CVE-2017-8855-h], RIOT-OS [Missing release memory: CVE-2019-15134-h] \\ \cline{4-4}
&&&  Mismatch DNS request and response (1m) - FreeRTOS[CVE-2018-16598-m] \\ \cline{2-4}
& \multirow{4}{*}{\textit{Extrinsic Bugs - }} & 15 & Nonce (1c) - wolfSSL [CVE-2019-6439-c] \\ \cline{4-4} 
& \multirow{4}{*}{\textbf{Side channel}}      && Timing Side channel (14,1h13m) - Mbed TLS[CVE-2020-16150-m, CVE-2020-10941-m, CVE-2020-10932-m, CVE-2019-18222-m, CVE-2019-16910-m, CVE-2018-0498-m, CVE-2018-0497-m], wolfSSL [CVE-2020-11735-m, CVE-2020-11713-h, CVE-2019-13628-m, CVE-2016-7440-m, CVE-2019-19960-m, CVE-2016-7439-m, CVE-2016-7438-m] \\ \hline                                                                   
\end{tabular}
\end{table*}
\end{comment}


\begin{table}[!t]
	\center
	\scriptsize
	\vspace{-0.3cm}
	\caption{Vulnerability discovery for Cortex-M firmware}
	\vspace{-0.3cm}
	\setlength\tabcolsep{0.5ex}
	\rowcolors{2}{white}{gray!15}
	\label{tab:bug-finding}
	\begin{threeparttable}
		\begin{tabular}{l|l|l|ccc|ccc}
			\hline 
			\rowcolor{white}
			& Project & Year& \begin{tabular}[l]{@{}l@{}}\cellcolor{white} \rotatebox[origin=c]{90}{Input} \end{tabular}& \begin{tabular}[l]{@{}l@{}}\cellcolor{white} \rotatebox[origin=c]{90}{Target} \end{tabular}& \begin{tabular}[c]{@{}l@{}}\cellcolor{white} \rotatebox[origin=c]{90}{ISA} \end{tabular}&
			\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\cellcolor{white}Peripheral\\\cellcolor{white}Modeling \end{tabular}}&
			\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\cellcolor{white}I/O\\\cellcolor{white}Interaction\end{tabular}} &\begin{tabular}[c]{@{}c@{}}\cellcolor{white}Support\\\cellcolor{white}Fuzzing \end{tabular} \TBstrut{4ex}{-2.7ex} \\ \hline \hline
            \cellcolor{white}&FirmWare~\cite{firmwire}	&2022&&&&  &&  \\
            \cellcolor{white}&P$^2$IM~\cite{feng2020p}  &2020&C&R &v7 &&&\supportlevel{10}  \\
			\cellcolor{white}&DICE~\cite{mera2020dice}     &2020         &C&R &v7 &  &  &\supportlevel{10}  \\
            \cellcolor{white}&Laelaps~\cite{cao2020device}		&2020	&B&R &v7 &  &&\supportlevel{10}  \\
            \cellcolor{white}&$\mu$Emu~\cite{zhou2021automatic}  &2021   &B&R &v7 &  &&\supportlevel{10}  \\
            \cellcolor{white}&Jetset~\cite{jetset}	&2021&&&&  &&  \\
            \cellcolor{white}&Fuzzware~\cite{fuzzware}	&2022&&&&  &&\supportlevel{10}\\
            \cellcolor{white}&SEmu~\cite{semu}	&2022&&&&  &&  \\
            \multirow{-9}{*}{\cellcolor{white}\ref{Full firmware rehosting:}}&HALucinator~\cite{clements2020halucinator}	&2020&&&&  &&\supportlevel{10}\\
            \hline
            \cellcolor{white}&Avatar~\cite{avatar2}      &2018&&&&  &  &  \\
            \cellcolor{white}&Inception~\cite{cor2018}	&2018		&C&R &v7 &  &&  \\
            \multirow{-3}{*}{\cellcolor{white}\ref{Hardware-in-the-loop rehosting:}}&Frankenstein~\cite{Frankenstein} &2020&&&&  &  &  \\
            \hline
            \cellcolor{white}\ref{On-device fuzzing:}&$\mu$AFL~\cite{li2022mu}	&2022	&B&B&v7 &&&\supportlevel{10}\\ 
            \hline
            \cellcolor{white}&PASAN~\cite{kim2021pasan}      &2021       &C&R &v7 &&  &   \\
            \cellcolor{white}&FirmXRay~\cite{wen2020firmxray}	&2020	&B&B &v7 &&&\\
            \multirow{-3}{*}{\cellcolor{white}\ref{Static methods:}}&HEAPSTER~\cite{gritti2022heapster}	&2022	&B&B &- &&&\\
			%argXtract~\cite{sivakumaran2021argxtract} &B&R &v6/7 &\supportlevel{10}  &  &  \\
			%FIE~\cite{davidson2013fie}            &C&R &*  &  &\supportlevel{10}  &  \\
			\hline 
		\end{tabular}
		\begin{tablenotes}
		\item[] v6: Armv6-M, v7: Armv7-M, A: Cortex-A, R: Cortex-R, M: Cortex-M. \supportlevel{10}: Implement a specific security feature or need specific hardware support. 
		% \item[] Code and memory overhead shows the best case, run-time overhead shows the worst case.
		% \item[]: Bare-metal only or RTOSes. Input - source code; binary. Developer involvement - None; annotation; code modification.
		\end{tablenotes}  
	\end{threeparttable}
	\vspace{-0.5cm}
\end{table}

